Jailbreak Transferability Emerges from Shared Representations

Jailbreak transferability is the surprising phenomenon when an adversarial attack compromising one model also elicits harmful responses from other models. Despite widespread demonstrations, there is little consensus on why transfer is possible: is it a quirk of safety training, an artifact of model families, or a more fundamental property of representation learning? We present evidence that transferability emerges from shared representations rather than incidental flaws. Across 20 open-weight models and 33 jailbreak attacks, we find two factors that systematically shape transfer: (1) representational similarity under benign prompts, and (2) the strength of the jailbreak on the source model. To move beyond correlation, we show that deliberately increasing similarity through benign only distillation causally increases transfer. Our qualitative analyses reveal systematic transferability patterns across different types of jailbreaks. For example, persona-style jailbreaks transfer far more often than cipher-based prompts, consistent with the idea that natural-language attacks exploit models' shared representation space, whereas cipher-based attacks rely on idiosyncratic quirks that do not generalize. Together, these results reframe jailbreak transfer as a consequence of representation alignment rather than a fragile byproduct of safety training.

==> data/roc_a.tex <==
A B
0.0	0.0
0.07070902750871755	0.23997296079315006
0.07070902750871755	0.24087426768814782
0.07148392096086788	0.24087426768814782
0.07148392096086788	0.24132492113564669
0.07167764432390546	0.24132492113564669
0.07167764432390546	0.24177557458314555
0.07187136768694305	0.24177557458314555
0.07187136768694305	0.24222622803064445
0.07245253777605579	0.24222622803064445
0.07245253777605579	0.24245155475439387
0.07264626113909338	0.24245155475439387
0.07264626113909338	0.24312753492564218
0.07322743122820612	0.24312753492564218
0.07322743122820612	0.24335286164939163
0.07342115459124371	0.24335286164939163
0.07342115459124371	0.2438035150968905
0.07438977140643162	0.2438035150968905
0.07438977140643162	0.24425416854438936
0.0745834947694692	0.24425416854438936
0.0745834947694692	0.24470482199188823
0.07497094149554437	0.24470482199188823
0.07497094149554437	0.24515547543938712
0.07516466485858195	0.24515547543938712
0.07516466485858195	0.2458314556106354
0.0755521115846571	0.2458314556106354
0.0755521115846571	0.2462821090581343
0.07613328167376986	0.2462821090581343
0.07613328167376986	0.24650743578188372
0.07671445176288261	0.24650743578188372
0.07671445176288261	0.24673276250563317
0.07690817512592019	0.24673276250563317
0.07690817512592019	0.24853537629562866
0.07710189848895777	0.24853537629562866
0.07710189848895777	0.24966200991437584
0.07729562185199534	0.24966200991437584
0.07729562185199534	0.2501126633618747
0.07748934521503294	0.2501126633618747
0.07748934521503294	0.25033799008562413
0.0778767919411081	0.25033799008562413
0.0778767919411081	0.2505633168093736
0.07807051530414567	0.2505633168093736
0.07807051530414567	0.250788643533123
0.07826423866718327	0.250788643533123
0.07826423866718327	0.25101397025687244
0.0790391321193336	0.25101397025687244
0.0790391321193336	0.25146462370437134
0.07923285548237118	0.25146462370437134
0.07923285548237118	0.25191527715187023
0.07923285548237118	0.25214060387561965
0.07942657884540875	0.25214060387561965
0.07942657884540875	0.25236593059936907
0.07981402557148393	0.25236593059936907
0.07981402557148393	0.25259125732311855
0.0800077489345215	0.25259125732311855
0.0800077489345215	0.2534925642181163
0.08020147229755908	0.2534925642181163
0.08020147229755908	0.2537178909418657
0.08078264238667184	0.2537178909418657
0.08078264238667184	0.2539432176656151
0.081170089112747	0.2539432176656151
0.081170089112747	0.254393871113114
0.08136381247578459	0.254393871113114
0.08136381247578459	0.25461919783686343
0.08155753583882216	0.25461919783686343
0.08155753583882216	0.2555205047318612
0.08194498256489732	0.2555205047318612
0.08213870592793492	0.25574583145561064
0.0823324292909725	0.25574583145561064
0.0823324292909725	0.25642181162685895
0.08252615265401007	0.25642181162685895
0.08252615265401007	0.2566471383506084
0.08271987601704765	0.2566471383506084
0.08271987601704765	0.2573231185218567
0.08291359938008523	0.2573231185218567
0.08291359938008523	0.2575484452456061
0.0833010461061604	0.2575484452456061
0.0833010461061604	0.257999098693105
0.08349476946919798	0.257999098693105
0.08349476946919798	0.25890040558810273
0.08407593955831073	0.25890040558810273
0.08407593955831073	0.2591257323118522
0.08426966292134831	0.2591257323118522
0.08426966292134831	0.2598017124831005
0.08504455637349864	0.2598017124831005
0.08504455637349864	0.26025236593059936
0.08562572646261139	0.26025236593059936
0.08562572646261139	0.2609283461018477
0.08581944982564897	0.2609283461018477
0.08581944982564897	0.261604326273096
0.08601317318868655	0.261604326273096
0.08601317318868655	0.2618296529968454
0.08678806664083688	0.2618296529968454
0.08678806664083688	0.2620549797205949
0.08698179000387447	0.2620549797205949
0.08698179000387447	0.2622803064443443
0.08736923672994963	0.2622803064443443
0.08736923672994963	0.2627309598918432
0.08756296009298721	0.2627309598918432
0.08756296009298721	0.26318161333934204
0.08756296009298721	0.2634069400630915
0.0877566834560248	0.2634069400630915
0.0877566834560248	0.26453357368183866
0.08795040681906238	0.26453357368183866
0.08795040681906238	0.265209553853087
0.08833785354513754	0.265209553853087
0.08833785354513754	0.2661108607480847
0.08853157690817512	0.2661108607480847
0.08853157690817512	0.2663361874718342
0.08911274699728787	0.2663361874718342
0.08911274699728787	0.266786840919333
0.08930647036032545	0.266786840919333
0.08930647036032545	0.2672374943668319
0.0898876404494382	0.2672374943668319
0.0898876404494382	0.26768814781433076
0.09008136381247578	0.26768814781433076
0.09008136381247578	0.26791347453808023
0.09046881053855095	0.26791347453808023
0.09046881053855095	0.26836412798557907
0.09066253390158853	0.26836412798557907
0.09066253390158853	0.26881478143307797
0.09124370399070128	0.26881478143307797
0.09124370399070128	0.2690401081568274
0.09182487407981403	0.2690401081568274
0.09182487407981403	0.26926543488057686
0.09221232080588919	0.26926543488057686
0.09221232080588919	0.270392068499324
0.09240604416892677	0.270392068499324
0.09240604416892677	0.27061739522307343
0.09259976753196436	0.27061739522307343
0.09259976753196436	0.27129337539432175
0.09298721425803952	0.27129337539432175
0.09298721425803952	0.2715187021180712
0.09337466098411469	0.2715187021180712
0.09337466098411469	0.27309598918431727
0.09376210771018985	0.27309598918431727
0.09376210771018985	0.2744479495268139
0.094149554436265	0.2744479495268139
0.094149554436265	0.2751239296980622
0.09492444788841534	0.2751239296980622
0.09492444788841534	0.27534925642181163
0.09511817125145293	0.27534925642181163
0.09511817125145293	0.2757999098693105
0.09531189461449051	0.2757999098693105
0.09531189461449051	0.27670121676430826
0.09550561797752809	0.27670121676430826
0.09589306470360326	0.27670121676430826
0.09589306470360326	0.2769265434880577
0.09608678806664084	0.2769265434880577
0.09608678806664084	0.2778278503830554
0.09628051142967842	0.2778278503830554
0.09628051142967842	0.2782785038305543
0.09686168151879117	0.2782785038305543
0.09686168151879117	0.2785038305543037
0.09705540488182875	0.2785038305543037
0.09705540488182875	0.2789544840018026
0.0976365749709415	0.2789544840018026
0.0976365749709415	0.28030644434429924
0.09802402169701666	0.28030644434429924
0.09802402169701666	0.28053177106804866
0.09821774506005425	0.28053177106804866
0.09821774506005425	0.2807570977917981
0.0986051917861294	0.2807570977917981
0.0986051917861294	0.2814330779630464
0.09879891514916699	0.2814330779630464
0.09879891514916699	0.2821090581342947
0.09918636187524216	0.2821090581342947
0.09918636187524216	0.2823343848580442
0.09918636187524216	0.282785038305543
0.09918636187524216	0.28391167192429023
0.10034870205346764	0.28391167192429023
0.10034870205346764	0.28458765209553855
0.10073614877954282	0.28458765209553855
0.10073614877954282	0.28481297881928797
0.1009298721425804	0.28481297881928797
0.10112359550561797	0.2850383055430374
0.10112359550561797	0.28526363226678686
0.10131731886865555	0.28526363226678686
0.10131731886865555	0.2859396124380352
0.1018984889577683	0.2859396124380352
0.1018984889577683	0.286390265885534
0.10228593568384348	0.286390265885534
0.10228593568384348	0.2875168995042812
0.1030608291359938	0.2875168995042812
0.1030608291359938	0.28819287967552953
0.10325455249903139	0.28819287967552953
0.10325455249903139	0.28841820639927895
0.10364199922510654	0.28841820639927895
0.10364199922510654	0.2917981072555205
0.10383572258814414	0.2917981072555205
0.10383572258814414	0.29315006759801715
0.10402944595118171	0.29315006759801715
0.10402944595118171	0.29698062190175756
0.1042231693142193	0.29698062190175756
0.1042231693142193	0.2974312753492564
0.10441689267725687	0.2974312753492564
0.10441689267725687	0.2978819287967553
0.10461061604029447	0.2978819287967553
0.10461061604029447	0.2983325822442542
0.10480433940333204	0.2983325822442542
0.10480433940333204	0.2990085624155025
0.10499806276636962	0.2992338891392519
0.1053855094924448	0.2992338891392519
0.1053855094924448	0.29990986931050023
0.10557923285548237	0.29990986931050023
0.10557923285548237	0.30081117620549797
0.10577295621851995	0.30081117620549797
0.10577295621851995	0.3010365029292474
0.10596667958155753	0.3010365029292474
0.10596667958155753	0.302388463271744
0.10616040294459511	0.302388463271744
0.10616040294459511	0.3053177106804867
0.1063541263076327	0.3053177106804867
0.1063541263076327	0.30937359170797657
0.10654784967067028	0.30937359170797657
0.10654784967067028	0.313204146011717
0.10654784967067028	0.31365479945921587
0.10654784967067028	0.3152320865254619
0.10693529639674544	0.3152320865254619
0.10693529639674544	0.31726002703920686
0.10712901975978303	0.31726002703920686
0.10712901975978303	0.3181613339342046
0.10712901975978303	0.3186119873817035
0.10732274312282061	0.3186119873817035
0.10732274312282061	0.32154123479044616
0.10771018984889577	0.32154123479044616
0.10771018984889577	0.3226678684091933
0.10809763657497094	0.3226678684091933
0.10829135993800852	0.3226678684091933
0.10829135993800852	0.32424515547543936
0.1084850833010461	0.32424515547543936
0.1084850833010461	0.32469580892293826
0.1086788066640837	0.32469580892293826
0.1086788066640837	0.32514646237043715
0.10887253002712127	0.32514646237043715
0.10887253002712127	0.32830103650292924
0.10906625339015885	0.32830103650292924
0.10906625339015885	0.329202343397927
0.10925997675319643	0.329202343397927
0.10925997675319643	0.32942767012167645
0.10945370011623402	0.32942767012167645
0.10945370011623402	0.3305543037404236
0.10984114684230918	0.3305543037404236
0.10984114684230918	0.330779630464173
0.11003487020534676	0.330779630464173
0.11003487020534676	0.33258224425416855
0.11022859356838435	0.33258224425416855
0.11022859356838435	0.33370887787291575
0.11042231693142193	0.33370887787291575
0.11042231693142193	0.3341595313204146
0.11061604029445951	0.3341595313204146
0.11061604029445951	0.3346101847679135
0.11100348702053468	0.3346101847679135
0.11100348702053468	0.3348355114916629
0.11119721038357226	0.3348355114916629
0.11119721038357226	0.3355114916629112
0.11139093374660984	0.3355114916629112
0.11139093374660984	0.33641279855790895
0.11158465710964742	0.33641279855790895
0.11158465710964742	0.33708877872915727
0.11216582719876017	0.33708877872915727
0.11216582719876017	0.337990085624155
0.11235955056179775	0.337990085624155
0.11235955056179775	0.3382154123479045
0.11255327392483533	0.3382154123479045
0.11255327392483533	0.34001802613789994
0.11274699728787292	0.3402433528616494
0.1129407206509105	0.3402433528616494
0.1129407206509105	0.3409193330328977
0.11313444401394808	0.3409193330328977
0.11313444401394808	0.3424966200991438
0.11332816737698566	0.3424966200991438
0.11332816737698566	0.3427219468228932
0.11390933746609841	0.3427219468228932
0.11390933746609841	0.3431726002703921
0.11429678419217358	0.3431726002703921
0.11429678419217358	0.3438485804416404
0.11449050755521116	0.3438485804416404
0.11449050755521116	0.34429923388913924
0.11468423091824874	0.34429923388913924
0.11468423091824874	0.34474988733663814
0.11487795428128632	0.34474988733663814
0.11487795428128632	0.34497521406038756
0.11507167764432391	0.34497521406038756
0.11507167764432391	0.34565119423163587
0.11545912437039907	0.34565119423163587
0.11545912437039907	0.3465525011266336
0.11565284773343665	0.3465525011266336
0.11565284773343665	0.34745380802163134
0.11584657109647424	0.34745380802163134
0.11584657109647424	0.34790446146913023
0.11604029445951182	0.34790446146913023
0.11604029445951182	0.34880576836412797
0.11642774118558698	0.34880576836412797
0.11642774118558698	0.34970707525912575
0.11662146454862457	0.34970707525912575
0.11662146454862457	0.3499324019828752
0.11681518791166215	0.3499324019828752
0.11681518791166215	0.3501577287066246
0.1173963580007749	0.3501577287066246
0.1173963580007749	0.35038305543037407
0.11817125145292522	0.35038305543037407
0.11817125145292522	0.3506083821541235
0.11836497481596281	0.3506083821541235
0.11836497481596281	0.3508337088778729
0.11875242154203797	0.3508337088778729
0.11875242154203797	0.3512843623253718
0.11894614490507555	0.3512843623253718
0.11894614490507555	0.3515096890491212
0.11913986826811314	0.3515096890491212
0.11913986826811314	0.3519603424966201
0.11933359163115072	0.3519603424966201
0.11933359163115072	0.35241099594411895
0.11991476172026347	0.35241099594411895
0.11991476172026347	0.35286164939161785
0.12088337853545138	0.35286164939161785
0.12088337853545138	0.35308697611536727
0.12127082526152654	0.35308697611536727
0.12127082526152654	0.3537629562866156
0.12146454862456413	0.3537629562866156
0.12146454862456413	0.3542136097341145
0.12165827198760171	0.3542136097341145
0.12165827198760171	0.35691753041910773
0.12185199535063929	0.35691753041910773
0.12185199535063929	0.35714285714285715
0.12204571871367687	0.35714285714285715
0.12204571871367687	0.35781883731410546
0.12223944207671446	0.35781883731410546
0.12223944207671446	0.3584948174853538
0.12262688880278962	0.3584948174853538
0.12262688880278962	0.3587201442091032
0.12359550561797752	0.3587201442091032
0.12359550561797752	0.3591707976566021
0.1237892289810151	0.3591707976566021
0.1237892289810151	0.36029743127534924
0.1239829523440527	0.36029743127534924
0.1239829523440527	0.3605227579990987
0.12417667570709028	0.3605227579990987
0.12417667570709028	0.36097341144659756
0.12437039907012785	0.36097341144659756
0.12437039907012785	0.3616493916178459
0.12456412243316543	0.3616493916178459
0.12456412243316543	0.3618747183415953
0.1249515691592406	0.3618747183415953
0.1249515691592406	0.36210004506534477
0.12514529252227818	0.36210004506534477
0.12514529252227818	0.3623253717890942
0.12533901588531576	0.3623253717890942
0.12533901588531576	0.3627760252365931
0.12553273924835334	0.3627760252365931
0.12553273924835334	0.3632266786840919
0.12592018597442853	0.3632266786840919
0.12630763270050369	0.3632266786840919
0.127082526152654	0.3632266786840919
0.127082526152654	0.3636773321315908
0.12727624951569158	0.3636773321315908
0.12727624951569158	0.36457863902658855
0.12766369624176677	0.36457863902658855
0.12766369624176677	0.36502929247408744
0.12785741960480435	0.36502929247408744
0.12785741960480435	0.3659305993690852
0.12805114296784192	0.3659305993690852
0.12805114296784192	0.3661559260928346
0.1282448663308795	0.3661559260928346
0.1282448663308795	0.36638125281658407
0.12843858969391708	0.36638125281658407
0.12843858969391708	0.3670572329878324
0.12863231305695466	0.3670572329878324
0.12863231305695466	0.36773321315908064
0.12882603641999224	0.36773321315908064
0.12882603641999224	0.3679585398828301
0.12921348314606743	0.3679585398828301
0.12921348314606743	0.36885984677782785
0.129407206509105	0.36885984677782785
0.129407206509105	0.36998648039657506
0.12960092987214258	0.36998648039657506
0.12960092987214258	0.3702118071203245
0.12979465323518016	0.3702118071203245
0.12979465323518016	0.3704371338440739
0.12998837659821774	0.3704371338440739
0.12998837659821774	0.37066246056782337
0.13018209996125532	0.37066246056782337
0.13018209996125532	0.3708877872915728
0.1303758233242929	0.3708877872915728
0.1303758233242929	0.3711131140153222
0.13056954668733048	0.3711131140153222
0.13056954668733048	0.37133844073907163
0.13115071677644324	0.37133844073907163
0.13115071677644324	0.3715637674628211
0.13134444013948082	0.3715637674628211
0.13134444013948082	0.37201442091031994
0.13173188686555598	0.37201442091031994
0.13173188686555598	0.3722397476340694
0.13192561022859356	0.3722397476340694
0.13192561022859356	0.37246507435781884
0.13211933359163114	0.37246507435781884
0.13211933359163114	0.37336638125281657
0.13231305695466875	0.37336638125281657
0.13231305695466875	0.3749436683190626
0.13250678031770632	0.3749436683190626
0.13250678031770632	0.3751689950428121
0.13289422704378148	0.3751689950428121
0.13289422704378148	0.37561964849031093
0.13308795040681906	0.37561964849031093
0.13308795040681906	0.37697160883280756
0.13347539713289422	0.37697160883280756
0.13347539713289422	0.37719693555655703
0.13405656722200698	0.37719693555655703
0.13405656722200698	0.37742226228030645
0.13425029058504456	0.37742226228030645
0.13425029058504456	0.37809824245155477
0.13444401394808214	0.37809824245155477
0.13444401394808214	0.3785488958990536
0.1348314606741573	0.3785488958990536
0.1348314606741573	0.3787742226228031
0.13502518403719488	0.3787742226228031
0.13502518403719488	0.3792248760703019
0.13521890740023246	0.3792248760703019
0.13521890740023246	0.38102748986029744
0.13580007748934522	0.38102748986029744
0.13580007748934522	0.38170347003154576
0.1359938008523828	0.38170347003154576
0.1359938008523828	0.38237945020279407
0.13618752421542038	0.38237945020279407
0.13618752421542038	0.3826047769265435
0.13638124757845796	0.3826047769265435
0.13638124757845796	0.3830554303740424
0.13657497094149554	0.3830554303740424
0.13657497094149554	0.38485804416403785
0.13676869430453312	0.38485804416403785
0.13676869430453312	0.38508337088778727
0.1371561410306083	0.38508337088778727
0.1371561410306083	0.38530869761153674
0.13754358775668346	0.38530869761153674
0.13754358775668346	0.3862100045065345
0.13773731111972104	0.3862100045065345
0.13773731111972104	0.3864353312302839
0.13773731111972104	0.3868859846777828
0.13831848120883378	0.3868859846777828
0.13831848120883378	0.3871113114015322
0.13870592793490896	0.3871113114015322
0.13870592793490896	0.3877872915727805
0.13889965129794654	0.3877872915727805
0.13889965129794654	0.38801261829652994
0.1392870980240217	0.38801261829652994
0.1392870980240217	0.38936457863902657
0.13948082138705928	0.38936457863902657
0.13948082138705928	0.38958990536277605
0.13967454475009686	0.38958990536277605
0.13967454475009686	0.3911671924290221
0.13986826811313444	0.3911671924290221
0.13986826811313444	0.39274447949526814
0.13986826811313444	0.39319513294276703
0.14006199147617202	0.39319513294276703
0.14006199147617202	0.3936457863902659
0.14025571483920962	0.3936457863902659
0.14025571483920962	0.3949977467327625
0.1404494382022472	0.3949977467327625
0.1404494382022472	0.3954484001802614
0.14064316156528478	0.3954484001802614
0.14064316156528478	0.39634970707525913
0.14122433165439752	0.39634970707525913
0.14122433165439752	0.39702568724650744
0.14161177838047267	0.39702568724650744
0.14161177838047267	0.39747634069400634
0.14277411855869818	0.39747634069400634
0.14277411855869818	0.3981523208652546
0.1433552886478109	0.3981523208652546
0.1433552886478109	0.3986029743127535
0.14354901201084852	0.3986029743127535
0.14354901201084852	0.3992789544840018
0.1437427353738861	0.3992789544840018
0.1437427353738861	0.3997296079315007
0.14393645873692368	0.3997296079315007
0.14393645873692368	0.40085624155024785
0.14413018209996126	0.40085624155024785
0.14413018209996126	0.40108156827399727
0.14432390546299884	0.40108156827399727
0.14432390546299884	0.40265885534024337
0.14451762882603642	0.40265885534024337
0.14451762882603642	0.4028841820639928
0.144711352189074	0.4028841820639928
0.144711352189074	0.4031095087877422
0.14490507555211157	0.4031095087877422
0.14490507555211157	0.40401081568274
0.14509879891514918	0.40401081568274
0.14509879891514918	0.4042361424064894
0.14529252227818676	0.4042361424064894
0.14529252227818676	0.40446146913023884
0.14567996900426192	0.40446146913023884
0.14567996900426192	0.40513744930148715
0.1458736923672995	0.40513744930148715
0.1458736923672995	0.40536277602523657
0.14606741573033707	0.40536277602523657
0.14606741573033707	0.40626408292023436
0.14626113909337465	0.40626408292023436
0.14626113909337465	0.4069400630914827
0.14664858581944984	0.4069400630914827
0.14664858581944984	0.4071653898152321
0.14722975590856258	0.4071653898152321
0.14722975590856258	0.4073907165389815
0.14742347927160016	0.4073907165389815
0.14742347927160016	0.407616043262731
0.14761720263463773	0.407616043262731
0.14761720263463773	0.4080666967102298
0.1478109259976753	0.4080666967102298
0.1478109259976753	0.40919333032897703
0.1480046493607129	0.40919333032897703
0.1480046493607129	0.4096439837764759
0.14819837272375047	0.4096439837764759
0.14819837272375047	0.4103199639477242
0.14839209608678808	0.4103199639477242
0.14839209608678808	0.4121225777377197
0.14877954281286324	0.4121225777377197
0.14877954281286324	0.41234790446146913
0.14897326617590081	0.41234790446146913
0.14897326617590081	0.412798557908968
0.14936071290197597	0.412798557908968
0.14936071290197597	0.41324921135646686
0.14955443626501355	0.41324921135646686
0.14955443626501355	0.41347453808021634
0.14974815962805113	0.41347453808021634
0.14974815962805113	0.4148264984227129
0.14994188299108874	0.4148264984227129
0.14994188299108874	0.4157278053177107
0.15013560635412632	0.4157278053177107
0.15013560635412632	0.416403785488959
0.1503293297171639	0.416403785488959
0.1503293297171639	0.41753041910770616
0.15091049980627663	0.41753041910770616
0.15091049980627663	0.4182063992789545
0.1511042231693142	0.4182063992789545
0.1511042231693142	0.4188823794502028
0.1514916698953894	0.4188823794502028
0.1514916698953894	0.4197836863452005
0.15168539325842698	0.4197836863452005
0.15168539325842698	0.42000901306895
0.15187911662146455	0.42000901306895
0.15187911662146455	0.42045966651644884
0.15207283998450213	0.42045966651644884
0.15207283998450213	0.42091031996394773
0.1522665633475397	0.42091031996394773
0.1522665633475397	0.42136097341144657
0.1524602867105773	0.42136097341144657
0.1524602867105773	0.42181162685894547
0.15265401007361487	0.42181162685894547
0.15265401007361487	0.4229382604776927
0.15284773343665245	0.4229382604776927
0.15284773343665245	0.4245155475439387
0.15304145679969003	0.4245155475439387
0.15304145679969003	0.4256421811626859
0.15323518016272764	0.4256421811626859
0.15323518016272764	0.42654348805768366
0.1536226268888028	0.42654348805768366
0.1536226268888028	0.427219468228932
0.15401007361487795	0.427219468228932
0.15401007361487795	0.428796755295178
0.15420379697791553	0.428796755295178
0.15420379697791553	0.4310500225326724
0.1543975203409531	0.4310500225326724
0.1543975203409531	0.4312753492564218
0.1545912437039907	0.4312753492564218
0.1545912437039907	0.4319513294276701
0.15497869043006587	0.4319513294276701
0.15497869043006587	0.43217665615141954
0.15517241379310345	0.43217665615141954
0.15517241379310345	0.432401982875169
0.15536613715614103	0.432401982875169
0.15536613715614103	0.43352861649391616
0.1555598605191786	0.43352861649391616
0.1555598605191786	0.43397926994141506
0.1557535838822162	0.43397926994141506
0.1557535838822162	0.4342045966651645
0.15652847733436653	0.4342045966651645
0.15652847733436653	0.43442992338891395
0.1567222006974041	0.43442992338891395
0.1567222006974041	0.43465525011266337
0.1569159240604417	0.43465525011266337
0.1569159240604417	0.43645786390265884
0.15710964742347927	0.43645786390265884
0.15710964742347927	0.4366831906264083
0.15730337078651685	0.4366831906264083
0.15730337078651685	0.43690851735015773
0.157690817512592	0.43690851735015773
0.157690817512592	0.4373591707976566
0.15788454087562961	0.4373591707976566
0.15788454087562961	0.439612438035151
0.1580782642386672	0.439612438035151
0.1580782642386672	0.44118972510139703
0.15827198760170477	0.44118972510139703
0.15827198760170477	0.44141505182514645
0.15846571096474235	0.44141505182514645
0.15846571096474235	0.4416403785488959
0.15865943432777993	0.4416403785488959
0.15865943432777993	0.44254168544389366
0.1588531576908175	0.44254168544389366
0.1588531576908175	0.4427670121676431
0.15924060441689267	0.4427670121676431
0.15924060441689267	0.443217665615142
0.15962805114296785	0.443217665615142
0.15962805114296785	0.4434429923388914
0.15982177450600543	0.4434429923388914
0.15982177450600543	0.4436683190626408
0.160015497869043	0.4436683190626408
0.160015497869043	0.44434429923388913
0.1602092212320806	0.44434429923388913
0.1602092212320806	0.44524560612888686
0.16040294459511817	0.44524560612888686
0.16040294459511817	0.4465975664713835
0.16059666795815575	0.4465975664713835
0.16059666795815575	0.44885083370887785
0.1609841146842309	0.44885083370887785
0.1609841146842309	0.44930148715637674
0.1613715614103061	0.44930148715637674
0.1613715614103061	0.45042812077512395
0.16156528477334367	0.45042812077512395
0.16156528477334367	0.45200540784137
0.16195273149941883	0.45200540784137
0.16195273149941883	0.4522307345651194
0.1621464548624564	0.4522307345651194
0.1621464548624564	0.45245606128886884
0.162340178225494	0.45245606128886884
0.162340178225494	0.4533573681838666
0.16253390158853157	0.4533573681838666
0.16253390158853157	0.45358269490761605
0.16272762495156917	0.45358269490761605
0.16272762495156917	0.45380802163136547
0.16311507167764433	0.45380802163136547
0.16311507167764433	0.45425867507886436
0.16311507167764433	0.4547093285263632
0.1635025184037195	0.4547093285263632
0.1635025184037195	0.4553853086976115
0.16369624176675707	0.4553853086976115
0.16369624176675707	0.455610635421361
0.16408368849283222	0.455610635421361
0.16408368849283222	0.45741324921135645
0.16427741185586983	0.45741324921135645
0.16427741185586983	0.45786390265885535
0.1644711352189074	0.45786390265885535
0.1644711352189074	0.4589905362776025
0.164664858581945	0.4589905362776025
0.164664858581945	0.460793150067598
0.16485858194498257	0.460793150067598
0.16485858194498257	0.46146913023884634
0.16505230530802015	0.46146913023884634
0.16505230530802015	0.4630464173050924
0.16524602867105773	0.4630464173050924
0.16524602867105773	0.4632717440288418
0.1654397520340953	0.4632717440288418
0.1654397520340953	0.4641730509238396
0.16563347539713288	0.4641730509238396
0.16563347539713288	0.46575033799008564
0.16582719876017046	0.46575033799008564
0.16582719876017046	0.4662009914375845
0.16602092212320807	0.4662009914375845
0.16602092212320807	0.4673276250563317
0.16621464548624565	0.4673276250563317
0.16621464548624565	0.46845425867507884
0.16640836884928323	0.46845425867507884
0.16640836884928323	0.4711581793600721
0.1666020922123208	0.4711581793600721
0.1666020922123208	0.47138350608382157
0.16679581557535839	0.47138350608382157
0.16679581557535839	0.4725101397025687
0.16698953893839596	0.4725101397025687
0.16698953893839596	0.47408742676881477
0.16718326230143354	0.47408742676881477
0.16718326230143354	0.4756647138350608
0.16737698566447112	0.4756647138350608
0.16737698566447112	0.47634069400630913
0.16757070902750873	0.47634069400630913
0.16757070902750873	0.47746732762505634
0.1677644323905463	0.47769265434880576
0.1677644323905463	0.47814330779630465
0.1679581557535839	0.47814330779630465
0.1679581557535839	0.47881928796755296
0.16815187911662147	0.47881928796755296
0.16815187911662147	0.4808472284812979
0.16853932584269662	0.4808472284812979
0.16853932584269662	0.48129788192879674
0.1687330492057342	0.48129788192879674
0.1687330492057342	0.4821991888237945
0.16892677256877178	0.4821991888237945
0.16892677256877178	0.4833258224425417
0.1691204959318094	0.4833258224425417
0.1691204959318094	0.4837764758900406
0.16950794265788455	0.4837764758900406
0.16950794265788455	0.4853537629562866
0.16970166602092213	0.4853537629562866
0.16970166602092213	0.48557908968003605
0.1698953893839597	0.48557908968003605
0.1698953893839597	0.48602974312753494
0.17028283611003486	0.48602974312753494
0.17028283611003486	0.4882830103650293
0.17047655947307244	0.4882830103650293
0.17047655947307244	0.4885083370887787
0.17067028283611002	0.4885083370887787
0.17067028283611002	0.49053627760252366
0.17086400619914763	0.49053627760252366
0.17086400619914763	0.49098693105002256
0.17125145292522279	0.49098693105002256
0.17125145292522279	0.491212257773772
0.17125145292522279	0.4916629112212708
0.17125145292522279	0.4918882379450203
0.17144517628826036	0.4918882379450203
0.17144517628826036	0.49369085173501576
0.17163889965129794	0.49369085173501576
0.17163889965129794	0.49481748535376296
0.1720263463773731	0.49481748535376296
0.1720263463773731	0.4961694456962596
0.17222006974041068	0.4961694456962596
0.17222006974041068	0.496394772420009
0.17260751646648587	0.496394772420009
0.17260751646648587	0.49662009914375843
0.17280123982952345	0.49662009914375843
0.17280123982952345	0.49774673276250564
0.17280123982952345	0.49819738621000453
0.17280123982952345	0.5
0.17299496319256102	0.5
0.17299496319256102	0.5004506534474988
0.17338240991863618	0.5004506534474988
0.17338240991863618	0.5024785939612438
0.17357613328167376	0.5024785939612438
0.17357613328167376	0.5045065344749887
0.17396358000774895	0.5045065344749887
0.17396358000774895	0.5051825146462371
0.17415730337078653	0.5051825146462371
0.17415730337078653	0.5054078413699865
0.1743510267338241	0.5054078413699865
0.1743510267338241	0.5060838215412348
0.17454475009686168	0.5060838215412348
0.17454475009686168	0.5090130689499774
0.17473847345989926	0.5090130689499774
0.17473847345989926	0.5094637223974764
0.17493219682293684	0.5094637223974764
0.17493219682293684	0.5096890491212258
0.17570709027508719	0.5096890491212258
0.17570709027508719	0.5114916629112213
0.17590081363812476	0.5114916629112213
0.17590081363812476	0.5135196034249662
0.17609453700116234	0.5135196034249662
0.17609453700116234	0.5139702568724651
0.17628826036419992	0.5139702568724651
0.17628826036419992	0.5148715637674628
0.17667570709027508	0.5148715637674628
0.17667570709027508	0.51599819738621
0.17706315381635024	0.51599819738621
0.17706315381635024	0.5182514646237044
0.17725687717938785	0.5182514646237044
0.17725687717938785	0.5187021180712033
0.177644323905463	0.5187021180712033
0.177644323905463	0.5189274447949527
0.17803177063153816	0.5189274447949527
0.17803177063153816	0.5191527715187021
0.17822549399457574	0.5191527715187021
0.17822549399457574	0.519603424966201
0.17841921735761332	0.519603424966201
0.17841921735761332	0.5200540784136999
0.1786129407206509	0.5200540784136999
0.1786129407206509	0.5218566922036953
0.17900038744672608	0.5218566922036953
0.17900038744672608	0.5229833258224426
0.17919411080976366	0.5229833258224426
0.17919411080976366	0.5241099594411898
0.17996900426191398	0.5241099594411898
0.17996900426191398	0.5245606128886886
0.18035645098798916	0.5245606128886886
0.18035645098798916	0.524785939612438
0.18055017435102674	0.524785939612438
0.18055017435102674	0.5252365930599369
0.18074389771406432	0.5252365930599369
0.18074389771406432	0.5256872465074358
0.1809376210771019	0.5256872465074358
0.1809376210771019	0.526813880126183
0.18113134444013948	0.526813880126183
0.18113134444013948	0.5270392068499324
0.18151879116621464	0.5270392068499324
0.18151879116621464	0.5279405137449301
0.18171251452925222	0.5279405137449301
0.18171251452925222	0.5281658404686795
0.1820999612553274	0.5281658404686795
0.1820999612553274	0.5290671473636773
0.18248740798140256	0.5290671473636773
0.18248740798140256	0.5295178008111762
0.18287485470747772	0.5295178008111762
0.18287485470747772	0.5313204146011717
0.1830685780705153	0.5313204146011717
0.1830685780705153	0.5315457413249212
0.18326230143355288	0.5315457413249212
0.18326230143355288	0.5322217214961694
0.18384347152266564	0.5322217214961694
0.18384347152266564	0.5324470482199188
0.18442464161177838	0.5324470482199188
0.18442464161177838	0.5326723749436684
0.18461836497481596	0.5326723749436684
0.18461836497481596	0.5328977016674178
0.18481208833785354	0.5328977016674178
0.18481208833785354	0.5344749887336638
0.18500581170089112	0.5344749887336638
0.18500581170089112	0.5351509689049121
0.18519953506392872	0.5351509689049121
0.18519953506392872	0.5369535826949076
0.1853932584269663	0.5369535826949076
0.1853932584269663	0.5371789094186571
0.18558698179000388	0.5371789094186571
0.18558698179000388	0.5380802163136548
0.18597442851607904	0.5380802163136548
0.18597442851607904	0.5383055430374042
0.18616815187911662	0.5383055430374042
0.18616815187911662	0.5387561964849031
0.1863618752421542	0.5387561964849031
0.1863618752421542	0.5389815232086526
0.18655559860519177	0.5389815232086526
0.18655559860519177	0.5403334835511492
0.18713676869430454	0.5403334835511492
0.18713676869430454	0.5412347904461469
0.18733049205734212	0.5412347904461469
0.18733049205734212	0.5414601171698964
0.18810538550949243	0.5414601171698964
0.18810538550949243	0.5425867507886435
0.18829910887253	0.5425867507886435
0.18829910887253	0.5439387111311401
0.18849283223556762	0.5439387111311401
0.18849283223556762	0.5441640378548895
0.1886865555986052	0.5441640378548895
0.1886865555986052	0.5443893645786391
0.18888027896164278	0.5443893645786391
0.18888027896164278	0.5450653447498873
0.18984889577683067	0.5450653447498873
0.18984889577683067	0.5455159981973862
0.19023634250290586	0.5455159981973862
0.19023634250290586	0.5457413249211357
0.19043006586594344	0.5457413249211357
0.19043006586594344	0.546417305092384
0.19062378922898102	0.546417305092384
0.19062378922898102	0.5466426318161334
0.1908175125920186	0.5466426318161334
0.1908175125920186	0.5482199188823794
0.19101123595505617	0.5482199188823794
0.19101123595505617	0.5484452456061288
0.19120495931809375	0.5484452456061288
0.19120495931809375	0.5488958990536278
0.19139868268113133	0.5488958990536278
0.19139868268113133	0.5497972059486255
0.19178612940720652	0.5497972059486255
0.19178612940720652	0.5506985128436233
0.1919798527702441	0.5506985128436233
0.1919798527702441	0.5511491662911221
0.19217357613328168	0.5511491662911221
0.19217357613328168	0.5520504731861199
0.19256102285935683	0.5520504731861199
0.19256102285935683	0.5529517800811177
0.1927547462223944	0.5529517800811177
0.1927547462223944	0.5531771068048671
0.192948469585432	0.5531771068048671
0.192948469585432	0.555205047318612
0.1931421929484696	0.555205047318612
0.1931421929484696	0.5556557007661108
0.19333591631150718	0.5556557007661108
0.19333591631150718	0.5558810274898603
0.19352963967454476	0.5558810274898603
0.19352963967454476	0.556782334384858
0.19391708640061991	0.556782334384858
0.19391708640061991	0.5570076611086074
0.19449825648973265	0.5570076611086074
0.19449825648973265	0.5574583145561064
0.19488570321580784	0.5574583145561064
0.19488570321580784	0.5579089680036052
0.19507942657884542	0.5579089680036052
0.19507942657884542	0.5583596214511041
0.19566059666795815	0.5583596214511041
0.19566059666795815	0.5590356016223524
0.19585432003099573	0.5590356016223524
0.19585432003099573	0.5592609283461019
0.1962417667570709	0.5592609283461019
0.1962417667570709	0.5597115817936007
0.1964354901201085	0.5597115817936007
0.1964354901201085	0.5599369085173501
0.19682293684618365	0.5599369085173501
0.19682293684618365	0.5601622352410996
0.1974041069352964	0.5601622352410996
0.1974041069352964	0.5603875619648491
0.19779155366137155	0.5603875619648491
0.19779155366137155	0.5615141955835962
0.19817900038744674	0.5615141955835962
0.19817900038744674	0.5621901757548445
0.19837272375048431	0.5621901757548445
0.19837272375048431	0.5626408292023434
0.19876017047655947	0.5626408292023434
0.19876017047655947	0.5630914826498423
0.19895389383959705	0.5630914826498423
0.19895389383959705	0.5635421360973412
0.19914761720263463	0.5635421360973412
0.19914761720263463	0.5648940964398378
0.1993413405656722	0.5648940964398378
0.1993413405656722	0.565570076611086
0.19953506392870982	0.565570076611086
0.19953506392870982	0.566020730058585
0.19992251065478497	0.566020730058585
0.19992251065478497	0.5662460567823344
0.20108485083301045	0.5662460567823344
0.20108485083301045	0.5671473636773321
0.20127857419604805	0.5671473636773321
0.20127857419604805	0.567598017124831
0.2016660209221232	0.567598017124831
0.2016660209221232	0.5682739972960793
0.2018597442851608	0.5682739972960793
0.2018597442851608	0.5684993240198287
0.20205346764819837	0.5684993240198287
0.20205346764819837	0.5687246507435781
0.20224719101123595	0.5687246507435781
0.20224719101123595	0.5698512843623253
0.2026346377373111	0.5698512843623253
0.2026346377373111	0.5700766110860748
0.20340953118946145	0.5700766110860748
0.20340953118946145	0.5705272645335737
0.2037969779155366	0.5705272645335737
0.2037969779155366	0.5707525912573231
0.20476559473072453	0.5707525912573231
0.20476559473072453	0.5709779179810726
0.20554048818287485	0.5709779179810726
0.20554048818287485	0.571203244704822
0.20592793490895	0.571203244704822
0.20592793490895	0.5714285714285714
0.2061216582719876	0.5714285714285714
0.2061216582719876	0.5716538981523208
0.2063153816350252	0.5716538981523208
0.2063153816350252	0.5721045515998198
0.20670282836110035	0.5721045515998198
0.20670282836110035	0.5723298783235692
0.20689655172413793	0.5723298783235692
0.20689655172413793	0.572780531771068
0.20747772181325067	0.572780531771068
0.20747772181325067	0.573231185218567
0.20786516853932585	0.573231185218567
0.20786516853932585	0.5736818386660658
0.208252615265401	0.5736818386660658
0.208252615265401	0.5743578188373141
0.20864006199147617	0.5743578188373141
0.20864006199147617	0.574808472284813
0.20902750871755132	0.574808472284813
0.20902750871755132	0.5754844524560613
0.2096086788066641	0.5754844524560613
0.2096086788066641	0.5757097791798107
0.21018984889577683	0.5757097791798107
0.21018984889577683	0.5761604326273096
0.21057729562185198	0.5761604326273096
0.21057729562185198	0.5763857593510591
0.21096474234792717	0.5763857593510591
0.21096474234792717	0.5772870662460567
0.21115846571096475	0.5772870662460567
0.21115846571096475	0.5775123929698062
0.21135218907400233	0.5777377196935557
0.21173963580007749	0.5777377196935557
0.21173963580007749	0.578413699864804
0.21193335916311506	0.578413699864804
0.21193335916311506	0.5795403334835512
0.21212708252615264	0.5795403334835512
0.21212708252615264	0.5797656602073006
0.21309569934134057	0.5797656602073006
0.21309569934134057	0.57999098693105
0.21425803951956607	0.57999098693105
0.21425803951956607	0.580441640378549
0.21445176288260365	0.580441640378549
0.21445176288260365	0.5808922938260478
0.2148392096086788	0.5808922938260478
0.2148392096086788	0.5813429472735466
0.21503293297171638	0.5813429472735466
0.21503293297171638	0.581568273997296
0.21522665633475396	0.581568273997296
0.21522665633475396	0.582018927444795
0.21561410306082915	0.582018927444795
0.21561410306082915	0.5826949076160433
0.2160015497869043	0.5826949076160433
0.2160015497869043	0.5829202343397927
0.21619527314994189	0.5829202343397927
0.21619527314994189	0.5831455610635421
0.21658271987601704	0.5831455610635421
0.21658271987601704	0.583596214511041
0.21677644323905462	0.583596214511041
0.21677644323905462	0.5838215412347905
0.2169701666020922	0.5838215412347905
0.2169701666020922	0.5847228481297881
0.21774506005424255	0.5847228481297881
0.21774506005424255	0.5860748084722848
0.21793878341728012	0.5860748084722848
0.21793878341728012	0.5863001351960343
0.2181325067803177	0.5863001351960343
0.2181325067803177	0.5867507886435331
0.21871367686943044	0.5867507886435331
0.21871367686943044	0.587201442091032
0.21890740023246805	0.587201442091032
0.21890740023246805	0.5878774222622803
0.2192948469585432	0.5878774222622803
0.2192948469585432	0.5883280757097792
0.21968229368461836	0.5883280757097792
0.21968229368461836	0.5885534024335286
0.22006974041069352	0.5885534024335286
0.22006974041069352	0.588778729157278
0.2202634637737311	0.588778729157278
0.2202634637737311	0.589229382604777
0.2204571871367687	0.589229382604777
0.2204571871367687	0.5896800360522758
0.22065091049980629	0.5896800360522758
0.22065091049980629	0.5905813429472736
0.22103835722588144	0.5905813429472736
0.22103835722588144	0.590806669671023
0.2214258039519566	0.590806669671023
0.2214258039519566	0.5910319963947724
0.22161952731499418	0.5910319963947724
0.22161952731499418	0.5914826498422713
0.22200697404106937	0.5914826498422713
0.22200697404106937	0.5919333032897701
0.22239442076714452	0.5919333032897701
0.22239442076714452	0.5923839567372691
0.2225881441301821	0.5923839567372691
0.2225881441301821	0.5926092834610185
0.22278186749321968	0.5926092834610185
0.22278186749321968	0.5930599369085173
0.22297559085625726	0.5930599369085173
0.22297559085625726	0.5935105903560163
0.22336303758233242	0.5935105903560163
0.22336303758233242	0.5937359170797657
0.22355676094537	0.5937359170797657
0.22355676094537	0.5941865705272645
0.2237504843084076	0.5941865705272645
0.2237504843084076	0.594411897251014
0.22413793103448276	0.594411897251014
0.22413793103448276	0.5948625506985128
0.22433165439752034	0.5948625506985128
0.22433165439752034	0.59598918431726
0.22452537776055792	0.59598918431726
0.22452537776055792	0.5966651644885084
0.2247191011235955	0.5966651644885084
0.2247191011235955	0.5971158179360072
0.22491282448663308	0.5971158179360072
0.22491282448663308	0.5973411446597566
0.22530027121270826	0.5973411446597566
0.22530027121270826	0.598017124831005
0.22549399457574584	0.598017124831005
0.22549399457574584	0.5982424515547544
0.22568771793878342	0.5982424515547544
0.22568771793878342	0.5989184317260027
0.22607516466485858	0.5989184317260027
0.22607516466485858	0.5991437584497521
0.22626888802789616	0.5991437584497521
0.22626888802789616	0.5993690851735016
0.22646261139093374	0.5993690851735016
0.22646261139093374	0.5998197386210005
0.22665633475397132	0.5998197386210005
0.22665633475397132	0.6007210455159981
0.22723750484308408	0.6007210455159981
0.22723750484308408	0.6016223524109959
0.22781867493219682	0.6016223524109959
0.22781867493219682	0.6018476791347454
0.2280123982952344	0.6018476791347454
0.2280123982952344	0.6020730058584948
0.22820612165827198	0.6020730058584948
0.22820612165827198	0.6022983325822443
0.22839984502130958	0.6022983325822443
0.22839984502130958	0.6027489860297431
0.22859356838434716	0.6027489860297431
0.22859356838434716	0.6029743127534926
0.22936846183649748	0.6029743127534926
0.22936846183649748	0.6038756196484903
0.22994963192561022	0.6038756196484903
0.22994963192561022	0.6041009463722398
0.23014335528864782	0.6041009463722398
0.23014335528864782	0.6045515998197386
0.2303370786516854	0.6045515998197386
0.2303370786516854	0.6050022532672374
0.23111197210383572	0.6050022532672374
0.23111197210383572	0.605227579990987
0.2313056954668733	0.605227579990987
0.2313056954668733	0.6054529067147364
0.23149941882991087	0.6054529067147364
0.23149941882991087	0.6059035601622352
0.23188686555598606	0.6059035601622352
0.23188686555598606	0.6061288868859847
0.2324680356450988	0.6061288868859847
0.2324680356450988	0.606804867057233
0.23266175900813638	0.606804867057233
0.23266175900813638	0.6070301937809824
0.23285548237117396	0.6070301937809824
0.23285548237117396	0.6077061739522307
0.23324292909724914	0.6077061739522307
0.23324292909724914	0.6086074808472285
0.23343665246028672	0.6086074808472285
0.23343665246028672	0.6090581342947273
0.2336303758233243	0.6090581342947273
0.2336303758233243	0.6092834610184767
0.23382409918636188	0.6092834610184767
0.23382409918636188	0.6095087877422263
0.23421154591243704	0.6095087877422263
0.23421154591243704	0.6097341144659757
0.23440526927547461	0.6097341144659757
0.23440526927547461	0.6099594411897251
0.2345989926385122	0.6099594411897251
0.2345989926385122	0.6101847679134745
0.2347927160015498	0.6101847679134745
0.2347927160015498	0.610410094637224
0.23498643936458738	0.610410094637224
0.23498643936458738	0.6106354213609734
0.23518016272762496	0.6106354213609734
0.23518016272762496	0.6108607480847228
0.23537388609066254	0.6108607480847228
0.23537388609066254	0.6110860748084723
0.2357613328167377	0.6110860748084723
0.2357613328167377	0.6117620549797206
0.23614877954281285	0.6117620549797206
0.23614877954281285	0.61198738170347
0.2369236729949632	0.61198738170347
0.2369236729949632	0.612438035150969
0.23711739635800078	0.612438035150969
0.23711739635800078	0.6126633618747184
0.23731111972103835	0.6126633618747184
0.23731111972103835	0.6131140153222172
0.2378922898101511	0.6131140153222172
0.2378922898101511	0.6133393420459666
0.2380860131731887	0.6133393420459666
0.2380860131731887	0.614015322217215
0.23827973653622628	0.614015322217215
0.23827973653622628	0.6144659756647138
0.2390546299883766	0.6144659756647138
0.2390546299883766	0.615592609283461
0.23944207671445175	0.615592609283461
0.23944207671445175	0.6158179360072105
0.23982952344052694	0.6158179360072105
0.23982952344052694	0.6160432627309599
0.24002324680356452	0.6160432627309599
0.24002324680356452	0.6169445696259577
0.24041069352963967	0.6169445696259577
0.24041069352963967	0.6171698963497071
0.24060441689267725	0.6171698963497071
0.24060441689267725	0.6173952230734565
0.2409918636187524	0.6173952230734565
0.2409918636187524	0.6176205497972059
0.24118558698179	0.6176205497972059
0.24118558698179	0.6194231635872014
0.24176675707090275	0.6194231635872014
0.24176675707090275	0.6200991437584498
0.2423479271600155	0.6200991437584498
0.2423479271600155	0.6203244704821992
0.243510267338241	0.6203244704821992
0.243510267338241	0.620775123929698
0.24370399070127857	0.620775123929698
0.24370399070127857	0.6219017575484452
0.24389771406431615	0.6219017575484452
0.24389771406431615	0.6223524109959441
0.24409143742735373	0.6223524109959441
0.24409143742735373	0.622803064443443
0.2442851607903913	0.622803064443443
0.2442851607903913	0.6234790446146913
0.24525377760557923	0.6234790446146913
0.24525377760557923	0.6237043713384407
0.24583494769469197	0.6237043713384407
0.24583494769469197	0.6241550247859396
0.24602867105772958	0.6241550247859396
0.24602867105772958	0.6248310049571879
0.24641611778380473	0.6248310049571879
0.24641611778380473	0.6252816584046867
0.2489345215032933	0.6252816584046867
0.2489345215032933	0.6257323118521857
0.24912824486633087	0.6257323118521857
0.24912824486633087	0.6259576385759351
0.24970941495544363	0.6259576385759351
0.24970941495544363	0.6261829652996845
0.25029058504455637	0.6261829652996845
0.25029058504455637	0.626408292023434
0.25048430840759395	0.626408292023434
0.25048430840759395	0.6268589454709329
0.2506780317706315	0.6268589454709329
0.2506780317706315	0.6270842721946823
0.2508717551336691	0.6270842721946823
0.2508717551336691	0.6275349256421812
0.2510654784967067	0.6275349256421812
0.2510654784967067	0.6277602523659306
0.25145292522278184	0.6277602523659306
0.25145292522278184	0.62798557908968
0.25184037194885706	0.62798557908968
0.25184037194885706	0.6282109058134294
0.2522278186749322	0.6282109058134294
0.2522278186749322	0.6288868859846778
0.25261526540100737	0.6288868859846778
0.25261526540100737	0.6291122127084272
0.25358388221619527	0.6291122127084272
0.25358388221619527	0.6302388463271744
0.25377760557923285	0.6302388463271744
0.25377760557923285	0.6304641730509238
0.2539713289422704	0.6304641730509238
0.2539713289422704	0.6309148264984227
0.25455249903138316	0.6309148264984227
0.25455249903138316	0.6311401532221721
0.25610228593568385	0.6311401532221721
0.25610228593568385	0.6313654799459216
0.25629600929872143	0.6313654799459216
0.25629600929872143	0.6318161333934205
0.256489732661759	0.6318161333934205
0.256489732661759	0.6320414601171699
0.25707090275087174	0.6320414601171699
0.25707090275087174	0.6322667868409193
0.2576520728399845	0.6322667868409193
0.2576520728399845	0.6327174402884183
0.25784579620302206	0.6327174402884183
0.25784579620302206	0.6329427670121677
0.2580395195660597	0.6329427670121677
0.2580395195660597	0.6340694006309149
0.25862068965517243	0.6340694006309149
0.25862068965517243	0.6342947273546643
0.2590081363812476	0.6342947273546643
0.2590081363812476	0.6349707075259126
0.25920185974428517	0.6349707075259126
0.25920185974428517	0.6354213609734114
0.26017047655947306	0.6354213609734114
0.26017047655947306	0.6356466876971609
0.26036419992251064	0.6356466876971609
0.26036419992251064	0.6358720144209103
0.2605579232855482	0.6358720144209103
0.2605579232855482	0.6365479945921586
0.2607516466485858	0.6365479945921586
0.2607516466485858	0.6369986480396576
0.2613328167376986	0.6369986480396576
0.2613328167376986	0.637223974763407
0.26152654010073617	0.637223974763407
0.26152654010073617	0.6378999549346552
0.26172026346377375	0.6378999549346552
0.26172026346377375	0.6381252816584047
0.2621077101898489	0.6381252816584047
0.2621077101898489	0.6383506083821541
0.26268888027896165	0.6383506083821541
0.26268888027896165	0.6385759351059036
0.2630763270050368	0.6385759351059036
0.2630763270050368	0.638801261829653
0.26365749709414954	0.638801261829653
0.26365749709414954	0.6390265885534024
0.2638512204571871	0.6390265885534024
0.2638512204571871	0.6392519152771519
0.2644323905462999	0.6392519152771519
0.2644323905462999	0.6397025687246507
0.26481983727237507	0.6397025687246507
0.26481983727237507	0.6401532221721496
0.2654010073614878	0.6401532221721496
0.2654010073614878	0.6403785488958991
0.2655947307245254	0.6403785488958991
0.2655947307245254	0.6408292023433979
0.26578845408756296	0.6408292023433979
0.26578845408756296	0.6410545290671473
0.2661759008136381	0.6410545290671473
0.2661759008136381	0.6412798557908967
0.26695079426578844	0.6412798557908967
0.26695079426578844	0.6417305092383957
0.2673382409918636	0.6417305092383957
0.2673382409918636	0.6426318161333934
0.2675319643549012	0.6426318161333934
0.2675319643549012	0.6433077963046417
0.2698566447113522	0.6433077963046417
0.2698566447113522	0.64398377647589
0.27005036807438976	0.64398377647589
0.27005036807438976	0.6442091031996395
0.27024409143742734	0.6442091031996395
0.27024409143742734	0.644434429923389
0.27160015497869044	0.644434429923389
0.27160015497869044	0.6446597566471384
0.2719876017047656	0.6446597566471384
0.2719876017047656	0.6448850833708878
0.27237504843084076	0.6448850833708878
0.27237504843084076	0.6451104100946372
0.2727624951569159	0.6451104100946372
0.2727624951569159	0.6453357368183866
0.2729562185199535	0.6453357368183866
0.2729562185199535	0.645561063542136
0.27334366524602866	0.645561063542136
0.27334366524602866	0.6457863902658856
0.27353738860906623	0.6457863902658856
0.27353738860906623	0.6464623704371338
0.2737311119721038	0.6464623704371338
0.2737311119721038	0.6466876971608833
0.2739248353351414	0.6466876971608833
0.2739248353351414	0.6469130238846327
0.2743122820612166	0.6469130238846327
0.2743122820612166	0.6471383506083822
0.2750871755133669	0.6471383506083822
0.2750871755133669	0.6482649842271293
0.2752808988764045	0.6482649842271293
0.2752808988764045	0.6489409643983777
0.27586206896551724	0.6489409643983777
0.27586206896551724	0.6491662911221271
0.2760557923285548	0.6491662911221271
0.2760557923285548	0.6493916178458765
0.27683068578070513	0.6493916178458765
0.27683068578070513	0.6498422712933754
0.2772181325067803	0.6498422712933754
0.2772181325067803	0.6500675980171249
0.2777993025958931	0.6500675980171249
0.2777993025958931	0.6502929247408743
0.2785741960480434	0.6502929247408743
0.2785741960480434	0.6505182514646237
0.27915536613715614	0.6505182514646237
0.27915536613715614	0.6518702118071203
0.2793490895001937	0.6518702118071203
0.2793490895001937	0.6520955385308698
0.2795428128632313	0.6520955385308698
0.2795428128632313	0.6523208652546192
0.27993025958930645	0.6523208652546192
0.27993025958930645	0.6525461919783686
0.28012398295234403	0.6525461919783686
0.28012398295234403	0.652771518702118
0.2803177063153816	0.652771518702118
0.2803177063153816	0.653222172149617
0.28051142967841924	0.653222172149617
0.28051142967841924	0.6534474988733664
0.2807051530414568	0.6534474988733664
0.2807051530414568	0.6538981523208652
0.2808988764044944	0.6538981523208652
0.2808988764044944	0.6541234790446147
0.28128632313056956	0.6541234790446147
0.28128632313056956	0.6545741324921136
0.2820612165827199	0.6545741324921136
0.2820612165827199	0.654799459215863
0.2826423866718326	0.654799459215863
0.2826423866718326	0.6557007661108607
0.28322355676094535	0.6557007661108607
0.28322355676094535	0.6559260928346102
0.28341728012398293	0.6559260928346102
0.28341728012398293	0.6568273997296079
0.2836110034870205	0.6568273997296079
0.2836110034870205	0.6575033799008563
0.28380472685005814	0.6575033799008563
0.28380472685005814	0.6577287066246057
0.2839984502130957	0.6577287066246057
0.2839984502130957	0.6579540333483551
0.2841921735761333	0.6579540333483551
0.2841921735761333	0.6581793600721045
0.28477334366524604	0.6581793600721045
0.28477334366524604	0.658404686795854
0.2849670670282836	0.658404686795854
0.2849670670282836	0.6586300135196034
0.28554823711739635	0.6586300135196034
0.28554823711739635	0.6588553402433529
0.2861294072065091	0.6588553402433529
0.2861294072065091	0.6595313204146012
0.28632313056954667	0.6595313204146012
0.28632313056954667	0.6597566471383506
0.28651685393258425	0.6597566471383506
0.28651685393258425	0.6599819738621
0.2867105772956218	0.6599819738621
0.2867105772956218	0.6602073005858495
0.2874854707477722	0.6602073005858495
0.2874854707477722	0.660432627309599
0.2876791941108098	0.660432627309599
0.2876791941108098	0.6608832807570978
0.28806664083688494	0.6608832807570978
0.28806664083688494	0.6611086074808472
0.2882603641999225	0.6611086074808472
0.2882603641999225	0.6613339342045966
0.2884540875629601	0.6613339342045966
0.2884540875629601	0.661559260928346
0.28864781092599767	0.661559260928346
0.28864781092599767	0.662009914375845
0.289422704378148	0.662009914375845
0.289422704378148	0.6624605678233438
0.2900038744672607	0.6624605678233438
0.2900038744672607	0.6626858945470933
0.29039132119333594	0.6626858945470933
0.29039132119333594	0.6631365479945922
0.2907787679194111	0.6631365479945922
0.2907787679194111	0.6638125281658405
0.2909724912824487	0.6638125281658405
0.2909724912824487	0.6644885083370887
0.29135993800852383	0.6644885083370887
0.29135993800852383	0.6649391617845877
0.2915536613715614	0.6649391617845877
0.2915536613715614	0.6653898152320865
0.2927160015497869	0.6653898152320865
0.2927160015497869	0.6656151419558359
0.29290972491282447	0.6656151419558359
0.29290972491282447	0.6658404686795854
0.29349089500193726	0.6658404686795854
0.29349089500193726	0.6660657954033349
0.2942657884540876	0.6660657954033349
0.2942657884540876	0.6665164488508337
0.29465323518016273	0.6665164488508337
0.29465323518016273	0.667192429022082
0.2950406819062379	0.667192429022082
0.2950406819062379	0.6674177557458315
0.29523440526927547	0.6674177557458315
0.29523440526927547	0.6678684091933303
0.2956218519953506	0.6678684091933303
0.2956218519953506	0.6685443893645786
0.2960092987214258	0.6685443893645786
0.2960092987214258	0.668769716088328
0.29620302208446336	0.668769716088328
0.29620302208446336	0.669220369535827
0.29639674544750094	0.669220369535827
0.29639674544750094	0.6696710229833258
0.29697791553661373	0.6696710229833258
0.29697791553661373	0.6705723298783236
0.2973653622626889	0.6705723298783236
0.2973653622626889	0.670797656602073
0.29755908562572647	0.670797656602073
0.29755908562572647	0.6714736367733213
0.29794653235180163	0.6714736367733213
0.29794653235180163	0.6719242902208202
0.29852770244091437	0.6719242902208202
0.29852770244091437	0.6721496169445697
0.29872142580395195	0.6721496169445697
0.29872142580395195	0.6723749436683191
0.2991088725300271	0.6723749436683191
0.2991088725300271	0.6726002703920685
0.2996900426191399	0.6726002703920685
0.2996900426191399	0.6728255971158179
0.30007748934521505	0.6728255971158179
0.30007748934521505	0.6737269040108157
0.30027121270825263	0.6737269040108157
0.30027121270825263	0.6739522307345651
0.3006586594343278	0.6739522307345651
0.3006586594343278	0.6741775574583145
0.30104610616040295	0.6741775574583145
0.30104610616040295	0.674402884182064
0.3012398295234405	0.674402884182064
0.3012398295234405	0.6746282109058134
0.3016272762495157	0.6746282109058134
0.3016272762495157	0.6748535376295629
0.30201472297559084	0.6748535376295629
0.30201472297559084	0.6750788643533123
0.3022084463386284	0.6750788643533123
0.3022084463386284	0.6753041910770617
0.302402169701666	0.6753041910770617
0.302402169701666	0.6757548445245606
0.3037582332429291	0.6757548445245606
0.3037582332429291	0.67598017124831
0.30414567996900427	0.67598017124831
0.30414567996900427	0.6762054979720595
0.304726850058117	0.6762054979720595
0.304726850058117	0.676430824695809
0.30511429678419216	0.676430824695809
0.30511429678419216	0.6771068048670572
0.3058891902363425	0.6771068048670572
0.3058891902363425	0.6777827850383056
0.3062766369624177	0.6777827850383056
0.3062766369624177	0.6782334384858044
0.30666408368849285	0.6782334384858044
0.30666408368849285	0.6784587652095538
0.30685780705153043	0.6784587652095538
0.30685780705153043	0.6786840919333033
0.3087950406819062	0.6786840919333033
0.3087950406819062	0.6791347453808022
0.3091824874079814	0.6791347453808022
0.3091824874079814	0.679585398828301
0.3095699341340566	0.679585398828301
0.3095699341340566	0.6800360522757999
0.3101511042231693	0.6800360522757999
0.3101511042231693	0.6802613789995493
0.3105385509492445	0.6802613789995493
0.3105385509492445	0.6804867057232988
0.31073227431228206	0.6804867057232988
0.31073227431228206	0.6807120324470483
0.3115071677644324	0.6807120324470483
0.3115071677644324	0.6811626858945471
0.31189461449050754	0.6811626858945471
0.31189461449050754	0.6813880126182965
0.3128632313056955	0.6813880126182965
0.3128632313056955	0.6820639927895449
0.3134444013948082	0.6820639927895449
0.3134444013948082	0.6825146462370437
0.3136381247578458	0.6825146462370437
0.3136381247578458	0.683190626408292
0.3138318481208834	0.683190626408292
0.3138318481208834	0.6834159531320415
0.31421929484695854	0.6834159531320415
0.31421929484695854	0.6836412798557909
0.3148004649360713	0.6836412798557909
0.3148004649360713	0.6838666065795403
0.31518791166214644	0.6838666065795403
0.31518791166214644	0.6840919333032898
0.315381635025184	0.6840919333032898
0.315381635025184	0.6843172600270392
0.3155753583882216	0.6843172600270392
0.3155753583882216	0.6845425867507886
0.31576908175125923	0.6845425867507886
0.31576908175125923	0.684767913474538
0.3161565284773344	0.684767913474538
0.3161565284773344	0.6849932401982876
0.31654397520340954	0.6849932401982876
0.31654397520340954	0.685218566922037
0.3169314219294847	0.685218566922037
0.3169314219294847	0.6854438936457864
0.3179000387446726	0.6854438936457864
0.3179000387446726	0.6858945470932852
0.3180937621077102	0.6858945470932852
0.3180937621077102	0.6863452005407842
0.31848120883378533	0.6863452005407842
0.31848120883378533	0.686795853988283
0.3192561022859357	0.686795853988283
0.3192561022859357	0.6872465074357819
0.31983727237504844	0.6872465074357819
0.31983727237504844	0.6876971608832808
0.320030995738086	0.6876971608832808
0.320030995738086	0.6885984677782785
0.3204184424641612	0.6885984677782785
0.3204184424641612	0.6888237945020279
0.3209996125532739	0.6888237945020279
0.3209996125532739	0.6892744479495269
0.3211933359163115	0.6892744479495269
0.3211933359163115	0.6894997746732763
0.32158078264238665	0.6894997746732763
0.32158078264238665	0.6897251013970257
0.322355676094537	0.6897251013970257
0.322355676094537	0.6899504281207751
0.3227431228206122	0.6899504281207751
0.3227431228206122	0.6901757548445245
0.3235180162727625	0.6901757548445245
0.3235180162727625	0.6906264082920235
0.3237117396358001	0.6906264082920235
0.3237117396358001	0.6908517350157729
0.3242929097249128	0.6908517350157729
0.3242929097249128	0.692429022082019
0.324680356450988	0.692429022082019
0.324680356450988	0.6928796755295178
0.32506780317706313	0.6928796755295178
0.32506780317706313	0.6931050022532672
0.32545524990313834	0.6931050022532672
0.32545524990313834	0.6933303289770166
0.3256489732661759	0.6933303289770166
0.3256489732661759	0.6935556557007662
0.3258426966292135	0.6935556557007662
0.3258426966292135	0.694006309148265
0.32623014335528866	0.694006309148265
0.32623014335528866	0.6942316358720144
0.3268113134444014	0.6942316358720144
0.3268113134444014	0.6944569625957638
0.32816737698566445	0.6944569625957638
0.32816737698566445	0.6946822893195133
0.32836110034870203	0.6946822893195133
0.32836110034870203	0.6951329427670122
0.32874854707477724	0.6951329427670122
0.32874854707477724	0.6958089229382605
0.32971716388996514	0.6958089229382605
0.32971716388996514	0.6969355565570077
0.3302983339790779	0.6969355565570077
0.3302983339790779	0.6971608832807571
0.33049205734211545	0.6971608832807571
0.33049205734211545	0.6978368634520055
0.3308795040681906	0.6978368634520055
0.3308795040681906	0.6980621901757549
0.3322355676094537	0.6980621901757549
0.3322355676094537	0.6989634970707526
0.3324292909724913	0.6989634970707526
0.3324292909724913	0.699188823794502
0.33359163115071677	0.699188823794502
0.33359163115071677	0.7000901306894998
0.3341728012398295	0.7000901306894998
0.3341728012398295	0.7003154574132492
0.3343665246028671	0.7003154574132492
0.3343665246028671	0.7005407841369986
0.33456024796590467	0.7005407841369986
0.33456024796590467	0.7007661108607481
0.33475397132894225	0.7007661108607481
0.33475397132894225	0.7016674177557458
0.3349476946919799	0.7016674177557458
0.3349476946919799	0.7018927444794952
0.33533514141805504	0.7018927444794952
0.33533514141805504	0.7025687246507436
0.3355288647810926	0.7025687246507436
0.3355288647810926	0.7032447048219919
0.33630375823324293	0.7032447048219919
0.33630375823324293	0.7036953582694908
0.3366912049593181	0.7036953582694908
0.3366912049593181	0.7039206849932402
0.33707865168539325	0.7039206849932402
0.33707865168539325	0.7043713384407391
0.337659821774506	0.7043713384407391
0.337659821774506	0.7045966651644885
0.33785354513754356	0.7045966651644885
0.33785354513754356	0.7052726453357369
0.33804726850058114	0.7052726453357369
0.33804726850058114	0.706399278954484
0.33862843858969394	0.706399278954484
0.33862843858969394	0.7066246056782335
0.3392096086788067	0.7066246056782335
0.3392096086788067	0.7068499324019829
0.3405656722200697	0.7068499324019829
0.3405656722200697	0.7070752591257323
0.3409531189461449	0.7070752591257323
0.3409531189461449	0.7075259125732312
0.34114684230918246	0.7075259125732312
0.34114684230918246	0.7077512392969806
0.34134056567222004	0.7077512392969806
0.34134056567222004	0.7082018927444795
0.34172801239829526	0.7082018927444795
0.34172801239829526	0.7086525461919784
0.34250290585044557	0.7086525461919784
0.34250290585044557	0.7088778729157278
0.34269662921348315	0.7088778729157278
0.34269662921348315	0.7091031996394772
0.34347152266563347	0.7091031996394772
0.34347152266563347	0.7097791798107256
0.3440526927547462	0.7097791798107256
0.3440526927547462	0.7104551599819738
0.34444013948082136	0.7104551599819738
0.34444013948082136	0.7109058134294728
0.34502130956993415	0.7109058134294728
0.34502130956993415	0.7111311401532222
0.34521503293297173	0.7111311401532222
0.34521503293297173	0.711581793600721
0.3454087562960093	0.711581793600721
0.3454087562960093	0.7118071203244705
0.34579620302208447	0.7118071203244705
0.34579620302208447	0.7120324470482199
0.34598992638512205	0.7120324470482199
0.34598992638512205	0.7122577737719693
0.3461836497481596	0.7122577737719693
0.3461836497481596	0.7124831004957188
0.3463773731111972	0.7124831004957188
0.3463773731111972	0.7127084272194683
0.34676481983727236	0.7127084272194683
0.34676481983727236	0.7129337539432177
0.3473459899263851	0.7129337539432177
0.3473459899263851	0.715187021180712
0.34773343665246026	0.715187021180712
0.34773343665246026	0.7158630013519603
0.3487020534676482	0.7158630013519603
0.3487020534676482	0.7167643082469581
0.3488957768306858	0.7167643082469581
0.3488957768306858	0.7174402884182064
0.3496706702828361	0.7174402884182064
0.3496706702828361	0.7181162685894548
0.35005811700891126	0.7181162685894548
0.35005811700891126	0.7183415953132042
0.3508330104610616	0.7183415953132042
0.3508330104610616	0.7185669220369536
0.3510267338240992	0.7185669220369536
0.3510267338240992	0.7194682289319513
0.3512204571871368	0.7194682289319513
0.3512204571871368	0.7199188823794502
0.35160790391321195	0.7199188823794502
0.35160790391321195	0.7201442091031997
0.35180162727624953	0.7201442091031997
0.35180162727624953	0.7203695358269491
0.3521890740023247	0.7203695358269491
0.3521890740023247	0.7212708427219469
0.35238279736536227	0.7212708427219469
0.35238279736536227	0.7214961694456963
0.3539325842696629	0.7214961694456963
0.3539325842696629	0.7217214961694457
0.3545137543587757	0.7217214961694457
0.3545137543587757	0.722397476340694
0.35490120108485085	0.722397476340694
0.35490120108485085	0.7226228030644435
0.3550949244478884	0.7226228030644435
0.3550949244478884	0.7228481297881929
0.3560635412630763	0.7228481297881929
0.3560635412630763	0.7230734565119423
0.3564509879891515	0.7230734565119423
0.3564509879891515	0.7232987832356917
0.3572258814413018	0.7232987832356917
0.3572258814413018	0.7242000901306895
0.357613328167377	0.7242000901306895
0.357613328167377	0.7255520504731862
0.35800077489345217	0.7255520504731862
0.35800077489345217	0.7257773771969356
0.35819449825648975	0.7257773771969356
0.35819449825648975	0.7271293375394322
0.3583882216195273	0.7271293375394322
0.3583882216195273	0.7273546642631816
0.3585819449825649	0.7273546642631816
0.3585819449825649	0.7280306444344299
0.35916311507167764	0.7280306444344299
0.35916311507167764	0.7287066246056783
0.3595505617977528	0.7287066246056783
0.3595505617977528	0.7289319513294277
0.3597442851607904	0.7289319513294277
0.3597442851607904	0.7298332582244255
0.36013173188686554	0.7298332582244255
0.36013173188686554	0.7300585849481749
0.36071290197597833	0.7300585849481749
0.36071290197597833	0.7302839116719243
0.3609066253390159	0.7302839116719243
0.3609066253390159	0.7307345651194231
0.3611003487020535	0.7307345651194231
0.3611003487020535	0.7311852185669221
0.36129407206509107	0.7311852185669221
0.36129407206509107	0.7316358720144209
0.3616815187911662	0.7316358720144209
0.3616815187911662	0.7318611987381703
0.3618752421542038	0.7318611987381703
0.3618752421542038	0.7323118521856692
0.36226268888027896	0.7323118521856692
0.36226268888027896	0.7325371789094186
0.36245641224331654	0.7325371789094186
0.36245641224331654	0.7329878323569176
0.3628438589693917	0.7329878323569176
0.3628438589693917	0.7334384858044164
0.363618752421542	0.7334384858044164
0.363618752421542	0.7336638125281658
0.3640061991476172	0.7336638125281658
0.3640061991476172	0.7341144659756648
0.3643936458736924	0.7341144659756648
0.3643936458736924	0.734790446146913
0.36458736923672996	0.734790446146913
0.36458736923672996	0.7354664263181613
0.36478109259976754	0.7354664263181613
0.36478109259976754	0.7365930599369085
0.3653622626888803	0.7365930599369085
0.3653622626888803	0.7368183866606579
0.36574970941495544	0.7368183866606579
0.36574970941495544	0.7370437133844074
0.3661371561410306	0.7370437133844074
0.3661371561410306	0.7372690401081569
0.3663308795040682	0.7372690401081569
0.3663308795040682	0.7379450202794051
0.36652460286710575	0.7379450202794051
0.36652460286710575	0.7381703470031545
0.36671832623014333	0.7381703470031545
0.36671832623014333	0.738395673726904
0.3669120495931809	0.738395673726904
0.3669120495931809	0.7386210004506535
0.36710577295621855	0.7386210004506535
0.36710577295621855	0.7388463271744029
0.3672994963192561	0.7388463271744029
0.3672994963192561	0.7390716538981523
0.3676869430453313	0.7390716538981523
0.3676869430453313	0.7392969806219017
0.36807438977140644	0.7392969806219017
0.36807438977140644	0.7395223073456512
0.36884928322355676	0.7395223073456512
0.36884928322355676	0.7397476340694006
0.36904300658659434	0.7397476340694006
0.36904300658659434	0.7399729607931501
0.37020534676481986	0.7399729607931501
0.37020534676481986	0.740423614240649
0.370592793490895	0.740423614240649
0.370592793490895	0.7406489409643984
0.37117396358000776	0.7406489409643984
0.37117396358000776	0.7410995944118972
0.3715614103060829	0.7410995944118972
0.3715614103060829	0.7413249211356467
0.3717551336691205	0.7413249211356467
0.3717551336691205	0.7415502478593962
0.3719488570321581	0.7415502478593962
0.3719488570321581	0.7417755745831456
0.37233630375823323	0.7417755745831456
0.37233630375823323	0.742000901306895
0.37349864393645876	0.742000901306895
0.37349864393645876	0.7424515547543938
0.3738860906625339	0.7424515547543938
0.3738860906625339	0.7426768814781433
0.3742735373886091	0.7426768814781433
0.3742735373886091	0.7433528616493916
0.37446726075164666	0.7433528616493916
0.37446726075164666	0.743578188373141
0.37466098411468424	0.743578188373141
0.37466098411468424	0.7438035150968905
0.3750484308407594	0.7438035150968905
0.3750484308407594	0.7440288418206399
0.37543587756683455	0.7440288418206399
0.37543587756683455	0.7444794952681388
0.3760170476559473	0.7444794952681388
0.3760170476559473	0.7453808021631365
0.37621077101898487	0.7453808021631365
0.37621077101898487	0.7456061288868859
0.37679194110809766	0.7456061288868859
0.37679194110809766	0.7458314556106355
0.37795428128632313	0.7458314556106355
0.37795428128632313	0.7462821090581343
0.38008523827973656	0.7462821090581343
0.38008523827973656	0.7465074357818837
0.3806664083688493	0.7465074357818837
0.3806664083688493	0.7469580892293826
0.38124757845796203	0.7469580892293826
0.38124757845796203	0.7476340694006309
0.3816350251840372	0.7476340694006309
0.3816350251840372	0.7478593961243803
0.38221619527314993	0.7478593961243803
0.38221619527314993	0.7480847228481298
0.3824099186361875	0.7480847228481298
0.3824099186361875	0.7487607030193781
0.3826036419992251	0.7487607030193781
0.3826036419992251	0.749211356466877
0.38337853545137546	0.749211356466877
0.38337853545137546	0.7494366831906264
0.3839597055404882	0.7494366831906264
0.3839597055404882	0.7496620099143758
0.38434715226656335	0.7496620099143758
0.38434715226656335	0.7498873366381252
0.38454087562960093	0.7498873366381252
0.38454087562960093	0.7501126633618748
0.3849283223556761	0.7501126633618748
0.3849283223556761	0.7505633168093736
0.38531576908175125	0.7505633168093736
0.38531576908175125	0.7510139702568724
0.3857032158078264	0.7510139702568724
0.3857032158078264	0.7516899504281208
0.38609066253390156	0.7516899504281208
0.38609066253390156	0.7519152771518702
0.38686555598605193	0.7519152771518702
0.38686555598605193	0.7523659305993691
0.3870592793490895	0.7523659305993691
0.3870592793490895	0.7534925642181163
0.38744672607516467	0.7534925642181163
0.38744672607516467	0.7537178909418657
0.3880278961642774	0.7537178909418657
0.3880278961642774	0.7539432176656151
0.38841534289035257	0.7539432176656151
0.38841534289035257	0.7541685443893645
0.3895776830685781	0.7541685443893645
0.3895776830685781	0.7543938711131141
0.3903525765207284	0.7543938711131141
0.3903525765207284	0.7550698512843623
0.390546299883766	0.7550698512843623
0.390546299883766	0.7552951780081117
0.39074002324680357	0.7552951780081117
0.39074002324680357	0.7555205047318612
0.3911274699728787	0.7555205047318612
0.3911274699728787	0.7561964849031095
0.3915149166989539	0.7561964849031095
0.3915149166989539	0.7566471383506084
0.39170864006199146	0.7566471383506084
0.39170864006199146	0.7570977917981072
0.3922898101511042	0.7570977917981072
0.3922898101511042	0.7573231185218567
0.3924835335141418	0.7573231185218567
0.3924835335141418	0.757999098693105
0.392870980240217	0.757999098693105
0.392870980240217	0.7584497521406038
0.3930647036032546	0.7584497521406038
0.3930647036032546	0.7589004055881028
0.39345215032932973	0.7589004055881028
0.39345215032932973	0.7591257323118522
0.3936458736923673	0.7591257323118522
0.3936458736923673	0.7593510590356016
0.3938395970554049	0.7593510590356016
0.3938395970554049	0.759576385759351
0.39403332041844247	0.759576385759351
0.39403332041844247	0.7600270392068499
0.39500193723363036	0.7600270392068499
0.39500193723363036	0.7602523659305994
0.39519566059666794	0.7602523659305994
0.39519566059666794	0.7609283461018477
0.3953893839597055	0.7609283461018477
0.3953893839597055	0.7613789995493465
0.3957768306857807	0.7613789995493465
0.3957768306857807	0.761604326273096
0.3961642774118559	0.761604326273096
0.3961642774118559	0.7618296529968455
0.39674544750096863	0.7618296529968455
0.39674544750096863	0.7625056331680937
0.3979077876791941	0.7625056331680937
0.3979077876791941	0.7627309598918431
0.3986826811313444	0.7627309598918431
0.3986826811313444	0.7640829202343398
0.3994575745834948	0.7640829202343398
0.3994575745834948	0.7643082469580892
0.4000387446726075	0.7643082469580892
0.4000387446726075	0.7647589004055881
0.40061991476172026	0.7647589004055881
0.40061991476172026	0.765209553853087
0.40081363812475784	0.765209553853087
0.40081363812475784	0.7658855340243352
0.4010073614877954	0.7658855340243352
0.4010073614877954	0.7661108607480848
0.401201084850833	0.7661108607480848
0.401201084850833	0.7665615141955836
0.40178225493994574	0.7665615141955836
0.40178225493994574	0.766786840919333
0.4021697016660209	0.766786840919333
0.4021697016660209	0.7672374943668319
0.40313831848120885	0.7672374943668319
0.40313831848120885	0.7674628210905814
0.4033320418442464	0.7674628210905814
0.4033320418442464	0.7688147814330779
0.4044943820224719	0.7688147814330779
0.4044943820224719	0.7690401081568274
0.4046881053855095	0.7690401081568274
0.4046881053855095	0.7692654348805769
0.40488182874854706	0.7692654348805769
0.40488182874854706	0.7697160883280757
0.40507555211158464	0.7697160883280757
0.40507555211158464	0.7699414150518251
0.40546299883765985	0.7699414150518251
0.40546299883765985	0.7703920684993241
0.405850445563735	0.7703920684993241
0.405850445563735	0.7717440288418207
0.40643161565284774	0.7717440288418207
0.40643161565284774	0.7719693555655701
0.4068190623789229	0.7719693555655701
0.4068190623789229	0.7721946822893195
0.40720650910499806	0.7721946822893195
0.40720650910499806	0.7726453357368184
0.40836884928322353	0.7726453357368184
0.40836884928322353	0.7730959891843172
0.4085625726462611	0.7730959891843172
0.4085625726462611	0.7733213159080667
0.4091437427353739	0.7733213159080667
0.4091437427353739	0.7735466426318162
0.4093374660984115	0.7735466426318162
0.4093374660984115	0.7737719693555656
0.4101123595505618	0.7737719693555656
0.4101123595505618	0.7742226228030644
0.4110809763657497	0.7742226228030644
0.4110809763657497	0.7744479495268138
0.41204959318093765	0.7744479495268138
0.41204959318093765	0.7746732762505634
0.41398682681131344	0.7746732762505634
0.41398682681131344	0.7753492564218116
0.41476172026346375	0.7753492564218116
0.41476172026346375	0.775574583145561
0.4155366137156141	0.775574583145561
0.4155366137156141	0.7760252365930599
0.41611778380472686	0.7760252365930599
0.41611778380472686	0.7762505633168094
0.4166989538938396	0.7762505633168094
0.4166989538938396	0.7764758900405588
0.4168926772568772	0.7764758900405588
0.4168926772568772	0.7767012167643083
0.41728012398295233	0.7767012167643083
0.41728012398295233	0.7769265434880577
0.4174738473459899	0.7769265434880577
0.4174738473459899	0.7771518702118071
0.4176675707090275	0.7771518702118071
0.4176675707090275	0.7773771969355565
0.4190236342502906	0.7773771969355565
0.4190236342502906	0.777602523659306
0.41960480433940334	0.777602523659306
0.41960480433940334	0.7778278503830555
0.4207671445176288	0.7778278503830555
0.4207671445176288	0.7780531771068049
0.4209608678806664	0.7780531771068049
0.4209608678806664	0.7789544840018026
0.4223169314219295	0.7789544840018026
0.4223169314219295	0.7794051374493015
0.42386671832623013	0.7794051374493015
0.42386671832623013	0.7796304641730509
0.4240604416892677	0.7796304641730509
0.4240604416892677	0.7798557908968003
0.4242541650523053	0.7798557908968003
0.4242541650523053	0.7803064443442992
0.42522278186749324	0.7803064443442992
0.42522278186749324	0.7809824245155476
0.4254165052305308	0.7809824245155476
0.4254165052305308	0.7816584046867958
0.42677256877179387	0.7816584046867958
0.42677256877179387	0.7825597115817936
0.42716001549786903	0.7825597115817936
0.42716001549786903	0.782785038305543
0.4273537388609066	0.782785038305543
0.4273537388609066	0.7832356917530419
0.42774118558698176	0.7832356917530419
0.42774118558698176	0.7836863452005408
0.42832235567609456	0.7836863452005408
0.42832235567609456	0.7843623253717891
0.4290972491282449	0.7843623253717891
0.4290972491282449	0.7845876520955385
0.42929097249128245	0.7845876520955385
0.42929097249128245	0.7852636322667869
0.4306470360325455	0.7852636322667869
0.4306470360325455	0.7854889589905363
0.4321968229368462	0.7854889589905363
0.4321968229368462	0.7857142857142857
0.43239054629988377	0.7857142857142857
0.43239054629988377	0.7859396124380351
0.43277799302595893	0.7859396124380351
0.43277799302595893	0.7863902658855341
0.43335916311507167	0.7863902658855341
0.43335916311507167	0.7866155926092835
0.4339403332041844	0.7866155926092835
0.4339403332041844	0.7870662460567823
0.434134056567222	0.7870662460567823
0.434134056567222	0.7879675529517801
0.4345215032932972	0.7879675529517801
0.4345215032932972	0.7881928796755295
0.4347152266563348	0.7881928796755295
0.4347152266563348	0.7886435331230284
0.43490895001937235	0.7886435331230284
0.43490895001937235	0.7888688598467778
0.4374273537388609	0.7888688598467778
0.4374273537388609	0.7890941865705272
0.4376210771018985	0.7890941865705272
0.4376210771018985	0.7893195132942767
0.4397520340953119	0.7893195132942767
0.4397520340953119	0.7895448400180262
0.44072065091049983	0.7895448400180262
0.44072065091049983	0.7908968003605228
0.44168926772568773	0.7908968003605228
0.44168926772568773	0.7911221270842722
0.4418829910887253	0.7911221270842722
0.4418829910887253	0.791572780531771
0.4420767144517629	0.791572780531771
0.4420767144517629	0.7920234339792699
0.4428516079039132	0.7920234339792699
0.4428516079039132	0.7922487607030194
0.4430453312669508	0.7922487607030194
0.4430453312669508	0.7933753943217665
0.44343277799302594	0.7933753943217665
0.44343277799302594	0.793600721045516
0.4438202247191011	0.793600721045516
0.4438202247191011	0.7940513744930149
0.44401394808213873	0.7940513744930149
0.44401394808213873	0.7942767012167643
0.4442076714451763	0.7942767012167643
0.4442076714451763	0.7945020279405137
0.4444013948082139	0.7945020279405137
0.4444013948082139	0.7949526813880127
0.4453700116234018	0.7949526813880127
0.4453700116234018	0.7951780081117621
0.44575745834947694	0.7951780081117621
0.44575745834947694	0.7958539882830103
0.44653235180162726	0.7958539882830103
0.44653235180162726	0.7960793150067598
0.4469197985277024	0.7960793150067598
0.4469197985277024	0.7965299684542587
0.4482758620689655	0.7965299684542587
0.4482758620689655	0.797205948625507
0.4484695854320031	0.797205948625507
0.4484695854320031	0.7974312753492564
0.4486633087950407	0.7974312753492564
0.4486633087950407	0.7976566020730058
0.44885703215807826	0.7976566020730058
0.44885703215807826	0.7978819287967553
0.45001937233630374	0.7978819287967553
0.45001937233630374	0.7981072555205048
0.45040681906237895	0.7981072555205048
0.45040681906237895	0.7983325822442542
0.4507942657884541	0.7983325822442542
0.4507942657884541	0.7985579089680036
0.45118171251452927	0.7985579089680036
0.45118171251452927	0.798783235691753
0.45215032932971716	0.798783235691753
0.45215032932971716	0.7990085624155024
0.45234405269275474	0.7990085624155024
0.45234405269275474	0.7992338891392519
0.4525377760557923	0.7992338891392519
0.4525377760557923	0.7994592158630014
0.45370011623401785	0.7994592158630014
0.45370011623401785	0.7996845425867508
0.4542812863231306	0.7996845425867508
0.4542812863231306	0.7999098693105002
0.4548624564122433	0.7999098693105002
0.4548624564122433	0.8001351960342497
0.45563734986439364	0.8001351960342497
0.45563734986439364	0.8003605227579991
0.4583494769469198	0.8003605227579991
0.4583494769469198	0.8010365029292474
0.45873692367299496	0.8010365029292474
0.45873692367299496	0.8012618296529969
0.45893064703603254	0.8012618296529969
0.45893064703603254	0.8014871563767463
0.4593180937621077	0.8014871563767463
0.4593180937621077	0.8017124831004957
0.45989926385122043	0.8017124831004957
0.45989926385122043	0.8021631365479945
0.4604804339403332	0.8021631365479945
0.4604804339403332	0.8023884632717441
0.4608678806664084	0.8023884632717441
0.4608678806664084	0.8026137899954935
0.46125532739248354	0.8026137899954935
0.46125532739248354	0.8028391167192429
0.46203022084463385	0.8028391167192429
0.46203022084463385	0.8030644434429923
0.46222394420767143	0.8030644434429923
0.46222394420767143	0.8035150968904912
0.4626113909337466	0.8035150968904912
0.4626113909337466	0.8039657503379901
0.46280511429678417	0.8039657503379901
0.46280511429678417	0.8041910770617395
0.46299883765982175	0.8041910770617395
0.46299883765982175	0.8046417305092384
0.4639674544750097	0.8046417305092384
0.4639674544750097	0.8048670572329878
0.46551724137931033	0.8048670572329878
0.46551724137931033	0.8050923839567373
0.46609841146842307	0.8050923839567373
0.46609841146842307	0.8053177106804867
0.46667958155753586	0.8053177106804867
0.46667958155753586	0.8057683641279856
0.4672607516466486	0.8057683641279856
0.4672607516466486	0.805993690851735
0.4680356450987989	0.805993690851735
0.4680356450987989	0.8062190175754844
0.4682293684618365	0.8062190175754844
0.4682293684618365	0.8064443442992338
0.46881053855094923	0.8064443442992338
0.46881053855094923	0.8071203244704822
0.4690042619139868	0.8071203244704822
0.4690042619139868	0.8073456511942316
0.46939170864006197	0.8073456511942316
0.46939170864006197	0.807570977917981
0.4705540488182875	0.807570977917981
0.4705540488182875	0.8077963046417305
0.4707477721813251	0.8077963046417305
0.4707477721813251	0.80802163136548
0.47113521890740023	0.80802163136548
0.47113521890740023	0.8084722848129788
0.4715226656334754	0.8084722848129788
0.4715226656334754	0.8086976115367283
0.47171638899651297	0.8086976115367283
0.47171638899651297	0.8089229382604777
0.4721038357225881	0.8089229382604777
0.4721038357225881	0.8091482649842271
0.47268500581170086	0.8091482649842271
0.47268500581170086	0.8093735917079765
0.4728787291747385	0.8093735917079765
0.4728787291747385	0.8098242451554755
0.47345989926385124	0.8098242451554755
0.47345989926385124	0.8100495718792249
0.4736536226268888	0.8100495718792249
0.4736536226268888	0.8105002253267237
0.4738473459899264	0.8105002253267237
0.4738473459899264	0.8107255520504731
0.4748159628051143	0.8107255520504731
0.4748159628051143	0.8109508787742227
0.4755908562572646	0.8109508787742227
0.4755908562572646	0.8116268589454709
0.47675319643549013	0.8116268589454709
0.47675319643549013	0.8118521856692203
0.4769469197985277	0.8118521856692203
0.4769469197985277	0.8123028391167192
0.47752808988764045	0.8123028391167192
0.47752808988764045	0.8127534925642181
0.47772181325067803	0.8127534925642181
0.47772181325067803	0.8129788192879676
0.47985277024409145	0.8129788192879676
0.47985277024409145	0.813204146011717
0.48004649360712903	0.813204146011717
0.48004649360712903	0.8136547994592158
0.48082138705927935	0.8136547994592158
0.48082138705927935	0.8138801261829653
0.4812088337853545	0.8138801261829653
0.4812088337853545	0.8141054529067148
0.48159628051142966	0.8141054529067148
0.48159628051142966	0.8143307796304642
0.48179000387446724	0.8143307796304642
0.48179000387446724	0.8145561063542136
0.4837272375048431	0.8145561063542136
0.4837272375048431	0.814781433077963
0.4852770244091437	0.814781433077963
0.4852770244091437	0.815232086525462
0.4854707477721813	0.815232086525462
0.4854707477721813	0.8154574132492114
0.48624564122433167	0.8154574132492114
0.48624564122433167	0.8156827399729608
0.48721425803951957	0.8156827399729608
0.48721425803951957	0.8159080666967102
0.4876017047655947	0.8159080666967102
0.4876017047655947	0.8163587201442091
0.4887640449438202	0.8163587201442091
0.4887640449438202	0.8165840468679585
0.48895776830685783	0.8165840468679585
0.48895776830685783	0.8170347003154574
0.4899263851220457	0.8170347003154574
0.4899263851220457	0.8172600270392069
0.4901201084850833	0.8172600270392069
0.4901201084850833	0.8174853537629563
0.49147617202634636	0.8174853537629563
0.49147617202634636	0.8179360072104551
0.49205734211545915	0.8179360072104551
0.49205734211545915	0.8183866606579541
0.49283223556760947	0.8183866606579541
0.49283223556760947	0.8186119873817035
0.4936071290197598	0.8186119873817035
0.4936071290197598	0.8188373141054529
0.49399457574583494	0.8188373141054529
0.49399457574583494	0.8190626408292023
0.49476946919798526	0.8190626408292023
0.49476946919798526	0.8195132942767012
0.4957380860131732	0.8195132942767012
0.4957380860131732	0.8197386210004507
0.49612553273924836	0.8197386210004507
0.49612553273924836	0.8199639477242001
0.4967067028283611	0.8199639477242001
0.4967067028283611	0.8201892744479495
0.49728787291747384	0.8201892744479495
0.49728787291747384	0.820414601171699
0.497675319643549	0.820414601171699
0.497675319643549	0.8208652546191978
0.49941882991088726	0.8208652546191978
0.49941882991088726	0.8215412347904462
0.5003874467260752	0.8215412347904462
0.5003874467260752	0.821991888237945
0.5017435102673382	0.821991888237945
0.5017435102673382	0.8222172149616944
0.5052305308020147	0.8222172149616944
0.5052305308020147	0.8224425416854438
0.5061991476172026	0.8224425416854438
0.5061991476172026	0.8231185218566922
0.5067803177063154	0.8231185218566922
0.5067803177063154	0.8233438485804416
0.5087175513366912	0.8233438485804416
0.5087175513366912	0.823569175304191
0.5098798915149167	0.823569175304191
0.5098798915149167	0.82401982875169
0.5112359550561798	0.82401982875169
0.5112359550561798	0.8242451554754394
0.5114296784192174	0.8242451554754394
0.5114296784192174	0.8244704821991888
0.5120108485083301	0.8244704821991888
0.5120108485083301	0.8249211356466877
0.5139480821387059	0.8249211356466877
0.5139480821387059	0.8251464623704371
0.5141418055017435	0.8251464623704371
0.5141418055017435	0.8253717890941866
0.5147229755908562	0.8253717890941866
0.5147229755908562	0.825597115817936
0.5154978690430065	0.825597115817936
0.5154978690430065	0.8260477692654349
0.5166602092212321	0.8260477692654349
0.5166602092212321	0.8262730959891843
0.5170476559473073	0.8262730959891843
0.5170476559473073	0.8267237494366831
0.5174351026733824	0.8267237494366831
0.5174351026733824	0.8269490761604327
0.5184037194885703	0.8269490761604327
0.5184037194885703	0.8271744028841821
0.5195660596667958	0.8271744028841821
0.5195660596667958	0.8273997296079315
0.519953506392871	0.8273997296079315
0.519953506392871	0.8276250563316809
0.5201472297559085	0.8276250563316809
0.5201472297559085	0.8278503830554303
0.5211158465710964	0.8278503830554303
0.5211158465710964	0.8280757097791798
0.5215032932971716	0.8280757097791798
0.5215032932971716	0.8283010365029293
0.5226656334753972	0.8283010365029293
0.5226656334753972	0.8285263632266787
0.5230530802014723	0.8285263632266787
0.5230530802014723	0.8289770166741776
0.5236342502905851	0.8289770166741776
0.5236342502905851	0.829202343397927
0.5240216970166602	0.829202343397927
0.5240216970166602	0.8294276701216764
0.5251840371948857	0.8294276701216764
0.5251840371948857	0.8296529968454258
0.5257652072839984	0.8296529968454258
0.5257652072839984	0.8298783235691753
0.5261526540100736	0.8298783235691753
0.5261526540100736	0.8303289770166742
0.5263463773731112	0.8303289770166742
0.5263463773731112	0.8305543037404236
0.5269275474622239	0.8305543037404236
0.5269275474622239	0.831230283911672
0.5275087175513367	0.831230283911672
0.5275087175513367	0.8314556106354214
0.5277024409143742	0.8314556106354214
0.5277024409143742	0.8316809373591708
0.5286710577295621	0.8316809373591708
0.5286710577295621	0.8319062640829202
0.5296396745447501	0.8319062640829202
0.5296396745447501	0.8321315908066697
0.5298333979077877	0.8321315908066697
0.5298333979077877	0.8323569175304191
0.5311894614490508	0.8323569175304191
0.5311894614490508	0.8325822442541685
0.5317706315381635	0.8325822442541685
0.5317706315381635	0.832807570977918
0.5325455249903138	0.832807570977918
0.5325455249903138	0.8330328977016674
0.532932971716389	0.8330328977016674
0.532932971716389	0.8334835511491663
0.5335141418055017	0.8334835511491663
0.5335141418055017	0.8337088778729157
0.5344827586206896	0.8337088778729157
0.5344827586206896	0.8339342045966651
0.5346764819837272	0.8339342045966651
0.5346764819837272	0.8341595313204146
0.5358388221619528	0.8341595313204146
0.5358388221619528	0.8343848580441641
0.5368074389771407	0.8343848580441641
0.5368074389771407	0.8346101847679135
0.5377760557923286	0.8346101847679135
0.5377760557923286	0.8348355114916629
0.5379697791553661	0.8348355114916629
0.5379697791553661	0.8350608382154123
0.5383572258814413	0.8350608382154123
0.5383572258814413	0.8352861649391617
0.5391321193335916	0.8352861649391617
0.5391321193335916	0.8355114916629113
0.5399070127857419	0.8355114916629113
0.5399070127857419	0.8357368183866607
0.5430065865943433	0.8357368183866607
0.5430065865943433	0.8361874718341595
0.5433940333204185	0.8361874718341595
0.5433940333204185	0.836412798557909
0.543587756683456	0.836412798557909
0.543587756683456	0.8366381252816584
0.5441689267725688	0.8366381252816584
0.5441689267725688	0.8368634520054078
0.5449438202247191	0.8368634520054078
0.5449438202247191	0.8370887787291573
0.5462998837659822	0.8370887787291573
0.5462998837659822	0.8375394321766562
0.5474622239442076	0.8375394321766562
0.5474622239442076	0.8377647589004056
0.5478496706702828	0.8377647589004056
0.5478496706702828	0.837990085624155
0.5480433940333204	0.837990085624155
0.5480433940333204	0.838440739071654
0.5486245641224332	0.838440739071654
0.5486245641224332	0.8386660657954034
0.5490120108485084	0.8386660657954034
0.5490120108485084	0.8391167192429022
0.5495931809376211	0.8391167192429022
0.5495931809376211	0.8393420459666516
0.5503680743897714	0.8393420459666516
0.5503680743897714	0.839567372690401
0.5507555211158466	0.839567372690401
0.5507555211158466	0.8397926994141505
0.5509492444788842	0.8397926994141505
0.5509492444788842	0.8400180261379
0.5511429678419217	0.8400180261379
0.5511429678419217	0.8402433528616494
0.5515304145679969	0.8402433528616494
0.5515304145679969	0.8404686795853988
0.5517241379310345	0.8404686795853988
0.5517241379310345	0.8406940063091483
0.5530802014722975	0.8406940063091483
0.5530802014722975	0.8409193330328977
0.5540488182874854	0.8409193330328977
0.5540488182874854	0.8411446597566471
0.5548237117396358	0.8411446597566471
0.5548237117396358	0.841595313204146
0.5569546687330492	0.841595313204146
0.5569546687330492	0.8418206399278955
0.5571483920960868	0.8418206399278955
0.5571483920960868	0.8420459666516449
0.5573421154591244	0.8420459666516449
0.5573421154591244	0.8429472735466427
0.5594730724525377	0.8429472735466427
0.5594730724525377	0.8431726002703921
0.5600542425416505	0.8431726002703921
0.5600542425416505	0.8436232537178909
0.5604416892677256	0.8436232537178909
0.5604416892677256	0.8438485804416404
0.5612165827198761	0.8438485804416404
0.5612165827198761	0.8440739071653898
0.5614103060829136	0.8440739071653898
0.5614103060829136	0.8447498873366381
0.5631538163502519	0.8447498873366381
0.5631538163502519	0.8449752140603876
0.5639287098024022	0.8449752140603876
0.5639287098024022	0.8456511942316358
0.5643161565284773	0.8456511942316358
0.5643161565284773	0.8458765209553853
0.5645098798915149	0.8458765209553853
0.5645098798915149	0.8465525011266336
0.5648973266175901	0.8465525011266336
0.5648973266175901	0.847228481297882
0.5650910499806276	0.847228481297882
0.5650910499806276	0.8474538080216314
0.5660596667958155	0.8474538080216314
0.5660596667958155	0.8476791347453808
0.5664471135218907	0.8476791347453808
0.5664471135218907	0.8479044614691302
0.5670282836110034	0.8479044614691302
0.5670282836110034	0.8483551149166291
0.568190623789229	0.8483551149166291
0.568190623789229	0.8485804416403786
0.5709027508717551	0.8485804416403786
0.5709027508717551	0.848805768364128
0.5714839209608679	0.848805768364128
0.5714839209608679	0.8490310950878774
0.571871367686943	0.8490310950878774
0.571871367686943	0.8494817485353763
0.5720650910499806	0.8494817485353763
0.5720650910499806	0.8497070752591257
0.5730337078651685	0.8497070752591257
0.5730337078651685	0.8499324019828751
0.5736148779542812	0.8499324019828751
0.5736148779542812	0.8501577287066246
0.5738086013173189	0.8501577287066246
0.5738086013173189	0.8506083821541235
0.5745834947694692	0.8506083821541235
0.5745834947694692	0.8508337088778729
0.575164664858582	0.8508337088778729
0.575164664858582	0.8510590356016223
0.5776830685780705	0.8510590356016223
0.5776830685780705	0.8512843623253717
0.5784579620302208	0.8512843623253717
0.5784579620302208	0.8515096890491213
0.5802014722975591	0.8515096890491213
0.5802014722975591	0.852410995944119
0.581170089112747	0.852410995944119
0.581170089112747	0.8526363226678684
0.5813638124757846	0.8526363226678684
0.5813638124757846	0.8528616493916178
0.5815575358388222	0.8528616493916178
0.5815575358388222	0.8530869761153673
0.5819449825648974	0.8530869761153673
0.5819449825648974	0.8533123028391167
0.5821387059279349	0.8533123028391167
0.5821387059279349	0.8535376295628662
0.5825261526540101	0.8535376295628662
0.5825261526540101	0.8537629562866156
0.5827198760170477	0.8537629562866156
0.5827198760170477	0.853988283010365
0.5831073227431228	0.853988283010365
0.5831073227431228	0.8546642631816134
0.5836884928322356	0.8546642631816134
0.5836884928322356	0.8548895899053628
0.5846571096474235	0.8548895899053628
0.5846571096474235	0.8553402433528616
0.5850445563734986	0.8553402433528616
0.5850445563734986	0.855565570076611
0.5854320030995738	0.855565570076611
0.5854320030995738	0.8557908968003605
0.5860131731886865	0.8557908968003605
0.5860131731886865	0.8562415502478594
0.5867880666408369	0.8562415502478594
0.5867880666408369	0.8564668769716088
0.5873692367299497	0.8564668769716088
0.5873692367299497	0.8566922036953583
0.5875629600929873	0.8566922036953583
0.5875629600929873	0.8569175304191077
0.5877566834560248	0.8569175304191077
0.5877566834560248	0.8571428571428571
0.5889190236342503	0.8571428571428571
0.5889190236342503	0.8573681838666066
0.5891127469972879	0.8573681838666066
0.5891127469972879	0.857593510590356
0.5893064703603255	0.857593510590356
0.5893064703603255	0.8582694907616043
0.5910499806276637	0.8582694907616043
0.5910499806276637	0.8587201442091033
0.5920185974428516	0.8587201442091033
0.5920185974428516	0.8591707976566021
0.5924060441689267	0.8591707976566021
0.5924060441689267	0.8602974312753493
0.5927934908950019	0.8602974312753493
0.5927934908950019	0.8605227579990987
0.5931809376210772	0.8605227579990987
0.5931809376210772	0.8609734114465976
0.5939558310732275	0.8609734114465976
0.5939558310732275	0.861198738170347
0.594149554436265	0.861198738170347
0.594149554436265	0.8614240648940964
0.5943432777993026	0.8614240648940964
0.5943432777993026	0.8618747183415953
0.5945370011623402	0.8618747183415953
0.5945370011623402	0.8621000450653448
0.5953118946144905	0.8621000450653448
0.5953118946144905	0.8623253717890942
0.5962805114296784	0.8623253717890942
0.5962805114296784	0.8625506985128436
0.596474234792716	0.8625506985128436
0.596474234792716	0.8630013519603424
0.5966679581557536	0.8630013519603424
0.5966679581557536	0.8634520054078414
0.5972491282448663	0.8634520054078414
0.5972491282448663	0.8636773321315908
0.5974428516079039	0.8636773321315908
0.5974428516079039	0.8639026588553402
0.5976365749709415	0.8639026588553402
0.5976365749709415	0.8641279855790897
0.5982177450600542	0.8641279855790897
0.5982177450600542	0.8643533123028391
0.5984114684230918	0.8643533123028391
0.5984114684230918	0.8645786390265886
0.599767531964355	0.8645786390265886
0.599767531964355	0.8650292924740874
0.6009298721425804	0.8650292924740874
0.6009298721425804	0.8654799459215863
0.601123595505618	0.8654799459215863
0.601123595505618	0.8657052726453357
0.6020922123208059	0.8657052726453357
0.6020922123208059	0.8659305993690851
0.6022859356838435	0.8659305993690851
0.6022859356838435	0.8661559260928346
0.602479659046881	0.8661559260928346
0.602479659046881	0.8663812528165841
0.6028671057729562	0.8663812528165841
0.6028671057729562	0.8666065795403335
0.6032545524990314	0.8666065795403335
0.6032545524990314	0.8670572329878323
0.6040294459511817	0.8670572329878323
0.6040294459511817	0.8672825597115817
0.604804339403332	0.8672825597115817
0.604804339403332	0.8675078864353313
0.6051917861294072	0.8675078864353313
0.6051917861294072	0.8679585398828301
0.6053855094924447	0.8679585398828301
0.6053855094924447	0.868409193330329
0.60577295621852	0.868409193330329
0.60577295621852	0.8688598467778279
0.6071290197597831	0.8688598467778279
0.6071290197597831	0.8693105002253267
0.6082913599380085	0.8693105002253267
0.6082913599380085	0.869986480396575
0.6084850833010461	0.869986480396575
0.6084850833010461	0.8708877872915728
0.6086788066640837	0.8708877872915728
0.6086788066640837	0.8711131140153222
0.6092599767531964	0.8711131140153222
0.6092599767531964	0.8713384407390716
0.609453700116234	0.8713384407390716
0.609453700116234	0.8717890941865706
0.6098411468423092	0.8717890941865706
0.6098411468423092	0.87201442091032
0.6102285935683843	0.87201442091032
0.6102285935683843	0.8729157278053177
0.6104223169314219	0.8729157278053177
0.6104223169314219	0.8731410545290671
0.6106160402944595	0.8731410545290671
0.6106160402944595	0.8733663812528166
0.6110034870205346	0.8733663812528166
0.6110034870205346	0.873591707976566
0.6135218907400233	0.873591707976566
0.6135218907400233	0.8742676881478143
0.6144905075552112	0.8742676881478143
0.6144905075552112	0.8744930148715637
0.6154591243703991	0.8744930148715637
0.6154591243703991	0.8749436683190627
0.6158465710964742	0.8749436683190627
0.6158465710964742	0.8756196484903109
0.616427741185587	0.8756196484903109
0.616427741185587	0.8760703019378098
0.6166214645486245	0.8760703019378098
0.6166214645486245	0.8762956286615593
0.6168151879116621	0.8762956286615593
0.6168151879116621	0.8765209553853087
0.6175900813638124	0.8765209553853087
0.6175900813638124	0.8774222622803064
0.61778380472685	0.8774222622803064
0.61778380472685	0.8778729157278053
0.6181712514529252	0.8778729157278053
0.6181712514529252	0.8783235691753042
0.618752421542038	0.8783235691753042
0.618752421542038	0.8785488958990536
0.6189461449050756	0.8785488958990536
0.6189461449050756	0.878774222622803
0.6193335916311508	0.878774222622803
0.6193335916311508	0.8789995493465526
0.6195273149941883	0.8789995493465526
0.6195273149941883	0.879224876070302
0.6199147617202635	0.879224876070302
0.6199147617202635	0.8794502027940514
0.6212708252615265	0.8794502027940514
0.6212708252615265	0.8796755295178008
0.6216582719876017	0.8796755295178008
0.6216582719876017	0.8801261829652997
0.6218519953506393	0.8801261829652997
0.6218519953506393	0.8805768364127986
0.6220457187136769	0.8805768364127986
0.6220457187136769	0.880802163136548
0.622433165439752	0.880802163136548
0.622433165439752	0.8810274898602974
0.6226268888027896	0.8810274898602974
0.6226268888027896	0.8814781433077963
0.6232080588919023	0.8814781433077963
0.6232080588919023	0.8817034700315457
0.6235955056179775	0.8817034700315457
0.6235955056179775	0.8819287967552952
0.6251452925222782	0.8819287967552952
0.6251452925222782	0.8828301036502929
0.6253390158853158	0.8828301036502929
0.6253390158853158	0.8830554303740423
0.6259201859744286	0.8830554303740423
0.6259201859744286	0.8832807570977917
0.6265013560635413	0.8832807570977917
0.6265013560635413	0.8839567372690401
0.6268888027896165	0.8839567372690401
0.6268888027896165	0.8841820639927895
0.6272762495156916	0.8841820639927895
0.6272762495156916	0.8846327174402884
0.6274699728787292	0.8846327174402884
0.6274699728787292	0.8848580441640379
0.6284385896939171	0.8848580441640379
0.6284385896939171	0.8850833708877873
0.6286323130569547	0.8850833708877873
0.6286323130569547	0.8853086976115367
0.6290197597830298	0.8853086976115367
0.6290197597830298	0.8855340243352862
0.6292134831460674	0.8855340243352862
0.6292134831460674	0.8857593510590356
0.6296009298721426	0.8857593510590356
0.6296009298721426	0.885984677782785
0.6299883765982177	0.885984677782785
0.6299883765982177	0.8862100045065344
0.6319256102285936	0.8862100045065344
0.6319256102285936	0.886435331230284
0.6321193335916312	0.886435331230284
0.6321193335916312	0.8866606579540334
0.6323130569546688	0.8866606579540334
0.6323130569546688	0.8868859846777828
0.6327005036807439	0.8868859846777828
0.6327005036807439	0.8873366381252816
0.6328942270437815	0.8873366381252816
0.6328942270437815	0.887561964849031
0.634056567222007	0.887561964849031
0.634056567222007	0.8877872915727806
0.6348314606741573	0.8877872915727806
0.6348314606741573	0.88801261829653
0.63541263076327	0.88801261829653
0.63541263076327	0.8886885984677783
0.6356063541263076	0.8886885984677783
0.6356063541263076	0.8891392519152772
0.6359938008523828	0.8891392519152772
0.6359938008523828	0.889589905362776
0.6363812475784579	0.889589905362776
0.6363812475784579	0.8900405588102749
0.6375435877566834	0.8900405588102749
0.6375435877566834	0.8907165389815233
0.637737311119721	0.8907165389815233
0.637737311119721	0.8909418657052727
0.6379310344827587	0.8909418657052727
0.6379310344827587	0.8913925191527715
0.6381247578457963	0.8913925191527715
0.6381247578457963	0.8916178458765209
0.6383184812088338	0.8916178458765209
0.6383184812088338	0.8918431726002704
0.638705927934909	0.8918431726002704
0.638705927934909	0.8929698062190176
0.6388996512979466	0.8929698062190176
0.6388996512979466	0.893195132942767
0.6402557148392096	0.893195132942767
0.6402557148392096	0.8936457863902659
0.6404494382022472	0.8936457863902659
0.6404494382022472	0.8938711131140153
0.6406431615652848	0.8938711131140153
0.6406431615652848	0.8940964398377648
0.6410306082913599	0.8940964398377648
0.6410306082913599	0.8943217665615142
0.6416117783804727	0.8943217665615142
0.6416117783804727	0.8945470932852636
0.6421929484695854	0.8945470932852636
0.6421929484695854	0.8949977467327626
0.6439364587369236	0.8949977467327626
0.6439364587369236	0.8956737269040108
0.6443239054629989	0.8956737269040108
0.6443239054629989	0.8961243803515097
0.6445176288260365	0.8961243803515097
0.6445176288260365	0.8963497070752591
0.6452925222781868	0.8963497070752591
0.6452925222781868	0.8972510139702569
0.6458736923672995	0.8972510139702569
0.6458736923672995	0.8977016674177557
0.6460674157303371	0.8977016674177557
0.6460674157303371	0.8979269941415052
0.6462611390933747	0.8979269941415052
0.6462611390933747	0.8986029743127535
0.6464548624564123	0.8986029743127535
0.6464548624564123	0.8990536277602523
0.6472297559085626	0.8990536277602523
0.6472297559085626	0.8992789544840019
0.6485858194498256	0.8992789544840019
0.6485858194498256	0.8997296079315007
0.6487795428128632	0.8997296079315007
0.6487795428128632	0.8999549346552501
0.6489732661759008	0.8999549346552501
0.6489732661759008	0.9001802613789995
0.6491669895389384	0.9001802613789995
0.6491669895389384	0.900405588102749
0.649360712901976	0.900405588102749
0.649360712901976	0.9013068949977467
0.6499418829910887	0.9013068949977467
0.6499418829910887	0.9017575484452456
0.6503293297171638	0.9017575484452456
0.6503293297171638	0.902433528616494
0.6505230530802014	0.902433528616494
0.6505230530802014	0.9028841820639928
0.6507167764432391	0.9028841820639928
0.6507167764432391	0.9031095087877422
0.6518791166214646	0.9031095087877422
0.6518791166214646	0.9033348355114916
0.6524602867105773	0.9033348355114916
0.6524602867105773	0.903560162235241
0.6532351801627276	0.903560162235241
0.6532351801627276	0.9037854889589906
0.6534289035257652	0.9037854889589906
0.6534289035257652	0.9042361424064894
0.654010073614878	0.9042361424064894
0.654010073614878	0.9044614691302388
0.655366137156141	0.9044614691302388
0.655366137156141	0.9051374493014872
0.6557535838822162	0.9051374493014872
0.6557535838822162	0.9053627760252366
0.6561410306082913	0.9053627760252366
0.6561410306082913	0.905588102748986
0.6565284773343665	0.905588102748986
0.6565284773343665	0.9058134294727355
0.6574970941495545	0.9058134294727355
0.6574970941495545	0.9064894096439837
0.6576908175125921	0.9064894096439837
0.6576908175125921	0.9071653898152321
0.6580782642386672	0.9071653898152321
0.6580782642386672	0.9078413699864804
0.6592406044168927	0.9078413699864804
0.6592406044168927	0.909193330328977
0.6594343277799303	0.909193330328977
0.6594343277799303	0.9094186570527264
0.6598217745060054	0.9094186570527264
0.6598217745060054	0.9096439837764759
0.6609841146842309	0.9096439837764759
0.6609841146842309	0.9100946372239748
0.6613715614103061	0.9100946372239748
0.6613715614103061	0.9103199639477242
0.6617590081363812	0.9103199639477242
0.6617590081363812	0.9105452906714736
0.6621464548624564	0.9105452906714736
0.6621464548624564	0.910770617395223
0.662340178225494	0.910770617395223
0.662340178225494	0.911221270842722
0.6627276249515691	0.911221270842722
0.6627276249515691	0.9114465975664714
0.6629213483146067	0.9114465975664714
0.6629213483146067	0.9116719242902208
0.6638899651297947	0.9116719242902208
0.6638899651297947	0.9118972510139702
0.6644711352189074	0.9118972510139702
0.6644711352189074	0.9125732311852186
0.664664858581945	0.9125732311852186
0.664664858581945	0.9130238846327174
0.6654397520340953	0.9130238846327174
0.6654397520340953	0.9134745380802163
0.6656334753971329	0.9134745380802163
0.6656334753971329	0.9139251915277152
0.6660209221232081	0.9139251915277152
0.6660209221232081	0.9141505182514646
0.6664083688492832	0.9141505182514646
0.6664083688492832	0.9143758449752141
0.6666020922123208	0.9143758449752141
0.6666020922123208	0.9146011716989635
0.6681518791166214	0.9146011716989635
0.6681518791166214	0.9150518251464623
0.6687330492057342	0.9150518251464623
0.6687330492057342	0.9152771518702119
0.6700891127469973	0.9152771518702119
0.6700891127469973	0.9157278053177107
0.6704765594730725	0.9157278053177107
0.6704765594730725	0.9159531320414601
0.6708640061991477	0.9159531320414601
0.6708640061991477	0.916403785488959
0.6718326230143356	0.916403785488959
0.6718326230143356	0.9166291122127084
0.6728012398295234	0.9166291122127084
0.6728012398295234	0.9170797656602073
0.6737698566447113	0.9170797656602073
0.6737698566447113	0.9173050923839567
0.6739635800077489	0.9173050923839567
0.6739635800077489	0.9175304191077062
0.6747384734598992	0.9175304191077062
0.6747384734598992	0.9177557458314556
0.675319643549012	0.9177557458314556
0.675319643549012	0.9182063992789545
0.6757070902750871	0.9182063992789545
0.6757070902750871	0.918431726002704
0.6759008136381247	0.918431726002704
0.6759008136381247	0.9191077061739522
0.6760945370011623	0.9191077061739522
0.6760945370011623	0.9193330328977016
0.6770631538163503	0.9193330328977016
0.6770631538163503	0.919558359621451
0.6782254939945758	0.919558359621451
0.6782254939945758	0.9197836863452006
0.6788066640836885	0.9197836863452006
0.6788066640836885	0.92000901306895
0.6795815575358388	0.92000901306895
0.6795815575358388	0.9206849932401983
0.6805501743510267	0.9206849932401983
0.6805501743510267	0.9211356466876972
0.6807438977140643	0.9211356466876972
0.6807438977140643	0.9213609734114466
0.6809376210771019	0.9213609734114466
0.6809376210771019	0.921586300135196
0.6811313444401395	0.921586300135196
0.6811313444401395	0.9218116268589455
0.6817125145292522	0.9218116268589455
0.6817125145292522	0.9222622803064443
0.6819062378922898	0.9222622803064443
0.6819062378922898	0.9224876070301938
0.6820999612553273	0.9224876070301938
0.6820999612553273	0.9227129337539433
0.6822936846183649	0.9227129337539433
0.6822936846183649	0.9229382604776927
0.6830685780705154	0.9229382604776927
0.6830685780705154	0.9233889139251915
0.6832623014335529	0.9233889139251915
0.6832623014335529	0.9238395673726904
0.6834560247965905	0.9238395673726904
0.6834560247965905	0.9242902208201893
0.6840371948857032	0.9242902208201893
0.6840371948857032	0.9247408742676881
0.6842309182487408	0.9247408742676881
0.6842309182487408	0.925191527715187
0.6844246416117784	0.925191527715187
0.6844246416117784	0.9256421811626859
0.684618364974816	0.9256421811626859
0.684618364974816	0.9260928346101848
0.6850058117008911	0.9260928346101848
0.6850058117008911	0.9265434880576836
0.6855869817900039	0.9265434880576836
0.6855869817900039	0.926768814781433
0.6863618752421542	0.926768814781433
0.6863618752421542	0.9274447949526814
0.6867493219682294	0.9274447949526814
0.6867493219682294	0.9276701216764308
0.6873304920573421	0.9276701216764308
0.6873304920573421	0.9278954484001802
0.68829910887253	0.9278954484001802
0.68829910887253	0.9281207751239297
0.6886865555986051	0.9281207751239297
0.6886865555986051	0.9290220820189274
0.6888802789616427	0.9290220820189274
0.6888802789616427	0.9292474087426769
0.6900426191398683	0.9292474087426769
0.6900426191398683	0.9294727354664263
0.6902363425029059	0.9294727354664263
0.6902363425029059	0.9296980621901757
0.6927547462223944	0.9296980621901757
0.6927547462223944	0.9299233889139252
0.6933359163115071	0.9299233889139252
0.6933359163115071	0.9301487156376747
0.6937233630375823	0.9301487156376747
0.6937233630375823	0.9303740423614241
0.6941108097636575	0.9303740423614241
0.6941108097636575	0.9310500225326723
0.6950794265788454	0.9310500225326723
0.6950794265788454	0.9312753492564219
0.6966292134831461	0.9312753492564219
0.6966292134831461	0.9317260027039207
0.6997287872917474	0.9317260027039207
0.6997287872917474	0.9319513294276701
0.7014722975590856	0.9319513294276701
0.7014722975590856	0.9321766561514195
0.7018597442851607	0.9321766561514195
0.7018597442851607	0.932401982875169
0.7020534676481984	0.932401982875169
0.7020534676481984	0.9326273095989185
0.702247191011236	0.9326273095989185
0.702247191011236	0.9328526363226679
0.7030220844633863	0.9328526363226679
0.7030220844633863	0.9330779630464173
0.7032158078264239	0.9330779630464173
0.7032158078264239	0.9333032897701667
0.7036032545524991	0.9333032897701667
0.7036032545524991	0.9335286164939162
0.7043781480046494	0.9335286164939162
0.7043781480046494	0.9337539432176656
0.7047655947307245	0.9337539432176656
0.7047655947307245	0.933979269941415
0.7053467648198373	0.933979269941415
0.7053467648198373	0.9342045966651645
0.7055404881828748	0.9342045966651645
0.7055404881828748	0.9348805768364128
0.7068965517241379	0.9348805768364128
0.7068965517241379	0.9351059035601622
0.7070902750871755	0.9351059035601622
0.7070902750871755	0.9355565570076612
0.7078651685393258	0.9355565570076612
0.7078651685393258	0.93600721045516
0.7084463386284386	0.93600721045516
0.7084463386284386	0.9362325371789094
0.7103835722588144	0.9362325371789094
0.7103835722588144	0.9364578639026588
0.7109647423479272	0.9364578639026588
0.7109647423479272	0.9373591707976566
0.7111584657109647	0.9373591707976566
0.7111584657109647	0.937584497521406
0.7115459124370399	0.937584497521406
0.7115459124370399	0.9378098242451555
0.7136768694304533	0.9378098242451555
0.7136768694304533	0.9380351509689049
0.7138705927934909	0.9380351509689049
0.7138705927934909	0.9382604776926543
0.7148392096086789	0.9382604776926543
0.7148392096086789	0.9384858044164038
0.7158078264238668	0.9384858044164038
0.7158078264238668	0.9387111311401533
0.7160015497869043	0.9387111311401533
0.7160015497869043	0.9389364578639027
0.7165827198760171	0.9389364578639027
0.7165827198760171	0.9391617845876521
0.7169701666020922	0.9391617845876521
0.7169701666020922	0.9393871113114015
0.7171638899651298	0.9393871113114015
0.7171638899651298	0.9396124380351509
0.7183262301433553	0.9396124380351509
0.7183262301433553	0.9402884182063993
0.7185199535063929	0.9402884182063993
0.7185199535063929	0.9407390716538981
0.7191011235955056	0.9407390716538981
0.7191011235955056	0.9409643983776476
0.7194885703215808	0.9409643983776476
0.7194885703215808	0.941189725101397
0.7196822936846183	0.941189725101397
0.7196822936846183	0.9418657052726453
0.7202634637737311	0.9418657052726453
0.7202634637737311	0.9420910319963948
0.7206509104998062	0.9420910319963948
0.7206509104998062	0.9423163587201442
0.7208446338628438	0.9423163587201442
0.7208446338628438	0.9425416854438936
0.7212320805889191	0.9425416854438936
0.7212320805889191	0.9427670121676431
0.7223944207671446	0.9427670121676431
0.7223944207671446	0.9429923388913926
0.7231693142192949	0.9429923388913926
0.7231693142192949	0.943217665615142
0.7239442076714452	0.943217665615142
0.7239442076714452	0.9434429923388914
0.7260751646648586	0.9434429923388914
0.7260751646648586	0.9438936457863902
0.7264626113909337	0.9438936457863902
0.7264626113909337	0.9441189725101397
0.7268500581170089	0.9441189725101397
0.7268500581170089	0.9445696259576386
0.7293684618364975	0.9445696259576386
0.7293684618364975	0.9450202794051374
0.7297559085625727	0.9450202794051374
0.7297559085625727	0.9454709328526363
0.7307245253777606	0.9454709328526363
0.7307245253777606	0.9456962595763858
0.7322743122820612	0.9456962595763858
0.7322743122820612	0.9459215863001352
0.7326617590081363	0.9459215863001352
0.7326617590081363	0.9465975664713835
0.7328554823711739	0.9465975664713835
0.7328554823711739	0.9470482199188823
0.7342115459124371	0.9470482199188823
0.7342115459124371	0.9472735466426319
0.7344052692754747	0.9472735466426319
0.7344052692754747	0.9477242000901307
0.7353738860906626	0.9477242000901307
0.7353738860906626	0.9479495268138801
0.7361487795428129	0.9479495268138801
0.7361487795428129	0.9481748535376295
0.7367299496319256	0.9481748535376295
0.7367299496319256	0.948400180261379
0.7369236729949632	0.948400180261379
0.7369236729949632	0.9488508337088779
0.7378922898101511	0.9488508337088779
0.7378922898101511	0.9490761604326273
0.7380860131731887	0.9490761604326273
0.7380860131731887	0.9493014871563767
0.7394420767144517	0.9493014871563767
0.7394420767144517	0.9495268138801262
0.7396358000774893	0.9495268138801262
0.7396358000774893	0.949977467327625
0.7400232468035645	0.949977467327625
0.7400232468035645	0.9502027940513745
0.7413793103448276	0.9502027940513745
0.7413793103448276	0.950428120775124
0.7415730337078652	0.950428120775124
0.7415730337078652	0.9506534474988734
0.7431228206121658	0.9506534474988734
0.7431228206121658	0.9508787742226228
0.7438977140643162	0.9508787742226228
0.7438977140643162	0.9511041009463722
0.7456412243316544	0.9511041009463722
0.7456412243316544	0.9513294276701216
0.7473847345989927	0.9513294276701216
0.7473847345989927	0.9515547543938712
0.7479659046881054	0.9515547543938712
0.7479659046881054	0.9517800811176206
0.749515691592406	0.9517800811176206
0.749515691592406	0.95200540784137
0.7497094149554436	0.95200540784137
0.7497094149554436	0.9522307345651194
0.7516466485858194	0.9522307345651194
0.7516466485858194	0.9524560612888688
0.751840371948857	0.9524560612888688
0.751840371948857	0.9526813880126183
0.7524215420379697	0.9526813880126183
0.7524215420379697	0.9529067147363678
0.7533901588531577	0.9529067147363678
0.7533901588531577	0.9531320414601172
0.7561022859356838	0.9531320414601172
0.7561022859356838	0.9533573681838666
0.7568771793878342	0.9533573681838666
0.7568771793878342	0.953582694907616
0.7570709027508717	0.953582694907616
0.7570709027508717	0.9538080216313655
0.7584269662921348	0.9538080216313655
0.7584269662921348	0.9540333483551149
0.7590081363812475	0.9540333483551149
0.7590081363812475	0.9542586750788643
0.7603641999225107	0.9542586750788643
0.7603641999225107	0.9544840018026138
0.7607516466485859	0.9544840018026138
0.7607516466485859	0.9547093285263633
0.7609453700116234	0.9547093285263633
0.7609453700116234	0.9549346552501127
0.7624951569159241	0.9549346552501127
0.7624951569159241	0.9551599819738621
0.7640449438202247	0.9551599819738621
0.7640449438202247	0.9553853086976115
0.7673382409918637	0.9553853086976115
0.7673382409918637	0.9556106354213609
0.7677256877179388	0.9556106354213609
0.7677256877179388	0.9558359621451105
0.768113134444014	0.9558359621451105
0.768113134444014	0.9562866155926093
0.7690817512592019	0.9562866155926093
0.7690817512592019	0.9565119423163587
0.7692754746222394	0.9565119423163587
0.7692754746222394	0.9567372690401081
0.7704378148004649	0.9567372690401081
0.7704378148004649	0.9569625957638576
0.774118558698179	0.9569625957638576
0.774118558698179	0.9574132492113565
0.7750871755133669	0.9574132492113565
0.7750871755133669	0.9576385759351059
0.7762495156915924	0.9576385759351059
0.7762495156915924	0.9580892293826048
0.7770244091437427	0.9580892293826048
0.7770244091437427	0.9583145561063542
0.7774118558698179	0.9583145561063542
0.7774118558698179	0.9585398828301036
0.777799302595893	0.9585398828301036
0.777799302595893	0.9587652095538531
0.7781867493219682	0.9587652095538531
0.7781867493219682	0.9589905362776026
0.7787679194110809	0.9589905362776026
0.7787679194110809	0.959215863001352
0.7791553661371562	0.959215863001352
0.7791553661371562	0.9596665164488508
0.7843858969391708	0.9596665164488508
0.7843858969391708	0.9598918431726002
0.7851607903913211	0.9598918431726002
0.7851607903913211	0.9601171698963497
0.7859356838434716	0.9601171698963497
0.7859356838434716	0.9603424966200992
0.7867105772956219	0.9603424966200992
0.7867105772956219	0.9605678233438486
0.7888415342890353	0.9605678233438486
0.7888415342890353	0.960793150067598
0.7923285548237118	0.960793150067598
0.7923285548237118	0.9610184767913474
0.7932971716388997	0.9610184767913474
0.7932971716388997	0.9612438035150969
0.7971716388996513	0.9612438035150969
0.7971716388996513	0.9614691302388463
0.7991088725300272	0.9614691302388463
0.7991088725300272	0.9616944569625958
0.8072452537776056	0.9616944569625958
0.8072452537776056	0.9619197836863452
0.8109259976753197	0.9619197836863452
0.8109259976753197	0.9621451104100947
0.81170089112747	0.9621451104100947
0.81170089112747	0.9623704371338441
0.8128632313056955	0.9623704371338441
0.8128632313056955	0.9625957638575935
0.8144130182099961	0.9625957638575935
0.8144130182099961	0.9628210905813429
0.8163502518403719	0.9628210905813429
0.8163502518403719	0.9630464173050924
0.8179000387446727	0.9630464173050924
0.8179000387446727	0.9632717440288419
0.8182874854707478	0.9632717440288419
0.8182874854707478	0.9634970707525913
0.818674932196823	0.9634970707525913
0.818674932196823	0.9637223974763407
0.8208058891902363	0.9637223974763407
0.8208058891902363	0.9639477242000901
0.8221619527314994	0.9639477242000901
0.8221619527314994	0.9641730509238395
0.8248740798140256	0.9641730509238395
0.8248740798140256	0.964398377647589
0.8254552499031383	0.964398377647589
0.8254552499031383	0.9646237043713385
0.8339790778767919	0.9646237043713385
0.8339790778767919	0.9648490310950879
0.8351414180550174	0.9648490310950879
0.8351414180550174	0.9650743578188373
0.8390158853157691	0.9650743578188373
0.8390158853157691	0.9652996845425867
0.8392096086788067	0.9652996845425867
0.8392096086788067	0.9655250112663362
0.8442464161177838	0.9655250112663362
0.8442464161177838	0.9657503379900856
0.844633862843859	0.9657503379900856
0.844633862843859	0.9659756647138351
0.8450213095699342	0.9659756647138351
0.8450213095699342	0.9662009914375845
0.8502518403719489	0.9662009914375845
0.8502518403719489	0.966426318161334
0.8525765207283998	0.966426318161334
0.8525765207283998	0.9666516448850834
0.855288647810926	0.9666516448850834
0.855288647810926	0.9668769716088328
0.857613328167377	0.9668769716088328
0.9043006586594343	0.9677782785038306
0.9066253390158853	0.9677782785038306
0.9066253390158853	0.96800360522758
0.9114684230918249	0.96800360522758
0.9114684230918249	0.9682289319513294
0.9174738473459899	0.9682289319513294
0.9174738473459899	0.9684542586750788
0.9180550174351026	0.9684542586750788
0.9180550174351026	0.9686795853988283
0.9221232080588919	0.9686795853988283
0.9221232080588919	0.9689049121225778
0.9223169314219295	0.9689049121225778
0.9223169314219295	0.9691302388463272
0.9225106547849671	0.9691302388463272
0.9225106547849671	0.9693555655700766
0.9273537388609067	0.9693555655700766
0.9273537388609067	0.969580892293826
0.9275474622239442	0.969580892293826
0.9275474622239442	0.9698062190175755
0.9285160790391321	0.9698062190175755
0.9285160790391321	0.9700315457413249
0.9325842696629213	0.9700315457413249
0.9325842696629213	0.9702568724650743
0.9335528864781093	0.9702568724650743
0.9335528864781093	0.9704821991888238
0.9352963967454475	0.9704821991888238
0.9352963967454475	0.9707075259125733
0.9416892677256877	0.9707075259125733
0.9416892677256877	0.9709328526363227
0.9422704378148005	0.9709328526363227
0.9422704378148005	0.9711581793600721
0.9449825648973266	0.9711581793600721
0.9449825648973266	0.9713835060838215
0.9453700116234017	0.9713835060838215
0.9453700116234017	0.9716088328075709
0.94711352189074	0.9716088328075709
0.94711352189074	0.9718341595313205
0.9484695854320031	0.9718341595313205
0.9484695854320031	0.9720594862550699
0.9498256489732662	0.9720594862550699
0.9498256489732662	0.9722848129788193
0.9515691592406044	0.9722848129788193
0.9515691592406044	0.9725101397025687
0.9519566059666796	0.9725101397025687
0.9519566059666796	0.9727354664263181
0.9531189461449051	0.9727354664263181
0.9531189461449051	0.9729607931500676
0.9544750096861682	0.9729607931500676
0.9544750096861682	0.973186119873817
0.9558310732274312	0.973186119873817
0.9558310732274312	0.9734114465975665
0.9593180937621077	0.9734114465975665
0.9593180937621077	0.9736367733213159
0.9597055404881829	0.9736367733213159
0.9597055404881829	0.9738621000450653
0.9598992638512205	0.9738621000450653
0.9598992638512205	0.9743127534925642
0.9606741573033708	0.9743127534925642
0.9606741573033708	0.9745380802163136
0.9608678806664084	0.9745380802163136
0.9608678806664084	0.9747634069400631
0.9629988376598217	0.9747634069400631
0.9629988376598217	0.975214060387562
0.9637737311119721	0.975214060387562
0.9637737311119721	0.9754393871113114
0.9639674544750096	0.9754393871113114
0.9639674544750096	0.9756647138350608
0.9641611778380472	0.9756647138350608
0.9641611778380472	0.9758900405588102
0.9643549012010848	0.9758900405588102
0.9643549012010848	0.9761153672825598
0.9664858581944983	0.9761153672825598
0.9664858581944983	0.9763406940063092
0.967067028283611	0.9763406940063092
0.967067028283611	0.9765660207300586
0.9672607516466486	0.9765660207300586
0.9672607516466486	0.976791347453808
0.9680356450987989	0.976791347453808
0.9680356450987989	0.9772420009013069
0.9695854320030995	0.9772420009013069
0.9695854320030995	0.9774673276250563
0.9701666020922123	0.9774673276250563
0.9701666020922123	0.9776926543488058
0.9705540488182874	0.9776926543488058
0.9705540488182874	0.9783686345200541
0.9715226656334754	0.9783686345200541
0.9715226656334754	0.9785939612438035
0.9726850058117009	0.9785939612438035
0.9726850058117009	0.9788192879675529
0.9744285160790391	0.9788192879675529
0.9744285160790391	0.9797205948625507
0.9748159628051143	0.9797205948625507
0.9748159628051143	0.9799459215863001
0.9752034095311894	0.9799459215863001
0.9752034095311894	0.9801712483100495
0.9763657497094149	0.9801712483100495
0.9763657497094149	0.9806219017575485
0.9767531964354901	0.9806219017575485
0.9767531964354901	0.9808472284812979
0.9773343665246028	0.9808472284812979
0.9773343665246028	0.9815232086525462
0.9783029833397908	0.9815232086525462
0.9783029833397908	0.9817485353762956
0.9788841534289036	0.9817485353762956
0.9788841534289036	0.9821991888237945
0.9790778767919411	0.9821991888237945
0.9790778767919411	0.982424515547544
0.9792716001549787	0.982424515547544
0.9792716001549787	0.9826498422712934
0.9796590468810539	0.9826498422712934
0.9796590468810539	0.9828751689950428
0.9814025571483921	0.9828751689950428
0.9814025571483921	0.9831004957187922
0.9815962805114297	0.9831004957187922
0.9815962805114297	0.9833258224425416
0.9817900038744672	0.9833258224425416
0.9817900038744672	0.9837764758900406
0.98237117396358	0.9837764758900406
0.98237117396358	0.9842271293375394
0.9829523440526927	0.9842271293375394
0.9829523440526927	0.9846777827850383
0.9839209608678806	0.9846777827850383
0.9839209608678806	0.9853537629562866
0.9852770244091438	0.9853537629562866
0.9852770244091438	0.985579089680036
0.9854707477721814	0.985579089680036
0.9854707477721814	0.9862550698512844
0.9860519178612941	0.9862550698512844
0.9860519178612941	0.9864803965750338
0.9864393645873692	0.9864803965750338
0.9864393645873692	0.9869310500225327
0.9866330879504068	0.9869310500225327
0.9866330879504068	0.9871563767462821
0.9868268113134444	0.9871563767462821
0.9868268113134444	0.9876070301937809
0.9874079814025571	0.9876070301937809
0.9874079814025571	0.9880576836412799
0.9881828748547075	0.9880576836412799
0.9881828748547075	0.9885083370887787
0.9887640449438202	0.9885083370887787
0.9891514916698954	0.9900856241550248
0.9897326617590081	0.9900856241550248
0.9897326617590081	0.9905362776025236
0.9899263851220457	0.9905362776025236
0.9899263851220457	0.9907616043262731
0.9905075552111585	0.9907616043262731
0.9905075552111585	0.991212257773772
0.9912824486633088	0.991212257773772
0.9912824486633088	0.9914375844975214
0.9914761720263464	0.9914375844975214
0.9914761720263464	0.9916629112212708
0.9920573421154592	0.9916629112212708
0.9920573421154592	0.9918882379450202
0.9922510654784967	0.9918882379450202
0.9922510654784967	0.9921135646687698
0.9926385122045719	0.9921135646687698
0.9926385122045719	0.9923388913925192
0.9928322355676095	0.9923388913925192
0.9928322355676095	0.9930148715637674
0.993025958930647	0.9930148715637674
0.993025958930647	0.9934655250112663
0.9938008523827974	0.9934655250112663
0.9938008523827974	0.9939161784587652
0.9945757458349477	0.9939161784587652
0.9945757458349477	0.9945921586300135
0.9947694691979853	0.9945921586300135
0.9947694691979853	0.9948174853537629
0.9949631925610228	0.9948174853537629
0.9949631925610228	0.9950428120775124
0.995350639287098	0.9950428120775124
0.995350639287098	0.9952681388012619
0.9965129794653235	0.9952681388012619
0.9965129794653235	0.9954934655250113
0.9972878729174739	0.9954934655250113
0.9972878729174739	0.9957187922487607
0.9978690430065866	0.9957187922487607
0.9978690430065866	0.9963947724200091
0.9982564897326618	0.9963947724200091
0.9982564897326618	0.9966200991437585
0.9984502130956994	0.9966200991437585
0.9984502130956994	0.9970707525912573
0.998643936458737	0.9970707525912573
0.998643936458737	0.9975214060387562
0.9990313831848121	0.9975214060387562
0.9990313831848121	0.9977467327625056
0.9992251065478497	0.9977467327625056
0.9992251065478497	0.9979720594862551
0.9994188299108873	0.9979720594862551
0.9994188299108873	0.9981973862100045
0.9998062766369624	0.9981973862100045
0.9998062766369624	0.998422712933754
1.0	0.998422712933754
1.0	1.0

==> data/roc_b.tex <==
A B
0.0	0.0
0.0	0.0003456619426201175
0.0	0.0017283097131005876
0.0001490979573579842	0.0017283097131005876
0.0001490979573579842	0.002073971655720705
0.0001490979573579842	0.00276529554096094
0.0002981959147159684	0.00276529554096094
0.0002981959147159684	0.009332872450743173
0.0004472938720739526	0.009332872450743173
0.0004472938720739526	0.012098167991704113
0.0005963918294319368	0.012098167991704113
0.0005963918294319368	0.013480815762184583
0.0011927836588638736	0.013480815762184583
0.0011927836588638736	0.015554787417905289
0.0013418816162218577	0.015554787417905289
0.0013418816162218577	0.015900449360525405
0.001490979573579842	0.015900449360525405
0.001490979573579842	0.017283097131005877
0.0016400775309378262	0.017283097131005877
0.0016400775309378262	0.018320082958866227
0.0017891754882958103	0.018320082958866227
0.0017891754882958103	0.018665744901486345
0.0019382734456537946	0.018665744901486345
0.0019382734456537946	0.020394054614586935
0.0023855673177277472	0.020394054614586935
0.0023855673177277472	0.020739716557207053
0.0026837632324437154	0.020739716557207053
0.0026837632324437154	0.024196335983408226
0.0028328611898017	0.024196335983408226
0.0028328611898017	0.027307293466989284
0.0028328611898017	0.02799861735222952
0.003131057104517668	0.02799861735222952
0.003131057104517668	0.029726927065330106
0.0032801550618756525	0.029726927065330106
0.0032801550618756525	0.03180089872105081
0.0032801550618756525	0.032492222606291046
0.0032801550618756525	0.0335292084341514
0.0032801550618756525	0.034220532319391636
0.0034292530192336365	0.034220532319391636
0.0034292530192336365	0.03491185620463187
0.0035783509765916206	0.03491185620463187
0.0035783509765916206	0.03525751814725199
0.0037274489339496047	0.03525751814725199
0.0037274489339496047	0.03767715174559281
0.003876546891307589	0.03767715174559281
0.003876546891307589	0.040096785343933634
0.004025644848665574	0.040096785343933634
0.004025644848665574	0.04182509505703422
0.004174742806023557	0.04182509505703422
0.004174742806023557	0.042170756999654335
0.004323840763381542	0.042170756999654335
0.004323840763381542	0.04597303836847563
0.0044729387207395254	0.04597303836847563
0.0044729387207395254	0.04908399585205669
0.00462203667809751	0.04908399585205669
0.00462203667809751	0.05772554441755963
0.0047711346354554944	0.05772554441755963
0.0047711346354554944	0.058762530245419976
0.005069330550171463	0.058762530245419976
0.005069330550171463	0.06360179744210162
0.005218428507529447	0.06360179744210162
0.005218428507529447	0.06947805046664363
0.005367526464887431	0.06947805046664363
0.005367526464887431	0.07016937435188386
0.005516624422245415	0.07016937435188386
0.005516624422245415	0.07189768406498445
0.0056657223796034	0.07189768406498445
0.0056657223796034	0.07328033183546491
0.005814820336961383	0.07328033183546491
0.005814820336961383	0.07811959903214656
0.005963918294319368	0.07811959903214656
0.005963918294319368	0.07915658486000691
0.006113016251677352	0.07915658486000691
0.006113016251677352	0.08157621845834774
0.006262114209035336	0.08157621845834774
0.006262114209035336	0.08745247148288973
0.0064112121663933205	0.08745247148288973
0.0064112121663933205	0.09125475285171103
0.006560310123751305	0.09125475285171103
0.006560310123751305	0.09194607673695127
0.006709408081109289	0.09194607673695127
0.006709408081109289	0.09540269616315243
0.006858506038467273	0.09540269616315243
0.006858506038467273	0.09713100587625302
0.007007603995825258	0.09713100587625302
0.007007603995825258	0.09816799170411337
0.007156701953183241	0.09816799170411337
0.007156701953183241	0.09885931558935361
0.007454897867899209	0.09885931558935361
0.007454897867899209	0.09920497753197373
0.007753093782615178	0.09920497753197373
0.007753093782615178	0.09955063947459385
0.007902191739973162	0.09955063947459385
0.007902191739973162	0.10369858278603526
0.008051289697331147	0.10369858278603526
0.008051289697331147	0.1085378499827169
0.008200387654689131	0.1085378499827169
0.008200387654689131	0.10957483581057725
0.008349485612047115	0.10957483581057725
0.008349485612047115	0.11268579329415832
0.008647681526763084	0.11268579329415832
0.008647681526763084	0.11337711717939855
0.008796779484121067	0.11337711717939855
0.008796779484121067	0.11648807466297961
0.009094975398837036	0.11648807466297961
0.009094975398837036	0.11752506049083995
0.00924407335619502	0.11752506049083995
0.00924407335619502	0.11787072243346007
0.009393171313553004	0.11787072243346007
0.009393171313553004	0.11925337020394054
0.009542269270910989	0.11925337020394054
0.009542269270910989	0.11959903214656066
0.009691367228268973	0.11959903214656066
0.009691367228268973	0.11994469408918078
0.009840465185626956	0.11994469408918078
0.009840465185626956	0.12270998963014172
0.009989563142984942	0.12270998963014172
0.009989563142984942	0.12340131351538196
0.010138661100342925	0.12340131351538196
0.010138661100342925	0.12512962322848253
0.010436857015058894	0.12512962322848253
0.010436857015058894	0.12547528517110265
0.010884150887132847	0.12547528517110265
0.010884150887132847	0.12582094711372277
0.011182346801848814	0.12582094711372277
0.011182346801848814	0.1261666090563429
0.0113314447592068	0.1261666090563429
0.0113314447592068	0.12685793294158312
0.012226032503354705	0.12685793294158312
0.012226032503354705	0.12754925682682336
0.012375130460712688	0.12754925682682336
0.012524228418070672	0.12789491876944348
0.012524228418070672	0.1282405807120636
0.012822424332786641	0.1282405807120636
0.012822424332786641	0.1285862426546837
0.012971522290144625	0.1285862426546837
0.012971522290144625	0.12893190459730383
0.013418816162218577	0.12893190459730383
0.013418816162218577	0.12927756653992395
0.013567914119576563	0.12927756653992395
0.013567914119576563	0.12996889042516419
0.013717012076934546	0.12996889042516419
0.013717012076934546	0.13169720013826478
0.01386611003429253	0.13169720013826478
0.01386611003429253	0.1320428620808849
0.014164305949008499	0.1320428620808849
0.014164305949008499	0.132388524023505
0.014313403906366482	0.132388524023505
0.014313403906366482	0.13273418596612513
0.014611599821082451	0.13273418596612513
0.014611599821082451	0.13377117179398548
0.014760697778440435	0.13377117179398548
0.014760697778440435	0.1341168337366056
0.014909795735798419	0.1341168337366056
0.014909795735798419	0.13446249567922572
0.015058893693156404	0.13446249567922572
0.015058893693156404	0.1358451434497062
0.015655285522588342	0.1358451434497062
0.015655285522588342	0.1361908053923263
0.016251677352020277	0.1361908053923263
0.016251677352020277	0.13688212927756654
0.016400775309378262	0.13688212927756654
0.016400775309378262	0.13861043899066713
0.01669897122409423	0.13861043899066713
0.01669897122409423	0.13895610093328725
0.016848069181452215	0.13930176287590737
0.016848069181452215	0.1396474248185275
0.017295363053526167	0.1396474248185275
0.017295363053526167	0.1399930867611476
0.017444461010884153	0.1399930867611476
0.017444461010884153	0.14103007258900796
0.017593558968242134	0.14103007258900796
0.017593558968242134	0.14137573453162808
0.01774265692560012	0.14137573453162808
0.01774265692560012	0.1417213964742482
0.017891754882958102	0.1417213964742482
0.017891754882958102	0.1420670584168683
0.018040852840316087	0.14241272035948843
0.018040852840316087	0.14275838230210855
0.018189950797674072	0.14275838230210855
0.018189950797674072	0.1444866920152091
0.018637244669748025	0.1444866920152091
0.018637244669748025	0.14517801590044935
0.018786342627106007	0.14517801590044935
0.018786342627106007	0.14586933978568958
0.01923363649917996	0.14586933978568958
0.01923363649917996	0.1462150017283097
0.019382734456537945	0.1462150017283097
0.019382734456537945	0.14656066367092982
0.01953183241389593	0.14656066367092982
0.01953183241389593	0.14863463532665053
0.019680930371253912	0.14863463532665053
0.019680930371253912	0.14898029726927065
0.019830028328611898	0.14898029726927065
0.019830028328611898	0.14932595921189076
0.019979126285969883	0.14932595921189076
0.019979126285969883	0.15070860698237123
0.020128224243327865	0.15070860698237123
0.020128224243327865	0.15105426892499135
0.02027732220068585	0.15105426892499135
0.02027732220068585	0.15139993086761147
0.020575518115401818	0.15139993086761147
0.020575518115401818	0.1520912547528517
0.020724616072759803	0.1520912547528517
0.020724616072759803	0.15347390252333218
0.02132100790219174	0.15347390252333218
0.02132100790219174	0.1538195644659523
0.021470105859549723	0.1538195644659523
0.021470105859549723	0.15416522640857241
0.021917399731623675	0.15416522640857241
0.021917399731623675	0.15623919806429312
0.022215595646339646	0.15623919806429312
0.022215595646339646	0.15658486000691324
0.022364693603697628	0.15658486000691324
0.022364693603697628	0.15693052194953336
0.023557477262561504	0.15693052194953336
0.023557477262561504	0.1579675077773937
0.02415386909199344	0.1579675077773937
0.02415386909199344	0.15831316972001383
0.02460116296406739	0.15831316972001383
0.02460116296406739	0.15900449360525407
0.024750260921425377	0.15900449360525407
0.024750260921425377	0.1596958174904943
0.025048456836141344	0.1596958174904943
0.025048456836141344	0.16004147943311442
0.02519755479349933	0.16004147943311442
0.02519755479349933	0.16038714137573454
0.025346652750857315	0.16038714137573454
0.025346652750857315	0.1614241272035949
0.025793946622931267	0.1614241272035949
0.025793946622931267	0.161769789146215
0.02594304458028925	0.161769789146215
0.02594304458028925	0.16211545108883513
0.026539436409721187	0.16211545108883513
0.026539436409721187	0.1634980988593156
0.026837632324437154	0.1634980988593156
0.026837632324437154	0.16453508468717595
0.02698673028179514	0.16453508468717595
0.02698673028179514	0.16488074662979607
0.027135828239153125	0.16488074662979607
0.027135828239153125	0.1655720705150363
0.027434024153869092	0.1655720705150363
0.027434024153869092	0.1679917041133771
0.02773222006858506	0.1679917041133771
0.02773222006858506	0.1700656757690978
0.027881318025943045	0.1700656757690978
0.027881318025943045	0.17041133771171793
0.02803041598330103	0.17041133771171793
0.02803041598330103	0.17110266159695817
0.028328611898016998	0.17110266159695817
0.028328611898016998	0.1717939854821984
0.028477709855374983	0.1717939854821984
0.028477709855374983	0.17248530936743864
0.028626807812732965	0.17248530936743864
0.028626807812732965	0.17317663325267887
0.02877590577009095	0.17317663325267887
0.02877590577009095	0.1773245765641203
0.028925003727448936	0.1773245765641203
0.028925003727448936	0.17870722433460076
0.029074101684806918	0.17870722433460076
0.029074101684806918	0.18181818181818182
0.029223199642164903	0.18181818181818182
0.029223199642164903	0.18458347735914277
0.02937229759952289	0.18458347735914277
0.02937229759952289	0.18562046318700312
0.02952139555688087	0.18562046318700312
0.02952139555688087	0.18769443484272383
0.029670493514238856	0.18769443484272383
0.029670493514238856	0.1897684064984445
0.029968689428954823	0.1897684064984445
0.029968689428954823	0.19011406844106463
0.030117787386312808	0.19011406844106463
0.030117787386312808	0.19080539232630486
0.030415983301028775	0.19080539232630486
0.030415983301028775	0.19184237815416522
0.031012375130460713	0.19184237815416522
0.031012375130460713	0.19253370203940545
0.031161473087818695	0.19253370203940545
0.031161473087818695	0.19287936398202557
0.03175786491725063	0.19287936398202557
0.03175786491725063	0.19391634980988592
0.03190696287460862	0.19391634980988592
0.03190696287460862	0.19426201175250604
0.03235425674668257	0.19426201175250604
0.03235425674668257	0.1952989975803664
0.03250335470404055	0.1952989975803664
0.03250335470404055	0.19599032146560663
0.03265245266139854	0.19599032146560663
0.03265245266139854	0.19702730729346699
0.032801550618756524	0.19702730729346699
0.032801550618756524	0.19771863117870722
0.033099746533472495	0.19771863117870722
0.033099746533472495	0.19806429312132734
0.03339794244818846	0.19806429312132734
0.03339794244818846	0.19875561700656758
0.03369613836290443	0.19875561700656758
0.03369613836290443	0.19979260283442793
0.033845236320262415	0.19979260283442793
0.033845236320262415	0.20048392671966817
0.03414343223497838	0.20048392671966817
0.03414343223497838	0.20152091254752852
0.03444162814969435	0.20152091254752852
0.03444162814969435	0.20221223643276875
0.03473982406441032	0.20221223643276875
0.03473982406441032	0.2032492222606291
0.034888922021768305	0.2032492222606291
0.034888922021768305	0.20359488420324923
0.03518711793648427	0.20359488420324923
0.03518711793648427	0.20394054614586934
0.035336215893842254	0.20394054614586934
0.035336215893842254	0.20636017974421017
0.03548531385120024	0.20636017974421017
0.03548531385120024	0.20808848945731076
0.03593260772327419	0.20808848945731076
0.03593260772327419	0.20843415139993088
0.036081705680632174	0.20843415139993088
0.036081705680632174	0.21016246111303147
0.03623080363799016	0.21016246111303147
0.03623080363799016	0.21050812305565159
0.03652899955270613	0.21050812305565159
0.03652899955270613	0.21223643276875215
0.036827195467422094	0.21223643276875215
0.036827195467422094	0.21361908053923262
0.03727448933949605	0.21361908053923262
0.03727448933949605	0.21431040442447286
0.037572685254212014	0.21431040442447286
0.037572685254212014	0.2153473902523332
0.037870881168927985	0.2153473902523332
0.037870881168927985	0.21845834773591427
0.03801997912628597	0.21845834773591427
0.03801997912628597	0.2188040096785344
0.038169077083643956	0.2188040096785344
0.038169077083643956	0.2191496716211545
0.03831817504100194	0.2191496716211545
0.03831817504100194	0.21949533356377463
0.038616370955717905	0.21949533356377463
0.038616370955717905	0.22018665744901486
0.039361860742507825	0.22018665744901486
0.039361860742507825	0.22053231939163498
0.03951095869986581	0.22053231939163498
0.03951095869986581	0.2208779813342551
0.039660056657223795	0.2208779813342551
0.039660056657223795	0.22156930521949533
0.03980915461458178	0.22156930521949533
0.03980915461458178	0.22191496716211545
0.04010735052929775	0.22191496716211545
0.04010735052929775	0.22433460076045628
0.04025644848665573	0.22433460076045628
0.04025644848665573	0.2246802627030764
0.040405546444013715	0.2246802627030764
0.040405546444013715	0.2267542343587971
0.0405546444013717	0.2267542343587971
0.0405546444013717	0.22744555824403734
0.04085284031608767	0.22744555824403734
0.04085284031608767	0.22813688212927757
0.041449232145519606	0.22813688212927757
0.041449232145519606	0.2288282060145178
0.04159833010287759	0.2288282060145178
0.04159833010287759	0.22917386795713793
0.042194721932309526	0.22917386795713793
0.042194721932309526	0.22986519184237816
0.04234381988966751	0.22986519184237816
0.04234381988966751	0.2305565157276184
0.042492917847025496	0.2305565157276184
0.042492917847025496	0.23090217767023852
0.04279111376174147	0.23090217767023852
0.04279111376174147	0.2326304873833391
0.042940211719099446	0.2326304873833391
0.042940211719099446	0.23297614932595923
0.04308930967645743	0.23297614932595923
0.04308930967645743	0.23332181126857934
0.043238407633815416	0.23332181126857934
0.043238407633815416	0.23366747321119943
0.04353660354853139	0.23366747321119943
0.04353660354853139	0.2347044590390598
0.04368570150588937	0.2347044590390598
0.04368570150588937	0.2350501209816799
0.04428209333532131	0.2350501209816799
0.04428209333532131	0.23574144486692014
0.044729387207395256	0.23574144486692014
0.044729387207395256	0.23608710680954026
0.04487848516475324	0.23608710680954026
0.04487848516475324	0.2371240926374006
0.04517668107946921	0.2371240926374006
0.04517668107946921	0.23746975458002073
0.04547487699418518	0.23746975458002073
0.04547487699418518	0.23781541652264085
0.04562397495154316	0.23781541652264085
0.04562397495154316	0.23850674040788108
0.04577307290890115	0.23850674040788108
0.04577307290890115	0.23954372623574144
0.04592217086625913	0.23954372623574144
0.04592217086625913	0.24161769789146215
0.04636946473833309	0.24161769789146215
0.04636946473833309	0.24196335983408226
0.04651856269569107	0.24196335983408226
0.04651856269569107	0.24334600760456274
0.04681675861040704	0.24334600760456274
0.04681675861040704	0.24369166954718285
0.04696585656776502	0.24369166954718285
0.04696585656776502	0.24403733148980297
0.04726405248248099	0.24403733148980297
0.04726405248248099	0.2443829934324231
0.04756224839719696	0.2443829934324231
0.04756224839719696	0.24507431731766333
0.04771134635455494	0.24507431731766333
0.04771134635455494	0.24611130314552368
0.04786044431191293	0.24611130314552368
0.04786044431191293	0.24680262703076392
0.04800954226927091	0.24680262703076392
0.04800954226927091	0.24991358451434498
0.04830773818398688	0.24991358451434498
0.04830773818398688	0.2509505703422053
0.04845683614134486	0.2509505703422053
0.04845683614134486	0.25164189422744554
0.04860593409870285	0.25164189422744554
0.04860593409870285	0.2519875561700657
0.0490532279707768	0.2519875561700657
0.0490532279707768	0.2526788800553059
0.04950052184285075	0.2526788800553059
0.04950052184285075	0.253024541997926
0.04964961980020874	0.253024541997926
0.04964961980020874	0.25337020394054616
0.049798717757566724	0.25337020394054616
0.049798717757566724	0.25578983753888695
0.05024601162964067	0.25578983753888695
0.05024601162964067	0.2571724853093674
0.05099150141643059	0.2571724853093674
0.05099150141643059	0.25786380919460766
0.05114059937378858	0.25786380919460766
0.05114059937378858	0.25890079502246804
0.051289697331146564	0.25890079502246804
0.051289697331146564	0.25924645696508813
0.05143879528850455	0.25924645696508813
0.05143879528850455	0.2595921189077083
0.051587893245862534	0.2595921189077083
0.051587893245862534	0.2602834427929485
0.05173699120322051	0.2602834427929485
0.05173699120322051	0.261666090563429
0.05218428507529447	0.261666090563429
0.05218428507529447	0.2627030763912893
0.052333383032652454	0.2627030763912893
0.052333383032652454	0.2637400622191497
0.05322797077680036	0.2637400622191497
0.05322797077680036	0.2640857241617698
0.05352616669151632	0.2640857241617698
0.05352616669151632	0.26443138610438993
0.05367526464887431	0.26443138610438993
0.05367526464887431	0.26477704804701
0.05427165647830625	0.26477704804701
0.05427165647830625	0.26512270998963017
0.05442075443566423	0.26512270998963017
0.05442075443566423	0.2658140338748704
0.054569852393022214	0.2658140338748704
0.054569852393022214	0.26685101970273073
0.054868048307738185	0.26685101970273073
0.054868048307738185	0.26788800553059106
0.05501714626509617	0.26788800553059106
0.055166244222454155	0.2682336674732112
0.055613538094528105	0.2682336674732112
0.055613538094528105	0.27099896301417215
0.05576263605188609	0.27099896301417215
0.05576263605188609	0.27341859661251294
0.055911734009244075	0.27341859661251294
0.055911734009244075	0.27652955409609403
0.05606083196660206	0.27652955409609403
0.05606083196660206	0.27722087798133427
0.05620992992396004	0.27722087798133427
0.05620992992396004	0.279294849637055
0.056359027881318025	0.279294849637055
0.056359027881318025	0.2799861735222952
0.05650812583867601	0.2799861735222952
0.05650812583867601	0.2813688212927757
0.056657223796033995	0.2813688212927757
0.056657223796033995	0.282405807120636
0.05680632175339198	0.282405807120636
0.05680632175339198	0.28275146906325616
0.056955419710749966	0.28275146906325616
0.056955419710749966	0.28309713100587625
0.057104517668107944	0.28309713100587625
0.057104517668107944	0.28482544071897686
0.05725361562546593	0.28482544071897686
0.05725361562546593	0.2858624265468372
0.057700909497539886	0.2858624265468372
0.057700909497539886	0.2879363982025579
0.05785000745489787	0.2879363982025579
0.05785000745489787	0.28966470791565846
0.058148203369613835	0.28966470791565846
0.058148203369613835	0.2938126512270999
0.05829730132697182	0.2938126512270999
0.05829730132697182	0.29415831316972
0.058446399284329806	0.29415831316972
0.058446399284329806	0.2945039751123401
0.05874459519904578	0.2945039751123401
0.05874459519904578	0.2976149325959212
0.058893693156403755	0.2976149325959212
0.058893693156403755	0.2979605945385413
0.059191889071119726	0.2979605945385413
0.059191889071119726	0.29899758036640167
0.05934098702847771	0.29899758036640167
0.05934098702847771	0.2996889042516419
0.059490084985835696	0.2996889042516419
0.059490084985835696	0.300034566194262
0.05978828090055166	0.300034566194262
0.05978828090055166	0.30245419979260285
0.059937378857909646	0.30245419979260285
0.059937378857909646	0.3034911856204632
0.060235574772625616	0.3034911856204632
0.060235574772625616	0.3038368475630833
0.06053377068734158	0.3038368475630833
0.06053377068734158	0.3041825095057034
0.060682868644699565	0.3041825095057034
0.060682868644699565	0.3055651572761839
0.06083196660205755	0.3055651572761839
0.06083196660205755	0.30591081921880403
0.060981064559415536	0.30591081921880403
0.060981064559415536	0.3062564811614241
0.06113016251677352	0.3062564811614241
0.06113016251677352	0.3072934669892845
0.06127926047413151	0.3072934669892845
0.06127926047413151	0.30833045281714483
0.061726554346205456	0.30833045281714483
0.061726554346205456	0.308676114759765
0.06202475026092143	0.308676114759765
0.06202475026092143	0.30902177670238506
0.06217384821827941	0.30902177670238506
0.06217384821827941	0.31005876253024545
0.06232294617563739	0.31005876253024545
0.06232294617563739	0.31040442447286554
0.062472044132995376	0.31040442447286554
0.062472044132995376	0.31144141030072586
0.06262114209035337	0.31144141030072586
0.06262114209035337	0.311787072243346
0.06306843596242731	0.311787072243346
0.06306843596242731	0.31247839612858624
0.06351572983450127	0.31247839612858624
0.06351572983450127	0.3131697200138265
0.06366482779185925	0.3131697200138265
0.06366482779185925	0.31489802972692704
0.06381392574921724	0.31489802972692704
0.06381392574921724	0.3152436916695472
0.06396302370657522	0.3152436916695472
0.06396302370657522	0.31697200138264775
0.06411212166393321	0.31697200138264775
0.06411212166393321	0.3173176633252679
0.0642612196212912	0.3173176633252679
0.0642612196212912	0.32008295886622884
0.06455941553600715	0.32008295886622884
0.06455941553600715	0.3238852402350501
0.06470851349336514	0.3238852402350501
0.06470851349336514	0.3269961977186312
0.06485761145072312	0.3269961977186312
0.06485761145072312	0.32768752160387143
0.06515580736543909	0.32768752160387143
0.06515580736543909	0.32872450743173176
0.06530490532279708	0.32872450743173176
0.06530490532279708	0.329415831316972
0.06664678693901893	0.329415831316972
0.06664678693901893	0.3328724507431732
0.0669449828537349	0.3328724507431732
0.0669449828537349	0.33425509851365365
0.06709408081109289	0.33425509851365365
0.06709408081109289	0.3349464223988939
0.06724317876845087	0.3349464223988939
0.06724317876845087	0.3356377462841341
0.06739227672580886	0.3356377462841341
0.06739227672580886	0.3370203940546146
0.06769047264052483	0.3370203940546146
0.06769047264052483	0.33840304182509506
0.06783957059788281	0.33840304182509506
0.06783957059788281	0.33874870376771515
0.0679886685552408	0.33874870376771515
0.0679886685552408	0.33978568959557554
0.06813776651259877	0.33978568959557554
0.06813776651259877	0.3401313515381956
0.06828686446995676	0.3401313515381956
0.06828686446995676	0.34220532319391633
0.06843596242731474	0.34220532319391633
0.06843596242731474	0.3432423090217767
0.06858506038467273	0.3432423090217767
0.06858506038467273	0.3446249567922572
0.06873415834203071	0.3446249567922572
0.06873415834203071	0.34842723816107846
0.06903235425674668	0.34842723816107846
0.06903235425674668	0.3491185620463187
0.06918145221410467	0.3491185620463187
0.06918145221410467	0.3501555478741791
0.06933055017146265	0.3501555478741791
0.06933055017146265	0.35050120981679916
0.06962874608617863	0.35050120981679916
0.06962874608617863	0.35153819564465955
0.06977784404353661	0.35153819564465955
0.06977784404353661	0.35188385758727964
0.06992694200089458	0.35188385758727964
0.06992694200089458	0.35257518147251987
0.07022513791561055	0.35257518147251987
0.07022513791561055	0.35292084341514
0.07037423587296854	0.35292084341514
0.07037423587296854	0.35395782924300034
0.07052333383032652	0.35395782924300034
0.07052333383032652	0.3577601106118216
0.07067243178768451	0.3577601106118216
0.07067243178768451	0.35810577255444176
0.0708215297450425	0.35810577255444176
0.0708215297450425	0.358797096439682
0.07097062770240048	0.358797096439682
0.07097062770240048	0.36156239198064294
0.07111972565975846	0.36156239198064294
0.07111972565975846	0.36363636363636365
0.07141792157447444	0.36363636363636365
0.07141792157447444	0.364673349464224
0.07156701953183241	0.364673349464224
0.07156701953183241	0.3653646733494642
0.07171611748919039	0.3653646733494642
0.07171611748919039	0.36605599723470444
0.07186521544654838	0.36605599723470444
0.07186521544654838	0.36778430694780506
0.07201431340390636	0.36778430694780506
0.07201431340390636	0.3688212927756654
0.07231250931862233	0.3688212927756654
0.07231250931862233	0.36916695471828553
0.07246160727598032	0.36916695471828553
0.07246160727598032	0.3708952644313861
0.0726107052333383	0.3708952644313861
0.0726107052333383	0.37366055997234704
0.07275980319069629	0.37366055997234704
0.07275980319069629	0.3740062219149672
0.07290890114805428	0.3740062219149672
0.07290890114805428	0.376425855513308
0.07305799910541226	0.376425855513308
0.07305799910541226	0.3788454891116488
0.07335619502012822	0.3788454891116488
0.07335619502012822	0.38126512270998963
0.0735052929774862	0.38126512270998963
0.0735052929774862	0.3840304182509506
0.07395258684956016	0.3840304182509506
0.07395258684956016	0.38437608019357067
0.07410168480691814	0.38437608019357067
0.07410168480691814	0.3847217421361908
0.07425078276427613	0.3847217421361908
0.07425078276427613	0.3850674040788109
0.07439988072163412	0.3850674040788109
0.07439988072163412	0.3871413757345316
0.0745489786789921	0.3871413757345316
0.0745489786789921	0.388178361562392
0.07469807663635009	0.388178361562392
0.07469807663635009	0.3905979951607328
0.07484717459370807	0.3905979951607328
0.07484717459370807	0.3937089526443139
0.07529446846578201	0.3937089526443139
0.07529446846578201	0.3961285862426547
0.07544356642314	0.3961285862426547
0.07544356642314	0.3982025578983754
0.07559266438049798	0.3982025578983754
0.07559266438049798	0.3988938817836156
0.07574176233785597	0.3988938817836156
0.07574176233785597	0.4044244728655375
0.07589086029521395	0.4044244728655375
0.07589086029521395	0.4047701348081576
0.07603995825257194	0.4047701348081576
0.07603995825257194	0.4085724161769789
0.07618905620992993	0.4085724161769789
0.07618905620992993	0.408918078119599
0.07633815416728791	0.408918078119599
0.07633815416728791	0.40960940200483925
0.07663635008200388	0.40960940200483925
0.07663635008200388	0.4123746975458002
0.07678544803936187	0.4123746975458002
0.07678544803936187	0.4141030072589008
0.07693454599671984	0.4141030072589008
0.07693454599671984	0.4196335983408227
0.07708364395407782	0.4196335983408227
0.07708364395407782	0.420670584168683
0.07723274191143581	0.420670584168683
0.07723274191143581	0.4241272035948842
0.0773818398687938	0.4241272035948842
0.0773818398687938	0.4275838230210854
0.07753093782615178	0.4275838230210854
0.07753093782615178	0.4286208088489457
0.07782913374086775	0.4286208088489457
0.07782913374086775	0.42896647079156586
0.07797823169822574	0.42896647079156586
0.07797823169822574	0.42931213273418595
0.07812732965558372	0.42931213273418595
0.07812732965558372	0.4317317663325268
0.0782764276129417	0.4317317663325268
0.0782764276129417	0.4338057379882475
0.07842552557029969	0.4338057379882475
0.07842552557029969	0.43484272381610783
0.07857462352765768	0.43484272381610783
0.07857462352765768	0.44106463878326996
0.07902191739973162	0.44106463878326996
0.07902191739973162	0.4414103007258901
0.0791710153570896	0.4414103007258901
0.0791710153570896	0.4459039059799516
0.07932011331444759	0.4459039059799516
0.07932011331444759	0.44694089180781194
0.07946921127180558	0.44694089180781194
0.07946921127180558	0.450051849291393
0.07976740718652155	0.450051849291393
0.07976740718652155	0.45074317317663326
0.07991650514387953	0.45074317317663326
0.07991650514387953	0.4517801590044936
0.08006560310123752	0.4517801590044936
0.08006560310123752	0.45212582094711373
0.0802147010585955	0.45212582094711373
0.0802147010585955	0.4548911164880747
0.08036379901595349	0.4548911164880747
0.08036379901595349	0.4555824403733149
0.08051289697331146	0.4555824403733149
0.08051289697331146	0.45661942620117524
0.08081109288802743	0.45661942620117524
0.08081109288802743	0.4611130314552368
0.0811092888027434	0.4611130314552368
0.0811092888027434	0.46180435534047704
0.08125838676010139	0.46180435534047704
0.08125838676010139	0.4635326650535776
0.08140748471745937	0.4635326650535776
0.08140748471745937	0.46422398893881783
0.08155658267481736	0.46422398893881783
0.08155658267481736	0.46491531282405807
0.08185477858953333	0.46491531282405807
0.08185477858953333	0.46871759419287934
0.0821529745042493	0.46871759419287934
0.0821529745042493	0.4697545800207397
0.08230207246160727	0.4697545800207397
0.08230207246160727	0.47079156584860005
0.08245117041896526	0.47079156584860005
0.08245117041896526	0.47251987556170066
0.08260026837632324	0.47251987556170066
0.08260026837632324	0.47597649498790184
0.08274936633368123	0.47597649498790184
0.08274936633368123	0.4766678188731421
0.08289846429103921	0.4766678188731421
0.08289846429103921	0.4797787763567231
0.0830475622483972	0.4797787763567231
0.0830475622483972	0.48254407189768406
0.08319666020575518	0.48254407189768406
0.08319666020575518	0.48358105772554444
0.08334575816311317	0.48358105772554444
0.08334575816311317	0.48565502938126515
0.08364395407782914	0.48565502938126515
0.08364395407782914	0.4870376771517456
0.08379305203518712	0.4870376771517456
0.08379305203518712	0.4873833390943657
0.08409124794990308	0.4873833390943657
0.08409124794990308	0.48772900103698585
0.08424034590726107	0.48772900103698585
0.08424034590726107	0.4884203249222261
0.08438944386461905	0.4884203249222261
0.08438944386461905	0.49014863463532665
0.08453854182197704	0.49014863463532665
0.08453854182197704	0.4929139301762876
0.08468763977933502	0.4929139301762876
0.08468763977933502	0.49809885931558934
0.08483673773669301	0.49809885931558934
0.08483673773669301	0.5019011406844106
0.08498583569405099	0.5019011406844106
0.08498583569405099	0.5022468026270308
0.08528403160876696	0.5022468026270308
0.08528403160876696	0.5053577601106118
0.08543312956612495	0.5053577601106118
0.08543312956612495	0.5084687175941929
0.0857313254808409	0.5084687175941929
0.0857313254808409	0.5091600414794332
0.08588042343819889	0.5091600414794332
0.08588042343819889	0.5098513653646733
0.08602952139555688	0.5098513653646733
0.08602952139555688	0.5108883511925337
0.08617861935291486	0.5108883511925337
0.08617861935291486	0.511925337020394
0.08632771731027285	0.511925337020394
0.08632771731027285	0.5122709989630142
0.08662591322498882	0.5122709989630142
0.08662591322498882	0.5136536467334947
0.08692410913970479	0.5136536467334947
0.08692410913970479	0.5181472519875562
0.08707320709706277	0.5181472519875562
0.08707320709706277	0.5184929139301763
0.08722230505442076	0.5184929139301763
0.08722230505442076	0.5198755617006567
0.08737140301177874	0.5198755617006567
0.08737140301177874	0.520566885585897
0.08796779484121067	0.520566885585897
0.08796779484121067	0.5216038714137573
0.08811689279856866	0.5216038714137573
0.08811689279856866	0.5236778430694781
0.08826599075592664	0.5236778430694781
0.08826599075592664	0.5247148288973384
0.0887132846280006	0.5247148288973384
0.0887132846280006	0.5250604908399585
0.08886238258535858	0.5250604908399585
0.08886238258535858	0.5260974766678189
0.08916057850007456	0.5260974766678189
0.08916057850007456	0.5267888005530591
0.08930967645743253	0.5267888005530591
0.08930967645743253	0.5278257863809195
0.08945877441479051	0.5278257863809195
0.08945877441479051	0.5292084341514
0.0896078723721485	0.5292084341514
0.0896078723721485	0.532319391634981
0.08975697032950648	0.532319391634981
0.08975697032950648	0.5343933632907016
0.08990606828686447	0.5343933632907016
0.08990606828686447	0.5350846871759419
0.09005516624422245	0.5350846871759419
0.09005516624422245	0.5368129968890425
0.09020426420158044	0.5368129968890425
0.09020426420158044	0.5399239543726235
0.09035336215893842	0.5399239543726235
0.09035336215893842	0.5406152782578638
0.09050246011629641	0.5406152782578638
0.09050246011629641	0.5423435879709644
0.09080065603101238	0.5423435879709644
0.09080065603101238	0.5426892499135845
0.09094975398837037	0.5426892499135845
0.09094975398837037	0.5440718976840649
0.09109885194572834	0.5440718976840649
0.09109885194572834	0.5482198409955064
0.09124794990308632	0.5482198409955064
0.09124794990308632	0.5489111648807466
0.09139704786044431	0.5489111648807466
0.09139704786044431	0.5509851365364673
0.09169524377516028	0.5509851365364673
0.09169524377516028	0.5520221223643277
0.09184434173251826	0.5520221223643277
0.09184434173251826	0.5523677843069478
0.09199343968987625	0.5523677843069478
0.09199343968987625	0.5530591081921881
0.0924407335619502	0.5530591081921881
0.0924407335619502	0.5537504320774282
0.09258983151930819	0.5537504320774282
0.09258983151930819	0.5554787417905289
0.09303712539138213	0.5554787417905289
0.09303712539138213	0.5568613895610093
0.09318622334874012	0.5568613895610093
0.09318622334874012	0.5572070515036295
0.0933353213060981	0.5572070515036295
0.0933353213060981	0.5578983753888697
0.09363351722081407	0.5578983753888697
0.09363351722081407	0.5603180089872105
0.09393171313553005	0.5603180089872105
0.09393171313553005	0.5610093328724507
0.09408081109288803	0.5610093328724507
0.09408081109288803	0.5655029381265123
0.09422990905024602	0.5655029381265123
0.09422990905024602	0.5661942620117525
0.094379007007604	0.5661942620117525
0.094379007007604	0.5665399239543726
0.09467720292231996	0.5665399239543726
0.09467720292231996	0.567922571724853
0.09482630087967794	0.567922571724853
0.09482630087967794	0.5699965433805738
0.09497539883703593	0.5699965433805738
0.09497539883703593	0.5703422053231939
0.09512449679439391	0.5703422053231939
0.09512449679439391	0.570687867265814
0.09542269270910989	0.570687867265814
0.09542269270910989	0.5713791911510543
0.09557179066646787	0.5713791911510543
0.09557179066646787	0.5720705150362945
0.09586998658118384	0.5720705150362945
0.09586998658118384	0.5727618389215348
0.09646637841061577	0.5727618389215348
0.09646637841061577	0.5731075008641549
0.09661547636797375	0.5731075008641549
0.09661547636797375	0.5741444866920152
0.09691367228268973	0.5741444866920152
0.09691367228268973	0.5755271344624957
0.09706277024004771	0.5755271344624957
0.09706277024004771	0.5762184583477359
0.09751006411212167	0.5762184583477359
0.09751006411212167	0.5765641202903561
0.09765916206947965	0.5765641202903561
0.09765916206947965	0.5769097822329762
0.09780826002683764	0.5769097822329762
0.09780826002683764	0.5772554441755963
0.09795735798419562	0.5772554441755963
0.09795735798419562	0.5776011061182164
0.09825555389891158	0.5776011061182164
0.09825555389891158	0.5789837538886968
0.09840465185626956	0.5789837538886968
0.09840465185626956	0.5820947113722779
0.09870284777098554	0.5820947113722779
0.09870284777098554	0.5824403733148981
0.09885194572834352	0.5824403733148981
0.09885194572834352	0.5827860352575182
0.0990010436857015	0.5827860352575182
0.0990010436857015	0.5834773591427583
0.09929923960041748	0.5834773591427583
0.09929923960041748	0.5841686830279986
0.09944833755777546	0.5841686830279986
0.09944833755777546	0.5845143449706187
0.0998956314298494	0.5845143449706187
0.0998956314298494	0.5848600069132388
0.10004472938720739	0.5848600069132388
0.10004472938720739	0.585205668855859
0.10019382734456538	0.585205668855859
0.10019382734456538	0.5855513307984791
0.10034292530192336	0.5855513307984791
0.10034292530192336	0.5862426546837193
0.10049202325928135	0.5862426546837193
0.10049202325928135	0.5872796405115797
0.10079021917399732	0.5872796405115797
0.10079021917399732	0.5876253024541997
0.1009393171313553	0.5876253024541997
0.1009393171313553	0.5886622882820601
0.10123751304607127	0.5886622882820601
0.10123751304607127	0.5928102315935015
0.10168480691814522	0.5928102315935015
0.10168480691814522	0.5931558935361216
0.1018339048755032	0.5931558935361216
0.1018339048755032	0.5952298651918424
0.10228119874757716	0.5952298651918424
0.10228119874757716	0.5959211890770826
0.10243029670493514	0.5959211890770826
0.10243029670493514	0.5962668510197028
0.10257939466229313	0.5962668510197028
0.10257939466229313	0.5966125129623229
0.10272849261965111	0.5966125129623229
0.10272849261965111	0.597303836847563
0.10302668853436708	0.597303836847563
0.10302668853436708	0.5979951607328033
0.10317578649172507	0.5979951607328033
0.10317578649172507	0.600069132388524
0.10332488444908305	0.600069132388524
0.10332488444908305	0.6007604562737643
0.10347398240644103	0.6007604562737643
0.10347398240644103	0.6014517801590045
0.10362308036379901	0.6014517801590045
0.10362308036379901	0.6021431040442448
0.10392127627851498	0.6021431040442448
0.10392127627851498	0.6028344279294849
0.10407037423587297	0.6028344279294849
0.10407037423587297	0.6042170756999654
0.10421947219323095	0.6042170756999654
0.10421947219323095	0.6045627376425855
0.10436857015058894	0.6045627376425855
0.10436857015058894	0.605945385413066
0.10451766810794692	0.605945385413066
0.10451766810794692	0.6066367092983063
0.1048158640226629	0.6066367092983063
0.1048158640226629	0.6076736951261666
0.10496496198002088	0.6076736951261666
0.10496496198002088	0.6083650190114068
0.10511405993737886	0.6083650190114068
0.10511405993737886	0.6087106809540269
0.10526315789473684	0.6087106809540269
0.10526315789473684	0.6090563428966471
0.10541225585209482	0.6090563428966471
0.10541225585209482	0.6097476667818873
0.10556135380945281	0.6097476667818873
0.10556135380945281	0.6114759764949879
0.10571045176681079	0.6114759764949879
0.10571045176681079	0.6118216384376081
0.10600864768152676	0.6118216384376081
0.10600864768152676	0.6135499481507086
0.10645594155360072	0.6135499481507086
0.10645594155360072	0.6138956100933287
0.1066050395109587	0.6138956100933287
0.1066050395109587	0.614586933978569
0.10690323542567466	0.614586933978569
0.10690323542567466	0.6156239198064293
0.10735052929774862	0.6156239198064293
0.10735052929774862	0.6163152436916696
0.1074996272551066	0.6163152436916696
0.1074996272551066	0.6180435534047701
0.10764872521246459	0.6180435534047701
0.10764872521246459	0.6187348772900104
0.10779782316982257	0.6187348772900104
0.10779782316982257	0.6190805392326305
0.10794692112718056	0.6190805392326305
0.10794692112718056	0.6194262011752506
0.10809601908453854	0.6194262011752506
0.10809601908453854	0.6197718631178707
0.1085433129566125	0.6197718631178707
0.1085433129566125	0.6201175250604909
0.10869241091397047	0.6201175250604909
0.10869241091397047	0.620463187003111
0.10884150887132846	0.620463187003111
0.10884150887132846	0.6215001728309714
0.10899060682868644	0.6215001728309714
0.10899060682868644	0.6218458347735915
0.10913970478604443	0.6218458347735915
0.10913970478604443	0.6232284825440719
0.1094379007007604	0.6232284825440719
0.1094379007007604	0.6256481161424127
0.11018339048755033	0.6256481161424127
0.11018339048755033	0.6291047355686139
0.11033248844490831	0.6291047355686139
0.11033248844490831	0.629450397511234
0.11048158640226628	0.629450397511234
0.11048158640226628	0.6301417213964743
0.11063068435962427	0.6301417213964743
0.11063068435962427	0.6304873833390944
0.11107797823169822	0.6304873833390944
0.11107797823169822	0.6308330452817145
0.11122707618905621	0.6308330452817145
0.11122707618905621	0.6318700311095748
0.1113761741464142	0.6318700311095748
0.1113761741464142	0.6322156930521949
0.11152527210377218	0.6322156930521949
0.11152527210377218	0.6329070169374352
0.11167437006113017	0.6329070169374352
0.11167437006113017	0.6339440027652955
0.11182346801848815	0.6339440027652955
0.11182346801848815	0.6342896647079157
0.11212166393320412	0.6342896647079157
0.11212166393320412	0.6346353266505358
0.11256895780527806	0.6346353266505358
0.11256895780527806	0.635326650535776
0.11286715371999403	0.635326650535776
0.11286715371999403	0.6360179744210163
0.11301625167735202	0.6360179744210163
0.11301625167735202	0.6391289319045973
0.11331444759206799	0.6391289319045973
0.11331444759206799	0.6394745938472174
0.11346354554942598	0.6394745938472174
0.11346354554942598	0.6415485655029382
0.11361264350678396	0.6415485655029382
0.11361264350678396	0.6446595229865192
0.11376174146414195	0.6446595229865192
0.11376174146414195	0.6456965088143796
0.11450723125093186	0.6456965088143796
0.11450723125093186	0.6460421707569997
0.11465632920828984	0.6460421707569997
0.11465632920828984	0.6463878326996197
0.1151036230803638	0.6463878326996197
0.1151036230803638	0.6467334946422398
0.11540181899507977	0.6467334946422398
0.11540181899507977	0.6484618043553405
0.11570001490979574	0.6484618043553405
0.11570001490979574	0.6488074662979606
0.11584911286715371	0.6488074662979606
0.11584911286715371	0.6491531282405807
0.11614730878186968	0.6491531282405807
0.11614730878186968	0.6515727618389215
0.11674370061130163	0.6515727618389215
0.11674370061130163	0.6522640857241617
0.11689279856865961	0.6522640857241617
0.11689279856865961	0.6526097476667819
0.1170418965260176	0.6526097476667819
0.1170418965260176	0.652955409609402
0.11719099448337558	0.652955409609402
0.11719099448337558	0.6536467334946422
0.11734009244073357	0.6536467334946422
0.11734009244073357	0.6553750432077429
0.11748919039809155	0.6553750432077429
0.11748919039809155	0.656066367092983
0.11763828835544952	0.656066367092983
0.11763828835544952	0.6567576909782233
0.11778738631280751	0.6567576909782233
0.11778738631280751	0.6577946768060836
0.11838377814223945	0.6577946768060836
0.11838377814223945	0.6581403387487038
0.11868197405695542	0.6581403387487038
0.11868197405695542	0.6591773245765641
0.11927836588638735	0.6591773245765641
0.11927836588638735	0.6598686484618044
0.11942746384374534	0.6598686484618044
0.11942746384374534	0.6612512962322848
0.11957656180110332	0.6612512962322848
0.11957656180110332	0.6615969581749049
0.1197256597584613	0.6615969581749049
0.1197256597584613	0.661942620117525
0.11987475771581929	0.661942620117525
0.11987475771581929	0.6626339440027653
0.12002385567317728	0.6626339440027653
0.12002385567317728	0.6629796059453854
0.12017295363053526	0.6629796059453854
0.12017295363053526	0.6633252678880055
0.12032205158789325	0.6633252678880055
0.12032205158789325	0.6636709298306257
0.12047114954525123	0.6636709298306257
0.12047114954525123	0.6643622537158659
0.12106754137468316	0.6643622537158659
0.12106754137468316	0.664707915658486
0.12121663933204115	0.664707915658486
0.12121663933204115	0.6653992395437263
0.12136573728939913	0.6653992395437263
0.12136573728939913	0.6657449014863464
0.1216639332041151	0.6657449014863464
0.1216639332041151	0.6667818873142067
0.12240942299090503	0.6667818873142067
0.12240942299090503	0.6671275492568268
0.12255852094826301	0.6671275492568268
0.12255852094826301	0.6674732111994469
0.12285671686297897	0.6674732111994469
0.12285671686297897	0.6688558589699274
0.12300581482033696	0.6688558589699274
0.12300581482033696	0.6698928447977878
0.12315491277769494	0.6698928447977878
0.12315491277769494	0.6702385067404079
0.1236022066497689	0.6702385067404079
0.1236022066497689	0.670584168683028
0.12375130460712688	0.670584168683028
0.12375130460712688	0.6709298306256481
0.12390040256448487	0.6709298306256481
0.12390040256448487	0.6736951261666091
0.12404950052184285	0.6736951261666091
0.12404950052184285	0.6740407881092292
0.12419859847920084	0.6740407881092292
0.12419859847920084	0.6757690978223297
0.12449679439391681	0.6757690978223297
0.12449679439391681	0.6768060836501901
0.12464589235127478	0.6768060836501901
0.12464589235127478	0.6778430694780505
0.12479499030863277	0.6778430694780505
0.12479499030863277	0.6781887314206706
0.12494408826599075	0.6781887314206706
0.12494408826599075	0.6785343933632907
0.12539138213806472	0.6785343933632907
0.12539138213806472	0.6788800553059108
0.12554048009542268	0.6788800553059108
0.12554048009542268	0.6795713791911511
0.12568957805278066	0.6795713791911511
0.12568957805278066	0.6809540269616315
0.12583867601013865	0.6809540269616315
0.12583867601013865	0.6812996889042516
0.12598777396749664	0.6812996889042516
0.12598777396749664	0.6816453508468717
0.1262859698822126	0.6816453508468717
0.1262859698822126	0.6826823366747321
0.1264350678395706	0.6826823366747321
0.1264350678395706	0.6830279986173522
0.12673326375428656	0.6830279986173522
0.12673326375428656	0.6847563083304529
0.12688236171164455	0.6847563083304529
0.12688236171164455	0.6861389561009333
0.12718055762636052	0.6861389561009333
0.12718055762636052	0.6864846180435534
0.1273296555837185	0.6864846180435534
0.1273296555837185	0.6875216038714138
0.1274787535410765	0.6875216038714138
0.1274787535410765	0.688212927756654
0.12762785149843447	0.688212927756654
0.12762785149843447	0.6885585896992741
0.12777694945579246	0.6885585896992741
0.12777694945579246	0.6892499135845144
0.12792604741315045	0.6892499135845144
0.12792604741315045	0.6906325613549948
0.12807514537050843	0.6906325613549948
0.12807514537050843	0.6920152091254753
0.1285224392425824	0.6920152091254753
0.1285224392425824	0.6933978568959558
0.12882063515729836	0.6933978568959558
0.12882063515729836	0.6944348427238161
0.12896973311465634	0.6944348427238161
0.12896973311465634	0.6965088143795368
0.1291188310720143	0.6965088143795368
0.1291188310720143	0.697200138264777
0.12941702698673027	0.697200138264777
0.12941702698673027	0.6975458002073972
0.12971522290144624	0.6975458002073972
0.12971522290144624	0.6978914621500173
0.12986432085880423	0.6978914621500173
0.12986432085880423	0.6996197718631179
0.1300134188161622	0.6996197718631179
0.1300134188161622	0.7010024196335983
0.1301625167735202	0.7010024196335983
0.1301625167735202	0.7016937435188386
0.13031161473087818	0.7016937435188386
0.13031161473087818	0.7020394054614587
0.13046071268823617	0.7020394054614587
0.13046071268823617	0.7041133771171794
0.13075890860295214	0.7041133771171794
0.13075890860295214	0.7051503629450397
0.13090800656031013	0.7051503629450397
0.13090800656031013	0.7054960248876598
0.13135530043238408	0.7054960248876598
0.13135530043238408	0.70584168683028
0.13165349634710005	0.70584168683028
0.13165349634710005	0.7065330107155202
0.13180259430445804	0.7065330107155202
0.13180259430445804	0.7068786726581403
0.132100790219174	0.7068786726581403
0.132100790219174	0.7072243346007605
0.13269718204860592	0.7072243346007605
0.13269718204860592	0.7079156584860007
0.1328462800059639	0.7079156584860007
0.1328462800059639	0.7082613204286208
0.13314447592067988	0.7082613204286208
0.13314447592067988	0.7092983062564812
0.13374086775011182	0.7092983062564812
0.13374086775011182	0.7103352920843415
0.1338899657074698	0.7103352920843415
0.1338899657074698	0.7110266159695817
0.1340390636648278	0.7110266159695817
0.1340390636648278	0.7113722779122018
0.13463545549425973	0.7113722779122018
0.13463545549425973	0.711717939854822
0.13478455345161772	0.711717939854822
0.13478455345161772	0.7120636017974421
0.1350827493663337	0.7120636017974421
0.1350827493663337	0.7124092637400622
0.13523184732369167	0.7124092637400622
0.13523184732369167	0.7127549256826823
0.13538094528104966	0.7127549256826823
0.13538094528104966	0.7134462495679226
0.13553004323840764	0.7134462495679226
0.13553004323840764	0.7141375734531628
0.13567914119576563	0.7141375734531628
0.13567914119576563	0.714828897338403
0.1359773371104816	0.714828897338403
0.1359773371104816	0.7158658831662634
0.13612643506783956	0.7158658831662634
0.13612643506783956	0.7162115451088835
0.13642463098255553	0.7162115451088835
0.13642463098255553	0.7169028689941237
0.1365737289399135	0.7169028689941237
0.1365737289399135	0.7172485309367439
0.13687192485462948	0.7172485309367439
0.13687192485462948	0.7193225025924646
0.13746831668406143	0.7193225025924646
0.13746831668406143	0.7196681645350846
0.1376174146414194	0.7196681645350846
0.1376174146414194	0.7203594884203249
0.1377665125987774	0.7203594884203249
0.1377665125987774	0.720705150362945
0.13791561055613538	0.720705150362945
0.13791561055613538	0.7213964742481853
0.13821380647085135	0.7213964742481853
0.13821380647085135	0.7220877981334255
0.13836290442820934	0.7220877981334255
0.13836290442820934	0.7231247839612859
0.1386611003429253	0.7231247839612859
0.1386611003429253	0.723470445903906
0.1388101983002833	0.723470445903906
0.1388101983002833	0.7238161078465261
0.13925749217235725	0.7238161078465261
0.13925749217235725	0.7245074317317663
0.13940659012971524	0.7245074317317663
0.13940659012971524	0.7248530936743864
0.13955568808707322	0.7248530936743864
0.13955568808707322	0.7258900795022468
0.13970478604443118	0.7258900795022468
0.13970478604443118	0.726581403387487
0.13985388400178916	0.726581403387487
0.13985388400178916	0.7272727272727273
0.14030117787386312	0.7272727272727273
0.14030117787386312	0.7279640511579675
0.1404502758312211	0.7279640511579675
0.1404502758312211	0.7283097131005877
0.1405993737885791	0.7283097131005877
0.1405993737885791	0.7290010369858279
0.14074847174593708	0.7290010369858279
0.14074847174593708	0.7296923608710681
0.14089756970329506	0.7296923608710681
0.14089756970329506	0.7300380228136882
0.14119576561801103	0.7300380228136882
0.14119576561801103	0.7317663325267888
0.14134486357536902	0.7317663325267888
0.14134486357536902	0.7324576564120291
0.141493961532727	0.7324576564120291
0.141493961532727	0.7328033183546492
0.141643059490085	0.7328033183546492
0.141643059490085	0.7341859661251297
0.14179215744744297	0.7341859661251297
0.14179215744744297	0.7352229519529899
0.14223945131951693	0.7352229519529899
0.14223945131951693	0.7359142758382302
0.1425376472342329	0.7359142758382302
0.1425376472342329	0.7362599377808503
0.14268674519159089	0.7362599377808503
0.14268674519159089	0.7369512616660906
0.14283584314894887	0.7369512616660906
0.14283584314894887	0.7372969236087107
0.14298494110630686	0.7372969236087107
0.14298494110630686	0.7383339094365711
0.14313403906366481	0.7383339094365711
0.14313403906366481	0.7386795713791912
0.14358133293573877	0.7386795713791912
0.14358133293573877	0.7390252333218112
0.14387952885045474	0.7390252333218112
0.14387952885045474	0.7393708952644313
0.14402862680781273	0.7393708952644313
0.14402862680781273	0.7400622191496716
0.1443268227225287	0.7400622191496716
0.1443268227225287	0.741099204977532
0.14492321455196064	0.741099204977532
0.14492321455196064	0.7417905288627722
0.1452214104666766	0.7417905288627722
0.1452214104666766	0.7421361908053923
0.1453705084240346	0.7421361908053923
0.1453705084240346	0.7431731766332527
0.14551960638139258	0.7431731766332527
0.14551960638139258	0.743864500518493
0.14581780229610855	0.743864500518493
0.14581780229610855	0.744210162461113
0.14611599821082452	0.744210162461113
0.14611599821082452	0.7445558244037331
0.1464141941255405	0.7445558244037331
0.1464141941255405	0.7452471482889734
0.14656329208289848	0.7452471482889734
0.14656329208289848	0.7466297960594539
0.1470105859549724	0.7466297960594539
0.1470105859549724	0.7473211199446941
0.14745787982704636	0.7473211199446941
0.14745787982704636	0.7476667818873142
0.14760697778440435	0.7476667818873142
0.14760697778440435	0.7483581057725545
0.14775607574176233	0.7483581057725545
0.14775607574176233	0.7504320774282751
0.1480542716564783	0.7504320774282751
0.1480542716564783	0.7507777393708953
0.14865066348591024	0.7507777393708953
0.14865066348591024	0.7511234013135154
0.14879976144326823	0.7511234013135154
0.14879976144326823	0.7518147251987556
0.1490979573579842	0.7518147251987556
0.1490979573579842	0.752851711026616
0.14939615327270017	0.752851711026616
0.14939615327270017	0.7531973729692361
0.14954525123005816	0.7531973729692361
0.14954525123005816	0.7535430349118563
0.1501416430594901	0.7535430349118563
0.1501416430594901	0.7545800207397165
0.15088713284628	0.7545800207397165
0.15088713284628	0.7549256826823367
0.15103623080363798	0.7549256826823367
0.15103623080363798	0.755962668510197
0.15118532876099597	0.755962668510197
0.15118532876099597	0.7563083304528171
0.15148352467571194	0.7563083304528171
0.15148352467571194	0.7566539923954373
0.15163262263306992	0.7566539923954373
0.15163262263306992	0.7569996543380574
0.1517817205904279	0.7569996543380574
0.1517817205904279	0.7576909782232976
0.1519308185477859	0.7576909782232976
0.1519308185477859	0.7580366401659178
0.15207991650514388	0.7580366401659178
0.15207991650514388	0.759073625993778
0.15252721037721784	0.759073625993778
0.15252721037721784	0.7594192879363982
0.15267630833457582	0.7594192879363982
0.15267630833457582	0.7601106118216384
0.15342179812136575	0.7601106118216384
0.15342179812136575	0.7608019357068787
0.15357089607872373	0.7608019357068787
0.15357089607872373	0.761838921534739
0.1537199940360817	0.761838921534739
0.1537199940360817	0.7628759073625994
0.15401818995079766	0.7628759073625994
0.15401818995079766	0.7635672312478397
0.15416728790815565	0.7635672312478397
0.15416728790815565	0.7639128931904597
0.1546145817802296	0.7639128931904597
0.1546145817802296	0.7642585551330798
0.15491277769494557	0.7642585551330798
0.15491277769494557	0.7646042170756999
0.15536007156701953	0.7646042170756999
0.15536007156701953	0.7649498790183201
0.1558073654390935	0.7649498790183201
0.1558073654390935	0.7652955409609402
0.15595646339645147	0.7652955409609402
0.15595646339645147	0.7659868648461804
0.15625465931116744	0.7659868648461804
0.15625465931116744	0.7663325267888006
0.15640375726852543	0.7663325267888006
0.15640375726852543	0.7666781887314207
0.15700014909795737	0.7666781887314207
0.15700014909795737	0.7673695126166609
0.1572983450126733	0.7673695126166609
0.1572983450126733	0.7677151745592811
0.15774563888474727	0.7677151745592811
0.15774563888474727	0.7680608365019012
0.15804383479946324	0.7680608365019012
0.15804383479946324	0.7684064984445212
0.15819293275682123	0.7684064984445212
0.15819293275682123	0.7687521603871413
0.1583420307141792	0.7687521603871413
0.1583420307141792	0.7690978223297615
0.15878932458625317	0.7690978223297615
0.15878932458625317	0.770480470100242
0.15893842254361115	0.770480470100242
0.15893842254361115	0.7715174559281023
0.15908752050096914	0.7715174559281023
0.15908752050096914	0.7722087798133426
0.15923661845832712	0.7722087798133426
0.15923661845832712	0.7729001036985828
0.15968391233040108	0.7729001036985828
0.15968391233040108	0.773245765641203
0.15998210824511705	0.773245765641203
0.15998210824511705	0.773591427583823
0.16013120620247503	0.773591427583823
0.16013120620247503	0.7739370895264431
0.16028030415983302	0.7739370895264431
0.16028030415983302	0.7742827514690632
0.16087669598926493	0.7742827514690632
0.16087669598926493	0.7746284134116834
0.16102579394662292	0.7746284134116834
0.16102579394662292	0.7749740753543035
0.16251677352020277	0.7749740753543035
0.16251677352020277	0.7756653992395437
0.16266587147756076	0.7756653992395437
0.16266587147756076	0.776356723124784
0.16341136126435069	0.776356723124784
0.16341136126435069	0.7767023850674041
0.16370955717906666	0.7767023850674041
0.16370955717906666	0.7770480470100242
0.16385865513642464	0.7770480470100242
0.16385865513642464	0.7777393708952645
0.16460414492321454	0.7777393708952645
0.16460414492321454	0.7791220186657449
0.16475324288057253	0.7791220186657449
0.16475324288057253	0.7798133425509851
0.1649023408379305	0.7798133425509851
0.1649023408379305	0.7801590044936052
0.1650514387952885	0.7801590044936052
0.1650514387952885	0.7805046664362254
0.16534963471000447	0.7805046664362254
0.16534963471000447	0.7808503283788455
0.16549873266736245	0.7808503283788455
0.16549873266736245	0.7811959903214656
0.16624422245415238	0.7811959903214656
0.16624422245415238	0.7829243000345661
0.16684061428358432	0.7829243000345661
0.16684061428358432	0.7832699619771863
0.1669897122409423	0.7832699619771863
0.1669897122409423	0.7836156239198064
0.16773520202773223	0.7836156239198064
0.16773520202773223	0.7839612858624265
0.1678842999850902	0.7839612858624265
0.1678842999850902	0.7843069478050466
0.16803339794244818	0.7843069478050466
0.16803339794244818	0.7849982716902869
0.16818249589980616	0.7849982716902869
0.16818249589980616	0.7856895955755271
0.16833159385716415	0.7856895955755271
0.16833159385716415	0.7863809194607674
0.16862978977188012	0.7863809194607674
0.16862978977188012	0.7867265814033875
0.1689279856865961	0.7867265814033875
0.1689279856865961	0.7874179052886278
0.16997167138810199	0.7874179052886278
0.16997167138810199	0.7877635672312479
0.17012076934545997	0.7877635672312479
0.17012076934545997	0.7881092291738679
0.17026986730281796	0.7881092291738679
0.17026986730281796	0.788454891116488
0.17041896526017594	0.788454891116488
0.17041896526017594	0.7894918769443484
0.17116445504696587	0.7894918769443484
0.17116445504696587	0.7905288627722088
0.1714626509616818	0.7905288627722088
0.1714626509616818	0.7908745247148289
0.1716117489190398	0.7908745247148289
0.1716117489190398	0.791220186657449
0.17176084687639778	0.791220186657449
0.17176084687639778	0.7915658486000692
0.17235723870582972	0.7915658486000692
0.17235723870582972	0.7919115105426893
0.17280453257790368	0.7919115105426893
0.17280453257790368	0.7922571724853094
0.17384821827940958	0.7922571724853094
0.17384821827940958	0.7926028344279294
0.17414641419412555	0.7926028344279294
0.17414641419412555	0.7932941583131697
0.17429551215148353	0.7932941583131697
0.17429551215148353	0.7936398202557898
0.17489190398091548	0.7936398202557898
0.17489190398091548	0.7939854821984099
0.17504100193827343	0.7939854821984099
0.17504100193827343	0.7953681299688904
0.17563739376770537	0.7953681299688904
0.17563739376770537	0.7960594538541307
0.17593558968242134	0.7960594538541307
0.17593558968242134	0.7964051157967508
0.17623378559713732	0.7964051157967508
0.17623378559713732	0.7967507777393709
0.17668107946921127	0.7967507777393709
0.17668107946921127	0.7977877635672312
0.1772774712986432	0.7977877635672312
0.1772774712986432	0.7981334255098513
0.1774265692560012	0.7981334255098513
0.1774265692560012	0.7988247493950916
0.17802296108543314	0.7988247493950916
0.17802296108543314	0.7991704113377117
0.17876845087222304	0.7991704113377117
0.17876845087222304	0.8002073971655721
0.17996123453108692	0.8002073971655721
0.17996123453108692	0.8005530591081922
0.18055762636051886	0.8005530591081922
0.18055762636051886	0.8015900449360526
0.18070672431787685	0.8015900449360526
0.18070672431787685	0.8019357068786727
0.1811540181899508	0.8019357068786727
0.1811540181899508	0.8022813688212928
0.18175041001938275	0.8022813688212928
0.18175041001938275	0.8026270307639128
0.18324138959296257	0.8026270307639128
0.18324138959296257	0.802972692706533
0.18353958550767854	0.802972692706533
0.18353958550767854	0.8033183546491531
0.18383778142239451	0.8033183546491531
0.18383778142239451	0.8036640165917732
0.1848814671239004	0.8036640165917732
0.1848814671239004	0.8040096785343933
0.18517966303861638	0.8040096785343933
0.18517966303861638	0.8043553404770135
0.1856269569106903	0.8043553404770135
0.1856269569106903	0.8047010024196336
0.1866706426121962	0.8047010024196336
0.1866706426121962	0.8050466643622537
0.18741613239898613	0.8050466643622537
0.18741613239898613	0.8053923263048738
0.18905620992992395	0.8053923263048738
0.18905620992992395	0.805737988247494
0.1896526017593559	0.805737988247494
0.1896526017593559	0.8060836501901141
0.19039809154614581	0.8060836501901141
0.19039809154614581	0.8067749740753543
0.1905471895035038	0.8067749740753543
0.1905471895035038	0.8078119599032146
0.1914417772476517	0.8078119599032146
0.1914417772476517	0.8081576218458347
0.19188907111972567	0.8081576218458347
0.19188907111972567	0.8095402696163152
0.19203816907708365	0.8095402696163152
0.19203816907708365	0.8098859315589354
0.1932309527359475	0.8098859315589354
0.1932309527359475	0.8102315935015555
0.1944237363948114	0.8102315935015555
0.1944237363948114	0.8109229173867957
0.19457283435216938	0.8109229173867957
0.19457283435216938	0.8112685793294159
0.19472193230952736	0.8112685793294159
0.19472193230952736	0.811614241272036
0.19502012822424333	0.811614241272036
0.19502012822424333	0.811959903214656
0.19695840166989712	0.811959903214656
0.19695840166989712	0.8123055651572761
0.1971074996272551	0.8123055651572761
0.1971074996272551	0.8126512270998963
0.19755479349932906	0.8126512270998963
0.19755479349932906	0.8133425509851365
0.19785298941404503	0.8133425509851365
0.19785298941404503	0.8136882129277566
0.198002087371403	0.8136882129277566
0.198002087371403	0.814725198755617
0.19844938124347697	0.814725198755617
0.19844938124347697	0.8154165226408573
0.19889667511555092	0.8154165226408573
0.19889667511555092	0.8157621845834774
0.1991948710302669	0.8157621845834774
0.1991948710302669	0.8161078465260975
0.19949306694498287	0.8161078465260975
0.19949306694498287	0.8167991704113378
0.20023855673177277	0.8167991704113378
0.20023855673177277	0.8171448323539579
0.20053675264648874	0.8171448323539579
0.20053675264648874	0.8174904942965779
0.2009840465185627	0.8174904942965779
0.2009840465185627	0.8181818181818182
0.20172953630535262	0.8181818181818182
0.20172953630535262	0.8188731420670584
0.2020277322200686	0.8188731420670584
0.2020277322200686	0.8195644659522987
0.20217683017742658	0.8195644659522987
0.20217683017742658	0.8202557898375389
0.20262412404950053	0.8202557898375389
0.20262412404950053	0.820601451780159
0.2029223199642165	0.820601451780159
0.2029223199642165	0.8209471137227792
0.2047114954525123	0.8209471137227792
0.2047114954525123	0.8212927756653993
0.20500969136722827	0.8212927756653993
0.20500969136722827	0.8219840995506394
0.20545698523930223	0.8219840995506394
0.20545698523930223	0.8223297614932595
0.20679886685552407	0.8223297614932595
0.20679886685552407	0.8226754234358797
0.207395258684956	0.8226754234358797
0.207395258684956	0.8230210853784998
0.20814074847174593	0.8230210853784998
0.20814074847174593	0.8233667473211199
0.2084389443864619	0.8233667473211199
0.2084389443864619	0.82371240926374
0.2085880423438199	0.82371240926374
0.2085880423438199	0.8240580712063602
0.20873714030117788	0.8240580712063602
0.20873714030117788	0.8244037331489803
0.20933353213060982	0.8244037331489803
0.20933353213060982	0.8257863809194608
0.21022811987475773	0.8257863809194608
0.21022811987475773	0.8268233667473212
0.21157000149097957	0.8268233667473212
0.21157000149097957	0.8271690286899412
0.2121663933204115	0.8271690286899412
0.2121663933204115	0.8278603525751814
0.21246458923512748	0.8278603525751814
0.21246458923512748	0.8282060145178016
0.21291188310720144	0.8282060145178016
0.21291188310720144	0.8285516764604217
0.21350827493663338	0.8285516764604217
0.21350827493663338	0.8288973384030418
0.2141046667660653	0.8288973384030418
0.2141046667660653	0.8295886622882821
0.21425376472342328	0.8295886622882821
0.21425376472342328	0.8299343242309022
0.21455196063813925	0.8299343242309022
0.21455196063813925	0.8302799861735223
0.21485015655285522	0.8302799861735223
0.21485015655285522	0.8306256481161424
0.2149992545102132	0.8306256481161424
0.2149992545102132	0.8309713100587626
0.21559564633964515	0.8309713100587626
0.21559564633964515	0.8313169720013827
0.21574474429700313	0.8313169720013827
0.21574474429700313	0.8316626339440027
0.217086625913225	0.8316626339440027
0.217086625913225	0.8320082958866228
0.21738482182794094	0.8320082958866228
0.21738482182794094	0.832353957829243
0.21798121365737289	0.832353957829243
0.21798121365737289	0.8326996197718631
0.21813031161473087	0.8326996197718631
0.21813031161473087	0.8333909436571033
0.21827940957208886	0.8333909436571033
0.21827940957208886	0.8337366055997235
0.21842850752944684	0.8337366055997235
0.21842850752944684	0.8354649153128241
0.2187267034441628	0.8354649153128241
0.2187267034441628	0.8365019011406845
0.2188758014015208	0.8365019011406845
0.2188758014015208	0.838230210853785
0.21917399731623677	0.838230210853785
0.21917399731623677	0.8385758727964051
0.2199194871030267	0.8385758727964051
0.2199194871030267	0.8392671966816454
0.22006858506038468	0.8392671966816454
0.22006858506038468	0.8399585205668856
0.22021768301774267	0.8399585205668856
0.22021768301774267	0.8406498444521259
0.22036678097510065	0.8406498444521259
0.22036678097510065	0.8416868302799861
0.22051587893245864	0.8416868302799861
0.22051587893245864	0.8420324922226063
0.22066497688981662	0.8420324922226063
0.22066497688981662	0.8427238161078465
0.22111227076189055	0.8427238161078465
0.22111227076189055	0.8434151399930868
0.22126136871924854	0.8434151399930868
0.22126136871924854	0.8447977877635672
0.22141046667660652	0.8447977877635672
0.22141046667660652	0.8461804355340476
0.2217086625913225	0.8461804355340476
0.2217086625913225	0.8482544071897684
0.22245415237811242	0.8482544071897684
0.22245415237811242	0.8489457310750086
0.2226032503354704	0.8489457310750086
0.2226032503354704	0.8496370549602489
0.22305054420754436	0.8496370549602489
0.22305054420754436	0.849982716902869
0.22334874012226033	0.849982716902869
0.22334874012226033	0.8503283788454891
0.22349783807961832	0.8503283788454891
0.22349783807961832	0.8513653646733494
0.2236469360369763	0.8513653646733494
0.2236469360369763	0.8517110266159695
0.22409422990905026	0.8517110266159695
0.22409422990905026	0.8524023505012098
0.22454152378112419	0.8524023505012098
0.22454152378112419	0.8541306602143104
0.22469062173848217	0.8541306602143104
0.22469062173848217	0.8548219840995507
0.22483971969584016	0.8548219840995507
0.22483971969584016	0.8555133079847909
0.22513791561055613	0.8555133079847909
0.22513791561055613	0.855858969927411
0.2254361115252721	0.855858969927411
0.2254361115252721	0.8562046318700312
0.22558520948263008	0.8562046318700312
0.22558520948263008	0.8572416176978914
0.22618160131206203	0.8572416176978914
0.22618160131206203	0.8575872796405116
0.22633069926942	0.8575872796405116
0.22633069926942	0.8589699274109921
0.226479797226778	0.8589699274109921
0.226479797226778	0.8593155893536122
0.22677799314149397	0.8593155893536122
0.22677799314149397	0.8596612512962323
0.22692709109885195	0.8596612512962323
0.22692709109885195	0.8600069132388524
0.22707618905620994	0.8600069132388524
0.22707618905620994	0.8603525751814726
0.22722528701356792	0.8603525751814726
0.22722528701356792	0.8606982371240927
0.2273743849709259	0.8606982371240927
0.2273743849709259	0.8613895610093328
0.22782167884299986	0.8613895610093328
0.22782167884299986	0.861735222951953
0.22797077680035782	0.861735222951953
0.22797077680035782	0.8620808848945731
0.2281198747577158	0.8620808848945731
0.2281198747577158	0.8624265468371932
0.22871626658714775	0.8624265468371932
0.22871626658714775	0.8627722087798133
0.22886536454450573	0.8627722087798133
0.22886536454450573	0.8631178707224335
0.22901446250186372	0.8631178707224335
0.22901446250186372	0.8634635326650536
0.22946175637393768	0.8634635326650536
0.22946175637393768	0.8638091946076737
0.22961085433129566	0.8638091946076737
0.22961085433129566	0.8641548565502938
0.2303563441180856	0.8641548565502938
0.2303563441180856	0.8648461804355341
0.23065454003280156	0.8648461804355341
0.23065454003280156	0.8651918423781542
0.23080363799015954	0.8651918423781542
0.23080363799015954	0.8658831662633945
0.23110183390487551	0.8658831662633945
0.23110183390487551	0.8683027998617352
0.23154912777694944	0.8683027998617352
0.23154912777694944	0.8689941237469755
0.23214551960638138	0.8689941237469755
0.23214551960638138	0.8700311095748358
0.23244371552109735	0.8700311095748358
0.23244371552109735	0.870722433460076
0.23259281347845534	0.870722433460076
0.23259281347845534	0.8714137573453162
0.2328910093931713	0.8714137573453162
0.2328910093931713	0.8717594192879364
0.2330401073505293	0.8717594192879364
0.2330401073505293	0.8721050812305565
0.23318920530788728	0.8721050812305565
0.23318920530788728	0.8731420670584169
0.23363649917996124	0.8731420670584169
0.23363649917996124	0.8752160387141376
0.2340837930520352	0.8752160387141376
0.2340837930520352	0.8755617006567576
0.23453108692410915	0.8755617006567576
0.23453108692410915	0.8762530245419979
0.23482928283882512	0.8762530245419979
0.23482928283882512	0.8772900103698583
0.2349783807961831	0.8772900103698583
0.2349783807961831	0.8779813342550985
0.23512747875354106	0.8779813342550985
0.23512747875354106	0.8783269961977186
0.23527657671089905	0.8783269961977186
0.23527657671089905	0.879363982025579
0.23557477262561502	0.879363982025579
0.23557477262561502	0.8804009678534394
0.235872968540331	0.8804009678534394
0.235872968540331	0.8807466297960594
0.23632026241240495	0.8807466297960594
0.23632026241240495	0.8814379536812997
0.23661845832712092	0.8814379536812997
0.23661845832712092	0.8821292775665399
0.2369166542418369	0.8821292775665399
0.2369166542418369	0.88247493950916
0.23721485015655286	0.88247493950916
0.23721485015655286	0.8831662633944003
0.23736394811391084	0.8831662633944003
0.23736394811391084	0.8842032492222607
0.23751304607126883	0.8842032492222607
0.23751304607126883	0.885240235050121
0.2385567317727747	0.885240235050121
0.2385567317727747	0.8862772208779813
0.23885492768749067	0.8862772208779813
0.23885492768749067	0.8866228828206014
0.23915312360220664	0.8866228828206014
0.23915312360220664	0.8873142067058417
0.23930222155956463	0.8873142067058417
0.23930222155956463	0.8883511925337021
0.2396004174742806	0.8883511925337021
0.2396004174742806	0.8890425164189423
0.23989861338899657	0.8890425164189423
0.23989861338899657	0.8904251641894227
0.24004771134635455	0.8904251641894227
0.24004771134635455	0.8907708261320428
0.24019680930371254	0.8907708261320428
0.24019680930371254	0.8914621500172831
0.2404950052184285	0.8914621500172831
0.2404950052184285	0.8918078119599032
0.24079320113314448	0.8918078119599032
0.24079320113314448	0.8921534739025233
0.24124049500521844	0.8921534739025233
0.24124049500521844	0.8942274455582441
0.24138959296257642	0.8942274455582441
0.24138959296257642	0.8945731075008642
0.2415386909199344	0.8945731075008642
0.2415386909199344	0.8949187694434843
0.24183688683465038	0.8949187694434843
0.24183688683465038	0.8952644313861043
0.2424332786640823	0.8952644313861043
0.2424332786640823	0.8956100933287245
0.24258237662144028	0.8956100933287245
0.24258237662144028	0.8959557552713446
0.24288057253615625	0.8959557552713446
0.24288057253615625	0.8963014172139647
0.24317876845087222	0.8963014172139647
0.24317876845087222	0.8966470791565848
0.2433278664082302	0.8966470791565848
0.2433278664082302	0.896992741099205
0.2434769643655882	0.896992741099205
0.2434769643655882	0.8973384030418251
0.24481884598181006	0.8973384030418251
0.24481884598181006	0.8976840649844452
0.24496794393916804	0.8976840649844452
0.24496794393916804	0.8980297269270653
0.245415237811242	0.8980297269270653
0.245415237811242	0.8983753888696855
0.24630982555538988	0.8983753888696855
0.24630982555538988	0.8987210508123056
0.24675711942746384	0.8987210508123056
0.24675711942746384	0.8990667127549257
0.24750260921425377	0.8990667127549257
0.24750260921425377	0.8994123746975458
0.24884449083047563	0.8994123746975458
0.24884449083047563	0.900103698582786
0.24944088265990755	0.900103698582786
0.24944088265990755	0.9007950224680262
0.2498881765319815	0.9007950224680262
0.2498881765319815	0.9011406844106464
0.2500372744893395	0.9011406844106464
0.2500372744893395	0.9018320082958866
0.25033547040405546	0.9018320082958866
0.25033547040405546	0.9021776702385067
0.2509318622334874	0.9021776702385067
0.2509318622334874	0.9025233321811269
0.2512300581482034	0.9025233321811269
0.2512300581482034	0.9032146560663671
0.2525719397644252	0.9032146560663671
0.2525719397644252	0.9039059799516074
0.2528701356791412	0.9039059799516074
0.2528701356791412	0.9045973038368476
0.2530192336364992	0.9045973038368476
0.2530192336364992	0.9049429657794676
0.25316833159385715	0.9049429657794676
0.25316833159385715	0.9052886277220878
0.25406291933800507	0.9052886277220878
0.25406291933800507	0.905979951607328
0.254659311167437	0.905979951607328
0.254659311167437	0.9066712754925683
0.254957507082153	0.9066712754925683
0.254957507082153	0.9073625993778085
0.25510660503951094	0.9073625993778085
0.25510660503951094	0.9077082613204286
0.25525570299686895	0.9077082613204286
0.25525570299686895	0.9083995852056689
0.2555538989115849	0.9083995852056689
0.2555538989115849	0.9090909090909091
0.2558520948263009	0.9090909090909091
0.2558520948263009	0.9097822329761494
0.25615029074101686	0.9097822329761494
0.25615029074101686	0.9101278949187694
0.2567466825704488	0.9101278949187694
0.2567466825704488	0.9104735568613895
0.25719397644252273	0.9104735568613895
0.25719397644252273	0.9108192188040097
0.25734307439988074	0.9108192188040097
0.25734307439988074	0.9111648807466298
0.25853585805874457	0.9111648807466298
0.25853585805874457	0.9115105426892499
0.2595795437602505	0.9115105426892499
0.2595795437602505	0.91185620463187
0.26017593558968244	0.91185620463187
0.26017593558968244	0.9122018665744901
0.2603250335470404	0.9122018665744901
0.2603250335470404	0.9125475285171103
0.2612196212911883	0.9125475285171103
0.2612196212911883	0.9128931904597304
0.2613687192485463	0.9128931904597304
0.2613687192485463	0.9132388524023505
0.2615178172059043	0.9132388524023505
0.2615178172059043	0.9135845143449706
0.2619651110779782	0.9135845143449706
0.2619651110779782	0.9139301762875908
0.2621142090353362	0.9139301762875908
0.2621142090353362	0.9142758382302109
0.2622633069926942	0.9142758382302109
0.2622633069926942	0.914621500172831
0.2624124049500522	0.914621500172831
0.2624124049500522	0.914967162115451
0.26256150290741015	0.914967162115451
0.26256150290741015	0.9153128240580712
0.26271060086476816	0.9153128240580712
0.26271060086476816	0.9156584860006913
0.26300879677948413	0.9156584860006913
0.26300879677948413	0.9163498098859315
0.2633069926942001	0.9163498098859315
0.2633069926942001	0.9166954718285517
0.2636051886089161	0.9166954718285517
0.2636051886089161	0.9170411337711718
0.26390338452363205	0.9170411337711718
0.26390338452363205	0.917732457656412
0.264201580438348	0.917732457656412
0.264201580438348	0.9184237815416523
0.26479797226777996	0.9184237815416523
0.26479797226777996	0.9191151054268925
0.2650961681824959	0.9191151054268925
0.2650961681824959	0.9194607673695127
0.2652452661398539	0.9194607673695127
0.2652452661398539	0.9198064293121327
0.26628895184135976	0.9198064293121327
0.26628895184135976	0.9201520912547528
0.2665871477560757	0.9201520912547528
0.2665871477560757	0.9204977531973729
0.26673624571343374	0.9204977531973729
0.26673624571343374	0.9208434151399931
0.2668853436707917	0.9208434151399931
0.2668853436707917	0.9211890770826132
0.26718353958550767	0.9211890770826132
0.26718353958550767	0.9215347390252333
0.26763083345758165	0.9215347390252333
0.26763083345758165	0.9218804009678534
0.26837632324437155	0.9218804009678534
0.26837632324437155	0.9222260629104736
0.2688236171164455	0.9222260629104736
0.2688236171164455	0.9229173867957138
0.2689727150738035	0.9229173867957138
0.2689727150738035	0.9232630487383339
0.27001640077530936	0.9232630487383339
0.27001640077530936	0.9236087106809541
0.2706127926047413	0.9236087106809541
0.2706127926047413	0.9239543726235742
0.27165647830624723	0.9239543726235742
0.27165647830624723	0.9249913584514345
0.2718055762636052	0.9249913584514345
0.2718055762636052	0.9260283442792948
0.27240196809303713	0.9260283442792948
0.27240196809303713	0.926374006221915
0.27299835992246907	0.926374006221915
0.27299835992246907	0.9267196681645351
0.273147457879827	0.9267196681645351
0.273147457879827	0.9270653301071552
0.2744893394960489	0.9270653301071552
0.2744893394960489	0.9274109920497753
0.2746384374534069	0.9274109920497753
0.2746384374534069	0.9277566539923955
0.2764276129417027	0.9277566539923955
0.2764276129417027	0.9281023159350156
0.2776203966005666	0.9281023159350156
0.2776203966005666	0.9284479778776357
0.27791859251528256	0.9284479778776357
0.27791859251528256	0.929484963705496
0.2800059639182943	0.929484963705496
0.2800059639182943	0.9298306256481161
0.2809005516624422	0.9298306256481161
0.2809005516624422	0.9301762875907362
0.2811987475771582	0.9301762875907362
0.2811987475771582	0.9305219495333564
0.2813478455345162	0.9305219495333564
0.2813478455345162	0.9308676114759765
0.28149694349187415	0.9308676114759765
0.28149694349187415	0.9312132734185966
0.28194423736394814	0.9312132734185966
0.28194423736394814	0.9315589353612167
0.2837334128522439	0.9315589353612167
0.2837334128522439	0.9319045973038369
0.2838825108096019	0.9319045973038369
0.2838825108096019	0.932250259246457
0.2840316087669599	0.932250259246457
0.2840316087669599	0.9325959211890771
0.2841807067243179	0.9325959211890771
0.2841807067243179	0.9329415831316972
0.28567168629789774	0.9329415831316972
0.28567168629789774	0.9332872450743174
0.2858207842552557	0.9332872450743174
0.2858207842552557	0.9336329070169375
0.28731176382883555	0.9336329070169375
0.28731176382883555	0.9343242309021776
0.2886536454450574	0.9343242309021776
0.2886536454450574	0.9346698928447977
0.28895184135977336	0.9346698928447977
0.28895184135977336	0.935361216730038
0.28925003727448934	0.935361216730038
0.28925003727448934	0.9357068786726581
0.2895482331892053	0.9357068786726581
0.2895482331892053	0.9360525406152782
0.2907410168480692	0.9360525406152782
0.2907410168480692	0.9363982025578984
0.292828388251081	0.9363982025578984
0.292828388251081	0.9367438645005185
0.2932756821231549	0.9367438645005185
0.2932756821231549	0.9370895264431386
0.2973013269718205	0.9370895264431386
0.2973013269718205	0.9374351883857587
0.2989414045027583	0.9374351883857587
0.2989414045027583	0.9377808503283789
0.2990905024601163	0.9377808503283789
0.2990905024601163	0.938126512270999
0.29923960041747427	0.938126512270999
0.29923960041747427	0.9384721742136191
0.3001341881616222	0.9384721742136191
0.3001341881616222	0.9388178361562391
0.30132697182048607	0.9388178361562391
0.30132697182048607	0.9395091600414794
0.3028179513940659	0.9395091600414794
0.3028179513940659	0.9402004839267196
0.30401073505292975	0.9402004839267196
0.30401073505292975	0.9405461458693398
0.3057999105412256	0.9405461458693398
0.3057999105412256	0.9408918078119599
0.31072014313403906	0.9408918078119599
0.31072014313403906	0.94123746975458
0.3120620247502609	0.94123746975458
0.3120620247502609	0.9415831316972001
0.31400029819591474	0.9415831316972001
0.31400029819591474	0.9419287936398203
0.3159385716415685	0.9419287936398203
0.3159385716415685	0.9422744555824404
0.3162367675562845	0.9422744555824404
0.3162367675562845	0.9426201175250605
0.3178768450872223	0.9426201175250605
0.3178768450872223	0.9429657794676806
0.3189205307887282	0.9429657794676806
0.3189205307887282	0.9433114414103008
0.32413895929625763	0.9433114414103008
0.32413895929625763	0.9436571033529209
0.3256299388698375	0.9436571033529209
0.3256299388698375	0.944348427238161
0.3260772327419114	0.944348427238161
0.3260772327419114	0.9446940891807812
0.32622633069926943	0.9446940891807812
0.32622633069926943	0.9450397511234013
0.3289100939317131	0.9450397511234013
0.3289100939317131	0.9453854130660214
0.3293573878037871	0.9453854130660214
0.3293573878037871	0.9457310750086415
0.32950648576114505	0.9457310750086415
0.32950648576114505	0.9460767369512617
0.3309974653347249	0.9460767369512617
0.3309974653347249	0.9464223988938818
0.3312956612494409	0.9464223988938818
0.3312956612494409	0.9467680608365019
0.3366631877143283	0.9467680608365019
0.3366631877143283	0.947113722779122
0.34188161622185775	0.947113722779122
0.34188161622185775	0.9474593847217422
0.3462054569852393	0.9474593847217422
0.3462054569852393	0.9478050466643623
0.349485612047115	0.9478050466643623
0.349485612047115	0.9481507086069824
0.3520202773222007	0.9481507086069824
0.3520202773222007	0.9484963705496025
0.35261666915163264	0.9484963705496025
0.35261666915163264	0.9488420324922227
0.35336215893842254	0.9488420324922227
0.35336215893842254	0.9491876944348427
0.3560459221708663	0.9491876944348427
0.3560459221708663	0.9498790183200829
0.3566423140002982	0.9498790183200829
0.3566423140002982	0.9502246802627031
0.3572387058297301	0.9502246802627031
0.3572387058297301	0.9505703422053232
0.36156254659311166	0.9505703422053232
0.36156254659311166	0.9509160041479433
0.3709557179066647	0.9509160041479433
0.3709557179066647	0.9512616660905634
0.3790070076039958	0.9512616660905634
0.3790070076039958	0.9516073280331836
0.3803488892202177	0.9516073280331836
0.3803488892202177	0.9519529899758037
0.38139257492172357	0.9519529899758037
0.38139257492172357	0.9522986519184238
0.3828835544953034	0.9522986519184238
0.3828835544953034	0.9526443138610439
0.3848218279409572	0.9526443138610439
0.3848218279409572	0.9529899758036641
0.38705829730132696	0.9529899758036641
0.38705829730132696	0.9533356377462842
0.38795288504547487	0.9533356377462842
0.38795288504547487	0.9536812996889042
0.38989115849112865	0.9536812996889042
0.3901893544058446	0.9536812996889042
0.395855076785448	0.9536812996889042
0.395855076785448	0.9540269616315243
0.396302370657522	0.9540269616315243
0.396302370657522	0.9543726235741445
0.4083793052035187	0.9543726235741445
0.4083793052035187	0.9547182855167646
0.41076487252124644	0.9547182855167646
0.41076487252124644	0.9554096094020048
0.4124049500521843	0.9554096094020048
0.4124049500521843	0.9557552713446249
0.41553600715670197	0.9557552713446249
0.41553600715670197	0.9561009332872451
0.41941255404800953	0.9561009332872451
0.41941255404800953	0.9564465952298652
0.42895482331892054	0.9564465952298652
0.42895482331892054	0.9567922571724853
0.43834799463247354	0.9567922571724853
0.43834799463247354	0.9571379191151054
0.44013717012076936	0.9571379191151054
0.44013717012076936	0.9574835810577256
0.4423736394811391	0.9574835810577256
0.4423736394811391	0.9578292430003457
0.4444610108841509	0.9578292430003457
0.4444610108841509	0.9581749049429658
0.452512300581482	0.9581749049429658
0.452512300581482	0.9585205668855858
0.4545996719844938	0.9585205668855858
0.4545996719844938	0.958866228828206
0.4593708066199493	0.958866228828206
0.4593708066199493	0.9592118907708261
0.4595199045773073	0.9592118907708261
0.4595199045773073	0.9595575527134462
0.46339645146861486	0.9595575527134462
0.46339645146861486	0.9599032146560663
0.47487699418517965	0.9599032146560663
0.47487699418517965	0.9602488765986865
0.47741165946026537	0.9602488765986865
0.47741165946026537	0.9605945385413066
0.47770985537498134	0.9605945385413066
0.47770985537498134	0.9609402004839267
0.49589980617265544	0.9609402004839267
0.49589980617265544	0.961631524369167
0.5014164305949008	0.961631524369167
0.5014164305949008	0.9619771863117871
0.5124496794393917	0.9619771863117871
0.5124496794393917	0.9623228482544072
0.5264648874310422	0.9623228482544072
0.5264648874310422	0.9626685101970273
0.528999552706128	0.9626685101970273
0.528999552706128	0.9630141721396475
0.5430147606977784	0.9630141721396475
0.5430147606977784	0.9633598340822676
0.5454003280155062	0.9633598340822676
0.5454003280155062	0.9637054960248876
0.5533025197554794	0.9637054960248876
0.5533025197554794	0.9640511579675077
0.5547934993290592	0.9640511579675077
0.5547934993290592	0.9643968199101279
0.5640375726852542	0.9643968199101279
0.5640375726852542	0.964742481852748
0.575667213359177	0.964742481852748
0.575667213359177	0.9650881437953681
0.5883405397346056	0.9650881437953681
0.5883405397346056	0.9654338057379882
0.5884896376919636	0.9654338057379882
0.5884896376919636	0.9657794676806084
0.594155360071567	0.9657794676806084
0.594155360071567	0.9661251296232285
0.5963918294319368	0.9661251296232285
0.5963918294319368	0.9664707915658486
0.6166691516326226	0.9664707915658486
0.6166691516326226	0.9668164535084687
0.622633069926942	0.9668164535084687
0.622633069926942	0.9671621154510889
0.6427612941702698	0.9671621154510889
0.6427612941702698	0.967507777393709
0.6570746980766363	0.967507777393709
0.6570746980766363	0.9678534393363291
0.659609363351722	0.9678534393363291
0.659609363351722	0.9681991012789491
0.6597584613090801	0.9681991012789491
0.6597584613090801	0.9685447632215693
0.660653049053228	0.9685447632215693
0.660653049053228	0.9688904251641894
0.6870433875055911	0.9688904251641894
0.6870433875055911	0.9692360871068095
0.7128373341285225	0.9692360871068095
0.7128373341285225	0.9695817490494296
0.7268525421201729	0.9695817490494296
0.7268525421201729	0.9699274109920498
0.7383330848367378	0.9699274109920498
0.7383330848367378	0.9702730729346699
0.7386312807514537	0.9702730729346699
0.7386312807514537	0.97061873487729
0.7444461010884151	0.97061873487729
0.7444461010884151	0.9709643968199101
0.7483226479797227	0.9709643968199101
0.7483226479797227	0.9713100587625303
0.7486208438944386	0.9713100587625303
0.7486208438944386	0.9716557207051504
0.7538392724019681	0.9716557207051504
0.7538392724019681	0.9720013826477705
0.7659162069479648	0.9720013826477705
0.7659162069479648	0.9723470445903906
0.7677053824362606	0.9723470445903906
0.7677053824362606	0.9726927065330108
0.7693454599671985	0.9726927065330108
0.7693454599671985	0.9730383684756309
0.7794841210675414	0.9730383684756309
0.7794841210675414	0.973384030418251
0.7820187863426271	0.973384030418251
0.7820187863426271	0.973729692360871
0.7869390189354406	0.973729692360871
0.7869390189354406	0.9740753543034912
0.7918592515282541	0.9740753543034912
0.7918592515282541	0.9744210162461113
0.8040852840316087	0.9744210162461113
0.8040852840316087	0.9747666781887314
0.8064708513493365	0.9747666781887314
0.8064708513493365	0.9751123401313515
0.8136275533025198	0.9751123401313515
0.8136275533025198	0.9754580020739717
0.8260026837632325	0.9754580020739717
0.8260026837632325	0.9758036640165918
0.8310720143134039	0.9758036640165918
0.8310720143134039	0.9761493259592119
0.8312211122707619	0.9761493259592119
0.8312211122707619	0.976494987901832
0.8552258834053973	0.976494987901832
0.896973311465633	0.9799516073280332
0.896973311465633	0.9802972692706533
0.9086029521395557	0.9802972692706533
0.9086029521395557	0.9806429312132734
0.933651408975697	0.9806429312132734
0.933651408975697	0.9809885931558935
0.9354405844639928	0.9809885931558935
0.9354405844639928	0.9813342550985137
0.9391680333979424	0.9813342550985137
0.9391680333979424	0.9816799170411338
0.9442373639481139	0.9816799170411338
0.9442373639481139	0.982371240926374
0.9592962576412704	0.982371240926374
0.9592962576412704	0.9827169028689942
0.9618309229163561	0.9827169028689942
0.9618309229163561	0.9830625648116142
0.9691367228268972	0.9830625648116142
0.9691367228268972	0.9834082267542343
0.9745042492917847	0.9834082267542343
0.9745042492917847	0.9837538886968544
0.9758461309080065	0.9837538886968544
0.9758461309080065	0.9840995506394746
0.9789771880125242	0.9840995506394746
0.9789771880125242	0.9844452125820947
0.9800208737140301	0.9844452125820947
0.9800208737140301	0.9847908745247148
0.9843447144774117	0.9847908745247148
0.9843447144774117	0.9851365364673349
0.9867302817951394	0.9851365364673349
0.9867302817951394	0.9854821984099551
0.9879230654540033	0.9854821984099551
0.9879230654540033	0.9861735222951953
0.991203220515879	0.9861735222951953
0.991203220515879	0.9865191842378154
0.9919487103026688	0.9865191842378154
0.9919487103026688	0.9868648461804356
0.9922469062173849	0.9868648461804356
0.9922469062173849	0.9872105081230557
0.9923960041747428	0.9872105081230557
0.9923960041747428	0.9875561700656758
0.9928432980468168	0.9875561700656758
0.9928432980468168	0.988247493950916
0.9935887878336067	0.988247493950916
0.9935887878336067	0.9889388178361562
0.9937378857909647	0.9889388178361562
0.9937378857909647	0.9892844797787763
0.9940360817056806	0.9892844797787763
0.9940360817056806	0.9896301417213965
0.9949306694498286	0.9896301417213965
0.9949306694498286	0.991012789491877
0.9955270612792605	0.991012789491877
0.9955270612792605	0.9913584514344971
0.9962725510660504	0.9913584514344971
0.9962725510660504	0.9927410992049776
0.9967198449381244	0.9927410992049776
0.9967198449381244	0.9934324230902177
0.9970180408528403	0.9934324230902177
0.9970180408528403	0.9937780850328379
0.9971671388101983	0.9937780850328379
0.9971671388101983	0.9944694089180781
0.9973162367675563	0.9944694089180781
0.9973162367675563	0.9948150708606982
0.9974653347249143	0.9948150708606982
0.9974653347249143	0.9951607328033184
0.9979126285969883	0.9951607328033184
0.9979126285969883	0.9955063947459385
0.9982108245117042	0.9955063947459385
0.9982108245117042	0.9961977186311787
0.9983599224690621	0.9961977186311787
0.9983599224690621	0.9975803664016591
0.9985090204264202	0.9975803664016591
0.9985090204264202	0.9989630141721396
0.9986581183837782	0.9989630141721396
0.9986581183837782	0.9993086761147598
0.9992545102132101	0.9993086761147598
0.9992545102132101	0.9996543380573799
0.9997018040852841	0.9996543380573799
0.9997018040852841	1.0
1.0	1.0

==> data/roc_c.tex <==
A B
0.0	0.0
0.00024509803921568627	0.0
0.00024509803921568627	0.00018115942028985507
0.0004901960784313725	0.00018115942028985507
0.0004901960784313725	0.00036231884057971015
0.000980392156862745	0.00036231884057971015
0.000980392156862745	0.0012681159420289854
0.0012254901960784314	0.0012681159420289854
0.0012254901960784314	0.0014492753623188406
0.00196078431372549	0.0014492753623188406
0.00196078431372549	0.002173913043478261
0.0022058823529411764	0.002173913043478261
0.0022058823529411764	0.002355072463768116
0.0024509803921568627	0.002355072463768116
0.0024509803921568627	0.002717391304347826
0.0029411764705882353	0.002717391304347826
0.0029411764705882353	0.004166666666666667
0.0031862745098039215	0.004166666666666667
0.0031862745098039215	0.005072463768115942
0.003676470588235294	0.005072463768115942
0.003676470588235294	0.005253623188405797
0.00392156862745098	0.005253623188405797
0.00392156862745098	0.006159420289855073
0.004166666666666667	0.006159420289855073
0.004166666666666667	0.007065217391304348
0.004411764705882353	0.007065217391304348
0.004411764705882353	0.007246376811594203
0.004656862745098039	0.007246376811594203
0.004656862745098039	0.007608695652173913
0.004901960784313725	0.007608695652173913
0.004901960784313725	0.007971014492753623
0.005147058823529412	0.007971014492753623
0.005147058823529412	0.008152173913043478
0.005392156862745098	0.008152173913043478
0.005392156862745098	0.009057971014492754
0.005637254901960784	0.009057971014492754
0.005637254901960784	0.00923913043478261
0.0058823529411764705	0.00923913043478261
0.0058823529411764705	0.009782608695652175
0.006127450980392157	0.009782608695652175
0.006127450980392157	0.010507246376811594
0.006372549019607843	0.010507246376811594
0.006372549019607843	0.010688405797101449
0.006617647058823529	0.010688405797101449
0.006617647058823529	0.010869565217391304
0.006862745098039216	0.010869565217391304
0.006862745098039216	0.011231884057971014
0.007352941176470588	0.011231884057971014
0.007352941176470588	0.011956521739130435
0.007598039215686274	0.011956521739130435
0.007598039215686274	0.013405797101449275
0.00784313725490196	0.013405797101449275
0.00784313725490196	0.01394927536231884
0.008088235294117648	0.01394927536231884
0.008088235294117648	0.014673913043478261
0.008333333333333333	0.014673913043478261
0.008333333333333333	0.016304347826086956
0.00857843137254902	0.016304347826086956
0.00857843137254902	0.017028985507246377
0.008823529411764706	0.017028985507246377
0.008823529411764706	0.017572463768115942
0.009068627450980393	0.017572463768115942
0.009068627450980393	0.017753623188405798
0.009313725490196078	0.017753623188405798
0.009313725490196078	0.01884057971014493
0.009558823529411765	0.01884057971014493
0.009558823529411765	0.01956521739130435
0.00980392156862745	0.01956521739130435
0.00980392156862745	0.020289855072463767
0.010049019607843138	0.020289855072463767
0.010049019607843138	0.021557971014492753
0.010294117647058823	0.021557971014492753
0.010294117647058823	0.022282608695652174
0.01053921568627451	0.022282608695652174
0.01053921568627451	0.02282608695652174
0.010784313725490196	0.02282608695652174
0.010784313725490196	0.02318840579710145
0.011029411764705883	0.02318840579710145
0.011029411764705883	0.024094202898550725
0.011519607843137256	0.024094202898550725
0.011519607843137256	0.025362318840579712
0.011764705882352941	0.025362318840579712
0.011764705882352941	0.02644927536231884
0.012009803921568628	0.02644927536231884
0.012009803921568628	0.02753623188405797
0.012254901960784314	0.02753623188405797
0.012254901960784314	0.027717391304347826
0.0125	0.027717391304347826
0.0125	0.02789855072463768
0.012745098039215686	0.02789855072463768
0.012745098039215686	0.028442028985507246
0.012990196078431373	0.028442028985507246
0.012990196078431373	0.030253623188405798
0.013235294117647059	0.030253623188405798
0.013235294117647059	0.03061594202898551
0.013480392156862746	0.03061594202898551
0.013480392156862746	0.03206521739130435
0.013725490196078431	0.03206521739130435
0.013725490196078431	0.03260869565217391
0.013970588235294118	0.03260869565217391
0.013970588235294118	0.03369565217391304
0.014215686274509804	0.03369565217391304
0.014215686274509804	0.034057971014492754
0.01446078431372549	0.034057971014492754
0.01446078431372549	0.03731884057971015
0.014705882352941176	0.03731884057971015
0.014705882352941176	0.03768115942028986
0.014950980392156863	0.03768115942028986
0.014950980392156863	0.03840579710144928
0.015196078431372549	0.03840579710144928
0.015196078431372549	0.03894927536231884
0.015441176470588236	0.03894927536231884
0.015441176470588236	0.04057971014492753
0.015931372549019607	0.04057971014492753
0.015931372549019607	0.041666666666666664
0.016176470588235296	0.041666666666666664
0.016176470588235296	0.042753623188405795
0.016666666666666666	0.042753623188405795
0.016666666666666666	0.04384057971014493
0.01764705882352941	0.04384057971014493
0.01764705882352941	0.04456521739130435
0.017892156862745097	0.04456521739130435
0.017892156862745097	0.04547101449275362
0.018137254901960786	0.04547101449275362
0.018137254901960786	0.04655797101449275
0.01838235294117647	0.04655797101449275
0.01838235294117647	0.04673913043478261
0.018627450980392157	0.04673913043478261
0.018627450980392157	0.04746376811594203
0.018872549019607842	0.04746376811594203
0.018872549019607842	0.04891304347826087
0.019362745098039216	0.04891304347826087
0.019362745098039216	0.05
0.0196078431372549	0.05
0.0196078431372549	0.05235507246376812
0.019852941176470587	0.05235507246376812
0.019852941176470587	0.05271739130434783
0.019852941176470587	0.05307971014492754
0.019852941176470587	0.05398550724637681
0.02034313725490196	0.05398550724637681
0.02034313725490196	0.05416666666666667
0.020588235294117647	0.05416666666666667
0.020588235294117647	0.0552536231884058
0.020833333333333332	0.0552536231884058
0.020833333333333332	0.05561594202898551
0.02107843137254902	0.05561594202898551
0.02107843137254902	0.05615942028985507
0.021323529411764706	0.05615942028985507
0.021323529411764706	0.05688405797101449
0.021568627450980392	0.05688405797101449
0.021568627450980392	0.057789855072463765
0.021813725490196077	0.057789855072463765
0.021813725490196077	0.06141304347826087
0.022058823529411766	0.06141304347826087
0.022058823529411766	0.06159420289855073
0.02230392156862745	0.06159420289855073
0.02230392156862745	0.0628623188405797
0.022549019607843137	0.0628623188405797
0.022549019607843137	0.06304347826086956
0.022794117647058822	0.06304347826086956
0.022794117647058822	0.06358695652173912
0.02303921568627451	0.06358695652173912
0.02303921568627451	0.06594202898550725
0.023284313725490197	0.06594202898550725
0.023284313725490197	0.0661231884057971
0.023529411764705882	0.0661231884057971
0.023529411764705882	0.06702898550724638
0.023774509803921567	0.06702898550724638
0.023774509803921567	0.06938405797101449
0.024019607843137256	0.06938405797101449
0.024019607843137256	0.06956521739130435
0.02426470588235294	0.06956521739130435
0.02426470588235294	0.06974637681159421
0.024754901960784313	0.06974637681159421
0.024754901960784313	0.07101449275362319
0.025	0.07101449275362319
0.025	0.07318840579710145
0.025245098039215687	0.07318840579710145
0.025245098039215687	0.07355072463768116
0.025490196078431372	0.07355072463768116
0.025490196078431372	0.07427536231884058
0.025735294117647058	0.07427536231884058
0.025735294117647058	0.07518115942028986
0.025980392156862746	0.07518115942028986
0.025980392156862746	0.07608695652173914
0.026225490196078432	0.07608695652173914
0.026225490196078432	0.0769927536231884
0.026470588235294117	0.0769927536231884
0.026470588235294117	0.07753623188405798
0.026715686274509803	0.07753623188405798
0.026715686274509803	0.07771739130434782
0.02696078431372549	0.07771739130434782
0.02696078431372549	0.08097826086956522
0.027205882352941177	0.08097826086956522
0.027205882352941177	0.0822463768115942
0.027450980392156862	0.0822463768115942
0.027450980392156862	0.08297101449275363
0.027941176470588237	0.08297101449275363
0.027941176470588237	0.08369565217391305
0.028186274509803922	0.08369565217391305
0.028186274509803922	0.08496376811594203
0.028431372549019607	0.08496376811594203
0.028431372549019607	0.08605072463768115
0.029166666666666667	0.08605072463768115
0.029166666666666667	0.08623188405797101
0.029411764705882353	0.08623188405797101
0.029411764705882353	0.08641304347826087
0.029656862745098038	0.08641304347826087
0.029656862745098038	0.08659420289855073
0.029901960784313727	0.08659420289855073
0.029901960784313727	0.0875
0.030147058823529412	0.0875
0.030147058823529412	0.08768115942028985
0.030392156862745098	0.08768115942028985
0.030392156862745098	0.08858695652173913
0.030637254901960783	0.08858695652173913
0.030637254901960783	0.09021739130434783
0.031127450980392157	0.09021739130434783
0.031127450980392157	0.09039855072463768
0.03137254901960784	0.09039855072463768
0.03137254901960784	0.09148550724637682
0.03161764705882353	0.09148550724637682
0.03161764705882353	0.09257246376811594
0.0321078431372549	0.09257246376811594
0.0321078431372549	0.09347826086956522
0.03235294117647059	0.09347826086956522
0.03235294117647059	0.09384057971014492
0.03259803921568628	0.09384057971014492
0.03259803921568628	0.09456521739130434
0.03284313725490196	0.09456521739130434
0.03284313725490196	0.09547101449275362
0.03308823529411765	0.09547101449275362
0.03308823529411765	0.09565217391304348
0.03333333333333333	0.09565217391304348
0.03333333333333333	0.09619565217391304
0.03357843137254902	0.09619565217391304
0.03357843137254902	0.09728260869565217
0.033823529411764704	0.09728260869565217
0.033823529411764704	0.09782608695652174
0.03431372549019608	0.09782608695652174
0.03431372549019608	0.10072463768115943
0.03480392156862745	0.10072463768115943
0.03480392156862745	0.10144927536231885
0.03504901960784314	0.10144927536231885
0.03504901960784314	0.10163043478260869
0.03529411764705882	0.10163043478260869
0.03529411764705882	0.10217391304347827
0.03553921568627451	0.10217391304347827
0.03553921568627451	0.10253623188405797
0.035784313725490194	0.10253623188405797
0.035784313725490194	0.10289855072463767
0.03602941176470588	0.10289855072463767
0.03602941176470588	0.1036231884057971
0.03651960784313726	0.1036231884057971
0.03651960784313726	0.10471014492753623
0.03676470588235294	0.10471014492753623
0.03676470588235294	0.10507246376811594
0.03700980392156863	0.10507246376811594
0.03700980392156863	0.10579710144927536
0.03725490196078431	0.10579710144927536
0.03725490196078431	0.10634057971014493
0.0375	0.10634057971014493
0.0375	0.10742753623188406
0.03799019607843137	0.10742753623188406
0.03799019607843137	0.10797101449275362
0.03823529411764706	0.10797101449275362
0.03823529411764706	0.1108695652173913
0.03848039215686275	0.1108695652173913
0.03848039215686275	0.11105072463768116
0.03872549019607843	0.11105072463768116
0.03872549019607843	0.11141304347826086
0.0392156862745098	0.11141304347826086
0.0392156862745098	0.1128623188405797
0.03946078431372549	0.1128623188405797
0.03946078431372549	0.11376811594202899
0.03995098039215686	0.11376811594202899
0.03995098039215686	0.11413043478260869
0.04019607843137255	0.11413043478260869
0.04019607843137255	0.11503623188405797
0.04044117647058824	0.11503623188405797
0.04044117647058824	0.11702898550724637
0.041176470588235294	0.11702898550724637
0.041176470588235294	0.11721014492753623
0.04142156862745098	0.11721014492753623
0.04142156862745098	0.11811594202898551
0.041666666666666664	0.11811594202898551
0.041666666666666664	0.11902173913043479
0.04191176470588235	0.11902173913043479
0.04191176470588235	0.11992753623188405
0.04215686274509804	0.11992753623188405
0.04215686274509804	0.12028985507246377
0.04240196078431373	0.12028985507246377
0.04240196078431373	0.12101449275362319
0.04264705882352941	0.12101449275362319
0.04264705882352941	0.12119565217391304
0.043137254901960784	0.12119565217391304
0.043137254901960784	0.1230072463768116
0.04338235294117647	0.1230072463768116
0.04338235294117647	0.12391304347826088
0.043627450980392155	0.12391304347826088
0.043627450980392155	0.12427536231884058
0.04411764705882353	0.12427536231884058
0.04411764705882353	0.1246376811594203
0.0446078431372549	0.1246376811594203
0.0446078431372549	0.12481884057971014
0.04485294117647059	0.12481884057971014
0.04485294117647059	0.1269927536231884
0.045098039215686274	0.1269927536231884
0.045098039215686274	0.12753623188405797
0.04534313725490196	0.12753623188405797
0.04534313725490196	0.12789855072463768
0.04583333333333333	0.12789855072463768
0.04583333333333333	0.1282608695652174
0.04632352941176471	0.1282608695652174
0.04632352941176471	0.12880434782608696
0.04656862745098039	0.12880434782608696
0.04656862745098039	0.13206521739130433
0.04681372549019608	0.13206521739130433
0.04681372549019608	0.13260869565217392
0.047058823529411764	0.13260869565217392
0.047058823529411764	0.13333333333333333
0.04730392156862745	0.13333333333333333
0.04730392156862745	0.13351449275362318
0.047549019607843135	0.13351449275362318
0.047549019607843135	0.13405797101449277
0.04779411764705882	0.13405797101449277
0.04779411764705882	0.1342391304347826
0.049019607843137254	0.1342391304347826
0.049019607843137254	0.13641304347826086
0.04926470588235294	0.13641304347826086
0.04926470588235294	0.1371376811594203
0.049509803921568625	0.1371376811594203
0.049509803921568625	0.13731884057971014
0.04975490196078431	0.13731884057971014
0.04975490196078431	0.1378623188405797
0.05	0.1378623188405797
0.05	0.13894927536231885
0.05024509803921569	0.13894927536231885
0.05024509803921569	0.14003623188405798
0.050490196078431374	0.14003623188405798
0.050490196078431374	0.1403985507246377
0.05073529411764706	0.1403985507246377
0.05073529411764706	0.14094202898550726
0.050980392156862744	0.14094202898550726
0.050980392156862744	0.14166666666666666
0.05122549019607843	0.14166666666666666
0.05122549019607843	0.14184782608695654
0.051470588235294115	0.14184782608695654
0.051470588235294115	0.14293478260869566
0.0517156862745098	0.14293478260869566
0.0517156862745098	0.14347826086956522
0.05220588235294118	0.14347826086956522
0.05220588235294118	0.1451086956521739
0.05269607843137255	0.1451086956521739
0.05269607843137255	0.14528985507246378
0.052941176470588235	0.14528985507246378
0.052941176470588235	0.14655797101449275
0.05318627450980392	0.14655797101449275
0.05318627450980392	0.1471014492753623
0.05367647058823529	0.1471014492753623
0.05367647058823529	0.14728260869565218
0.05367647058823529	0.14764492753623187
0.05367647058823529	0.14855072463768115
0.05392156862745098	0.14855072463768115
0.05392156862745098	0.14963768115942028
0.05416666666666667	0.14963768115942028
0.05416666666666667	0.15181159420289855
0.054411764705882354	0.15181159420289855
0.054411764705882354	0.1519927536231884
0.05465686274509804	0.1519927536231884
0.05465686274509804	0.15253623188405796
0.054901960784313725	0.15253623188405796
0.054901960784313725	0.15344202898550724
0.05514705882352941	0.15344202898550724
0.05514705882352941	0.1536231884057971
0.055392156862745096	0.1536231884057971
0.055392156862745096	0.15380434782608696
0.05563725490196078	0.15380434782608696
0.05563725490196078	0.15706521739130436
0.05588235294117647	0.15706521739130436
0.05588235294117647	0.15760869565217392
0.056372549019607844	0.15760869565217392
0.056372549019607844	0.15778985507246376
0.05661764705882353	0.15778985507246376
0.05661764705882353	0.15797101449275364
0.0571078431372549	0.15797101449275364
0.0571078431372549	0.15869565217391304
0.057352941176470586	0.15869565217391304
0.057352941176470586	0.1588768115942029
0.05759803921568627	0.1588768115942029
0.05759803921568627	0.15942028985507245
0.05784313725490196	0.15942028985507245
0.05784313725490196	0.161231884057971
0.05808823529411765	0.161231884057971
0.05808823529411765	0.16159420289855073
0.058333333333333334	0.16159420289855073
0.058333333333333334	0.16231884057971013
0.05857843137254902	0.16231884057971013
0.05857843137254902	0.16304347826086957
0.058823529411764705	0.16304347826086957
0.058823529411764705	0.16394927536231885
0.05906862745098039	0.16394927536231885
0.05906862745098039	0.1644927536231884
0.059313725490196076	0.1644927536231884
0.059313725490196076	0.16576086956521738
0.059803921568627454	0.16576086956521738
0.059803921568627454	0.16630434782608697
0.06004901960784314	0.16630434782608697
0.06004901960784314	0.1664855072463768
0.060294117647058824	0.1664855072463768
0.060294117647058824	0.16666666666666666
0.06053921568627451	0.16666666666666666
0.06053921568627451	0.1673913043478261
0.060784313725490195	0.1673913043478261
0.060784313725490195	0.16793478260869565
0.06102941176470588	0.16793478260869565
0.06102941176470588	0.1681159420289855
0.061274509803921566	0.1681159420289855
0.061274509803921566	0.17101449275362318
0.06151960784313725	0.17101449275362318
0.06151960784313725	0.17173913043478262
0.061764705882352944	0.17173913043478262
0.061764705882352944	0.17300724637681159
0.06200980392156863	0.17300724637681159
0.06200980392156863	0.17518115942028986
0.062254901960784315	0.17518115942028986
0.062254901960784315	0.1753623188405797
0.0625	0.1753623188405797
0.0625	0.17626811594202899
0.06274509803921569	0.17626811594202899
0.06274509803921569	0.1766304347826087
0.06299019607843137	0.1766304347826087
0.06299019607843137	0.17753623188405798
0.06323529411764706	0.17753623188405798
0.06323529411764706	0.17971014492753623
0.06348039215686274	0.17971014492753623
0.06348039215686274	0.1802536231884058
0.06372549019607843	0.1802536231884058
0.06372549019607843	0.1815217391304348
0.06397058823529411	0.1815217391304348
0.06397058823529411	0.18188405797101448
0.0642156862745098	0.18188405797101448
0.0642156862745098	0.18278985507246376
0.0644607843137255	0.18278985507246376
0.0644607843137255	0.18333333333333332
0.06470588235294118	0.18333333333333332
0.06470588235294118	0.18514492753623188
0.06495098039215687	0.18514492753623188
0.06495098039215687	0.18731884057971016
0.06519607843137255	0.18731884057971016
0.06519607843137255	0.1875
0.06593137254901961	0.1875
0.06593137254901961	0.18804347826086956
0.06642156862745098	0.18804347826086956
0.06642156862745098	0.18840579710144928
0.06666666666666667	0.18840579710144928
0.06666666666666667	0.18858695652173912
0.06691176470588235	0.18858695652173912
0.06691176470588235	0.1891304347826087
0.06715686274509804	0.1891304347826087
0.06715686274509804	0.19003623188405797
0.06740196078431372	0.19003623188405797
0.06740196078431372	0.19021739130434784
0.06764705882352941	0.19021739130434784
0.06764705882352941	0.19202898550724637
0.06813725490196078	0.19202898550724637
0.06813725490196078	0.19311594202898552
0.06838235294117648	0.19311594202898552
0.06838235294117648	0.1947463768115942
0.06862745098039216	0.1947463768115942
0.06862745098039216	0.19510869565217392
0.06887254901960785	0.19510869565217392
0.06887254901960785	0.19583333333333333
0.06911764705882353	0.19583333333333333
0.06911764705882353	0.1963768115942029
0.06936274509803922	0.1963768115942029
0.06936274509803922	0.1967391304347826
0.0696078431372549	0.1967391304347826
0.0696078431372549	0.19692028985507246
0.06985294117647059	0.19692028985507246
0.06985294117647059	0.19710144927536233
0.07009803921568628	0.19710144927536233
0.07009803921568628	0.19728260869565217
0.07034313725490196	0.19728260869565217
0.07034313725490196	0.19782608695652174
0.07058823529411765	0.19782608695652174
0.07058823529411765	0.1980072463768116
0.07083333333333333	0.1980072463768116
0.07083333333333333	0.1983695652173913
0.07107843137254902	0.1983695652173913
0.07107843137254902	0.19855072463768117
0.0713235294117647	0.19855072463768117
0.0713235294117647	0.19945652173913042
0.07181372549019607	0.19945652173913042
0.07181372549019607	0.2
0.07205882352941176	0.2
0.07205882352941176	0.20072463768115942
0.07230392156862746	0.20072463768115942
0.07230392156862746	0.20090579710144926
0.0732843137254902	0.20090579710144926
0.0732843137254902	0.20126811594202898
0.07352941176470588	0.20126811594202898
0.07352941176470588	0.20144927536231885
0.07377450980392157	0.20144927536231885
0.07377450980392157	0.20181159420289854
0.07426470588235294	0.20181159420289854
0.07426470588235294	0.2023550724637681
0.07450980392156863	0.2023550724637681
0.07450980392156863	0.20253623188405798
0.07475490196078431	0.20253623188405798
0.07475490196078431	0.20344202898550726
0.07524509803921568	0.20344202898550726
0.07524509803921568	0.2048913043478261
0.07549019607843137	0.2048913043478261
0.07549019607843137	0.20543478260869566
0.07622549019607844	0.20543478260869566
0.07622549019607844	0.20615942028985507
0.07671568627450981	0.20615942028985507
0.07671568627450981	0.20797101449275363
0.0769607843137255	0.20797101449275363
0.0769607843137255	0.20815217391304347
0.07720588235294118	0.20815217391304347
0.07720588235294118	0.2085144927536232
0.07745098039215687	0.2085144927536232
0.07745098039215687	0.20905797101449275
0.07794117647058824	0.20905797101449275
0.07794117647058824	0.20923913043478262
0.0784313725490196	0.20923913043478262
0.0784313725490196	0.20978260869565218
0.07867647058823529	0.20978260869565218
0.07867647058823529	0.2105072463768116
0.07916666666666666	0.2105072463768116
0.07916666666666666	0.2108695652173913
0.07965686274509803	0.2108695652173913
0.07965686274509803	0.21213768115942028
0.07990196078431372	0.21213768115942028
0.07990196078431372	0.21304347826086956
0.0803921568627451	0.21304347826086956
0.0803921568627451	0.21322463768115943
0.08063725490196079	0.21322463768115943
0.08063725490196079	0.21394927536231884
0.08088235294117647	0.21394927536231884
0.08088235294117647	0.2141304347826087
0.08137254901960785	0.2141304347826087
0.08137254901960785	0.21431159420289855
0.08161764705882353	0.21431159420289855
0.08161764705882353	0.21485507246376812
0.08186274509803922	0.21485507246376812
0.08186274509803922	0.21503623188405796
0.08259803921568627	0.21503623188405796
0.08259803921568627	0.21539855072463768
0.08284313725490196	0.21539855072463768
0.08284313725490196	0.21684782608695652
0.08308823529411764	0.21684782608695652
0.08308823529411764	0.21739130434782608
0.08333333333333333	0.21739130434782608
0.08333333333333333	0.21757246376811595
0.08357843137254901	0.21757246376811595
0.08357843137254901	0.21829710144927536
0.0838235294117647	0.21829710144927536
0.0838235294117647	0.2184782608695652
0.0840686274509804	0.2184782608695652
0.0840686274509804	0.21920289855072464
0.08455882352941177	0.21920289855072464
0.08455882352941177	0.21956521739130436
0.08504901960784314	0.21956521739130436
0.08504901960784314	0.22192028985507245
0.08529411764705883	0.22192028985507245
0.08529411764705883	0.22246376811594204
0.08553921568627451	0.22246376811594204
0.08553921568627451	0.223731884057971
0.0857843137254902	0.223731884057971
0.0857843137254902	0.22409420289855073
0.08602941176470588	0.22409420289855073
0.08602941176470588	0.225
0.08627450980392157	0.225
0.08627450980392157	0.2269927536231884
0.08651960784313725	0.2269927536231884
0.08651960784313725	0.22735507246376813
0.08700980392156862	0.22735507246376813
0.08700980392156862	0.22771739130434782
0.08725490196078431	0.22771739130434782
0.08725490196078431	0.22844202898550725
0.0875	0.22844202898550725
0.0875	0.22880434782608697
0.08774509803921568	0.22880434782608697
0.08774509803921568	0.2289855072463768
0.08799019607843138	0.2289855072463768
0.08799019607843138	0.22934782608695653
0.08848039215686275	0.22934782608695653
0.08848039215686275	0.23007246376811594
0.08897058823529412	0.23007246376811594
0.08897058823529412	0.23043478260869565
0.0892156862745098	0.23043478260869565
0.0892156862745098	0.23097826086956522
0.08946078431372549	0.23097826086956522
0.08946078431372549	0.23333333333333334
0.08970588235294118	0.23333333333333334
0.08970588235294118	0.23442028985507246
0.08995098039215686	0.23442028985507246
0.08995098039215686	0.23605072463768115
0.09019607843137255	0.23605072463768115
0.09019607843137255	0.23623188405797102
0.09044117647058823	0.23623188405797102
0.09044117647058823	0.23641304347826086
0.09068627450980392	0.23641304347826086
0.09068627450980392	0.23695652173913043
0.0909313725490196	0.23695652173913043
0.0909313725490196	0.23840579710144927
0.09117647058823529	0.23840579710144927
0.09117647058823529	0.2394927536231884
0.09142156862745097	0.2394927536231884
0.09142156862745097	0.2398550724637681
0.09166666666666666	0.2398550724637681
0.09166666666666666	0.24021739130434783
0.09215686274509804	0.24021739130434783
0.09215686274509804	0.24039855072463767
0.09240196078431373	0.24039855072463767
0.09240196078431373	0.2407608695652174
0.09264705882352942	0.2407608695652174
0.09264705882352942	0.24130434782608695
0.0928921568627451	0.24130434782608695
0.0928921568627451	0.24202898550724639
0.09313725490196079	0.24202898550724639
0.09313725490196079	0.2427536231884058
0.09362745098039216	0.2427536231884058
0.09362745098039216	0.24492753623188407
0.09387254901960784	0.24492753623188407
0.09387254901960784	0.24547101449275363
0.09411764705882353	0.24547101449275363
0.09411764705882353	0.24583333333333332
0.09436274509803921	0.24583333333333332
0.09436274509803921	0.2463768115942029
0.0946078431372549	0.2463768115942029
0.0946078431372549	0.24728260869565216
0.09485294117647058	0.24728260869565216
0.09485294117647058	0.24782608695652175
0.09509803921568627	0.24782608695652175
0.09509803921568627	0.2480072463768116
0.09534313725490196	0.2480072463768116
0.09534313725490196	0.2483695652173913
0.09558823529411764	0.2483695652173913
0.09558823529411764	0.24945652173913044
0.09583333333333334	0.24945652173913044
0.09583333333333334	0.24981884057971016
0.0965686274509804	0.24981884057971016
0.0965686274509804	0.2503623188405797
0.09705882352941177	0.2503623188405797
0.09705882352941177	0.2519927536231884
0.09730392156862745	0.2519927536231884
0.09730392156862745	0.25217391304347825
0.09754901960784314	0.25217391304347825
0.09754901960784314	0.2528985507246377
0.09779411764705882	0.2528985507246377
0.09779411764705882	0.2534420289855073
0.09803921568627451	0.2534420289855073
0.09803921568627451	0.2539855072463768
0.0982843137254902	0.2539855072463768
0.0982843137254902	0.2545289855072464
0.09877450980392156	0.2545289855072464
0.09877450980392156	0.2552536231884058
0.09926470588235294	0.2552536231884058
0.09926470588235294	0.2585144927536232
0.09950980392156862	0.2585144927536232
0.09950980392156862	0.2592391304347826
0.1	0.2592391304347826
0.1	0.2594202898550725
0.10024509803921569	0.2594202898550725
0.10024509803921569	0.25960144927536233
0.10049019607843138	0.25960144927536233
0.10049019607843138	0.2597826086956522
0.10073529411764706	0.2597826086956522
0.10073529411764706	0.26014492753623186
0.10098039215686275	0.26014492753623186
0.10098039215686275	0.26213768115942027
0.10122549019607843	0.26213768115942027
0.10122549019607843	0.2625
0.10147058823529412	0.2625
0.10147058823529412	0.26268115942028986
0.1017156862745098	0.26268115942028986
0.1017156862745098	0.2628623188405797
0.10196078431372549	0.2628623188405797
0.10196078431372549	0.26304347826086955
0.10245098039215686	0.26304347826086955
0.10245098039215686	0.2634057971014493
0.10269607843137254	0.2634057971014493
0.10269607843137254	0.26358695652173914
0.10294117647058823	0.26358695652173914
0.10294117647058823	0.26413043478260867
0.10318627450980392	0.26413043478260867
0.10318627450980392	0.2657608695652174
0.1036764705882353	0.2657608695652174
0.1036764705882353	0.2664855072463768
0.10392156862745099	0.2664855072463768
0.10392156862745099	0.2684782608695652
0.10416666666666667	0.2684782608695652
0.10416666666666667	0.2697463768115942
0.10465686274509804	0.2697463768115942
0.10465686274509804	0.27155797101449275
0.10490196078431373	0.27155797101449275
0.10490196078431373	0.27246376811594203
0.10514705882352941	0.27246376811594203
0.10514705882352941	0.27391304347826084
0.1053921568627451	0.27391304347826084
0.1053921568627451	0.27445652173913043
0.10588235294117647	0.27445652173913043
0.10588235294117647	0.2746376811594203
0.10612745098039215	0.2746376811594203
0.10612745098039215	0.275
0.10661764705882353	0.275
0.10661764705882353	0.2757246376811594
0.10686274509803921	0.2757246376811594
0.10686274509803921	0.2759057971014493
0.1071078431372549	0.2759057971014493
0.1071078431372549	0.27608695652173915
0.10735294117647058	0.27608695652173915
0.10735294117647058	0.2766304347826087
0.10784313725490197	0.2766304347826087
0.10784313725490197	0.2769927536231884
0.10808823529411765	0.2769927536231884
0.10808823529411765	0.27717391304347827
0.10833333333333334	0.27717391304347827
0.10833333333333334	0.2773550724637681
0.1090686274509804	0.2773550724637681
0.1090686274509804	0.27753623188405796
0.10931372549019608	0.27753623188405796
0.10931372549019608	0.2777173913043478
0.10955882352941176	0.2777173913043478
0.10955882352941176	0.2782608695652174
0.10980392156862745	0.2782608695652174
0.10980392156862745	0.2786231884057971
0.11004901960784313	0.2786231884057971
0.11004901960784313	0.27880434782608693
0.11078431372549019	0.27880434782608693
0.11078431372549019	0.27952898550724636
0.11102941176470588	0.27952898550724636
0.11102941176470588	0.2797101449275362
0.11127450980392156	0.2797101449275362
0.11127450980392156	0.2798913043478261
0.11176470588235295	0.2798913043478261
0.11176470588235295	0.28007246376811595
0.11225490196078432	0.28007246376811595
0.11225490196078432	0.2802536231884058
0.11274509803921569	0.2802536231884058
0.11274509803921569	0.2807971014492754
0.11323529411764706	0.2807971014492754
0.11323529411764706	0.28152173913043477
0.11348039215686274	0.28152173913043477
0.11348039215686274	0.2817028985507246
0.11397058823529412	0.2817028985507246
0.11397058823529412	0.2822463768115942
0.1142156862745098	0.2822463768115942
0.1142156862745098	0.28369565217391307
0.11446078431372549	0.28369565217391307
0.11446078431372549	0.2851449275362319
0.11470588235294117	0.2851449275362319
0.11470588235294117	0.2856884057971015
0.11519607843137254	0.2856884057971015
0.11519607843137254	0.2858695652173913
0.11544117647058824	0.2858695652173913
0.11544117647058824	0.286231884057971
0.11568627450980393	0.286231884057971
0.11568627450980393	0.28695652173913044
0.11642156862745098	0.28695652173913044
0.11642156862745098	0.2875
0.11666666666666667	0.2875
0.11666666666666667	0.28804347826086957
0.11691176470588235	0.28804347826086957
0.11691176470588235	0.28894927536231885
0.11715686274509804	0.28894927536231885
0.11715686274509804	0.2891304347826087
0.11764705882352941	0.2891304347826087
0.11764705882352941	0.28931159420289854
0.1178921568627451	0.28931159420289854
0.1178921568627451	0.2894927536231884
0.11838235294117647	0.2894927536231884
0.11838235294117647	0.29039855072463766
0.11887254901960784	0.29039855072463766
0.11887254901960784	0.2916666666666667
0.11936274509803922	0.2916666666666667
0.11936274509803922	0.29257246376811596
0.11960784313725491	0.29257246376811596
0.11960784313725491	0.2947463768115942
0.11985294117647059	0.2947463768115942
0.11985294117647059	0.2951086956521739
0.12009803921568628	0.2951086956521739
0.12009803921568628	0.29547101449275365
0.12034313725490196	0.29547101449275365
0.12034313725490196	0.2956521739130435
0.12058823529411765	0.2956521739130435
0.12058823529411765	0.296195652173913
0.12083333333333333	0.296195652173913
0.12083333333333333	0.29637681159420287
0.12205882352941176	0.29637681159420287
0.12205882352941176	0.29655797101449277
0.12230392156862745	0.29655797101449277
0.12230392156862745	0.29692028985507246
0.12254901960784313	0.29692028985507246
0.12254901960784313	0.29746376811594205
0.12279411764705882	0.29746376811594205
0.12279411764705882	0.2980072463768116
0.1232843137254902	0.2980072463768116
0.1232843137254902	0.298731884057971
0.12352941176470589	0.298731884057971
0.12352941176470589	0.3
0.12377450980392157	0.3
0.12377450980392157	0.30018115942028983
0.12401960784313726	0.30018115942028983
0.12401960784313726	0.3007246376811594
0.12426470588235294	0.3007246376811594
0.12426470588235294	0.30181159420289855
0.125	0.30181159420289855
0.125	0.30217391304347824
0.12524509803921569	0.30217391304347824
0.12524509803921569	0.3032608695652174
0.12573529411764706	0.3032608695652174
0.12573529411764706	0.30344202898550726
0.12598039215686274	0.30344202898550726
0.12598039215686274	0.30380434782608695
0.1267156862745098	0.30380434782608695
0.1267156862745098	0.30416666666666664
0.12696078431372548	0.30416666666666664
0.12696078431372548	0.30434782608695654
0.12720588235294117	0.30434782608695654
0.12720588235294117	0.30670289855072463
0.12745098039215685	0.30670289855072463
0.12745098039215685	0.3068840579710145
0.12769607843137254	0.3068840579710145
0.12769607843137254	0.3070652173913043
0.12794117647058822	0.3070652173913043
0.12794117647058822	0.3076086956521739
0.1284313725490196	0.3076086956521739
0.1284313725490196	0.30978260869565216
0.128921568627451	0.30978260869565216
0.128921568627451	0.3101449275362319
0.12916666666666668	0.3101449275362319
0.12916666666666668	0.3105072463768116
0.12965686274509805	0.3105072463768116
0.12965686274509805	0.3108695652173913
0.13014705882352942	0.3108695652173913
0.13014705882352942	0.31177536231884057
0.1303921568627451	0.31177536231884057
0.1303921568627451	0.3130434782608696
0.13088235294117648	0.3130434782608696
0.13088235294117648	0.31322463768115943
0.13112745098039216	0.31322463768115943
0.13112745098039216	0.3139492753623188
0.13137254901960785	0.3139492753623188
0.13137254901960785	0.3141304347826087
0.13161764705882353	0.3141304347826087
0.13161764705882353	0.31467391304347825
0.13186274509803922	0.31467391304347825
0.13186274509803922	0.315036231884058
0.1323529411764706	0.315036231884058
0.1323529411764706	0.31521739130434784
0.13259803921568628	0.31521739130434784
0.13259803921568628	0.3159420289855073
0.13284313725490196	0.3159420289855073
0.13284313725490196	0.31630434782608696
0.13308823529411765	0.31630434782608696
0.13308823529411765	0.31865942028985506
0.13333333333333333	0.31865942028985506
0.13333333333333333	0.3190217391304348
0.13357843137254902	0.3190217391304348
0.13357843137254902	0.31956521739130433
0.1340686274509804	0.31956521739130433
0.1340686274509804	0.3197463768115942
0.13431372549019607	0.3197463768115942
0.13431372549019607	0.3204710144927536
0.13455882352941176	0.3204710144927536
0.13455882352941176	0.32119565217391305
0.13504901960784313	0.32119565217391305
0.13504901960784313	0.3213768115942029
0.13529411764705881	0.3213768115942029
0.13529411764705881	0.322463768115942
0.1355392156862745	0.322463768115942
0.1355392156862745	0.32282608695652176
0.13578431372549019	0.32282608695652176
0.13578431372549019	0.3233695652173913
0.13602941176470587	0.3233695652173913
0.13602941176470587	0.32355072463768114
0.13627450980392156	0.32355072463768114
0.13627450980392156	0.3239130434782609
0.13651960784313724	0.3239130434782609
0.13651960784313724	0.3244565217391304
0.13700980392156864	0.3244565217391304
0.13700980392156864	0.32463768115942027
0.1377450980392157	0.32463768115942027
0.1377450980392157	0.325
0.13799019607843138	0.325
0.13799019607843138	0.32518115942028986
0.13872549019607844	0.32518115942028986
0.13872549019607844	0.3253623188405797
0.13897058823529412	0.3253623188405797
0.13897058823529412	0.32572463768115945
0.1392156862745098	0.32572463768115945
0.1392156862745098	0.3259057971014493
0.13970588235294118	0.3259057971014493
0.13970588235294118	0.326268115942029
0.14044117647058824	0.326268115942029
0.14044117647058824	0.32663043478260867
0.14068627450980392	0.32663043478260867
0.14068627450980392	0.32681159420289857
0.1409313725490196	0.32681159420289857
0.1409313725490196	0.32717391304347826
0.1411764705882353	0.32717391304347826
0.1411764705882353	0.32807971014492754
0.14142156862745098	0.32807971014492754
0.14142156862745098	0.32971014492753625
0.14215686274509803	0.32971014492753625
0.14215686274509803	0.33061594202898553
0.14313725490196078	0.33061594202898553
0.14313725490196078	0.3307971014492754
0.14338235294117646	0.3307971014492754
0.14338235294117646	0.33115942028985507
0.14411764705882352	0.33115942028985507
0.14411764705882352	0.33242753623188404
0.1448529411764706	0.33242753623188404
0.1448529411764706	0.3333333333333333
0.14583333333333334	0.3333333333333333
0.14583333333333334	0.33369565217391306
0.14607843137254903	0.33369565217391306
0.14607843137254903	0.33442028985507244
0.1465686274509804	0.33442028985507244
0.1465686274509804	0.33460144927536234
0.14681372549019608	0.33460144927536234
0.14681372549019608	0.3347826086956522
0.14705882352941177	0.3347826086956522
0.14705882352941177	0.336231884057971
0.14754901960784314	0.336231884057971
0.14754901960784314	0.33641304347826084
0.1480392156862745	0.33641304347826084
0.1480392156862745	0.3367753623188406
0.1482843137254902	0.3367753623188406
0.1482843137254902	0.33695652173913043
0.14926470588235294	0.33695652173913043
0.14926470588235294	0.33768115942028987
0.1497549019607843	0.33768115942028987
0.1497549019607843	0.33804347826086956
0.15	0.33804347826086956
0.15	0.3394927536231884
0.15073529411764705	0.3394927536231884
0.15073529411764705	0.3403985507246377
0.15122549019607842	0.3403985507246377
0.15122549019607842	0.3407608695652174
0.1514705882352941	0.3407608695652174
0.1514705882352941	0.34094202898550724
0.1517156862745098	0.34094202898550724
0.1517156862745098	0.3411231884057971
0.15196078431372548	0.3411231884057971
0.15196078431372548	0.3423913043478261
0.15220588235294116	0.3423913043478261
0.15220588235294116	0.34257246376811595
0.15245098039215688	0.34257246376811595
0.15245098039215688	0.3427536231884058
0.15269607843137256	0.3427536231884058
0.15269607843137256	0.3431159420289855
0.15294117647058825	0.3431159420289855
0.15294117647058825	0.34347826086956523
0.15318627450980393	0.34347826086956523
0.15318627450980393	0.3436594202898551
0.15343137254901962	0.3436594202898551
0.15343137254901962	0.3438405797101449
0.1536764705882353	0.3438405797101449
0.1536764705882353	0.34402173913043477
0.153921568627451	0.34402173913043477
0.153921568627451	0.3442028985507246
0.15441176470588236	0.3442028985507246
0.15441176470588236	0.3443840579710145
0.15465686274509804	0.3443840579710145
0.15465686274509804	0.3447463768115942
0.15514705882352942	0.3447463768115942
0.15514705882352942	0.3452898550724638
0.1553921568627451	0.3452898550724638
0.1553921568627451	0.34547101449275364
0.15612745098039216	0.34547101449275364
0.15612745098039216	0.34601449275362317
0.15637254901960784	0.34601449275362317
0.15637254901960784	0.3463768115942029
0.15661764705882353	0.3463768115942029
0.15661764705882353	0.34746376811594204
0.1571078431372549	0.34746376811594204
0.1571078431372549	0.34855072463768116
0.15784313725490196	0.34855072463768116
0.15784313725490196	0.34891304347826085
0.15808823529411764	0.34891304347826085
0.15808823529411764	0.3492753623188406
0.158578431372549	0.3492753623188406
0.158578431372549	0.3496376811594203
0.15931372549019607	0.3496376811594203
0.15931372549019607	0.35
0.16053921568627452	0.35
0.16053921568627452	0.3503623188405797
0.16151960784313726	0.3503623188405797
0.16151960784313726	0.3507246376811594
0.16200980392156863	0.3507246376811594
0.16200980392156863	0.3516304347826087
0.16225490196078432	0.3516304347826087
0.16225490196078432	0.3527173913043478
0.16323529411764706	0.3527173913043478
0.16323529411764706	0.3536231884057971
0.16348039215686275	0.3536231884057971
0.16348039215686275	0.3541666666666667
0.16470588235294117	0.3541666666666667
0.16470588235294117	0.35434782608695653
0.16519607843137254	0.35434782608695653
0.16519607843137254	0.35507246376811596
0.16544117647058823	0.35507246376811596
0.16544117647058823	0.3556159420289855
0.1659313725490196	0.3556159420289855
0.1659313725490196	0.35597826086956524
0.1661764705882353	0.35597826086956524
0.1661764705882353	0.3561594202898551
0.16642156862745097	0.3561594202898551
0.16642156862745097	0.35634057971014493
0.16691176470588234	0.35634057971014493
0.16691176470588234	0.3567028985507246
0.16789215686274508	0.3567028985507246
0.16789215686274508	0.35688405797101447
0.1681372549019608	0.35688405797101447
0.1681372549019608	0.35706521739130437
0.16911764705882354	0.35706521739130437
0.16911764705882354	0.3572463768115942
0.16936274509803922	0.3572463768115942
0.16936274509803922	0.35742753623188406
0.1696078431372549	0.35742753623188406
0.1696078431372549	0.35778985507246375
0.17034313725490197	0.35778985507246375
0.17034313725490197	0.35797101449275365
0.17058823529411765	0.35797101449275365
0.17058823529411765	0.3581521739130435
0.17083333333333334	0.3581521739130435
0.17083333333333334	0.35833333333333334
0.17107843137254902	0.35833333333333334
0.17107843137254902	0.358695652173913
0.1713235294117647	0.358695652173913
0.1713235294117647	0.35887681159420287
0.17181372549019608	0.35887681159420287
0.17181372549019608	0.36032608695652174
0.17230392156862745	0.36032608695652174
0.17230392156862745	0.3605072463768116
0.17254901960784313	0.3605072463768116
0.17254901960784313	0.36141304347826086
0.17352941176470588	0.36141304347826086
0.17352941176470588	0.3621376811594203
0.17377450980392156	0.3621376811594203
0.17377450980392156	0.36268115942028983
0.17401960784313725	0.36268115942028983
0.17401960784313725	0.36286231884057973
0.17426470588235293	0.36286231884057973
0.17426470588235293	0.3630434782608696
0.17450980392156862	0.3630434782608696
0.17450980392156862	0.36376811594202896
0.1747549019607843	0.36376811594202896
0.1747549019607843	0.3641304347826087
0.17622549019607844	0.3641304347826087
0.17622549019607844	0.36431159420289855
0.17647058823529413	0.36431159420289855
0.17647058823529413	0.3644927536231884
0.1769607843137255	0.3644927536231884
0.1769607843137255	0.36594202898550726
0.17745098039215687	0.36594202898550726
0.17745098039215687	0.3661231884057971
0.17769607843137256	0.3661231884057971
0.17769607843137256	0.36630434782608695
0.17794117647058824	0.36630434782608695
0.17794117647058824	0.3670289855072464
0.17818627450980393	0.3670289855072464
0.17818627450980393	0.36721014492753623
0.1784313725490196	0.36721014492753623
0.1784313725490196	0.3673913043478261
0.17892156862745098	0.3673913043478261
0.17892156862745098	0.3681159420289855
0.17916666666666667	0.3681159420289855
0.17916666666666667	0.3690217391304348
0.17941176470588235	0.3690217391304348
0.17941176470588235	0.36920289855072463
0.1803921568627451	0.36920289855072463
0.1803921568627451	0.3695652173913043
0.18063725490196078	0.3695652173913043
0.18063725490196078	0.3697463768115942
0.18112745098039215	0.3697463768115942
0.18112745098039215	0.36992753623188407
0.1818627450980392	0.36992753623188407
0.1818627450980392	0.37028985507246376
0.1821078431372549	0.37028985507246376
0.1821078431372549	0.3704710144927536
0.18284313725490195	0.3704710144927536
0.18284313725490195	0.3706521739130435
0.18308823529411763	0.3706521739130435
0.18308823529411763	0.37083333333333335
0.18382352941176472	0.37083333333333335
0.18382352941176472	0.3710144927536232
0.1840686274509804	0.3710144927536232
0.1840686274509804	0.37119565217391304
0.18504901960784315	0.37119565217391304
0.18504901960784315	0.3715579710144927
0.18529411764705883	0.3715579710144927
0.18529411764705883	0.3717391304347826
0.18553921568627452	0.3717391304347826
0.18553921568627452	0.3719202898550725
0.1857843137254902	0.3719202898550725
0.1857843137254902	0.3721014492753623
0.18627450980392157	0.3721014492753623
0.18627450980392157	0.37228260869565216
0.18651960784313726	0.37228260869565216
0.18651960784313726	0.372463768115942
0.18700980392156863	0.372463768115942
0.18700980392156863	0.3726449275362319
0.1892156862745098	0.3726449275362319
0.1892156862745098	0.37282608695652175
0.18946078431372548	0.37282608695652175
0.18946078431372548	0.3730072463768116
0.18970588235294117	0.3730072463768116
0.18970588235294117	0.3733695652173913
0.18995098039215685	0.3733695652173913
0.18995098039215685	0.37373188405797103
0.19117647058823528	0.37373188405797103
0.19117647058823528	0.3739130434782609
0.191421568627451	0.3739130434782609
0.191421568627451	0.3740942028985507
0.19240196078431374	0.3740942028985507
0.19240196078431374	0.3744565217391304
0.19264705882352942	0.3744565217391304
0.19264705882352942	0.3746376811594203
0.1928921568627451	0.3746376811594203
0.1928921568627451	0.37481884057971016
0.1931372549019608	0.37481884057971016
0.1931372549019608	0.37518115942028984
0.19362745098039216	0.37518115942028984
0.19362745098039216	0.3753623188405797
0.19411764705882353	0.3753623188405797
0.19411764705882353	0.3755434782608696
0.19558823529411765	0.3755434782608696
0.19558823529411765	0.3759057971014493
0.19583333333333333	0.3759057971014493
0.19583333333333333	0.3760869565217391
0.19607843137254902	0.3760869565217391
0.19607843137254902	0.37626811594202897
0.19681372549019607	0.37626811594202897
0.19681372549019607	0.3766304347826087
0.19730392156862744	0.3766304347826087
0.19730392156862744	0.37681159420289856
0.1980392156862745	0.37681159420289856
0.1980392156862745	0.3773550724637681
0.19828431372549019	0.3773550724637681
0.19828431372549019	0.3780797101449275
0.19852941176470587	0.3780797101449275
0.19852941176470587	0.3782608695652174
0.19901960784313724	0.3782608695652174
0.19901960784313724	0.3784420289855073
0.19926470588235295	0.3784420289855073
0.19926470588235295	0.3786231884057971
0.2	0.3786231884057971
0.2	0.3789855072463768
0.2002450980392157	0.3789855072463768
0.2002450980392157	0.3793478260869565
0.20098039215686275	0.3793478260869565
0.20098039215686275	0.3795289855072464
0.20147058823529412	0.3795289855072464
0.20147058823529412	0.3798913043478261
0.2017156862745098	0.3798913043478261
0.2017156862745098	0.38007246376811593
0.2019607843137255	0.38007246376811593
0.2019607843137255	0.3809782608695652
0.20220588235294118	0.3809782608695652
0.20220588235294118	0.3818840579710145
0.20294117647058824	0.3818840579710145
0.20294117647058824	0.38206521739130433
0.2034313725490196	0.38206521739130433
0.2034313725490196	0.3838768115942029
0.2036764705882353	0.3838768115942029
0.2036764705882353	0.3842391304347826
0.20416666666666666	0.3842391304347826
0.20416666666666666	0.384963768115942
0.20441176470588235	0.384963768115942
0.20441176470588235	0.38532608695652176
0.2051470588235294	0.38532608695652176
0.2051470588235294	0.3855072463768116
0.2053921568627451	0.3855072463768116
0.2053921568627451	0.38713768115942027
0.20563725490196078	0.38713768115942027
0.20563725490196078	0.3875
0.20612745098039215	0.3875
0.20612745098039215	0.38768115942028986
0.20710784313725492	0.38768115942028986
0.20710784313725492	0.3884057971014493
0.20784313725490197	0.3884057971014493
0.20784313725490197	0.38913043478260867
0.2088235294117647	0.38913043478260867
0.2088235294117647	0.38931159420289857
0.20980392156862746	0.38931159420289857
0.20980392156862746	0.3894927536231884
0.21004901960784314	0.3894927536231884
0.21004901960784314	0.39003623188405795
0.21151960784313725	0.39003623188405795
0.21151960784313725	0.39057971014492754
0.21274509803921568	0.39057971014492754
0.21274509803921568	0.39112318840579713
0.21323529411764705	0.39112318840579713
0.21323529411764705	0.3923913043478261
0.21446078431372548	0.3923913043478261
0.21446078431372548	0.39257246376811594
0.21470588235294116	0.39257246376811594
0.21470588235294116	0.3927536231884058
0.21495098039215688	0.3927536231884058
0.21495098039215688	0.39293478260869563
0.21568627450980393	0.39293478260869563
0.21568627450980393	0.39311594202898553
0.2161764705882353	0.39311594202898553
0.2161764705882353	0.3934782608695652
0.216421568627451	0.3934782608695652
0.216421568627451	0.3938405797101449
0.21691176470588236	0.3938405797101449
0.21691176470588236	0.39456521739130435
0.21715686274509804	0.39456521739130435
0.21715686274509804	0.39492753623188404
0.2181372549019608	0.39492753623188404
0.2181372549019608	0.3952898550724638
0.22009803921568627	0.3952898550724638
0.22009803921568627	0.3958333333333333
0.22083333333333333	0.3958333333333333
0.22083333333333333	0.3960144927536232
0.2213235294117647	0.3960144927536232
0.2213235294117647	0.39619565217391306
0.22181372549019607	0.39619565217391306
0.22181372549019607	0.3963768115942029
0.2235294117647059	0.3963768115942029
0.2235294117647059	0.39655797101449275
0.22377450980392158	0.39655797101449275
0.22377450980392158	0.3967391304347826
0.22450980392156863	0.3967391304347826
0.22450980392156863	0.39710144927536234
0.22475490196078432	0.39710144927536234
0.22475490196078432	0.3972826086956522
0.2252450980392157	0.3972826086956522
0.2252450980392157	0.39818840579710146
0.22549019607843138	0.39818840579710146
0.22549019607843138	0.39945652173913043
0.22598039215686275	0.39945652173913043
0.22598039215686275	0.40018115942028987
0.22622549019607843	0.40018115942028987
0.22622549019607843	0.4003623188405797
0.2267156862745098	0.4003623188405797
0.2267156862745098	0.40054347826086956
0.22794117647058823	0.40054347826086956
0.22794117647058823	0.401268115942029
0.22892156862745097	0.401268115942029
0.22892156862745097	0.4023550724637681
0.22916666666666666	0.4023550724637681
0.22916666666666666	0.40253623188405796
0.2299019607843137	0.40253623188405796
0.2299019607843137	0.4027173913043478
0.23088235294117648	0.4027173913043478
0.23088235294117648	0.4028985507246377
0.23112745098039217	0.4028985507246377
0.23112745098039217	0.4036231884057971
0.23161764705882354	0.4036231884057971
0.23161764705882354	0.40380434782608693
0.2321078431372549	0.40380434782608693
0.2321078431372549	0.4041666666666667
0.2323529411764706	0.4041666666666667
0.2323529411764706	0.4043478260869565
0.23284313725490197	0.4043478260869565
0.23284313725490197	0.4048913043478261
0.23308823529411765	0.4048913043478261
0.23308823529411765	0.40507246376811595
0.23333333333333334	0.40507246376811595
0.23333333333333334	0.40543478260869564
0.23357843137254902	0.40543478260869564
0.23357843137254902	0.4056159420289855
0.2340686274509804	0.4056159420289855
0.2340686274509804	0.4068840579710145
0.23431372549019608	0.4068840579710145
0.23431372549019608	0.4072463768115942
0.23431372549019608	0.40742753623188405
0.23529411764705882	0.40742753623188405
0.23529411764705882	0.4077898550724638
0.2355392156862745	0.4077898550724638
0.2355392156862745	0.40797101449275364
0.23676470588235293	0.40797101449275364
0.23676470588235293	0.4081521739130435
0.2375	0.4081521739130435
0.2375	0.4083333333333333
0.23774509803921567	0.4083333333333333
0.23774509803921567	0.40869565217391307
0.23848039215686276	0.40869565217391307
0.23848039215686276	0.4088768115942029
0.23897058823529413	0.4088768115942029
0.23897058823529413	0.4092391304347826
0.23921568627450981	0.4092391304347826
0.23921568627450981	0.40942028985507245
0.23970588235294119	0.40942028985507245
0.23970588235294119	0.4096014492753623
0.23995098039215687	0.4096014492753623
0.23995098039215687	0.4097826086956522
0.24044117647058824	0.4097826086956522
0.24044117647058824	0.40996376811594204
0.2409313725490196	0.40996376811594204
0.2409313725490196	0.4106884057971015
0.24142156862745098	0.4106884057971015
0.24142156862745098	0.4108695652173913
0.24166666666666667	0.4108695652173913
0.24166666666666667	0.411231884057971
0.24338235294117647	0.411231884057971
0.24338235294117647	0.41141304347826085
0.24362745098039215	0.41141304347826085
0.24362745098039215	0.4115942028985507
0.2443627450980392	0.4115942028985507
0.2443627450980392	0.41195652173913044
0.2446078431372549	0.41195652173913044
0.2446078431372549	0.4121376811594203
0.24558823529411763	0.4121376811594203
0.24558823529411763	0.41231884057971013
0.24583333333333332	0.41231884057971013
0.24583333333333332	0.4125
0.246078431372549	0.4125
0.246078431372549	0.4126811594202899
0.24632352941176472	0.4126811594202899
0.24632352941176472	0.4128623188405797
0.2465686274509804	0.4128623188405797
0.2465686274509804	0.41304347826086957
0.24877450980392157	0.41304347826086957
0.24877450980392157	0.41340579710144926
0.24975490196078431	0.41340579710144926
0.24975490196078431	0.41394927536231885
0.25049019607843137	0.41394927536231885
0.25049019607843137	0.4141304347826087
0.2512254901960784	0.4141304347826087
0.2512254901960784	0.41431159420289854
0.2517156862745098	0.41431159420289854
0.2517156862745098	0.4144927536231884
0.25269607843137254	0.4144927536231884
0.25269607843137254	0.4148550724637681
0.2529411764705882	0.4148550724637681
0.2529411764705882	0.4164855072463768
0.2531862745098039	0.4164855072463768
0.2531862745098039	0.4166666666666667
0.2536764705882353	0.4166666666666667
0.2536764705882353	0.4170289855072464
0.25392156862745097	0.4170289855072464
0.25392156862745097	0.4177536231884058
0.25416666666666665	0.4177536231884058
0.25416666666666665	0.41793478260869565
0.2551470588235294	0.41793478260869565
0.2551470588235294	0.4186594202898551
0.25563725490196076	0.4186594202898551
0.25563725490196076	0.41884057971014493
0.25588235294117645	0.41884057971014493
0.25588235294117645	0.41938405797101447
0.2566176470588235	0.41938405797101447
0.2566176470588235	0.41956521739130437
0.2568627450980392	0.41956521739130437
0.2568627450980392	0.41992753623188406
0.2571078431372549	0.41992753623188406
0.2571078431372549	0.4201086956521739
0.25882352941176473	0.4201086956521739
0.25882352941176473	0.42028985507246375
0.2590686274509804	0.42028985507246375
0.2590686274509804	0.4206521739130435
0.2595588235294118	0.4206521739130435
0.2595588235294118	0.4210144927536232
0.26029411764705884	0.4210144927536232
0.26029411764705884	0.4221014492753623
0.2612745098039216	0.4221014492753623
0.2612745098039216	0.42228260869565215
0.26151960784313727	0.42228260869565215
0.26151960784313727	0.42246376811594205
0.26176470588235295	0.42246376811594205
0.26176470588235295	0.4226449275362319
0.26200980392156864	0.4226449275362319
0.26200980392156864	0.42282608695652174
0.2622549019607843	0.42282608695652174
0.2622549019607843	0.4230072463768116
0.2629901960784314	0.4230072463768116
0.2629901960784314	0.42318840579710143
0.26348039215686275	0.42318840579710143
0.26348039215686275	0.423731884057971
0.26372549019607844	0.423731884057971
0.26372549019607844	0.42445652173913045
0.2642156862745098	0.42445652173913045
0.2642156862745098	0.4246376811594203
0.2644607843137255	0.4246376811594203
0.2644607843137255	0.425
0.26495098039215687	0.425
0.26495098039215687	0.4260869565217391
0.26519607843137255	0.4260869565217391
0.26519607843137255	0.42626811594202896
0.26544117647058824	0.42626811594202896
0.26544117647058824	0.4266304347826087
0.2656862745098039	0.4266304347826087
0.2656862745098039	0.4269927536231884
0.2659313725490196	0.4269927536231884
0.2659313725490196	0.42735507246376814
0.266421568627451	0.42735507246376814
0.266421568627451	0.4277173913043478
0.26691176470588235	0.4277173913043478
0.26691176470588235	0.42844202898550726
0.26715686274509803	0.42844202898550726
0.26715686274509803	0.4286231884057971
0.2678921568627451	0.4286231884057971
0.2678921568627451	0.4289855072463768
0.26887254901960783	0.4289855072463768
0.26887254901960783	0.4295289855072464
0.2693627450980392	0.4295289855072464
0.2693627450980392	0.42971014492753623
0.2696078431372549	0.42971014492753623
0.2696078431372549	0.4298913043478261
0.2698529411764706	0.4298913043478261
0.2698529411764706	0.4300724637681159
0.27009803921568626	0.4300724637681159
0.27009803921568626	0.4302536231884058
0.27034313725490194	0.4302536231884058
0.27034313725490194	0.4306159420289855
0.2713235294117647	0.4306159420289855
0.2713235294117647	0.4311594202898551
0.27156862745098037	0.4311594202898551
0.27156862745098037	0.43134057971014494
0.27328431372549017	0.43134057971014494
0.27328431372549017	0.43170289855072463
0.2735294117647059	0.43170289855072463
0.2735294117647059	0.4320652173913043
0.2740196078431373	0.4320652173913043
0.2740196078431373	0.4326086956521739
0.2754901960784314	0.4326086956521739
0.2754901960784314	0.4329710144927536
0.2757352941176471	0.4329710144927536
0.2757352941176471	0.43333333333333335
0.27647058823529413	0.43333333333333335
0.27647058823529413	0.4335144927536232
0.2767156862745098	0.4335144927536232
0.2767156862745098	0.43369565217391304
0.2772058823529412	0.43369565217391304
0.2772058823529412	0.4338768115942029
0.2774509803921569	0.4338768115942029
0.2774509803921569	0.4340579710144927
0.27769607843137256	0.4340579710144927
0.27769607843137256	0.4342391304347826
0.27794117647058825	0.4342391304347826
0.27794117647058825	0.4346014492753623
0.27818627450980393	0.4346014492753623
0.27818627450980393	0.434963768115942
0.2784313725490196	0.434963768115942
0.2784313725490196	0.4351449275362319
0.2786764705882353	0.4351449275362319
0.2786764705882353	0.4355072463768116
0.2791666666666667	0.4355072463768116
0.2791666666666667	0.4358695652173913
0.27941176470588236	0.4358695652173913
0.27941176470588236	0.4360507246376812
0.27965686274509804	0.4360507246376812
0.27965686274509804	0.4365942028985507
0.2803921568627451	0.4365942028985507
0.2803921568627451	0.4369565217391304
0.2806372549019608	0.4369565217391304
0.2806372549019608	0.43731884057971016
0.28088235294117647	0.43731884057971016
0.28088235294117647	0.43768115942028984
0.28112745098039216	0.43768115942028984
0.28112745098039216	0.4378623188405797
0.28137254901960784	0.4378623188405797
0.28137254901960784	0.43876811594202897
0.28161764705882353	0.43876811594202897
0.28161764705882353	0.4389492753623188
0.2818627450980392	0.4389492753623188
0.2818627450980392	0.4405797101449275
0.2821078431372549	0.4405797101449275
0.2821078431372549	0.4411231884057971
0.2833333333333333	0.4411231884057971
0.2833333333333333	0.4414855072463768
0.2840686274509804	0.4414855072463768
0.2840686274509804	0.44221014492753624
0.28431372549019607	0.44221014492753624
0.28431372549019607	0.44257246376811593
0.28480392156862744	0.44257246376811593
0.28480392156862744	0.44329710144927537
0.2850490196078431	0.44329710144927537
0.2850490196078431	0.4434782608695652
0.2855392156862745	0.4434782608695652
0.2855392156862745	0.4438405797101449
0.28602941176470587	0.4438405797101449
0.28602941176470587	0.4460144927536232
0.28627450980392155	0.4460144927536232
0.28627450980392155	0.44619565217391305
0.28651960784313724	0.44619565217391305
0.28651960784313724	0.4463768115942029
0.2872549019607843	0.4463768115942029
0.2872549019607843	0.4469202898550725
0.2875	0.4469202898550725
0.2875	0.44710144927536233
0.28774509803921566	0.44710144927536233
0.28774509803921566	0.447463768115942
0.28823529411764703	0.447463768115942
0.28823529411764703	0.44764492753623186
0.2889705882352941	0.44764492753623186
0.2889705882352941	0.44818840579710145
0.28921568627450983	0.44818840579710145
0.28921568627450983	0.44873188405797104
0.2894607843137255	0.44873188405797104
0.2894607843137255	0.4494565217391304
0.2897058823529412	0.4494565217391304
0.2897058823529412	0.44963768115942027
0.2901960784313726	0.44963768115942027
0.2901960784313726	0.44981884057971017
0.29068627450980394	0.44981884057971017
0.29068627450980394	0.45
0.2911764705882353	0.45
0.2911764705882353	0.4503623188405797
0.2916666666666667	0.4503623188405797
0.2916666666666667	0.45054347826086955
0.29191176470588237	0.45054347826086955
0.29191176470588237	0.451268115942029
0.29240196078431374	0.451268115942029
0.29240196078431374	0.4514492753623188
0.2926470588235294	0.4514492753623188
0.2926470588235294	0.4519927536231884
0.2928921568627451	0.4519927536231884
0.2928921568627451	0.45217391304347826
0.2933823529411765	0.45217391304347826
0.2933823529411765	0.45271739130434785
0.29411764705882354	0.45271739130434785
0.29411764705882354	0.45362318840579713
0.2946078431372549	0.45362318840579713
0.2946078431372549	0.4539855072463768
0.2948529411764706	0.4539855072463768
0.2948529411764706	0.45452898550724635
0.2950980392156863	0.45452898550724635
0.2950980392156863	0.45471014492753625
0.29534313725490197	0.45471014492753625
0.29534313725490197	0.45507246376811594
0.29583333333333334	0.45507246376811594
0.29583333333333334	0.45543478260869563
0.2963235294117647	0.45543478260869563
0.2963235294117647	0.45561594202898553
0.2965686274509804	0.45561594202898553
0.2965686274509804	0.4557971014492754
0.2968137254901961	0.4557971014492754
0.2968137254901961	0.4563405797101449
0.29705882352941176	0.4563405797101449
0.29705882352941176	0.45652173913043476
0.29730392156862745	0.45652173913043476
0.29730392156862745	0.45706521739130435
0.2977941176470588	0.45706521739130435
0.2977941176470588	0.4572463768115942
0.2982843137254902	0.4572463768115942
0.2982843137254902	0.45760869565217394
0.2985294117647059	0.45760869565217394
0.2985294117647059	0.4577898550724638
0.29877450980392156	0.4577898550724638
0.29877450980392156	0.4585144927536232
0.29901960784313725	0.4585144927536232
0.29901960784313725	0.45869565217391306
0.29926470588235293	0.45869565217391306
0.29926470588235293	0.4588768115942029
0.2995098039215686	0.4588768115942029
0.2995098039215686	0.45905797101449275
0.3	0.45905797101449275
0.3	0.45960144927536234
0.3002450980392157	0.45960144927536234
0.3002450980392157	0.46105072463768115
0.30049019607843136	0.46105072463768115
0.30049019607843136	0.461231884057971
0.30073529411764705	0.461231884057971
0.30073529411764705	0.46268115942028987
0.30098039215686273	0.46268115942028987
0.30098039215686273	0.46304347826086956
0.3017156862745098	0.46304347826086956
0.3017156862745098	0.4632246376811594
0.30196078431372547	0.4632246376811594
0.30196078431372547	0.4641304347826087
0.30220588235294116	0.4641304347826087
0.30220588235294116	0.46503623188405796
0.30269607843137253	0.46503623188405796
0.30269607843137253	0.4652173913043478
0.3029411764705882	0.4652173913043478
0.3029411764705882	0.46648550724637683
0.3031862745098039	0.46648550724637683
0.3031862745098039	0.46793478260869564
0.3034313725490196	0.46793478260869564
0.3034313725490196	0.46847826086956523
0.30392156862745096	0.46847826086956523
0.30392156862745096	0.4688405797101449
0.30416666666666664	0.4688405797101449
0.30416666666666664	0.4693840579710145
0.3044117647058823	0.4693840579710145
0.3044117647058823	0.46992753623188405
0.3053921568627451	0.46992753623188405
0.3053921568627451	0.4701086956521739
0.3056372549019608	0.4701086956521739
0.3056372549019608	0.4706521739130435
0.3058823529411765	0.4706521739130435
0.3058823529411765	0.47155797101449276
0.30637254901960786	0.47155797101449276
0.30637254901960786	0.4717391304347826
0.30661764705882355	0.4717391304347826
0.30661764705882355	0.4722826086956522
0.3071078431372549	0.4722826086956522
0.3071078431372549	0.47246376811594204
0.3075980392156863	0.47246376811594204
0.3075980392156863	0.4726449275362319
0.30808823529411766	0.4726449275362319
0.30808823529411766	0.47282608695652173
0.3090686274509804	0.47282608695652173
0.3090686274509804	0.473731884057971
0.3093137254901961	0.473731884057971
0.3093137254901961	0.47391304347826085
0.3095588235294118	0.47391304347826085
0.3095588235294118	0.4746376811594203
0.31004901960784315	0.4746376811594203
0.31004901960784315	0.47481884057971013
0.3110294117647059	0.47481884057971013
0.3110294117647059	0.4751811594202899
0.3112745098039216	0.4751811594202899
0.3112745098039216	0.4757246376811594
0.31176470588235294	0.4757246376811594
0.31176470588235294	0.47590579710144926
0.31200980392156863	0.47590579710144926
0.31200980392156863	0.47608695652173916
0.3122549019607843	0.47608695652173916
0.3122549019607843	0.47644927536231885
0.3125	0.47644927536231885
0.3125	0.4769927536231884
0.3127450980392157	0.4769927536231884
0.3127450980392157	0.4773550724637681
0.31299019607843137	0.4773550724637681
0.31299019607843137	0.4782608695652174
0.31323529411764706	0.4782608695652174
0.31323529411764706	0.47880434782608694
0.31348039215686274	0.47880434782608694
0.31348039215686274	0.4791666666666667
0.3137254901960784	0.4791666666666667
0.3137254901960784	0.4797101449275362
0.3139705882352941	0.4797101449275362
0.3139705882352941	0.47989130434782606
0.3142156862745098	0.47989130434782606
0.3142156862745098	0.48007246376811596
0.3144607843137255	0.48007246376811596
0.3144607843137255	0.4802536231884058
0.3156862745098039	0.4802536231884058
0.3156862745098039	0.4806159420289855
0.31666666666666665	0.4806159420289855
0.31666666666666665	0.48097826086956524
0.317156862745098	0.48097826086956524
0.317156862745098	0.4815217391304348
0.3174019607843137	0.4815217391304348
0.3174019607843137	0.48242753623188406
0.3178921568627451	0.48242753623188406
0.3178921568627451	0.48278985507246375
0.31838235294117645	0.48278985507246375
0.31838235294117645	0.483695652173913
0.3188725490196078	0.483695652173913
0.3188725490196078	0.4846014492753623
0.3196078431372549	0.4846014492753623
0.3196078431372549	0.48478260869565215
0.31985294117647056	0.48478260869565215
0.31985294117647056	0.48568840579710143
0.32009803921568625	0.48568840579710143
0.32009803921568625	0.48586956521739133
0.320343137254902	0.48586956521739133
0.320343137254902	0.48677536231884055
0.3205882352941177	0.48677536231884055
0.3205882352941177	0.48695652173913045
0.32083333333333336	0.48695652173913045
0.32083333333333336	0.4871376811594203
0.32132352941176473	0.4871376811594203
0.32132352941176473	0.48731884057971014
0.3215686274509804	0.48731884057971014
0.3215686274509804	0.4880434782608696
0.3218137254901961	0.4880434782608696
0.3218137254901961	0.48876811594202896
0.3220588235294118	0.48876811594202896
0.3220588235294118	0.48967391304347824
0.32230392156862747	0.48967391304347824
0.32230392156862747	0.4902173913043478
0.32303921568627453	0.4902173913043478
0.32303921568627453	0.4905797101449275
0.3232843137254902	0.4905797101449275
0.3232843137254902	0.49094202898550726
0.3235294117647059	0.49094202898550726
0.3235294117647059	0.49130434782608695
0.325	0.49130434782608695
0.325	0.4914855072463768
0.3252450980392157	0.4914855072463768
0.3252450980392157	0.4920289855072464
0.3254901960784314	0.4920289855072464
0.3254901960784314	0.49221014492753623
0.32598039215686275	0.49221014492753623
0.32598039215686275	0.4923913043478261
0.32622549019607844	0.4923913043478261
0.32622549019607844	0.4925724637681159
0.3269607843137255	0.4925724637681159
0.3269607843137255	0.4927536231884058
0.3272058823529412	0.4927536231884058
0.3272058823529412	0.49329710144927535
0.32769607843137255	0.49329710144927535
0.32769607843137255	0.4940217391304348
0.3286764705882353	0.4940217391304348
0.3286764705882353	0.49492753623188407
0.328921568627451	0.49492753623188407
0.328921568627451	0.49619565217391304
0.32965686274509803	0.49619565217391304
0.32965686274509803	0.4963768115942029
0.3303921568627451	0.4963768115942029
0.3303921568627451	0.4967391304347826
0.3306372549019608	0.4967391304347826
0.3306372549019608	0.49728260869565216
0.33137254901960783	0.49728260869565216
0.33137254901960783	0.497463768115942
0.3323529411764706	0.497463768115942
0.3323529411764706	0.4976449275362319
0.33259803921568626	0.4976449275362319
0.33259803921568626	0.4983695652173913
0.3333333333333333	0.4983695652173913
0.3333333333333333	0.4985507246376812
0.333578431372549	0.4985507246376812
0.333578431372549	0.49873188405797103
0.3338235294117647	0.49873188405797103
0.3338235294117647	0.4989130434782609
0.33406862745098037	0.4989130434782609
0.33406862745098037	0.4996376811594203
0.33431372549019606	0.4996376811594203
0.33431372549019606	0.5
0.33455882352941174	0.5
0.33455882352941174	0.5007246376811594
0.3352941176470588	0.5007246376811594
0.3352941176470588	0.5009057971014492
0.3360294117647059	0.5009057971014492
0.3360294117647059	0.5010869565217392
0.3362745098039216	0.5010869565217392
0.3362745098039216	0.501268115942029
0.3375	0.501268115942029
0.3375	0.5016304347826087
0.3379901960784314	0.5016304347826087
0.3379901960784314	0.5023550724637681
0.3382352941176471	0.5023550724637681
0.3382352941176471	0.5028985507246376
0.33848039215686276	0.5028985507246376
0.33848039215686276	0.5030797101449276
0.33897058823529413	0.5030797101449276
0.33897058823529413	0.5032608695652174
0.3392156862745098	0.5032608695652174
0.3392156862745098	0.5036231884057971
0.3394607843137255	0.5036231884057971
0.3394607843137255	0.503804347826087
0.3399509803921569	0.503804347826087
0.3399509803921569	0.5039855072463768
0.34019607843137256	0.5039855072463768
0.34019607843137256	0.5047101449275362
0.34068627450980393	0.5047101449275362
0.34068627450980393	0.5048913043478261
0.341421568627451	0.5048913043478261
0.341421568627451	0.5052536231884058
0.3416666666666667	0.5052536231884058
0.3416666666666667	0.5054347826086957
0.34191176470588236	0.5054347826086957
0.34191176470588236	0.5056159420289855
0.3426470588235294	0.5056159420289855
0.3426470588235294	0.5067028985507246
0.3426470588235294	0.5070652173913044
0.3426470588235294	0.5072463768115942
0.3431372549019608	0.5072463768115942
0.3431372549019608	0.5077898550724638
0.34387254901960784	0.5077898550724638
0.34387254901960784	0.508695652173913
0.3443627450980392	0.508695652173913
0.3443627450980392	0.5096014492753623
0.3448529411764706	0.5096014492753623
0.3448529411764706	0.509963768115942
0.34534313725490196	0.509963768115942
0.34534313725490196	0.5103260869565217
0.3458333333333333	0.5103260869565217
0.3458333333333333	0.5105072463768116
0.3465686274509804	0.5105072463768116
0.3465686274509804	0.511231884057971
0.34681372549019607	0.511231884057971
0.34681372549019607	0.5119565217391304
0.34705882352941175	0.5119565217391304
0.34705882352941175	0.5126811594202898
0.3477941176470588	0.5126811594202898
0.3477941176470588	0.5135869565217391
0.3480392156862745	0.5135869565217391
0.3480392156862745	0.5141304347826087
0.3482843137254902	0.5141304347826087
0.3482843137254902	0.5143115942028985
0.34852941176470587	0.5143115942028985
0.34852941176470587	0.5152173913043478
0.34877450980392155	0.5152173913043478
0.34877450980392155	0.5153985507246377
0.3492647058823529	0.5153985507246377
0.3492647058823529	0.5163043478260869
0.3495098039215686	0.5163043478260869
0.3495098039215686	0.5164855072463768
0.3497549019607843	0.5164855072463768
0.3497549019607843	0.5166666666666667
0.35	0.5166666666666667
0.35	0.5172101449275363
0.35024509803921566	0.5172101449275363
0.35024509803921566	0.5177536231884058
0.35049019607843135	0.5177536231884058
0.35049019607843135	0.5197463768115942
0.35073529411764703	0.5197463768115942
0.35073529411764703	0.519927536231884
0.3509803921568627	0.519927536231884
0.3509803921568627	0.5201086956521739
0.3522058823529412	0.5201086956521739
0.3522058823529412	0.5202898550724637
0.3524509803921569	0.5202898550724637
0.3524509803921569	0.5208333333333334
0.35318627450980394	0.5208333333333334
0.35318627450980394	0.5210144927536232
0.35343137254901963	0.5210144927536232
0.35343137254901963	0.5213768115942029
0.3541666666666667	0.5213768115942029
0.3541666666666667	0.5221014492753623
0.35490196078431374	0.5221014492753623
0.35490196078431374	0.5222826086956521
0.3551470588235294	0.5222826086956521
0.3551470588235294	0.5224637681159421
0.3553921568627451	0.5224637681159421
0.3553921568627451	0.5240942028985507
0.3556372549019608	0.5240942028985507
0.3556372549019608	0.5242753623188405
0.35612745098039217	0.5242753623188405
0.35612745098039217	0.5248188405797102
0.35637254901960785	0.5248188405797102
0.35637254901960785	0.525
0.3573529411764706	0.525
0.3573529411764706	0.5253623188405797
0.35784313725490197	0.5253623188405797
0.35784313725490197	0.5257246376811594
0.35808823529411765	0.5257246376811594
0.35808823529411765	0.5264492753623189
0.35833333333333334	0.5264492753623189
0.35833333333333334	0.5266304347826087
0.358578431372549	0.5266304347826087
0.358578431372549	0.5271739130434783
0.3588235294117647	0.5271739130434783
0.3588235294117647	0.5273550724637681
0.3590686274509804	0.5273550724637681
0.3590686274509804	0.5280797101449275
0.3593137254901961	0.5280797101449275
0.3593137254901961	0.5289855072463768
0.35980392156862745	0.5289855072463768
0.35980392156862745	0.5295289855072464
0.3607843137254902	0.5295289855072464
0.3607843137254902	0.5302536231884057
0.3610294117647059	0.5302536231884057
0.3610294117647059	0.5304347826086957
0.36127450980392156	0.5304347826086957
0.36127450980392156	0.5307971014492754
0.36151960784313725	0.5307971014492754
0.36151960784313725	0.5309782608695652
0.36176470588235293	0.5309782608695652
0.36176470588235293	0.5315217391304348
0.3620098039215686	0.5315217391304348
0.3620098039215686	0.5324275362318841
0.3625	0.5324275362318841
0.3625	0.532608695652174
0.36299019607843136	0.532608695652174
0.36299019607843136	0.533695652173913
0.36348039215686273	0.533695652173913
0.36348039215686273	0.5342391304347827
0.3642156862745098	0.5342391304347827
0.3642156862745098	0.5355072463768116
0.36446078431372547	0.5355072463768116
0.36446078431372547	0.5356884057971014
0.36470588235294116	0.5356884057971014
0.36470588235294116	0.5358695652173913
0.36495098039215684	0.5358695652173913
0.36495098039215684	0.5362318840579711
0.3654411764705882	0.5362318840579711
0.3654411764705882	0.5365942028985508
0.3656862745098039	0.5365942028985508
0.3656862745098039	0.5367753623188406
0.3659313725490196	0.5367753623188406
0.3659313725490196	0.5369565217391304
0.36666666666666664	0.5369565217391304
0.36666666666666664	0.5373188405797101
0.36764705882352944	0.5373188405797101
0.36764705882352944	0.5376811594202898
0.3678921568627451	0.5376811594202898
0.3678921568627451	0.5378623188405797
0.3681372549019608	0.5378623188405797
0.3681372549019608	0.5384057971014493
0.3683823529411765	0.5384057971014493
0.3683823529411765	0.5385869565217392
0.3686274509803922	0.5385869565217392
0.3686274509803922	0.5405797101449276
0.36887254901960786	0.5405797101449276
0.36887254901960786	0.5427536231884058
0.3696078431372549	0.5427536231884058
0.3696078431372549	0.5429347826086957
0.370343137254902	0.5429347826086957
0.370343137254902	0.5431159420289855
0.37058823529411766	0.5431159420289855
0.37058823529411766	0.5432971014492753
0.37083333333333335	0.5432971014492753
0.37083333333333335	0.5438405797101449
0.3715686274509804	0.5438405797101449
0.3715686274509804	0.5443840579710145
0.37230392156862746	0.5443840579710145
0.37230392156862746	0.5447463768115942
0.37254901960784315	0.5447463768115942
0.37254901960784315	0.5451086956521739
0.3730392156862745	0.5451086956521739
0.3730392156862745	0.5454710144927536
0.3732843137254902	0.5454710144927536
0.3732843137254902	0.5461956521739131
0.3735294117647059	0.5461956521739131
0.3735294117647059	0.5463768115942029
0.37401960784313726	0.5463768115942029
0.37401960784313726	0.5467391304347826
0.37450980392156863	0.5467391304347826
0.37450980392156863	0.5469202898550725
0.3747549019607843	0.5469202898550725
0.3747549019607843	0.547463768115942
0.375	0.547463768115942
0.375	0.5478260869565217
0.3752450980392157	0.5478260869565217
0.3752450980392157	0.5480072463768116
0.37549019607843137	0.5480072463768116
0.37549019607843137	0.548731884057971
0.37573529411764706	0.548731884057971
0.37573529411764706	0.5489130434782609
0.3764705882352941	0.5489130434782609
0.3764705882352941	0.5494565217391304
0.37720588235294117	0.5494565217391304
0.37720588235294117	0.5498188405797102
0.37745098039215685	0.5498188405797102
0.37745098039215685	0.5501811594202899
0.3779411764705882	0.5501811594202899
0.3779411764705882	0.5507246376811594
0.3784313725490196	0.5507246376811594
0.3784313725490196	0.5509057971014493
0.3786764705882353	0.5509057971014493
0.3786764705882353	0.551268115942029
0.37892156862745097	0.551268115942029
0.37892156862745097	0.5516304347826086
0.379656862745098	0.5516304347826086
0.379656862745098	0.5518115942028986
0.3799019607843137	0.5518115942028986
0.3799019607843137	0.5521739130434783
0.3803921568627451	0.5521739130434783
0.3803921568627451	0.5523550724637681
0.38063725490196076	0.5523550724637681
0.38063725490196076	0.552536231884058
0.3813725490196078	0.552536231884058
0.3813725490196078	0.5527173913043478
0.3816176470588235	0.5527173913043478
0.3816176470588235	0.553623188405797
0.3818627450980392	0.553623188405797
0.3818627450980392	0.5543478260869565
0.3821078431372549	0.5543478260869565
0.3821078431372549	0.5545289855072464
0.38235294117647056	0.5545289855072464
0.38235294117647056	0.5547101449275362
0.38259803921568625	0.5547101449275362
0.38259803921568625	0.5548913043478261
0.38333333333333336	0.5548913043478261
0.38333333333333336	0.5556159420289855
0.38357843137254904	0.5556159420289855
0.38357843137254904	0.5559782608695653
0.38382352941176473	0.5559782608695653
0.38382352941176473	0.5565217391304348
0.3843137254901961	0.5565217391304348
0.3843137254901961	0.5568840579710145
0.38480392156862747	0.5568840579710145
0.38480392156862747	0.557427536231884
0.38529411764705884	0.557427536231884
0.38529411764705884	0.5583333333333333
0.38553921568627453	0.5583333333333333
0.38553921568627453	0.5585144927536232
0.3857843137254902	0.5585144927536232
0.3857843137254902	0.5588768115942029
0.3860294117647059	0.5588768115942029
0.3860294117647059	0.5590579710144927
0.3862745098039216	0.5590579710144927
0.3862745098039216	0.5592391304347826
0.38651960784313727	0.5592391304347826
0.38651960784313727	0.5594202898550724
0.38676470588235295	0.5594202898550724
0.38676470588235295	0.5596014492753624
0.38700980392156864	0.5596014492753624
0.38700980392156864	0.5597826086956522
0.3872549019607843	0.5597826086956522
0.3872549019607843	0.5603260869565218
0.3875	0.5603260869565218
0.3875	0.5606884057971014
0.3877450980392157	0.5606884057971014
0.3877450980392157	0.5610507246376811
0.3879901960784314	0.5610507246376811
0.3879901960784314	0.5625
0.38823529411764707	0.5625
0.38823529411764707	0.5630434782608695
0.3892156862745098	0.5630434782608695
0.3892156862745098	0.5632246376811594
0.3894607843137255	0.5632246376811594
0.3894607843137255	0.5634057971014492
0.38995098039215687	0.5634057971014492
0.38995098039215687	0.5643115942028986
0.39019607843137255	0.5643115942028986
0.39019607843137255	0.5652173913043478
0.39044117647058824	0.5652173913043478
0.39044117647058824	0.5655797101449276
0.3906862745098039	0.5655797101449276
0.3906862745098039	0.5657608695652174
0.3909313725490196	0.5657608695652174
0.3909313725490196	0.5666666666666667
0.3911764705882353	0.5666666666666667
0.3911764705882353	0.5668478260869565
0.391421568627451	0.5668478260869565
0.391421568627451	0.5672101449275362
0.39166666666666666	0.5672101449275362
0.39166666666666666	0.5682971014492754
0.39215686274509803	0.5682971014492754
0.39215686274509803	0.5684782608695652
0.39338235294117646	0.5684782608695652
0.39338235294117646	0.568659420289855
0.3943627450980392	0.568659420289855
0.3943627450980392	0.5690217391304347
0.39534313725490194	0.5690217391304347
0.39534313725490194	0.5692028985507246
0.39558823529411763	0.5692028985507246
0.39558823529411763	0.5693840579710145
0.3958333333333333	0.5693840579710145
0.3958333333333333	0.5695652173913044
0.39656862745098037	0.5695652173913044
0.39656862745098037	0.5699275362318841
0.39681372549019606	0.5699275362318841
0.39681372549019606	0.5719202898550725
0.3980392156862745	0.5719202898550725
0.3980392156862745	0.5721014492753623
0.39828431372549017	0.5721014492753623
0.39828431372549017	0.5722826086956522
0.3985294117647059	0.5722826086956522
0.3985294117647059	0.572463768115942
0.3987745098039216	0.572463768115942
0.3987745098039216	0.5730072463768116
0.3990196078431373	0.5730072463768116
0.3990196078431373	0.5731884057971014
0.39926470588235297	0.5731884057971014
0.39926470588235297	0.5742753623188406
0.39950980392156865	0.5742753623188406
0.39950980392156865	0.5746376811594203
0.39975490196078434	0.5746376811594203
0.39975490196078434	0.575
0.4	0.575
0.4	0.5751811594202898
0.4002450980392157	0.5751811594202898
0.4002450980392157	0.5753623188405798
0.4004901960784314	0.5753623188405798
0.4004901960784314	0.576268115942029
0.40122549019607845	0.576268115942029
0.40122549019607845	0.5771739130434783
0.40147058823529413	0.5771739130434783
0.40147058823529413	0.5773550724637682
0.4017156862745098	0.5773550724637682
0.4017156862745098	0.577536231884058
0.4019607843137255	0.577536231884058
0.4019607843137255	0.5777173913043478
0.4022058823529412	0.5777173913043478
0.4022058823529412	0.5778985507246377
0.4024509803921569	0.5778985507246377
0.4024509803921569	0.5782608695652174
0.40269607843137256	0.5782608695652174
0.40269607843137256	0.5784420289855072
0.40465686274509804	0.5784420289855072
0.40465686274509804	0.5788043478260869
0.40490196078431373	0.5788043478260869
0.40490196078431373	0.5789855072463768
0.4051470588235294	0.5789855072463768
0.4051470588235294	0.5800724637681159
0.4053921568627451	0.5800724637681159
0.4053921568627451	0.5802536231884058
0.4056372549019608	0.5802536231884058
0.4056372549019608	0.5807971014492753
0.4068627450980392	0.5807971014492753
0.4068627450980392	0.581340579710145
0.4071078431372549	0.581340579710145
0.4071078431372549	0.5818840579710145
0.40784313725490196	0.5818840579710145
0.40784313725490196	0.5820652173913043
0.4083333333333333	0.5820652173913043
0.4083333333333333	0.5826086956521739
0.4090686274509804	0.5826086956521739
0.4090686274509804	0.5829710144927536
0.4105392156862745	0.5829710144927536
0.4105392156862745	0.5831521739130435
0.4107843137254902	0.5831521739130435
0.4107843137254902	0.5835144927536232
0.41127450980392155	0.5835144927536232
0.41127450980392155	0.5836956521739131
0.4122549019607843	0.5836956521739131
0.4122549019607843	0.5838768115942029
0.4125	0.5838768115942029
0.4125	0.5844202898550724
0.41299019607843135	0.5844202898550724
0.41299019607843135	0.5846014492753623
0.4134803921568627	0.5846014492753623
0.4134803921568627	0.5849637681159421
0.4139705882352941	0.5849637681159421
0.4139705882352941	0.5851449275362319
0.41421568627450983	0.5851449275362319
0.41421568627450983	0.5853260869565218
0.4144607843137255	0.5853260869565218
0.4144607843137255	0.5855072463768116
0.4147058823529412	0.5855072463768116
0.4147058823529412	0.5865942028985507
0.4149509803921569	0.5865942028985507
0.4149509803921569	0.5871376811594203
0.4151960784313726	0.5871376811594203
0.4151960784313726	0.5875
0.41568627450980394	0.5875
0.41568627450980394	0.5876811594202899
0.4161764705882353	0.5876811594202899
0.4161764705882353	0.5880434782608696
0.4166666666666667	0.5880434782608696
0.4166666666666667	0.5882246376811594
0.41691176470588237	0.5882246376811594
0.41691176470588237	0.5884057971014492
0.41715686274509806	0.5884057971014492
0.41715686274509806	0.5887681159420289
0.4176470588235294	0.5887681159420289
0.4176470588235294	0.5891304347826087
0.4178921568627451	0.5891304347826087
0.4178921568627451	0.590036231884058
0.41887254901960785	0.590036231884058
0.41887254901960785	0.5903985507246376
0.4196078431372549	0.5903985507246376
0.4196078431372549	0.5911231884057971
0.4200980392156863	0.5911231884057971
0.4200980392156863	0.5918478260869565
0.42034313725490197	0.5918478260869565
0.42034313725490197	0.5929347826086957
0.42083333333333334	0.5929347826086957
0.42083333333333334	0.5931159420289855
0.4215686274509804	0.5931159420289855
0.4215686274509804	0.5932971014492754
0.4218137254901961	0.5932971014492754
0.4218137254901961	0.5934782608695652
0.4230392156862745	0.5934782608695652
0.4230392156862745	0.5938405797101449
0.42401960784313725	0.5938405797101449
0.42401960784313725	0.5940217391304348
0.4245098039215686	0.5940217391304348
0.4245098039215686	0.5943840579710145
0.4252450980392157	0.5943840579710145
0.4252450980392157	0.5949275362318841
0.42549019607843136	0.5949275362318841
0.42549019607843136	0.5952898550724638
0.4262254901960784	0.5952898550724638
0.4262254901960784	0.5954710144927536
0.4264705882352941	0.5954710144927536
0.4264705882352941	0.596195652173913
0.42696078431372547	0.596195652173913
0.42696078431372547	0.5963768115942029
0.42720588235294116	0.5963768115942029
0.42720588235294116	0.5969202898550725
0.42745098039215684	0.5969202898550725
0.42745098039215684	0.597463768115942
0.4279411764705882	0.597463768115942
0.4279411764705882	0.5976449275362319
0.4284313725490196	0.5976449275362319
0.4284313725490196	0.5978260869565217
0.4294117647058823	0.5978260869565217
0.4294117647058823	0.5981884057971014
0.429656862745098	0.5981884057971014
0.429656862745098	0.5983695652173913
0.42990196078431375	0.5983695652173913
0.42990196078431375	0.5987318840579711
0.43014705882352944	0.5987318840579711
0.43014705882352944	0.5989130434782609
0.4303921568627451	0.5989130434782609
0.4303921568627451	0.5994565217391304
0.4306372549019608	0.5994565217391304
0.4306372549019608	0.5996376811594203
0.4308823529411765	0.5996376811594203
0.4308823529411765	0.5998188405797101
0.43161764705882355	0.5998188405797101
0.43161764705882355	0.6003623188405797
0.4321078431372549	0.6003623188405797
0.4321078431372549	0.6009057971014493
0.4323529411764706	0.6009057971014493
0.4323529411764706	0.6010869565217392
0.432843137254902	0.6010869565217392
0.432843137254902	0.6016304347826087
0.43308823529411766	0.6016304347826087
0.43308823529411766	0.6021739130434782
0.43357843137254903	0.6021739130434782
0.43357843137254903	0.6025362318840579
0.4338235294117647	0.6025362318840579
0.4338235294117647	0.6027173913043479
0.4340686274509804	0.6027173913043479
0.4340686274509804	0.6038043478260869
0.43504901960784315	0.6038043478260869
0.43504901960784315	0.6041666666666666
0.43529411764705883	0.6041666666666666
0.43529411764705883	0.6047101449275363
0.4355392156862745	0.6047101449275363
0.4355392156862745	0.6052536231884058
0.4360294117647059	0.6052536231884058
0.4360294117647059	0.6054347826086957
0.4362745098039216	0.6054347826086957
0.4362745098039216	0.6057971014492753
0.43676470588235294	0.6057971014492753
0.43676470588235294	0.606159420289855
0.43700980392156863	0.606159420289855
0.43700980392156863	0.6070652173913044
0.4377450980392157	0.6070652173913044
0.4377450980392157	0.6072463768115942
0.43799019607843137	0.6072463768115942
0.43799019607843137	0.6074275362318841
0.43823529411764706	0.6074275362318841
0.43823529411764706	0.6077898550724637
0.43848039215686274	0.6077898550724637
0.43848039215686274	0.6081521739130434
0.4387254901960784	0.6081521739130434
0.4387254901960784	0.6086956521739131
0.4389705882352941	0.6086956521739131
0.4389705882352941	0.6088768115942029
0.4392156862745098	0.6088768115942029
0.4392156862745098	0.6094202898550725
0.43970588235294117	0.6094202898550725
0.43970588235294117	0.6096014492753623
0.43995098039215685	0.6096014492753623
0.43995098039215685	0.6097826086956522
0.4411764705882353	0.6097826086956522
0.4411764705882353	0.6105072463768116
0.44142156862745097	0.6105072463768116
0.44142156862745097	0.611231884057971
0.44191176470588234	0.611231884057971
0.44191176470588234	0.6123188405797102
0.442156862745098	0.6123188405797102
0.442156862745098	0.6125
0.4424019607843137	0.6125
0.4424019607843137	0.6132246376811594
0.4426470588235294	0.6132246376811594
0.4426470588235294	0.6139492753623188
0.44338235294117645	0.6139492753623188
0.44338235294117645	0.6144927536231884
0.4446078431372549	0.6144927536231884
0.4446078431372549	0.6152173913043478
0.44485294117647056	0.6152173913043478
0.44485294117647056	0.6157608695652174
0.44509803921568625	0.6157608695652174
0.44509803921568625	0.616123188405797
0.445343137254902	0.616123188405797
0.445343137254902	0.6170289855072464
0.44607843137254904	0.6170289855072464
0.44607843137254904	0.6179347826086956
0.4468137254901961	0.6179347826086956
0.4468137254901961	0.6181159420289855
0.4470588235294118	0.6181159420289855
0.4470588235294118	0.6182971014492754
0.44754901960784316	0.6182971014492754
0.44754901960784316	0.6184782608695653
0.44779411764705884	0.6184782608695653
0.44779411764705884	0.618840579710145
0.4482843137254902	0.618840579710145
0.4482843137254902	0.6190217391304348
0.4485294117647059	0.6190217391304348
0.4485294117647059	0.6192028985507246
0.4487745098039216	0.6192028985507246
0.4487745098039216	0.6197463768115942
0.44901960784313727	0.6197463768115942
0.44901960784313727	0.6208333333333333
0.44926470588235295	0.6208333333333333
0.44926470588235295	0.6210144927536232
0.45	0.6210144927536232
0.45	0.6226449275362319
0.4502450980392157	0.6226449275362319
0.4502450980392157	0.6228260869565218
0.4504901960784314	0.6228260869565218
0.4504901960784314	0.6235507246376811
0.45098039215686275	0.6235507246376811
0.45098039215686275	0.623731884057971
0.45122549019607844	0.623731884057971
0.45122549019607844	0.6239130434782608
0.4517156862745098	0.6239130434782608
0.4517156862745098	0.625
0.4519607843137255	0.625
0.4519607843137255	0.6253623188405797
0.45245098039215687	0.6253623188405797
0.45245098039215687	0.6257246376811594
0.45294117647058824	0.6257246376811594
0.45294117647058824	0.626268115942029
0.45416666666666666	0.626268115942029
0.45416666666666666	0.6269927536231884
0.45465686274509803	0.6269927536231884
0.45465686274509803	0.6271739130434782
0.4549019607843137	0.6271739130434782
0.4549019607843137	0.6277173913043478
0.4553921568627451	0.6277173913043478
0.4553921568627451	0.6280797101449276
0.4556372549019608	0.6280797101449276
0.4556372549019608	0.6284420289855073
0.45612745098039215	0.6284420289855073
0.45612745098039215	0.6291666666666667
0.4568627450980392	0.6291666666666667
0.4568627450980392	0.630072463768116
0.45759803921568626	0.630072463768116
0.45759803921568626	0.6304347826086957
0.45784313725490194	0.6304347826086957
0.45784313725490194	0.6307971014492754
0.45808823529411763	0.6307971014492754
0.45808823529411763	0.6320652173913044
0.458578431372549	0.6320652173913044
0.458578431372549	0.6324275362318841
0.45906862745098037	0.6324275362318841
0.45906862745098037	0.6326086956521739
0.45931372549019606	0.6326086956521739
0.45931372549019606	0.6329710144927536
0.45955882352941174	0.6329710144927536
0.45955882352941174	0.6331521739130435
0.4600490196078431	0.6331521739130435
0.4600490196078431	0.6333333333333333
0.4602941176470588	0.6333333333333333
0.4602941176470588	0.6335144927536231
0.4605392156862745	0.6335144927536231
0.4605392156862745	0.633695652173913
0.46078431372549017	0.633695652173913
0.46078431372549017	0.6340579710144928
0.4610294117647059	0.6340579710144928
0.4610294117647059	0.6344202898550725
0.4612745098039216	0.6344202898550725
0.4612745098039216	0.6346014492753623
0.46225490196078434	0.6346014492753623
0.46225490196078434	0.6347826086956522
0.4625	0.6347826086956522
0.4625	0.6351449275362319
0.4632352941176471	0.6351449275362319
0.4632352941176471	0.6353260869565217
0.46348039215686276	0.6353260869565217
0.46348039215686276	0.6358695652173914
0.46372549019607845	0.6358695652173914
0.46372549019607845	0.6360507246376812
0.46397058823529413	0.6360507246376812
0.46397058823529413	0.6364130434782609
0.4642156862745098	0.6364130434782609
0.4642156862745098	0.6375
0.4644607843137255	0.6375
0.4644607843137255	0.6376811594202898
0.4649509803921569	0.6376811594202898
0.4649509803921569	0.6378623188405798
0.46519607843137256	0.6378623188405798
0.46519607843137256	0.6380434782608696
0.46544117647058825	0.6380434782608696
0.46544117647058825	0.6385869565217391
0.4661764705882353	0.6385869565217391
0.4661764705882353	0.638768115942029
0.46740196078431373	0.638768115942029
0.46740196078431373	0.6389492753623188
0.4676470588235294	0.6389492753623188
0.4676470588235294	0.6391304347826087
0.4681372549019608	0.6391304347826087
0.4681372549019608	0.6393115942028985
0.46838235294117647	0.6393115942028985
0.46838235294117647	0.6394927536231884
0.46862745098039216	0.6394927536231884
0.46862745098039216	0.6396739130434783
0.46887254901960784	0.6396739130434783
0.46887254901960784	0.6409420289855072
0.46911764705882353	0.6409420289855072
0.46911764705882353	0.6414855072463768
0.4693627450980392	0.6414855072463768
0.4693627450980392	0.6418478260869566
0.4696078431372549	0.6418478260869566
0.4696078431372549	0.6420289855072464
0.47034313725490196	0.6420289855072464
0.47034313725490196	0.6429347826086956
0.4708333333333333	0.6429347826086956
0.4708333333333333	0.6434782608695652
0.4713235294117647	0.6434782608695652
0.4713235294117647	0.6443840579710145
0.4715686274509804	0.6443840579710145
0.4715686274509804	0.6445652173913043
0.47181372549019607	0.6445652173913043
0.47181372549019607	0.644927536231884
0.47205882352941175	0.644927536231884
0.47205882352941175	0.6452898550724637
0.4732843137254902	0.6452898550724637
0.4732843137254902	0.6454710144927536
0.4742647058823529	0.6454710144927536
0.4742647058823529	0.6461956521739131
0.4745098039215686	0.6461956521739131
0.4745098039215686	0.6467391304347826
0.4747549019607843	0.6467391304347826
0.4747549019607843	0.6476449275362319
0.4759803921568627	0.6476449275362319
0.4759803921568627	0.6478260869565218
0.47671568627450983	0.6478260869565218
0.47671568627450983	0.6481884057971015
0.4772058823529412	0.6481884057971015
0.4772058823529412	0.6489130434782608
0.4776960784313726	0.6489130434782608
0.4776960784313726	0.6490942028985507
0.47818627450980394	0.6490942028985507
0.47818627450980394	0.6492753623188405
0.47843137254901963	0.6492753623188405
0.47843137254901963	0.6498188405797102
0.4786764705882353	0.6498188405797102
0.4786764705882353	0.6501811594202899
0.4791666666666667	0.6501811594202899
0.4791666666666667	0.6503623188405797
0.47941176470588237	0.6503623188405797
0.47941176470588237	0.6505434782608696
0.4806372549019608	0.6505434782608696
0.4806372549019608	0.6510869565217391
0.4808823529411765	0.6510869565217391
0.4808823529411765	0.6519927536231884
0.48112745098039217	0.6519927536231884
0.48112745098039217	0.6521739130434783
0.48137254901960785	0.6521739130434783
0.48137254901960785	0.6532608695652173
0.48161764705882354	0.6532608695652173
0.48161764705882354	0.6534420289855073
0.4818627450980392	0.6534420289855073
0.4818627450980392	0.6536231884057971
0.4821078431372549	0.6536231884057971
0.4821078431372549	0.653804347826087
0.4823529411764706	0.653804347826087
0.4823529411764706	0.6545289855072464
0.4825980392156863	0.6545289855072464
0.4825980392156863	0.6547101449275362
0.48333333333333334	0.6547101449275362
0.48333333333333334	0.6552536231884057
0.483578431372549	0.6552536231884057
0.483578431372549	0.6556159420289855
0.4838235294117647	0.6556159420289855
0.4838235294117647	0.6561594202898551
0.4840686274509804	0.6561594202898551
0.4840686274509804	0.6565217391304348
0.48455882352941176	0.6565217391304348
0.48455882352941176	0.6583333333333333
0.48480392156862745	0.6583333333333333
0.48480392156862745	0.658695652173913
0.48504901960784313	0.658695652173913
0.48504901960784313	0.6597826086956522
0.4857843137254902	0.6597826086956522
0.4857843137254902	0.6605072463768116
0.4860294117647059	0.6605072463768116
0.4860294117647059	0.6606884057971014
0.48627450980392156	0.6606884057971014
0.48627450980392156	0.6610507246376811
0.4877450980392157	0.6610507246376811
0.4877450980392157	0.6612318840579711
0.48823529411764705	0.6612318840579711
0.48823529411764705	0.6614130434782609
0.4889705882352941	0.6614130434782609
0.4889705882352941	0.6615942028985508
0.48946078431372547	0.6615942028985508
0.48946078431372547	0.6617753623188406
0.4904411764705882	0.6617753623188406
0.4904411764705882	0.6621376811594203
0.4906862745098039	0.6621376811594203
0.4906862745098039	0.6623188405797101
0.49117647058823527	0.6623188405797101
0.49117647058823527	0.6626811594202898
0.49142156862745096	0.6626811594202898
0.49142156862745096	0.6634057971014493
0.49166666666666664	0.6634057971014493
0.49166666666666664	0.6639492753623188
0.4919117647058823	0.6639492753623188
0.4919117647058823	0.6641304347826087
0.492156862745098	0.6641304347826087
0.492156862745098	0.6644927536231884
0.49240196078431375	0.6644927536231884
0.49240196078431375	0.6650362318840579
0.4928921568627451	0.6650362318840579
0.4928921568627451	0.6652173913043479
0.4931372549019608	0.6652173913043479
0.4931372549019608	0.6655797101449276
0.49411764705882355	0.6655797101449276
0.49411764705882355	0.6657608695652174
0.4946078431372549	0.6657608695652174
0.4946078431372549	0.6659420289855073
0.4950980392156863	0.6659420289855073
0.4950980392156863	0.6661231884057971
0.495343137254902	0.6661231884057971
0.495343137254902	0.6666666666666666
0.49558823529411766	0.6666666666666666
0.49558823529411766	0.6668478260869565
0.49583333333333335	0.6668478260869565
0.49583333333333335	0.6670289855072464
0.4965686274509804	0.6670289855072464
0.4965686274509804	0.6673913043478261
0.4968137254901961	0.6673913043478261
0.4968137254901961	0.667572463768116
0.49754901960784315	0.667572463768116
0.49754901960784315	0.6677536231884058
0.4982843137254902	0.6677536231884058
0.4982843137254902	0.668659420289855
0.4985294117647059	0.668659420289855
0.4985294117647059	0.6693840579710145
0.49926470588235294	0.6693840579710145
0.49926470588235294	0.6695652173913044
0.49950980392156863	0.6695652173913044
0.49950980392156863	0.6699275362318841
0.4997549019607843	0.6699275362318841
0.4997549019607843	0.6701086956521739
0.5	0.6701086956521739
0.5	0.6706521739130434
0.5002450980392157	0.6706521739130434
0.5002450980392157	0.6708333333333333
0.5004901960784314	0.6708333333333333
0.5004901960784314	0.6711956521739131
0.5007352941176471	0.6711956521739131
0.5007352941176471	0.6715579710144928
0.5009803921568627	0.6715579710144928
0.5009803921568627	0.6719202898550725
0.5012254901960784	0.6719202898550725
0.5012254901960784	0.6722826086956522
0.5014705882352941	0.6722826086956522
0.5014705882352941	0.672463768115942
0.5017156862745098	0.672463768115942
0.5017156862745098	0.6726449275362318
0.5022058823529412	0.6726449275362318
0.5022058823529412	0.6728260869565217
0.5024509803921569	0.6728260869565217
0.5024509803921569	0.6731884057971015
0.5029411764705882	0.6731884057971015
0.5029411764705882	0.6733695652173913
0.5044117647058823	0.6733695652173913
0.5044117647058823	0.673731884057971
0.504656862745098	0.673731884057971
0.504656862745098	0.6739130434782609
0.5051470588235294	0.6739130434782609
0.5051470588235294	0.6740942028985507
0.5053921568627451	0.6740942028985507
0.5056372549019608	0.6742753623188406
0.5056372549019608	0.6744565217391304
0.5058823529411764	0.6744565217391304
0.5058823529411764	0.6751811594202899
0.5061274509803921	0.6751811594202899
0.5061274509803921	0.6753623188405797
0.5063725490196078	0.6753623188405797
0.5063725490196078	0.6755434782608696
0.5071078431372549	0.6755434782608696
0.5071078431372549	0.676268115942029
0.5075980392156862	0.676268115942029
0.5075980392156862	0.6768115942028986
0.5080882352941176	0.6768115942028986
0.5080882352941176	0.6773550724637681
0.5083333333333333	0.6773550724637681
0.5083333333333333	0.677536231884058
0.508578431372549	0.677536231884058
0.508578431372549	0.6777173913043478
0.5095588235294117	0.6777173913043478
0.5095588235294117	0.678623188405797
0.5098039215686274	0.678623188405797
0.5098039215686274	0.678804347826087
0.5100490196078431	0.678804347826087
0.5100490196078431	0.6797101449275362
0.5102941176470588	0.6797101449275362
0.5102941176470588	0.6804347826086956
0.5105392156862745	0.6804347826086956
0.5105392156862745	0.6806159420289855
0.5107843137254902	0.6806159420289855
0.5107843137254902	0.6811594202898551
0.5112745098039215	0.6811594202898551
0.5112745098039215	0.6815217391304348
0.5115196078431372	0.6815217391304348
0.5115196078431372	0.6818840579710145
0.5120098039215686	0.6818840579710145
0.5120098039215686	0.6820652173913043
0.5122549019607843	0.6820652173913043
0.5122549019607843	0.682427536231884
0.5125	0.682427536231884
0.5125	0.6827898550724638
0.513235294117647	0.6827898550724638
0.513235294117647	0.6829710144927537
0.5144607843137254	0.6829710144927537
0.5144607843137254	0.6833333333333333
0.5151960784313725	0.6833333333333333
0.5151960784313725	0.6840579710144927
0.5159313725490197	0.6840579710144927
0.5159313725490197	0.6842391304347826
0.5161764705882353	0.6842391304347826
0.5161764705882353	0.6844202898550724
0.5169117647058824	0.6844202898550724
0.5169117647058824	0.6847826086956522
0.5171568627450981	0.6847826086956522
0.5171568627450981	0.6849637681159421
0.5176470588235295	0.6849637681159421
0.5176470588235295	0.6851449275362319
0.5178921568627451	0.6851449275362319
0.5178921568627451	0.6853260869565218
0.5181372549019608	0.6853260869565218
0.5181372549019608	0.6855072463768116
0.5191176470588236	0.6855072463768116
0.5191176470588236	0.6865942028985508
0.5193627450980393	0.6865942028985508
0.5193627450980393	0.6869565217391305
0.5196078431372549	0.6869565217391305
0.5196078431372549	0.6878623188405797
0.5200980392156863	0.6878623188405797
0.5200980392156863	0.6880434782608695
0.520343137254902	0.6880434782608695
0.520343137254902	0.6884057971014492
0.5208333333333334	0.6884057971014492
0.5208333333333334	0.6891304347826087
0.5210784313725491	0.6891304347826087
0.5210784313725491	0.6893115942028986
0.5213235294117647	0.6893115942028986
0.5213235294117647	0.6894927536231884
0.5220588235294118	0.6894927536231884
0.5220588235294118	0.6903985507246376
0.5225490196078432	0.6903985507246376
0.5225490196078432	0.6911231884057971
0.5230392156862745	0.6911231884057971
0.5230392156862745	0.6914855072463768
0.5235294117647059	0.6914855072463768
0.5235294117647059	0.6920289855072463
0.5237745098039216	0.6920289855072463
0.5237745098039216	0.6923913043478261
0.524264705882353	0.6923913043478261
0.524264705882353	0.6927536231884058
0.5245098039215687	0.6927536231884058
0.5245098039215687	0.6949275362318841
0.5247549019607843	0.6949275362318841
0.5247549019607843	0.6951086956521739
0.5257352941176471	0.6951086956521739
0.5257352941176471	0.6952898550724638
0.5262254901960784	0.6952898550724638
0.5262254901960784	0.6954710144927536
0.5267156862745098	0.6954710144927536
0.5267156862745098	0.6958333333333333
0.5274509803921569	0.6958333333333333
0.5274509803921569	0.6972826086956522
0.5279411764705882	0.6972826086956522
0.5279411764705882	0.697463768115942
0.5281862745098039	0.697463768115942
0.5281862745098039	0.6976449275362319
0.528921568627451	0.6976449275362319
0.528921568627451	0.6980072463768116
0.5291666666666667	0.6980072463768116
0.5291666666666667	0.7001811594202898
0.5294117647058824	0.7001811594202898
0.5294117647058824	0.7003623188405798
0.529656862745098	0.7003623188405798
0.529656862745098	0.7005434782608696
0.5303921568627451	0.7005434782608696
0.5303921568627451	0.7007246376811594
0.5306372549019608	0.7007246376811594
0.5306372549019608	0.7010869565217391
0.5308823529411765	0.7010869565217391
0.5308823529411765	0.7014492753623188
0.5316176470588235	0.7014492753623188
0.5316176470588235	0.7018115942028985
0.5318627450980392	0.7018115942028985
0.5318627450980392	0.7027173913043478
0.5321078431372549	0.7027173913043478
0.5321078431372549	0.7032608695652174
0.5325980392156863	0.7032608695652174
0.5325980392156863	0.7034420289855072
0.532843137254902	0.7034420289855072
0.532843137254902	0.7038043478260869
0.533578431372549	0.7038043478260869
0.533578431372549	0.7039855072463768
0.5338235294117647	0.7039855072463768
0.5338235294117647	0.7041666666666667
0.5343137254901961	0.7041666666666667
0.5343137254901961	0.7043478260869566
0.5350490196078431	0.7043478260869566
0.5350490196078431	0.7047101449275363
0.5357843137254902	0.7047101449275363
0.5357843137254902	0.7048913043478261
0.5367647058823529	0.7048913043478261
0.5367647058823529	0.7050724637681159
0.5375	0.7050724637681159
0.5375	0.7056159420289855
0.5377450980392157	0.7056159420289855
0.5377450980392157	0.7061594202898551
0.538235294117647	0.7061594202898551
0.538235294117647	0.7068840579710145
0.5394607843137255	0.7068840579710145
0.5394607843137255	0.7072463768115942
0.5397058823529411	0.7072463768115942
0.5397058823529411	0.7079710144927536
0.5401960784313725	0.7079710144927536
0.5401960784313725	0.7081521739130435
0.5406862745098039	0.7081521739130435
0.5406862745098039	0.7086956521739131
0.5414215686274509	0.7086956521739131
0.5414215686274509	0.7088768115942029
0.5426470588235294	0.7088768115942029
0.5426470588235294	0.7092391304347826
0.5428921568627451	0.7092391304347826
0.5428921568627451	0.7094202898550724
0.5431372549019607	0.7094202898550724
0.5431372549019607	0.7097826086956521
0.5443627450980392	0.7097826086956521
0.5443627450980392	0.7099637681159421
0.5448529411764705	0.7099637681159421
0.5448529411764705	0.7101449275362319
0.5455882352941176	0.7101449275362319
0.5455882352941176	0.7108695652173913
0.546078431372549	0.7108695652173913
0.546078431372549	0.7110507246376812
0.5463235294117647	0.7110507246376812
0.5463235294117647	0.7115942028985507
0.5465686274509803	0.7115942028985507
0.5465686274509803	0.7119565217391305
0.546813725490196	0.7119565217391305
0.546813725490196	0.7121376811594203
0.5470588235294118	0.7121376811594203
0.5470588235294118	0.7126811594202899
0.5473039215686275	0.7126811594202899
0.5473039215686275	0.7128623188405797
0.5475490196078432	0.7128623188405797
0.5475490196078432	0.7130434782608696
0.5480392156862746	0.7130434782608696
0.5480392156862746	0.7135869565217391
0.5482843137254902	0.7135869565217391
0.5482843137254902	0.7148550724637681
0.5485294117647059	0.7148550724637681
0.5485294117647059	0.715036231884058
0.5487745098039216	0.715036231884058
0.5487745098039216	0.7152173913043478
0.5490196078431373	0.7152173913043478
0.5490196078431373	0.7155797101449275
0.549264705882353	0.7155797101449275
0.549264705882353	0.7157608695652173
0.5495098039215687	0.7157608695652173
0.5495098039215687	0.7164855072463768
0.5497549019607844	0.7164855072463768
0.5497549019607844	0.7168478260869565
0.55	0.7168478260869565
0.55	0.7172101449275362
0.5509803921568628	0.7172101449275362
0.5509803921568628	0.7179347826086957
0.5514705882352942	0.7179347826086957
0.5514705882352942	0.7181159420289855
0.5519607843137255	0.7181159420289855
0.5519607843137255	0.7182971014492754
0.5536764705882353	0.7182971014492754
0.5536764705882353	0.7184782608695652
0.553921568627451	0.7184782608695652
0.553921568627451	0.7186594202898551
0.5544117647058824	0.7186594202898551
0.5544117647058824	0.7188405797101449
0.5549019607843138	0.7188405797101449
0.5549019607843138	0.7190217391304348
0.5553921568627451	0.7190217391304348
0.5553921568627451	0.7193840579710145
0.5556372549019608	0.7193840579710145
0.5556372549019608	0.7195652173913043
0.5558823529411765	0.7195652173913043
0.5558823529411765	0.7199275362318841
0.5571078431372549	0.7199275362318841
0.5571078431372549	0.7202898550724638
0.5573529411764706	0.7202898550724638
0.5573529411764706	0.7210144927536232
0.557843137254902	0.7210144927536232
0.557843137254902	0.721195652173913
0.5580882352941177	0.721195652173913
0.5580882352941177	0.7219202898550725
0.5588235294117647	0.7219202898550725
0.5588235294117647	0.7230072463768116
0.5590686274509804	0.7230072463768116
0.5590686274509804	0.7242753623188406
0.5593137254901961	0.7242753623188406
0.5593137254901961	0.7244565217391304
0.5595588235294118	0.7244565217391304
0.5595588235294118	0.7248188405797101
0.5600490196078431	0.7248188405797101
0.5600490196078431	0.725
0.5607843137254902	0.725
0.5607843137254902	0.7251811594202898
0.5615196078431373	0.7251811594202898
0.5615196078431373	0.7253623188405797
0.5625	0.7253623188405797
0.5625	0.7255434782608695
0.5632352941176471	0.7255434782608695
0.5632352941176471	0.7257246376811595
0.5642156862745098	0.7257246376811595
0.5642156862745098	0.7260869565217392
0.5647058823529412	0.7260869565217392
0.5647058823529412	0.726268115942029
0.5649509803921569	0.726268115942029
0.5649509803921569	0.7266304347826087
0.5656862745098039	0.7266304347826087
0.5656862745098039	0.7275362318840579
0.5661764705882353	0.7275362318840579
0.5661764705882353	0.7277173913043479
0.566421568627451	0.7277173913043479
0.566421568627451	0.7280797101449276
0.5666666666666667	0.7280797101449276
0.5666666666666667	0.7286231884057971
0.567156862745098	0.7286231884057971
0.567156862745098	0.7288043478260869
0.5674019607843137	0.7288043478260869
0.5674019607843137	0.7291666666666666
0.5681372549019608	0.7291666666666666
0.5681372549019608	0.7298913043478261
0.5683823529411764	0.7298913043478261
0.5683823529411764	0.7302536231884058
0.5686274509803921	0.7302536231884058
0.5686274509803921	0.7304347826086957
0.5688725490196078	0.7304347826086957
0.5688725490196078	0.7307971014492753
0.5691176470588235	0.7307971014492753
0.5691176470588235	0.7309782608695652
0.5693627450980392	0.7309782608695652
0.5693627450980392	0.731159420289855
0.5698529411764706	0.731159420289855
0.5698529411764706	0.7313405797101449
0.5703431372549019	0.7313405797101449
0.5703431372549019	0.7315217391304348
0.5708333333333333	0.7315217391304348
0.5708333333333333	0.7317028985507247
0.5713235294117647	0.7317028985507247
0.5713235294117647	0.7324275362318841
0.5723039215686274	0.7324275362318841
0.5723039215686274	0.7326086956521739
0.5725490196078431	0.7326086956521739
0.5725490196078431	0.7331521739130434
0.5727941176470588	0.7331521739130434
0.5727941176470588	0.7340579710144928
0.5732843137254902	0.7340579710144928
0.5732843137254902	0.7342391304347826
0.5742647058823529	0.7342391304347826
0.5742647058823529	0.7347826086956522
0.5745098039215686	0.7347826086956522
0.5745098039215686	0.7356884057971015
0.5754901960784313	0.7356884057971015
0.5754901960784313	0.7358695652173913
0.575735294117647	0.7358695652173913
0.575735294117647	0.736231884057971
0.5759803921568627	0.736231884057971
0.5759803921568627	0.7365942028985507
0.5762254901960784	0.7365942028985507
0.5762254901960784	0.7371376811594202
0.5767156862745098	0.7371376811594202
0.5767156862745098	0.7375
0.5772058823529411	0.7375
0.5772058823529411	0.7380434782608696
0.5774509803921568	0.7380434782608696
0.5774509803921568	0.7382246376811594
0.5776960784313725	0.7382246376811594
0.5776960784313725	0.7384057971014493
0.5784313725490197	0.7384057971014493
0.5784313725490197	0.7385869565217391
0.5786764705882353	0.7385869565217391
0.5786764705882353	0.738768115942029
0.5794117647058824	0.738768115942029
0.5794117647058824	0.7391304347826086
0.5803921568627451	0.7391304347826086
0.5803921568627451	0.7394927536231884
0.5806372549019608	0.7394927536231884
0.5806372549019608	0.7396739130434783
0.5813725490196079	0.7396739130434783
0.5813725490196079	0.740036231884058
0.5823529411764706	0.740036231884058
0.5823529411764706	0.7402173913043478
0.5833333333333334	0.7402173913043478
0.5833333333333334	0.7405797101449275
0.5838235294117647	0.7405797101449275
0.5838235294117647	0.7409420289855072
0.5843137254901961	0.7409420289855072
0.5843137254901961	0.741304347826087
0.5845588235294118	0.741304347826087
0.5845588235294118	0.7418478260869565
0.5850490196078432	0.7418478260869565
0.5850490196078432	0.7420289855072464
0.5855392156862745	0.7420289855072464
0.5855392156862745	0.7427536231884058
0.5857843137254902	0.7427536231884058
0.5857843137254902	0.7432971014492754
0.5860294117647059	0.7432971014492754
0.5860294117647059	0.743840579710145
0.5865196078431373	0.743840579710145
0.5865196078431373	0.7442028985507246
0.5872549019607843	0.7442028985507246
0.5872549019607843	0.7447463768115942
0.5877450980392157	0.7447463768115942
0.5877450980392157	0.744927536231884
0.5879901960784314	0.744927536231884
0.5879901960784314	0.7451086956521739
0.5887254901960784	0.7451086956521739
0.5887254901960784	0.7452898550724638
0.5889705882352941	0.7452898550724638
0.5889705882352941	0.7456521739130435
0.5892156862745098	0.7456521739130435
0.5892156862745098	0.7460144927536232
0.5894607843137255	0.7460144927536232
0.5894607843137255	0.746195652173913
0.5897058823529412	0.746195652173913
0.5897058823529412	0.7465579710144927
0.5904411764705882	0.7465579710144927
0.5904411764705882	0.7471014492753624
0.5906862745098039	0.7471014492753624
0.5906862745098039	0.7476449275362319
0.5909313725490196	0.7476449275362319
0.5909313725490196	0.7480072463768116
0.5919117647058824	0.7480072463768116
0.5919117647058824	0.7481884057971014
0.592156862745098	0.7481884057971014
0.592156862745098	0.7483695652173913
0.5926470588235294	0.7483695652173913
0.5926470588235294	0.7490942028985508
0.5928921568627451	0.7490942028985508
0.5928921568627451	0.7496376811594203
0.5933823529411765	0.7496376811594203
0.5933823529411765	0.75
0.5936274509803922	0.75
0.5936274509803922	0.7505434782608695
0.5941176470588235	0.7505434782608695
0.5941176470588235	0.7507246376811594
0.595343137254902	0.7507246376811594
0.595343137254902	0.7510869565217392
0.5955882352941176	0.7510869565217392
0.5955882352941176	0.7514492753623189
0.5965686274509804	0.7514492753623189
0.5965686274509804	0.7516304347826087
0.5973039215686274	0.7516304347826087
0.5973039215686274	0.7521739130434782
0.5975490196078431	0.7521739130434782
0.5975490196078431	0.7528985507246376
0.5977941176470588	0.7528985507246376
0.5977941176470588	0.7530797101449276
0.5980392156862745	0.7530797101449276
0.5980392156862745	0.7532608695652174
0.5985294117647059	0.7532608695652174
0.5985294117647059	0.7534420289855073
0.5992647058823529	0.7534420289855073
0.5992647058823529	0.7539855072463768
0.6012254901960784	0.7539855072463768
0.6012254901960784	0.7541666666666667
0.6017156862745098	0.7541666666666667
0.6017156862745098	0.7543478260869565
0.6019607843137255	0.7543478260869565
0.6019607843137255	0.7545289855072463
0.6022058823529411	0.7545289855072463
0.6022058823529411	0.7547101449275362
0.6024509803921568	0.7547101449275362
0.6024509803921568	0.7548913043478261
0.6031862745098039	0.7548913043478261
0.6031862745098039	0.755072463768116
0.6034313725490196	0.755072463768116
0.6034313725490196	0.7556159420289855
0.6049019607843137	0.7556159420289855
0.6049019607843137	0.7565217391304347
0.6061274509803921	0.7565217391304347
0.6061274509803921	0.7568840579710145
0.6063725490196078	0.7568840579710145
0.6063725490196078	0.7577898550724638
0.6071078431372549	0.7577898550724638
0.6071078431372549	0.7579710144927536
0.6078431372549019	0.7579710144927536
0.6078431372549019	0.7581521739130435
0.608578431372549	0.7581521739130435
0.608578431372549	0.758695652173913
0.6095588235294118	0.758695652173913
0.6095588235294118	0.758876811594203
0.6098039215686275	0.758876811594203
0.6098039215686275	0.7590579710144928
0.6102941176470589	0.7590579710144928
0.6102941176470589	0.7592391304347826
0.6105392156862746	0.7592391304347826
0.6105392156862746	0.7596014492753623
0.6122549019607844	0.7596014492753623
0.6122549019607844	0.7597826086956522
0.6125	0.7597826086956522
0.6125	0.7606884057971014
0.6129901960784314	0.7606884057971014
0.6129901960784314	0.7608695652173914
0.6137254901960785	0.7608695652173914
0.6137254901960785	0.7610507246376812
0.6142156862745098	0.7610507246376812
0.6142156862745098	0.761231884057971
0.6144607843137255	0.761231884057971
0.6144607843137255	0.7615942028985507
0.6147058823529412	0.7615942028985507
0.6147058823529412	0.7619565217391304
0.6149509803921569	0.7619565217391304
0.6149509803921569	0.7621376811594203
0.6154411764705883	0.7621376811594203
0.6154411764705883	0.7626811594202898
0.6166666666666667	0.7626811594202898
0.6166666666666667	0.7628623188405798
0.6169117647058824	0.7628623188405798
0.6169117647058824	0.7632246376811594
0.6171568627450981	0.7632246376811594
0.6171568627450981	0.7634057971014493
0.6181372549019608	0.7634057971014493
0.6181372549019608	0.7635869565217391
0.6186274509803922	0.7635869565217391
0.6186274509803922	0.7639492753623188
0.6200980392156863	0.7639492753623188
0.6200980392156863	0.7646739130434783
0.620343137254902	0.7646739130434783
0.620343137254902	0.765036231884058
0.621078431372549	0.765036231884058
0.621078431372549	0.7653985507246377
0.6213235294117647	0.7653985507246377
0.6213235294117647	0.7666666666666667
0.6220588235294118	0.7666666666666667
0.6220588235294118	0.7673913043478261
0.6223039215686275	0.7673913043478261
0.6223039215686275	0.7677536231884058
0.6232843137254902	0.7677536231884058
0.6232843137254902	0.7679347826086956
0.6235294117647059	0.7679347826086956
0.6235294117647059	0.7681159420289855
0.6237745098039216	0.7681159420289855
0.6237745098039216	0.7682971014492753
0.6240196078431373	0.7682971014492753
0.6240196078431373	0.7684782608695652
0.6242647058823529	0.7684782608695652
0.6242647058823529	0.7686594202898551
0.6247549019607843	0.7686594202898551
0.6247549019607843	0.7697463768115942
0.625	0.7697463768115942
0.625	0.769927536231884
0.6252450980392157	0.769927536231884
0.6252450980392157	0.7708333333333334
0.6257352941176471	0.7708333333333334
0.6257352941176471	0.7710144927536232
0.6259803921568627	0.7710144927536232
0.6259803921568627	0.7713768115942029
0.6264705882352941	0.7713768115942029
0.6264705882352941	0.7715579710144927
0.6276960784313725	0.7715579710144927
0.6276960784313725	0.7717391304347826
0.6281862745098039	0.7717391304347826
0.6281862745098039	0.7721014492753623
0.6286764705882353	0.7721014492753623
0.6286764705882353	0.7733695652173913
0.628921568627451	0.7733695652173913
0.628921568627451	0.7735507246376812
0.6294117647058823	0.7735507246376812
0.6294117647058823	0.7739130434782608
0.629656862745098	0.7739130434782608
0.629656862745098	0.7740942028985507
0.6299019607843137	0.7740942028985507
0.6299019607843137	0.7746376811594203
0.6303921568627451	0.7746376811594203
0.6303921568627451	0.7751811594202899
0.6311274509803921	0.7751811594202899
0.6311274509803921	0.7753623188405797
0.6313725490196078	0.7753623188405797
0.6313725490196078	0.7755434782608696
0.6318627450980392	0.7755434782608696
0.6318627450980392	0.7760869565217391
0.6325980392156862	0.7760869565217391
0.6325980392156862	0.7766304347826087
0.6328431372549019	0.7766304347826087
0.6328431372549019	0.7771739130434783
0.6330882352941176	0.7771739130434783
0.6330882352941176	0.7773550724637681
0.6333333333333333	0.7773550724637681
0.6333333333333333	0.7777173913043478
0.6338235294117647	0.7777173913043478
0.6338235294117647	0.7778985507246376
0.634313725490196	0.7778985507246376
0.634313725490196	0.7786231884057971
0.6348039215686274	0.7786231884057971
0.6348039215686274	0.7791666666666667
0.6352941176470588	0.7791666666666667
0.6352941176470588	0.7795289855072464
0.6357843137254902	0.7795289855072464
0.6357843137254902	0.7800724637681159
0.6360294117647058	0.7800724637681159
0.6360294117647058	0.7802536231884057
0.6367647058823529	0.7802536231884057
0.6367647058823529	0.7807971014492754
0.6392156862745098	0.7807971014492754
0.6392156862745098	0.7809782608695652
0.6397058823529411	0.7809782608695652
0.6397058823529411	0.7811594202898551
0.6399509803921568	0.7811594202898551
0.6399509803921568	0.7813405797101449
0.6404411764705882	0.7813405797101449
0.6404411764705882	0.7815217391304348
0.640686274509804	0.7815217391304348
0.640686274509804	0.7817028985507246
0.6409313725490197	0.7817028985507246
0.6409313725490197	0.7818840579710145
0.6416666666666667	0.7818840579710145
0.6416666666666667	0.7824275362318841
0.6419117647058824	0.7824275362318841
0.6419117647058824	0.7829710144927536
0.6428921568627451	0.7829710144927536
0.6428921568627451	0.7833333333333333
0.6431372549019608	0.7833333333333333
0.6431372549019608	0.7840579710144927
0.6436274509803922	0.7840579710144927
0.6436274509803922	0.7844202898550725
0.6441176470588236	0.7844202898550725
0.6441176470588236	0.7847826086956522
0.6443627450980393	0.7847826086956522
0.6443627450980393	0.7851449275362319
0.6446078431372549	0.7851449275362319
0.6446078431372549	0.7853260869565217
0.6448529411764706	0.7853260869565217
0.6448529411764706	0.7860507246376811
0.6450980392156863	0.7860507246376811
0.6450980392156863	0.7864130434782609
0.645343137254902	0.7864130434782609
0.645343137254902	0.7867753623188406
0.6463235294117647	0.7867753623188406
0.6463235294117647	0.7871376811594203
0.6465686274509804	0.7871376811594203
0.6465686274509804	0.7873188405797101
0.6470588235294118	0.7873188405797101
0.6470588235294118	0.7875
0.6473039215686275	0.7875
0.6473039215686275	0.7876811594202898
0.6475490196078432	0.7876811594202898
0.6475490196078432	0.7885869565217392
0.6480392156862745	0.7885869565217392
0.6480392156862745	0.7893115942028985
0.6482843137254902	0.7893115942028985
0.6482843137254902	0.7896739130434782
0.6485294117647059	0.7896739130434782
0.6485294117647059	0.7905797101449276
0.649264705882353	0.7905797101449276
0.649264705882353	0.7914855072463768
0.6497549019607843	0.7914855072463768
0.6497549019607843	0.7916666666666666
0.6502450980392157	0.7916666666666666
0.6502450980392157	0.7920289855072464
0.6504901960784314	0.7920289855072464
0.6504901960784314	0.7922101449275363
0.6507352941176471	0.7922101449275363
0.6507352941176471	0.7931159420289855
0.6514705882352941	0.7931159420289855
0.6514705882352941	0.7932971014492753
0.6522058823529412	0.7932971014492753
0.6522058823529412	0.7934782608695652
0.6524509803921569	0.7934782608695652
0.6524509803921569	0.7940217391304348
0.6529411764705882	0.7940217391304348
0.6529411764705882	0.7942028985507247
0.6536764705882353	0.7942028985507247
0.6536764705882353	0.7943840579710145
0.6541666666666667	0.7943840579710145
0.6541666666666667	0.7949275362318841
0.6544117647058824	0.7949275362318841
0.6544117647058824	0.7958333333333333
0.6549019607843137	0.7958333333333333
0.6549019607843137	0.7960144927536232
0.6553921568627451	0.7960144927536232
0.6553921568627451	0.7963768115942029
0.6556372549019608	0.7963768115942029
0.6556372549019608	0.7965579710144928
0.6558823529411765	0.7965579710144928
0.6558823529411765	0.7967391304347826
0.6561274509803922	0.7967391304347826
0.6561274509803922	0.7971014492753623
0.6563725490196078	0.7971014492753623
0.6563725490196078	0.7972826086956522
0.6566176470588235	0.7972826086956522
0.6566176470588235	0.7976449275362318
0.6571078431372549	0.7976449275362318
0.6571078431372549	0.7983695652173913
0.6580882352941176	0.7983695652173913
0.6580882352941176	0.7992753623188406
0.658578431372549	0.7992753623188406
0.658578431372549	0.7996376811594202
0.6590686274509804	0.7996376811594202
0.6590686274509804	0.7998188405797102
0.6595588235294118	0.7998188405797102
0.6595588235294118	0.8
0.6600490196078431	0.8
0.6600490196078431	0.8005434782608696
0.6602941176470588	0.8005434782608696
0.6602941176470588	0.8007246376811594
0.6605392156862745	0.8007246376811594
0.6605392156862745	0.8009057971014493
0.6612745098039216	0.8009057971014493
0.6612745098039216	0.801268115942029
0.6615196078431372	0.801268115942029
0.6615196078431372	0.8014492753623188
0.6622549019607843	0.8014492753623188
0.6622549019607843	0.8019927536231884
0.6625	0.8019927536231884
0.6625	0.8021739130434783
0.6627450980392157	0.8021739130434783
0.6627450980392157	0.8034420289855072
0.663235294117647	0.8034420289855072
0.663235294117647	0.8039855072463769
0.6642156862745098	0.8039855072463769
0.6642156862745098	0.8043478260869565
0.6644607843137255	0.8043478260869565
0.6644607843137255	0.8050724637681159
0.6647058823529411	0.8050724637681159
0.6647058823529411	0.8054347826086956
0.6651960784313725	0.8054347826086956
0.6651960784313725	0.8057971014492754
0.6656862745098039	0.8057971014492754
0.6656862745098039	0.8061594202898551
0.6664215686274509	0.8061594202898551
0.6664215686274509	0.8065217391304348
0.6666666666666666	0.8065217391304348
0.6666666666666666	0.8070652173913043
0.6669117647058823	0.8070652173913043
0.6669117647058823	0.8072463768115942
0.6676470588235294	0.8072463768115942
0.6676470588235294	0.807427536231884
0.6678921568627451	0.807427536231884
0.6678921568627451	0.8076086956521739
0.6681372549019607	0.8076086956521739
0.6681372549019607	0.8094202898550724
0.6683823529411764	0.8094202898550724
0.6683823529411764	0.8096014492753624
0.6691176470588235	0.8096014492753624
0.6691176470588235	0.8097826086956522
0.6693627450980392	0.8097826086956522
0.6693627450980392	0.8105072463768116
0.6698529411764705	0.8105072463768116
0.6698529411764705	0.8106884057971014
0.6700980392156862	0.8106884057971014
0.6700980392156862	0.8108695652173913
0.6703431372549019	0.8108695652173913
0.6703431372549019	0.8110507246376811
0.6708333333333333	0.8110507246376811
0.6708333333333333	0.8114130434782608
0.6713235294117647	0.8114130434782608
0.6713235294117647	0.8121376811594203
0.6715686274509803	0.8121376811594203
0.6715686274509803	0.8126811594202898
0.671813725490196	0.8126811594202898
0.671813725490196	0.8130434782608695
0.6720588235294118	0.8130434782608695
0.6720588235294118	0.8135869565217392
0.6723039215686275	0.8135869565217392
0.6723039215686275	0.8141304347826087
0.6727941176470589	0.8141304347826087
0.6727941176470589	0.8144927536231884
0.6730392156862746	0.8144927536231884
0.6730392156862746	0.8164855072463768
0.6732843137254902	0.8164855072463768
0.6732843137254902	0.8166666666666667
0.6735294117647059	0.8166666666666667
0.6735294117647059	0.8170289855072463
0.6737745098039216	0.8170289855072463
0.6737745098039216	0.8179347826086957
0.6740196078431373	0.8179347826086957
0.6740196078431373	0.8182971014492754
0.674264705882353	0.8182971014492754
0.674264705882353	0.8184782608695652
0.6745098039215687	0.8184782608695652
0.6745098039215687	0.8192028985507246
0.6747549019607844	0.8192028985507246
0.6747549019607844	0.8195652173913044
0.675	0.8195652173913044
0.675	0.8199275362318841
0.6752450980392157	0.8199275362318841
0.6752450980392157	0.8204710144927536
0.6762254901960785	0.8204710144927536
0.6762254901960785	0.8206521739130435
0.6767156862745098	0.8206521739130435
0.6767156862745098	0.8208333333333333
0.6774509803921569	0.8208333333333333
0.6774509803921569	0.821376811594203
0.6779411764705883	0.821376811594203
0.6779411764705883	0.8221014492753623
0.6791666666666667	0.8221014492753623
0.6791666666666667	0.8226449275362319
0.6794117647058824	0.8226449275362319
0.6794117647058824	0.8233695652173914
0.6799019607843138	0.8233695652173914
0.6799019607843138	0.8235507246376812
0.6801470588235294	0.8235507246376812
0.6801470588235294	0.823731884057971
0.6806372549019608	0.823731884057971
0.6806372549019608	0.8244565217391304
0.6813725490196079	0.8244565217391304
0.6813725490196079	0.8246376811594203
0.6818627450980392	0.8246376811594203
0.6818627450980392	0.8248188405797101
0.6823529411764706	0.8248188405797101
0.6823529411764706	0.8253623188405798
0.6825980392156863	0.8253623188405798
0.6825980392156863	0.8255434782608696
0.682843137254902	0.8255434782608696
0.682843137254902	0.8259057971014493
0.6833333333333333	0.8259057971014493
0.6833333333333333	0.8264492753623188
0.683578431372549	0.8264492753623188
0.683578431372549	0.8269927536231884
0.6840686274509804	0.8269927536231884
0.6840686274509804	0.8273550724637682
0.6845588235294118	0.8273550724637682
0.6845588235294118	0.8278985507246377
0.6848039215686275	0.8278985507246377
0.6848039215686275	0.8280797101449275
0.6852941176470588	0.8280797101449275
0.6852941176470588	0.8284420289855072
0.6855392156862745	0.8284420289855072
0.6855392156862745	0.8289855072463768
0.6860294117647059	0.8289855072463768
0.6860294117647059	0.8293478260869566
0.6862745098039216	0.8293478260869566
0.6862745098039216	0.8300724637681159
0.6867647058823529	0.8300724637681159
0.6867647058823529	0.8307971014492753
0.6872549019607843	0.8307971014492753
0.6872549019607843	0.8309782608695652
0.6879901960784314	0.8309782608695652
0.6879901960784314	0.8322463768115942
0.6882352941176471	0.8322463768115942
0.6882352941176471	0.832427536231884
0.6884803921568627	0.832427536231884
0.6884803921568627	0.8326086956521739
0.6894607843137255	0.8326086956521739
0.6894607843137255	0.8329710144927536
0.6897058823529412	0.8329710144927536
0.6897058823529412	0.8333333333333334
0.6899509803921569	0.8333333333333334
0.6899509803921569	0.8340579710144927
0.6901960784313725	0.8340579710144927
0.6901960784313725	0.8344202898550724
0.6904411764705882	0.8344202898550724
0.6904411764705882	0.8347826086956521
0.6906862745098039	0.8347826086956521
0.6906862745098039	0.8353260869565218
0.6909313725490196	0.8353260869565218
0.6909313725490196	0.8355072463768116
0.6911764705882353	0.8355072463768116
0.6911764705882353	0.8360507246376812
0.6916666666666667	0.8360507246376812
0.6916666666666667	0.8376811594202899
0.692156862745098	0.8376811594202899
0.692156862745098	0.8378623188405797
0.6924019607843137	0.8378623188405797
0.6924019607843137	0.8382246376811594
0.6926470588235294	0.8382246376811594
0.6926470588235294	0.8385869565217391
0.6928921568627451	0.8385869565217391
0.6928921568627451	0.8387681159420289
0.6931372549019608	0.8387681159420289
0.6931372549019608	0.8389492753623189
0.6936274509803921	0.8389492753623189
0.6936274509803921	0.8393115942028986
0.6938725490196078	0.8393115942028986
0.6938725490196078	0.8396739130434783
0.6943627450980392	0.8396739130434783
0.6943627450980392	0.840036231884058
0.6946078431372549	0.840036231884058
0.6946078431372549	0.8403985507246376
0.6948529411764706	0.8403985507246376
0.6948529411764706	0.8405797101449275
0.6950980392156862	0.8405797101449275
0.6950980392156862	0.8409420289855073
0.6958333333333333	0.8409420289855073
0.6958333333333333	0.841304347826087
0.6963235294117647	0.841304347826087
0.6963235294117647	0.8416666666666667
0.6970588235294117	0.8416666666666667
0.6970588235294117	0.842391304347826
0.6977941176470588	0.842391304347826
0.6977941176470588	0.8427536231884057
0.6985294117647058	0.8427536231884057
0.6985294117647058	0.8431159420289855
0.6987745098039215	0.8431159420289855
0.6987745098039215	0.8434782608695652
0.6992647058823529	0.8434782608695652
0.6992647058823529	0.8458333333333333
0.6995098039215686	0.8458333333333333
0.6995098039215686	0.8465579710144927
0.700735294117647	0.8465579710144927
0.700735294117647	0.8469202898550725
0.7009803921568627	0.8469202898550725
0.7009803921568627	0.8472826086956522
0.7012254901960784	0.8472826086956522
0.7012254901960784	0.8480072463768116
0.7019607843137254	0.8480072463768116
0.7019607843137254	0.8481884057971014
0.7022058823529411	0.8481884057971014
0.7022058823529411	0.8483695652173913
0.7024509803921568	0.8483695652173913
0.7024509803921568	0.8487318840579711
0.7029411764705882	0.8487318840579711
0.7029411764705882	0.8494565217391304
0.7036764705882353	0.8494565217391304
0.7036764705882353	0.851268115942029
0.703921568627451	0.851268115942029
0.703921568627451	0.8518115942028985
0.7041666666666667	0.8518115942028985
0.7041666666666667	0.8523550724637681
0.7046568627450981	0.8523550724637681
0.7046568627450981	0.8541666666666666
0.7049019607843138	0.8541666666666666
0.7049019607843138	0.8547101449275363
0.7051470588235295	0.8547101449275363
0.7051470588235295	0.8556159420289855
0.7053921568627451	0.8556159420289855
0.7053921568627451	0.8559782608695652
0.7056372549019608	0.8559782608695652
0.7056372549019608	0.856159420289855
0.7058823529411765	0.856159420289855
0.7058823529411765	0.8563405797101449
0.7066176470588236	0.8563405797101449
0.7066176470588236	0.8565217391304348
0.7071078431372549	0.8565217391304348
0.7071078431372549	0.8574275362318841
0.7073529411764706	0.8574275362318841
0.7073529411764706	0.8581521739130434
0.7075980392156863	0.8581521739130434
0.7075980392156863	0.8586956521739131
0.707843137254902	0.8586956521739131
0.707843137254902	0.8588768115942029
0.7080882352941177	0.8588768115942029
0.7080882352941177	0.8592391304347826
0.7083333333333334	0.8592391304347826
0.7083333333333334	0.8603260869565217
0.7088235294117647	0.8603260869565217
0.7088235294117647	0.8608695652173913
0.7095588235294118	0.8608695652173913
0.7095588235294118	0.8614130434782609
0.7100490196078432	0.8614130434782609
0.7100490196078432	0.8619565217391304
0.7102941176470589	0.8619565217391304
0.7102941176470589	0.8630434782608696
0.7110294117647059	0.8630434782608696
0.7110294117647059	0.8635869565217391
0.7125	0.8635869565217391
0.7125	0.8639492753623188
0.7129901960784314	0.8639492753623188
0.7129901960784314	0.8643115942028986
0.7132352941176471	0.8643115942028986
0.7132352941176471	0.8652173913043478
0.7134803921568628	0.8652173913043478
0.7134803921568628	0.8653985507246377
0.7137254901960784	0.8653985507246377
0.7137254901960784	0.8659420289855072
0.7139705882352941	0.8659420289855072
0.7139705882352941	0.866304347826087
0.7144607843137255	0.866304347826087
0.7144607843137255	0.8666666666666667
0.7147058823529412	0.8666666666666667
0.7147058823529412	0.8670289855072464
0.7149509803921569	0.8670289855072464
0.7149509803921569	0.8681159420289855
0.7159313725490196	0.8681159420289855
0.7159313725490196	0.8686594202898551
0.7161764705882353	0.8686594202898551
0.7161764705882353	0.8692028985507246
0.716421568627451	0.8692028985507246
0.716421568627451	0.8697463768115942
0.7166666666666667	0.8697463768115942
0.7166666666666667	0.8702898550724638
0.717156862745098	0.8702898550724638
0.717156862745098	0.871195652173913
0.7174019607843137	0.871195652173913
0.7174019607843137	0.8715579710144927
0.7183823529411765	0.8715579710144927
0.7183823529411765	0.8722826086956522
0.7186274509803922	0.8722826086956522
0.7186274509803922	0.8730072463768116
0.7188725490196078	0.8730072463768116
0.7188725490196078	0.8731884057971014
0.7191176470588235	0.8731884057971014
0.7191176470588235	0.8733695652173913
0.7196078431372549	0.8733695652173913
0.7196078431372549	0.8735507246376811
0.7200980392156863	0.8735507246376811
0.7200980392156863	0.873731884057971
0.720343137254902	0.873731884057971
0.720343137254902	0.8740942028985508
0.7205882352941176	0.8740942028985508
0.7205882352941176	0.8742753623188406
0.7208333333333333	0.8742753623188406
0.7208333333333333	0.8744565217391305
0.7215686274509804	0.8744565217391305
0.7215686274509804	0.8753623188405797
0.7218137254901961	0.8753623188405797
0.7218137254901961	0.8759057971014492
0.7225490196078431	0.8759057971014492
0.7225490196078431	0.876268115942029
0.7235294117647059	0.876268115942029
0.7235294117647059	0.8764492753623189
0.7237745098039216	0.8764492753623189
0.7237745098039216	0.8773550724637681
0.7240196078431372	0.8773550724637681
0.7240196078431372	0.8775362318840579
0.7245098039215686	0.8775362318840579
0.7245098039215686	0.8777173913043478
0.725	0.8777173913043478
0.725	0.8778985507246376
0.725735294117647	0.8778985507246376
0.725735294117647	0.8780797101449276
0.7259803921568627	0.8780797101449276
0.7259803921568627	0.8784420289855073
0.7264705882352941	0.8784420289855073
0.7264705882352941	0.878804347826087
0.7272058823529411	0.878804347826087
0.7272058823529411	0.8789855072463768
0.7274509803921568	0.8789855072463768
0.7274509803921568	0.8797101449275362
0.7276960784313725	0.8797101449275362
0.7276960784313725	0.8802536231884058
0.7279411764705882	0.8802536231884058
0.7279411764705882	0.8804347826086957
0.7281862745098039	0.8804347826086957
0.7281862745098039	0.881159420289855
0.7284313725490196	0.881159420289855
0.7284313725490196	0.8813405797101449
0.7286764705882353	0.8813405797101449
0.7286764705882353	0.8818840579710145
0.7289215686274509	0.8818840579710145
0.7289215686274509	0.8820652173913044
0.729656862745098	0.8820652173913044
0.729656862745098	0.8851449275362319
0.7299019607843137	0.8851449275362319
0.7299019607843137	0.8855072463768116
0.7303921568627451	0.8855072463768116
0.7303921568627451	0.8871376811594203
0.7316176470588235	0.8871376811594203
0.7316176470588235	0.8878623188405798
0.7318627450980392	0.8878623188405798
0.7318627450980392	0.8880434782608696
0.7321078431372549	0.8880434782608696
0.7321078431372549	0.8889492753623188
0.7330882352941176	0.8889492753623188
0.7330882352941176	0.8891304347826087
0.733578431372549	0.8891304347826087
0.733578431372549	0.8894927536231884
0.7338235294117647	0.8894927536231884
0.7338235294117647	0.8909420289855072
0.7340686274509803	0.8909420289855072
0.7340686274509803	0.8913043478260869
0.734313725490196	0.8913043478260869
0.734313725490196	0.8916666666666667
0.7345588235294118	0.8916666666666667
0.7345588235294118	0.8923913043478261
0.7348039215686275	0.8923913043478261
0.7348039215686275	0.8931159420289855
0.7355392156862746	0.8931159420289855
0.7355392156862746	0.8936594202898551
0.7357843137254902	0.8936594202898551
0.7357843137254902	0.8940217391304348
0.7362745098039216	0.8940217391304348
0.7362745098039216	0.8942028985507247
0.7365196078431373	0.8942028985507247
0.7365196078431373	0.8947463768115942
0.736764705882353	0.8947463768115942
0.736764705882353	0.8958333333333334
0.7375	0.8958333333333334
0.7375	0.8961956521739131
0.7382352941176471	0.8961956521739131
0.7382352941176471	0.8969202898550724
0.7384803921568628	0.8969202898550724
0.7384803921568628	0.8978260869565218
0.7389705882352942	0.8978260869565218
0.7389705882352942	0.8980072463768116
0.7392156862745098	0.8980072463768116
0.7392156862745098	0.8983695652173913
0.7397058823529412	0.8983695652173913
0.7397058823529412	0.8992753623188405
0.7399509803921569	0.8992753623188405
0.7399509803921569	0.8996376811594203
0.7401960784313726	0.8996376811594203
0.7401960784313726	0.8998188405797102
0.7404411764705883	0.8998188405797102
0.7404411764705883	0.9003623188405797
0.740686274509804	0.9003623188405797
0.740686274509804	0.9005434782608696
0.7409313725490196	0.9005434782608696
0.7409313725490196	0.9009057971014492
0.741421568627451	0.9009057971014492
0.741421568627451	0.9014492753623189
0.7416666666666667	0.9014492753623189
0.7416666666666667	0.9018115942028986
0.7419117647058824	0.9018115942028986
0.7419117647058824	0.9023550724637681
0.7424019607843138	0.9023550724637681
0.7424019607843138	0.902536231884058
0.7426470588235294	0.902536231884058
0.7426470588235294	0.9032608695652173
0.7428921568627451	0.9032608695652173
0.7428921568627451	0.903804347826087
0.7433823529411765	0.903804347826087
0.7433823529411765	0.9043478260869565
0.7436274509803922	0.9043478260869565
0.7436274509803922	0.9047101449275362
0.7438725490196079	0.9047101449275362
0.7438725490196079	0.9050724637681159
0.7441176470588236	0.9050724637681159
0.7441176470588236	0.9054347826086957
0.7450980392156863	0.9054347826086957
0.7450980392156863	0.9056159420289855
0.745343137254902	0.9056159420289855
0.745343137254902	0.9061594202898551
0.7458333333333333	0.9061594202898551
0.7458333333333333	0.9063405797101449
0.7468137254901961	0.9063405797101449
0.7468137254901961	0.9067028985507246
0.7470588235294118	0.9067028985507246
0.7470588235294118	0.9068840579710145
0.7473039215686275	0.9068840579710145
0.7473039215686275	0.9074275362318841
0.7475490196078431	0.9074275362318841
0.7475490196078431	0.9077898550724638
0.7495098039215686	0.9077898550724638
0.7495098039215686	0.9083333333333333
0.7497549019607843	0.9083333333333333
0.7497549019607843	0.9085144927536232
0.75	0.9085144927536232
0.75	0.908695652173913
0.7502450980392157	0.908695652173913
0.7502450980392157	0.9088768115942029
0.7512254901960784	0.9088768115942029
0.7512254901960784	0.9096014492753624
0.7519607843137255	0.9096014492753624
0.7519607843137255	0.909963768115942
0.7526960784313725	0.909963768115942
0.7526960784313725	0.9103260869565217
0.7529411764705882	0.9103260869565217
0.7529411764705882	0.9105072463768116
0.7541666666666667	0.9105072463768116
0.7541666666666667	0.9106884057971014
0.754656862745098	0.9106884057971014
0.754656862745098	0.9110507246376811
0.7549019607843137	0.9110507246376811
0.7549019607843137	0.9112318840579711
0.7553921568627451	0.9112318840579711
0.7553921568627451	0.9114130434782609
0.7561274509803921	0.9114130434782609
0.7561274509803921	0.9115942028985508
0.7568627450980392	0.9115942028985508
0.7568627450980392	0.9117753623188406
0.7578431372549019	0.9117753623188406
0.7578431372549019	0.9119565217391304
0.7580882352941176	0.9119565217391304
0.7580882352941176	0.9121376811594203
0.758578431372549	0.9121376811594203
0.758578431372549	0.9123188405797101
0.7588235294117647	0.9123188405797101
0.7588235294117647	0.9125
0.7595588235294117	0.9125
0.7595588235294117	0.9132246376811595
0.7598039215686274	0.9132246376811595
0.7598039215686274	0.9134057971014493
0.7600490196078431	0.9134057971014493
0.7600490196078431	0.9143115942028985
0.7605392156862745	0.9143115942028985
0.7605392156862745	0.9144927536231884
0.7615196078431372	0.9144927536231884
0.7615196078431372	0.9148550724637681
0.7617647058823529	0.9148550724637681
0.7617647058823529	0.9153985507246377
0.7620098039215686	0.9153985507246377
0.7620098039215686	0.9163043478260869
0.7622549019607843	0.9163043478260869
0.7622549019607843	0.9164855072463768
0.7625	0.9164855072463768
0.7625	0.9166666666666666
0.7629901960784313	0.9166666666666666
0.7629901960784313	0.9168478260869565
0.7642156862745098	0.9168478260869565
0.7642156862745098	0.9170289855072464
0.7647058823529411	0.9170289855072464
0.7647058823529411	0.9173913043478261
0.7649509803921568	0.9173913043478261
0.7649509803921568	0.9179347826086957
0.765686274509804	0.9179347826086957
0.765686274509804	0.9181159420289855
0.7666666666666667	0.9181159420289855
0.7666666666666667	0.9184782608695652
0.7671568627450981	0.9184782608695652
0.7671568627450981	0.918659420289855
0.7676470588235295	0.918659420289855
0.7676470588235295	0.9190217391304348
0.7683823529411765	0.9190217391304348
0.7683823529411765	0.9192028985507247
0.7686274509803922	0.9192028985507247
0.7686274509803922	0.9197463768115942
0.7698529411764706	0.9197463768115942
0.7698529411764706	0.9199275362318841
0.7705882352941177	0.9199275362318841
0.7705882352941177	0.9201086956521739
0.7720588235294118	0.9201086956521739
0.7720588235294118	0.9206521739130434
0.7725490196078432	0.9206521739130434
0.7725490196078432	0.9210144927536232
0.7730392156862745	0.9210144927536232
0.7730392156862745	0.9211956521739131
0.7732843137254902	0.9211956521739131
0.7732843137254902	0.9215579710144928
0.7740196078431373	0.9215579710144928
0.7740196078431373	0.9219202898550725
0.7745098039215687	0.9219202898550725
0.7745098039215687	0.9221014492753623
0.7752450980392157	0.9221014492753623
0.7752450980392157	0.9222826086956522
0.7754901960784314	0.9222826086956522
0.7754901960784314	0.9228260869565217
0.7759803921568628	0.9228260869565217
0.7759803921568628	0.9230072463768116
0.7769607843137255	0.9230072463768116
0.7769607843137255	0.9231884057971015
0.7779411764705882	0.9231884057971015
0.7779411764705882	0.923731884057971
0.7781862745098039	0.923731884057971
0.7781862745098039	0.9240942028985507
0.7784313725490196	0.9240942028985507
0.7784313725490196	0.9242753623188406
0.778921568627451	0.9242753623188406
0.778921568627451	0.9244565217391304
0.7791666666666667	0.9244565217391304
0.7791666666666667	0.9246376811594202
0.7794117647058824	0.9246376811594202
0.7794117647058824	0.9248188405797102
0.779656862745098	0.9248188405797102
0.779656862745098	0.9251811594202899
0.7801470588235294	0.9251811594202899
0.7801470588235294	0.9253623188405797
0.7803921568627451	0.9253623188405797
0.7803921568627451	0.9255434782608696
0.7821078431372549	0.9255434782608696
0.7821078431372549	0.9259057971014493
0.7823529411764706	0.9259057971014493
0.7823529411764706	0.9260869565217391
0.7825980392156863	0.9260869565217391
0.7825980392156863	0.9266304347826086
0.782843137254902	0.9266304347826086
0.782843137254902	0.9268115942028986
0.7833333333333333	0.9268115942028986
0.7833333333333333	0.9273550724637681
0.783578431372549	0.9273550724637681
0.783578431372549	0.927536231884058
0.7838235294117647	0.927536231884058
0.7838235294117647	0.9277173913043478
0.7843137254901961	0.9277173913043478
0.7843137254901961	0.9278985507246377
0.7845588235294118	0.9278985507246377
0.7845588235294118	0.9280797101449275
0.7848039215686274	0.9280797101449275
0.7848039215686274	0.928623188405797
0.7852941176470588	0.928623188405797
0.7852941176470588	0.928804347826087
0.7862745098039216	0.928804347826087
0.7862745098039216	0.9289855072463769
0.7867647058823529	0.9289855072463769
0.7867647058823529	0.9295289855072464
0.7870098039215686	0.9295289855072464
0.7870098039215686	0.9297101449275362
0.7872549019607843	0.9297101449275362
0.7872549019607843	0.9300724637681159
0.7875	0.9300724637681159
0.7875	0.9302536231884058
0.7877450980392157	0.9302536231884058
0.7877450980392157	0.9304347826086956
0.7879901960784313	0.9304347826086956
0.7879901960784313	0.9306159420289855
0.788235294117647	0.9306159420289855
0.788235294117647	0.9309782608695653
0.7884803921568627	0.9309782608695653
0.7884803921568627	0.9311594202898551
0.7887254901960784	0.9311594202898551
0.7887254901960784	0.9315217391304348
0.7894607843137255	0.9315217391304348
0.7894607843137255	0.9320652173913043
0.7901960784313725	0.9320652173913043
0.7901960784313725	0.9326086956521739
0.7904411764705882	0.9326086956521739
0.7904411764705882	0.9327898550724638
0.7906862745098039	0.9327898550724638
0.7906862745098039	0.9329710144927537
0.7909313725490196	0.9329710144927537
0.7909313725490196	0.9331521739130435
0.7911764705882353	0.9331521739130435
0.7911764705882353	0.9335144927536232
0.7924019607843137	0.9335144927536232
0.7924019607843137	0.9340579710144927
0.7926470588235294	0.9340579710144927
0.7926470588235294	0.9344202898550724
0.7936274509803921	0.9344202898550724
0.7936274509803921	0.9346014492753624
0.7946078431372549	0.9346014492753624
0.7946078431372549	0.9347826086956522
0.796813725490196	0.9347826086956522
0.796813725490196	0.9349637681159421
0.7973039215686275	0.9349637681159421
0.7973039215686275	0.9351449275362319
0.7977941176470589	0.9351449275362319
0.7977941176470589	0.9353260869565218
0.7980392156862746	0.9353260869565218
0.7980392156862746	0.9355072463768116
0.7987745098039216	0.9355072463768116
0.7987745098039216	0.9356884057971014
0.7990196078431373	0.9356884057971014
0.7990196078431373	0.9358695652173913
0.7997549019607844	0.9358695652173913
0.7997549019607844	0.936231884057971
0.8007352941176471	0.936231884057971
0.8007352941176471	0.9364130434782608
0.8009803921568628	0.9364130434782608
0.8009803921568628	0.9365942028985508
0.8014705882352942	0.9365942028985508
0.8014705882352942	0.9367753623188406
0.8019607843137255	0.9367753623188406
0.8019607843137255	0.9373188405797102
0.8022058823529412	0.9373188405797102
0.8022058823529412	0.9375
0.8024509803921569	0.9375
0.8024509803921569	0.9376811594202898
0.8029411764705883	0.9376811594202898
0.8029411764705883	0.9378623188405797
0.803186274509804	0.9378623188405797
0.803186274509804	0.9385869565217392
0.8041666666666667	0.9385869565217392
0.8041666666666667	0.938768115942029
0.8046568627450981	0.938768115942029
0.8046568627450981	0.9389492753623189
0.8049019607843138	0.9389492753623189
0.8049019607843138	0.9391304347826087
0.8051470588235294	0.9391304347826087
0.8051470588235294	0.9393115942028986
0.8053921568627451	0.9393115942028986
0.8053921568627451	0.9394927536231884
0.8056372549019608	0.9394927536231884
0.8056372549019608	0.9398550724637681
0.8058823529411765	0.9398550724637681
0.8058823529411765	0.9400362318840579
0.8075980392156863	0.9400362318840579
0.8075980392156863	0.9402173913043478
0.8110294117647059	0.9402173913043478
0.8110294117647059	0.9403985507246376
0.8122549019607843	0.9403985507246376
0.8122549019607843	0.9405797101449276
0.8127450980392157	0.9405797101449276
0.8127450980392157	0.9409420289855073
0.8132352941176471	0.9409420289855073
0.8132352941176471	0.9411231884057971
0.8147058823529412	0.9411231884057971
0.8147058823529412	0.9416666666666667
0.8156862745098039	0.9416666666666667
0.8156862745098039	0.9418478260869565
0.8181372549019608	0.9418478260869565
0.8181372549019608	0.9420289855072463
0.8186274509803921	0.9420289855072463
0.8186274509803921	0.9422101449275362
0.8188725490196078	0.9422101449275362
0.8188725490196078	0.9423913043478261
0.8198529411764706	0.9423913043478261
0.8198529411764706	0.942572463768116
0.8200980392156862	0.942572463768116
0.8200980392156862	0.9429347826086957
0.8208333333333333	0.9429347826086957
0.8208333333333333	0.9431159420289855
0.8215686274509804	0.9431159420289855
0.8215686274509804	0.943659420289855
0.821813725490196	0.943659420289855
0.821813725490196	0.9438405797101449
0.8220588235294117	0.9438405797101449
0.8220588235294117	0.9440217391304347
0.8223039215686274	0.9440217391304347
0.8223039215686274	0.9442028985507246
0.8230392156862745	0.9442028985507246
0.8230392156862745	0.9443840579710145
0.8232843137254902	0.9443840579710145
0.8232843137254902	0.9445652173913044
0.8235294117647058	0.9445652173913044
0.8235294117647058	0.9452898550724638
0.8237745098039215	0.9452898550724638
0.8237745098039215	0.9454710144927536
0.8252450980392156	0.9454710144927536
0.8252450980392156	0.9456521739130435
0.8254901960784313	0.9456521739130435
0.8254901960784313	0.9458333333333333
0.8276960784313725	0.9458333333333333
0.8276960784313725	0.9460144927536231
0.828186274509804	0.9460144927536231
0.828186274509804	0.9467391304347826
0.8291666666666667	0.9467391304347826
0.8291666666666667	0.9476449275362319
0.8294117647058824	0.9476449275362319
0.8294117647058824	0.9481884057971014
0.8299019607843138	0.9481884057971014
0.8299019607843138	0.9483695652173914
0.8313725490196079	0.9483695652173914
0.8313725490196079	0.9485507246376812
0.8316176470588236	0.9485507246376812
0.8316176470588236	0.9489130434782609
0.8318627450980393	0.9489130434782609
0.8318627450980393	0.9490942028985507
0.8325980392156863	0.9490942028985507
0.8325980392156863	0.9496376811594203
0.8338235294117647	0.9496376811594203
0.8338235294117647	0.9498188405797101
0.8345588235294118	0.9498188405797101
0.8345588235294118	0.9503623188405798
0.8355392156862745	0.9503623188405798
0.8355392156862745	0.9505434782608696
0.836764705882353	0.9505434782608696
0.836764705882353	0.9507246376811594
0.8375	0.9507246376811594
0.8375	0.9510869565217391
0.8382352941176471	0.9510869565217391
0.8382352941176471	0.951268115942029
0.8394607843137255	0.951268115942029
0.8394607843137255	0.9516304347826087
0.8406862745098039	0.9516304347826087
0.8406862745098039	0.9518115942028985
0.8411764705882353	0.9518115942028985
0.8411764705882353	0.9519927536231884
0.8426470588235294	0.9519927536231884
0.8426470588235294	0.9521739130434783
0.8433823529411765	0.9521739130434783
0.8433823529411765	0.9523550724637682
0.8446078431372549	0.9523550724637682
0.8446078431372549	0.952536231884058
0.8448529411764706	0.952536231884058
0.8448529411764706	0.9527173913043478
0.8450980392156863	0.9527173913043478
0.8450980392156863	0.9528985507246377
0.845343137254902	0.9528985507246377
0.845343137254902	0.9530797101449275
0.8455882352941176	0.9530797101449275
0.8455882352941176	0.9532608695652174
0.846078431372549	0.9532608695652174
0.846078431372549	0.9536231884057971
0.8463235294117647	0.9536231884057971
0.8463235294117647	0.9538043478260869
0.8468137254901961	0.9538043478260869
0.8468137254901961	0.9539855072463768
0.8470588235294118	0.9539855072463768
0.8470588235294118	0.9541666666666667
0.8473039215686274	0.9541666666666667
0.8473039215686274	0.9543478260869566
0.8475490196078431	0.9543478260869566
0.8475490196078431	0.9548913043478261
0.8480392156862745	0.9548913043478261
0.8480392156862745	0.9550724637681159
0.8497549019607843	0.9550724637681159
0.8497549019607843	0.9554347826086956
0.8517156862745098	0.9554347826086956
0.8517156862745098	0.9556159420289855
0.8522058823529411	0.9556159420289855
0.8522058823529411	0.9559782608695652
0.8529411764705882	0.9559782608695652
0.8529411764705882	0.9561594202898551
0.8534313725490196	0.9561594202898551
0.8534313725490196	0.9567028985507247
0.8536764705882353	0.9567028985507247
0.8536764705882353	0.9568840579710145
0.8539215686274509	0.9568840579710145
0.8539215686274509	0.9570652173913043
0.8541666666666666	0.9570652173913043
0.8541666666666666	0.9572463768115942
0.854656862745098	0.9572463768115942
0.854656862745098	0.957427536231884
0.8561274509803921	0.957427536231884
0.8561274509803921	0.9576086956521739
0.8566176470588235	0.9576086956521739
0.8566176470588235	0.9577898550724637
0.8578431372549019	0.9577898550724637
0.8578431372549019	0.9586956521739131
0.8580882352941176	0.9586956521739131
0.8580882352941176	0.9588768115942029
0.858578431372549	0.9588768115942029
0.858578431372549	0.9590579710144927
0.8590686274509803	0.9590579710144927
0.8590686274509803	0.9592391304347826
0.8598039215686275	0.9592391304347826
0.8598039215686275	0.9596014492753623
0.8600490196078432	0.9596014492753623
0.8600490196078432	0.9597826086956521
0.8607843137254902	0.9597826086956521
0.8607843137254902	0.9599637681159421
0.8610294117647059	0.9599637681159421
0.8610294117647059	0.9601449275362319
0.8615196078431373	0.9601449275362319
0.8615196078431373	0.9603260869565218
0.8627450980392157	0.9603260869565218
0.8627450980392157	0.9605072463768116
0.8637254901960785	0.9605072463768116
0.8637254901960785	0.9606884057971015
0.8639705882352942	0.9606884057971015
0.8639705882352942	0.9610507246376812
0.8642156862745098	0.9610507246376812
0.8642156862745098	0.961231884057971
0.8644607843137255	0.961231884057971
0.8644607843137255	0.9614130434782608
0.8647058823529412	0.9614130434782608
0.8647058823529412	0.9615942028985507
0.8649509803921569	0.9615942028985507
0.8649509803921569	0.9617753623188405
0.8666666666666667	0.9617753623188405
0.8666666666666667	0.9619565217391305
0.8676470588235294	0.9619565217391305
0.8676470588235294	0.9623188405797102
0.8678921568627451	0.9623188405797102
0.8678921568627451	0.9626811594202899
0.8683823529411765	0.9626811594202899
0.8683823529411765	0.9628623188405797
0.8691176470588236	0.9628623188405797
0.8691176470588236	0.9630434782608696
0.8696078431372549	0.9630434782608696
0.8696078431372549	0.9632246376811594
0.8705882352941177	0.9632246376811594
0.8705882352941177	0.9634057971014492
0.8718137254901961	0.9634057971014492
0.8718137254901961	0.9637681159420289
0.8720588235294118	0.9637681159420289
0.8720588235294118	0.9639492753623189
0.8730392156862745	0.9639492753623189
0.8730392156862745	0.9641304347826087
0.875	0.9641304347826087
0.875	0.9643115942028986
0.8752450980392157	0.9643115942028986
0.8752450980392157	0.9644927536231884
0.8757352941176471	0.9644927536231884
0.8757352941176471	0.9646739130434783
0.8759803921568627	0.9646739130434783
0.8759803921568627	0.9648550724637681
0.8794117647058823	0.9648550724637681
0.8794117647058823	0.9655797101449275
0.879656862745098	0.9655797101449275
0.879656862745098	0.9657608695652173
0.8813725490196078	0.9657608695652173
0.8813725490196078	0.9661231884057971
0.8818627450980392	0.9661231884057971
0.8818627450980392	0.966304347826087
0.8821078431372549	0.966304347826087
0.8821078431372549	0.9664855072463768
0.8825980392156862	0.9664855072463768
0.8825980392156862	0.9666666666666667
0.883578431372549	0.9666666666666667
0.883578431372549	0.9670289855072464
0.884313725490196	0.9670289855072464
0.884313725490196	0.9672101449275362
0.8850490196078431	0.9672101449275362
0.8850490196078431	0.967391304347826
0.8852941176470588	0.967391304347826
0.8852941176470588	0.9675724637681159
0.8855392156862745	0.9675724637681159
0.8855392156862745	0.9677536231884057
0.8857843137254902	0.9677536231884057
0.8857843137254902	0.9679347826086957
0.8865196078431372	0.9679347826086957
0.8865196078431372	0.9681159420289855
0.8872549019607843	0.9681159420289855
0.8872549019607843	0.9686594202898551
0.8877450980392156	0.9686594202898551
0.8877450980392156	0.9688405797101449
0.8879901960784313	0.9688405797101449
0.8879901960784313	0.9690217391304348
0.888235294117647	0.9690217391304348
0.888235294117647	0.9692028985507246
0.8884803921568627	0.9692028985507246
0.9436274509803921	0.9804347826086957
0.9441176470588235	0.9804347826086957
0.9441176470588235	0.9806159420289855
0.9463235294117647	0.9806159420289855
0.9463235294117647	0.9807971014492753
0.9480392156862745	0.9807971014492753
0.9480392156862745	0.9809782608695652
0.9487745098039215	0.9809782608695652
0.9487745098039215	0.981159420289855
0.9502450980392156	0.981159420289855
0.9502450980392156	0.9813405797101449
0.9509803921568627	0.9813405797101449
0.9509803921568627	0.9817028985507247
0.9512254901960784	0.9817028985507247
0.9512254901960784	0.9818840579710145
0.9529411764705882	0.9818840579710145
0.9529411764705882	0.9820652173913044
0.953186274509804	0.9820652173913044
0.953186274509804	0.9822463768115942
0.953921568627451	0.9822463768115942
0.953921568627451	0.9824275362318841
0.9541666666666667	0.9824275362318841
0.9541666666666667	0.9826086956521739
0.9544117647058824	0.9826086956521739
0.9544117647058824	0.9831521739130434
0.9546568627450981	0.9831521739130434
0.9546568627450981	0.9833333333333333
0.9556372549019608	0.9833333333333333
0.9556372549019608	0.9835144927536232
0.9561274509803922	0.9835144927536232
0.9561274509803922	0.9836956521739131
0.9563725490196079	0.9836956521739131
0.9563725490196079	0.9840579710144928
0.9571078431372549	0.9840579710144928
0.9571078431372549	0.9842391304347826
0.9590686274509804	0.9842391304347826
0.9590686274509804	0.9844202898550725
0.9593137254901961	0.9844202898550725
0.9593137254901961	0.9846014492753623
0.9627450980392157	0.9846014492753623
0.9627450980392157	0.9847826086956522
0.9649509803921569	0.9847826086956522
0.9649509803921569	0.984963768115942
0.9666666666666667	0.984963768115942
0.9666666666666667	0.9851449275362318
0.9678921568627451	0.9851449275362318
0.9678921568627451	0.9853260869565217
0.9700980392156863	0.9853260869565217
0.9700980392156863	0.9855072463768116
0.9720588235294118	0.9855072463768116
0.9720588235294118	0.9856884057971015
0.9727941176470588	0.9856884057971015
0.9727941176470588	0.9860507246376812
0.9732843137254902	0.9860507246376812
0.9732843137254902	0.986231884057971
0.975	0.986231884057971
0.975	0.9865942028985507
0.9754901960784313	0.9865942028985507
0.9754901960784313	0.9867753623188406
0.9759803921568627	0.9867753623188406
0.9759803921568627	0.9869565217391304
0.9762254901960784	0.9869565217391304
0.9762254901960784	0.9875
0.9764705882352941	0.9875
0.9764705882352941	0.9876811594202899
0.9772058823529411	0.9876811594202899
0.9772058823529411	0.9880434782608696
0.9789215686274509	0.9880434782608696
0.9789215686274509	0.9882246376811594
0.979656862745098	0.9882246376811594
0.979656862745098	0.9884057971014493
0.9799019607843137	0.9884057971014493
0.9799019607843137	0.988768115942029
0.9803921568627451	0.988768115942029
0.9803921568627451	0.9889492753623188
0.9806372549019607	0.9889492753623188
0.9806372549019607	0.9893115942028986
0.9813725490196078	0.9893115942028986
0.9813725490196078	0.9894927536231884
0.9825980392156862	0.9894927536231884
0.9825980392156862	0.9896739130434783
0.9830882352941176	0.9896739130434783
0.9830882352941176	0.9898550724637681
0.9840686274509803	0.9898550724637681
0.9840686274509803	0.990036231884058
0.9848039215686275	0.990036231884058
0.9848039215686275	0.9902173913043478
0.9855392156862746	0.9902173913043478
0.9855392156862746	0.9907608695652174
0.9857843137254902	0.9907608695652174
0.9857843137254902	0.9909420289855072
0.9860294117647059	0.9909420289855072
0.9860294117647059	0.991123188405797
0.9870098039215687	0.991123188405797
0.9870098039215687	0.9916666666666667
0.9872549019607844	0.9916666666666667
0.9872549019607844	0.9918478260869565
0.9875	0.9918478260869565
0.9875	0.9920289855072464
0.9879901960784314	0.9920289855072464
0.9879901960784314	0.9929347826086956
0.9892156862745098	0.9929347826086956
0.9892156862745098	0.9931159420289855
0.9897058823529412	0.9931159420289855
0.9897058823529412	0.9932971014492754
0.9899509803921569	0.9932971014492754
0.9899509803921569	0.9936594202898551
0.9904411764705883	0.9936594202898551
0.9904411764705883	0.993840579710145
0.9911764705882353	0.993840579710145
0.9911764705882353	0.9940217391304348
0.991421568627451	0.9940217391304348
0.991421568627451	0.9942028985507246
0.9916666666666667	0.9942028985507246
0.9916666666666667	0.9943840579710145
0.9919117647058824	0.9943840579710145
0.9919117647058824	0.9947463768115942
0.9926470588235294	0.9947463768115942
0.9926470588235294	0.994927536231884
0.9928921568627451	0.994927536231884
0.9928921568627451	0.9951086956521739
0.9931372549019608	0.9951086956521739
0.9931372549019608	0.9952898550724638
0.9936274509803922	0.9952898550724638
0.9936274509803922	0.9954710144927537
0.9943627450980392	0.9954710144927537
0.9943627450980392	0.9960144927536232
0.9946078431372549	0.9960144927536232
0.9946078431372549	0.996195652173913
0.9950980392156863	0.996195652173913
0.9950980392156863	0.9963768115942029
0.995343137254902	0.9963768115942029
0.995343137254902	0.9969202898550724
0.9958333333333333	0.9969202898550724
0.9958333333333333	0.9971014492753624
0.996078431372549	0.9971014492753624
0.996078431372549	0.9972826086956522
0.9968137254901961	0.9972826086956522
0.9968137254901961	0.9974637681159421
0.9973039215686275	0.9974637681159421
0.9973039215686275	0.9976449275362319
0.9977941176470588	0.9976449275362319
0.9977941176470588	0.9980072463768116
0.9980392156862745	0.9980072463768116
0.9980392156862745	0.9989130434782608
0.9982843137254902	0.9989130434782608
0.9982843137254902	0.9994565217391305
0.9987745098039216	0.9994565217391305
0.9987745098039216	0.9996376811594203
0.9992647058823529	0.9996376811594203
0.9992647058823529	0.9998188405797102
0.9997549019607843	0.9998188405797102
0.9997549019607843	1.0
1.0	1.0

==> fig/jailbreak_transfer_conceptual.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=\textwidth]{img/jailbreak_transfer_cropped.pdf}
\caption{\textbf{Jailbreak strength and model similarity predict transferability.} Given a harmful prompt, an attacker applies a jailbreaking method to the blue model with the intention of transferring the jailbreak to one of the other models. The generated jailbreak is strong with respect to the blue model: over multiple generations the judge scores the blue model responses as very helpful and harmful. The jailbreak transfers to the similar pink model, but not the dissimilar green model.}

\vspace{-0.5em}
\end{figure}

==> fig/over_obfuscation_conceptual.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=\textwidth]{img/over_obfuscation_cropped.pdf}
\caption{Over-obfuscation conceptual}
\end{figure}
